Batching and Optimal Multi-stage Bipartite Allocations

In several applications of real-time matching of demand to supply in online marketplaces, the platform allows for some latency to batch the demand and improve the efficiency. Motivated by these applications, we study the optimal trade-off between batching and inefficiency under adversarial arrival. As our base model, we consider K-stage variants of the vertex weighted b-matching in the adversarial setting, where online vertices arrive stage-wise and in K batches -- in contrast to online arrival. Our main result for this problem is an optimal (1-(1-1/K)^K)- competitive (fractional) matching algorithm, improving the classic (1-1/e) competitive ratio bound known for its online variant (Mehta et al., 2007; Aggarwal et al., 2011). We also extend this result to the rich model of multi-stage configuration allocation with free-disposals (Devanur et al., 2016), which is motivated by the display advertising in video streaming platforms. Our main technique is developing tools to vary the trade-off between "greedy-ness" and "hedging" of the algorithm across stages. We rely on a particular family of convex-programming based matchings that distribute the demand in a specifically balanced way among supply in different stages, while carefully modifying the balancedness of the resulting matching across stages. More precisely, we identify a sequence of polynomials with decreasing degrees to be used as strictly concave regularizers of the maximum weight matching linear program to form these convex programs. At each stage, our algorithm returns the corresponding regularized optimal solution as the matching of this stage (by solving the convex program). Using structural properties of these convex programs and recursively connecting the regularizers together, we develop a new multi-stage primal-dual framework to analyze the competitive ratio. We further show this algorithm is optimally competitive.

==> FN_ multi-stage matching + configuration allocation (MS Journal)/tex/adwords.tex <==
Recall that multi-stage AdWords 
problem is a variant of the multi-stage vertex 
weighted matching where 
(i) the weights (a.k.a., bids)
$\{b_{ij}\}_{(i,j)\in E}$
are assigned to edges;
(ii)
the matching constraint of 
each offline vertex $j\in \Driver$ is replaced with the budget constraint $\budget_j$;
and the goal 
is to maximize the total bids 
(a.k.a., used budgets) in the allocation.
Let $\minbudget = 
\min_{j\in \Driver}\budget_j$
be the smallest budget.
We discuss how to modify 
\Cref{alg:b-matching}
to output {fractional} solutions
for the $K$-stage AdWords problem
with competitive ratio $\cratio{K}$.
Then, using a standard 
randomized rounding technique,
we present a \emph{randomized} algorithm
that produces \emph{integral} solutions 
with competitive ratio 
$\cratio{K} - 
O(\sqrt{\log(\minbudget)/\minbudget})$.



\smallskip
\noindent\textbf{Fractional Multi-stage AdWords~} Consider a modification of 
\Cref{alg:b-matching}, where
(i) the convex program~\ref{eq:concave-k-bmatching}
is replaced with 
the modified convex program~\ref{eq:concave-adwords-k}
defined below,
and 
(ii) the update rule of 
$\{y_j\}$ is modified as 
$\forall j\in \Driver: y_j\gets y_j+\displaystyle\sum_{i\in\Rider_k}
b_{ij}x^*_{k,ij}$.
See the \emph{Polynomial Regularized Fractional AdWords} (\PRFAD) algorithm for a formal description (\Cref{alg:adwords fractional}):
    \begin{align}
\label{eq:concave-adwords-k}\tag{$\mathcal{P}_k^{\text{AdWords}}$}
    \begin{array}{lll}
       \xbf^*_k= \underset{\xbf}{\argmax} & 
        \displaystyle\sum_{(i,j) \in E_k}
b_{ij} {x_{ij}}
- \sum_{j\in \Driver}
\budget_j F_k\left(
\frac{y_j}{\budget_j}+
\sum_{i : (i,j)\in E_k}
\frac{b_{ij}x_{ij}}{\budget_j}
        \right)
        & \text{s.t.}\\
         &\displaystyle
         \sum_{j: (i,j)\in E_k} x_{ij} \leq 1
         & i\in \Rider_k\\
         & 
         \displaystyle\sum_{i: (i,j)\in E_k} 
         b_{ij}x_{ij} \leq 
         \budget_j-y_j
         & j\in \Driver\\
         &
        x_{ij} \geq 0 &
        (i, j) \in E_k
    \end{array}
\end{align}

\begin{algorithm}
 	\caption{Polynomial Regularized Fractional AdWords (\PRFAD)}
 	\label{alg:adwords fractional}
 	\KwIn{Number of batches/stages $K$}
%  	\vspace{1mm}
%  	\KwOut{SS.}
 	    \vspace{2mm}
 	    
    $\forall j\in\Driver:~y_j\gets 0$.

 	\vspace{1mm}
 	\For{stage $k=1$ to $K$}
 	{
 	\vspace{2mm}
 	\tcc{$k^{\textrm{th}}$ batch of vertices in $\Rider$, denoted by $\Rider_k$, arrives. Let $E_k$ denote the set of edges incident to vertices in $\Rider_k$.}
 	\vspace{2mm}
 	



   Given $\{y_j\}_{j\in \Driver}$ and subgraph $G_k=(\Rider_k,\Driver,E_k)$, solve $\xbf_k^*$
   from
   the convex program~\ref{eq:concave-adwords-k}.

$\forall j\in \Driver: y_j\gets y_j+\displaystyle\sum_{i\in\Rider_k}b_{ij}x^*_{k,ij}$.

Return $\xbf^*_k$ as the fractional AdWords allocation of stage $k$.

}
\end{algorithm}


\smallskip
\noindent\textbf{Rounding to an Integral Allocation~} To output integral solutions
in the $K$-stage AdWords problem, 
we apply a standard randomized rounding technique
as follows.
% \YF{do we need a citation for this
% sampling technique?}
At each stage $k$, find the optimal fractional solution
$\xbf_k^*$ of the convex
program \ref{eq:concave-adwords-k}
with adjusted budgets
$\{(1-\rho)\hat\budget_j\}_{j\in \Driver}$,
where $\rho = O(\sqrt{\log(\minbudget)/\minbudget})$
for a large enough constant in the big O notation.
% \footnote{It is not hard to verify that 
% $\rho = O(\sqrt{\log(\minbudget)/\minbudget})$.
% }
For each online vertex $i\in \Rider_k$,
sample an offline vertex $j\in\Driver$ independently 
with probability $\{x_{k,ij}^*\}_{j:(i,j)\in E_k}$.
If the offline vertex $j$ has enough budget for bid $b_{ij}$, allocate the online vertex $i$ to the offline vertex $j$. Otherwise, leave the online vertex $i$ unmatched.
Finally, update $\{y_j\}_{j\in \Driver}$
with the fractional solution $\xbf_k^*$ as before.
We refer to this algorithm as \emph{Polynomial Regularized Integral AdWords} (\PRIAD). See \Cref{alg:adwords integral}
for a formal description.

\begin{algorithm}
 	\caption{Polynomial Regularized Integral AdWords (\PRIAD)}
 	\label{alg:adwords integral}
 	\KwIn{Number of batches/stages $K$, parameter $\rho\in[0,1]$}
%  	\vspace{1mm}
%  	\KwOut{SS.}
 	    \vspace{2mm}
 	    
    $\forall j\in\Driver:~y_j\gets 0,
    \hat y_j \gets 0$.
    
%     $\rho = \underset{\rho\in[0,1]}{\argmin}
% ~1-\left(1-\rho\right)\left(1 - \exp\left(-\frac{\rho^2\minbudget}
%     {2-\rho}\right)\right)$.

 	\vspace{1mm}
 	\For{stage $k=1$ to $K$}
 	{
 	\vspace{2mm}
 	\tcc{$k^{\textrm{th}}$ batch of vertices in $\Rider$, denoted by $\Rider_k$, arrives. Let $E_k$ denote the set of edges incident to vertices in $\Rider_k$.}
 	\vspace{2mm}
 	

    Given $\{y_j\}_{j\in \Driver}$ and subgraph  $G_k=(\Rider_k,\Driver,E_k)$, solve $\xbf_k^*$
   from
   the convex  program~\ref{eq:concave-adwords-k} with
    adjusted budgets $\{(1-\rho)\budget_j\}_{j\in \Driver}$,
    and used budgets $\{y_j\}_{j\in \Driver}$.
    
    $\hat\xbf_k^* \gets \mathbf 0$.
    
 	\For{online vertex $i \in \Rider_k$}{
 	Sample offline vertex $j\sim \{x_{k,ij}^*\}_{j:(i,j)\in E_k}$.
 	
 	\If{$\hat y_j + b_{ij} \leq \budget_j$}{
 	    $\hat x_{k,ij}^* \gets 1$.
 	    
 	    $\hat y_j \gets \hat y_j + b_{ij}$.
 	}
 	}

$\forall j\in \Driver: y_j\gets y_j+\displaystyle\sum_{i\in\Rider_k} b_{ij}x^*_{k,ij}$.

Return $\hat\xbf^*_k$ as the integral AdWords allocation of stage $k$.

}
\end{algorithm}

We are now ready to describe the competitive ratio results of the multi-stage AdWords problem.
The proofs are deferred to \Cref{apx:adwords}.

\begin{theorem}[\textbf{Optimal Multi-stage Algorithm for Fractional AdWords}]
\label{thm:adwords fractional}
% \RN{is the statement of this theorem correct?}
In the $K$-stage fractional 
AdWords problem, \PRFAD~(\Cref{alg:adwords fractional})
is $\cratio{K}$-competitive, where $\cratio{K}=\cratioexp$.
\end{theorem}
\begin{theorem}[\textbf{Optimal Multi-stage Algorithm for AdWords with Large Budgets}]
\label{thm:adwords integral}
% \RN{is the statement of this theorem correct?}
In the $K$-stage integral
AdWords problem, \PRIAD~(\Cref{alg:adwords integral})
is \ $\left(\cratio{K} - O(\sqrt{\log(\minbudget)/\minbudget})\right)$-competitive, where $\cratio{K}=\cratioexp$.
\end{theorem}


\begin{remark}[\textbf{Optimality of the $\boldsymbol{\cratio{K}}$ Competitive Ratio for AdWords}]
Again, since the multi-stage AdWords problem generalizes
the multi-stage (fractional) unweighted matching problem (i.e., when $b_{ij}\in\{0,1\}$ and all budgets are $B_j=1$), 
% (i.e., the former approximates the latter
% by setting $b_{ij} = w_j$ for all $(i,j)\in E$
% and letting $\minbudget\rightarrow\infty$),
\Cref{thm:tightness} implies that
the competitive ratios in Theorems~\ref{thm:adwords fractional} and \ref{thm:adwords integral}
% is tight for $K$ 
have the optimal dependence on $K$
in the multi-stage AdWords problem, i.e., no integral or fractional multi-stage algorithm can obtain a competitive ratio better than $\cratio{K}$.
\end{remark}


==> FN_ multi-stage matching + configuration allocation (MS Journal)/tex/appendices.tex <==

\revcolor{\section{Connection Between Baseline and Extension Models}
\label{apx:connection}
We formally show that
the multi-stage configuration allocation 
generalizes the multi-stage vertex weighted matching.
To see this, we consider a reduction in which every instance in the vertex weighted matching 
can be thought as an
instance in the configuration allocation as follows:
Each advertiser $\driver$ has a unit demand 
($n_\driver = 1$).
The feasible configuration set encodes 
all edges $E$ in the baseline model
($\Config = E$).
Moreover, for every 
edge $(\rider\primed,\driver\primed)\in E$,
the corresponding
configuration $\config$ 
encodes the 
number of reserved impression $\{\alloci\}_{\rider,\driver}$
as 
$\alloci =\indicator{\rider = \rider\primed,
\driver = \driver\primed}$.
The 
per-impression prices are identical for each advertiser $j$ and only depend on the weight $w_j$ of the offline vertex $j$
($\weight_{\threeindex} =w_j \indicator{(i,j)\in E}$).
Finally, note that
since per-impression price are identical for each advertiser
and number of reserved impression $\{\alloci\}$
is encoded as the aforementioned indicator function,
without loss of generality, 
we can restrict attention to online algorithms 
whose allocations never exceed demand $\{n_\driver\}$
of advertisers, and thus
no
preemption or free disposal is needed.}



\section{Missing Proofs}
\label{sec:apx}
 \subsection{Proof of \Cref{prop:poly}}
 \label{apx:poly}
 

We first prove (i) by backward induction on $k$:
\begin{itemize}
    \item \textsl{Base case $(k = K-1)$:} The maximum of function $(1-y)f_{K}(x+y)=(1-y)\mathbb{I}\{x+y=1\}$ over $y\in[0,1-x]$ happens at $y^*=1-x$, and therefore $f_{K-1}(x)=x$. 
    \item \textsl{Inductive step $(k\in [K-2])$.}
Suppose $f_{k+1}(x)=(1-\frac{1-x}{K-k-1})^{K-k-1}$. Fix $x\in[0,1]$ and let $y^*=\underset{y\in[0,1-x]}{\argmax}~(1-y)f_{k+1}(x+y)$. By writing the first-order condition due to optimality of $y^*$, we have:
\begin{equation}
\label{eq:poly}
  \left(1-\frac{1-x-y^*}{K-k-1}\right)^{K-k-2}-y^*\left(1-\frac{1-x-y^*}{K-k-1}\right)^{K-k-2}
    -\left(1-\frac{1-x-y^*}{K-k-1}\right)^{K-k-1}= 0~,
\end{equation}
which implies that $y^*=\frac{1-x}{K-k}$. Note that $y^*\in[0,1-x]$. To check whether $y^*$ is the maximum point in $[0,1-x]$, we consider the second-order condition with respect to $y^*$. After algebraic simplifications, we have (details are omitted for brevity):
$$ \frac{\partial^2}{\partial^2 y}\left[(1-y)f_{k+1}(x+y)\right]_{y=y^*}=(x-2)(1-\frac{1-x-y^*}{K-k-1})^{K-k-3}\leq 0
$$
Plugging back $y^*=\frac{1-x}{K-k}$ into the objective, we have:
$$
f_k(x)=(1-\frac{1-x}{K-k})f_{k+1}(x+\frac{1-x}{K-k})=(1-\frac{1-x}{K-k})(1-\frac{1-x}{K-k})^{K-k-1}=(1-\frac{1-x}{K-k})^{K-k}~,
$$
as desired. 
\end{itemize}
Given (i), proof of (ii) is immediate as the polynomial $f_k(x)=(1-\frac{1-x}{K-k})^{K-k}$ is monotone increasing for $k\in[K-1]$. Also, (iii) simply holds as $(1-x)\leq e^{-x}$ when $x\in[0,1]$, and that $\lim_{N\to+\infty}(1-\frac{x}{N})^N=e^{-x}$ for $x\in[0,1]$. Finally, to prove (iv), consider defining $f_0(x)=\underset{y\in[0,1-x]}{\max}(1-y)f_1(x+y)$. Following the backward induction in the proof of (i), $f_0(x)\triangleq(1-(1-x)/K)^K$. Therefore, 
$$\underset{y\in[0,1]}{\min}1-(1-y)f_1(y)=1-\underset{y\in[0,1]}{\max}(1-y)f_1(y)=1-f_0(0)=\cratio{K}.
$$

 
% We first prove (i) by backward induction on $k$:
% \begin{itemize}
%     \item \textsl{Base case $(k = K-1)$:} The maximum of function $(1-y)f_{K}(x+y)=(1-y)\mathbb{I}\{x+y=1\}$ over $y\in[0,1-x]$ happens at $y^*=1-x$, and therefore $f_{K-1}(x)=x$. 
%     \item \textsl{Inductive step $(k\in [K-2])$.}
% Suppose $f_{k+1}(x)=(1-\frac{1-x}{K-k-1})^{K-k-1}$. Fix $x\in[0,1]$ and let $y^*=\underset{y\in[0,1-x]}{\argmax}~(1-y)f_{k+1}(x+y)$. By writing the first-order condition due to optimality of $y^*$, we have:
% \begin{equation}
% \label{eq:poly}
%   \left(1-\frac{1-x-y^*}{K-k-1}\right)^{K-k-2}-y^*\left(1-\frac{1-x-y^*}{K-k-1}\right)^{K-k-2}
%     -\left(1-\frac{1-x-y^*}{K-k-1}\right)^{K-k-1}= 0~,
% \end{equation}
% which implies that $y^*=\frac{1-x}{K-k}$. Note that $y^*\in[0,1-x]$. To check whether $y^*$ is the maximum point in $[0,1-x]$, we consider the second-order condition with respect to $y^*$. After algebraic simplifications, we have (details are omitted for brevity):
% $$ \frac{\partial^2}{\partial^2 y}\left[(1-y)f_{k+1}(x+y)\right]_{y=y^*}=(x-2)(1-\frac{1-x-y^*}{K-k-1})^{K-k-3}\leq 0
% $$
% Plugging back $y^*=\frac{1-x}{K-k}$ into the objective, we have:
% $$
% f_k(x)=(1-\frac{1-x}{K-k})f_{k+1}(x+\frac{1-x}{K-k})=(1-\frac{1-x}{K-k})(1-\frac{1-x}{K-k})^{K-k-1}=(1-\frac{1-x}{K-k})^{K-k}~,
% $$
% as desired. 
% \end{itemize}
% Given (i), proof of (ii) is immediate as the polynomial $f_k(x)=(1-\frac{1-x}{K-k})^{K-k}$ is monotone increasing for $k\in[K-1]$. Also, (iii) simply holds as $(1-x)\leq e^{-x}$ when $x\in[0,1]$, and that $\lim_{N\to+\infty}(1-\frac{x}{N})^N=e^{-x}$ for $x\in[0,1]$. Finally, to prove (vi), consider defining $f_0(x)=\underset{y\in[0,1-x]}{\max}(1-y)f_1(x+y)$. Following the backward induction in the proof of (i), $f_0(x)\triangleq(1-(1-x)/K)^K$. Therefore, 
% $$\underset{y\in[0,1]}{\min}1-(1-y)f_1(y)=1-\underset{y\in[0,1]}{\max}(1-y)f_1(y)=1-f_0(0)=\cratio{K}$$.\qed


% \subsection{Proof of \Cref{lemma:structure}}
% \label{apx:skeleton}


% In order for the proof, we investigate the program~\ref{eq:concave-k-bmatching} through convex strong duality. In particular, we first define the Lagrangian dual function $\Lag_k(\cdot)$ and then re-state the KKT optimality conditions of $\xbf^*_k$ in our specific convex program.
% \begin{definition}
% \label{def:lagrange}
% The \emph{Lagrangian dual} $\Lag_k(.)$ for the concave program~\ref{eq:concave-k-bmatching} is defined as:
% \begin{align*}
%     \Lag_k(\xbf,\lambdabf,\thetabf,\gammabf)\triangleq& \displaystyle\sum_{j\in \Driver}w_j\left(
%         \sum_{i:(i,j)\in E_k}x_{ij} - 
%         F_k\left(y_j+
%         \sum_{i: (i,j)\in E_k}x_{ij}\right)
%         \right) \\
%     &-\sum_{i\in \Rider_k}\lambda_i\left(\sum_{j:(i,j)\in E_k}x_{ij}-1\right)
%     -\sum_{j\in \Driver}\theta_j\left(\sum_{i:(i,j)\in E_k}x_{ij}+y_j-1\right)
%     \\
%     &+\sum_{(i,j)\in E_k}\gamma_{ij}x_{ij}~~,
% \end{align*}
% where $\{\lambda_i\}$, $\{\theta_j\}$, and $\{\gamma_{ij}\}$ are the \emph{Lagrange multipliers}, also known as the \emph{dual variables}, 
% corresponding to different constraints 
% in program~\ref{eq:concave-k-bmatching}.
% \end{definition}
% \begin{proposition}[\emph{Strong duality/KKT conditions}]
% \label{prop:kkt}
% Suppose $\xbf_k^*$ is the optimal solution of the concave program \ref{eq:concave-k-bmatching}. 
% Consider the Lagrangian dual $\Lag_k$, as in \Cref{def:lagrange}. Then:
% \begin{equation*}
%     \underset{\xbf}{\max}~\underset{\lambdabf,\thetabf,\gammabf}{\min}~\Lag_k(\xbf,\lambdabf,\thetabf,\gammabf)= \underset{\lambdabf,\thetabf,\gammabf}{\min}~\underset{\xbf}{\max}~\Lag_k(\xbf,\lambdabf,\thetabf,\gammabf)=\underset{\lambdabf,\thetabf,\gammabf}{\min}~\Lag_k(\xbf_k^*,\lambdabf,\thetabf,\gammabf)~~.
% \end{equation*}
% Moreover, if $\lambdabf^*$, $\thetabf^*$, and $\gammabf^*$ (together with $\xbf_k^*)$ are the solutions of the above minmax/maxmin, then:
% \begin{itemize}
%     \item (Stationarity)~~$\forall (i,j)\in E_k:~~\frac{\partial \Lag_k}
%     {\partial x_{ij}}(\xbf_k^*,\lambdabf^*,\thetabf^*,\gammabf^*)=0,$
%     \item (Dual feasibility)~~$\forall i\in \Rider_k,j\in \Driver,(i,j)\in E_k:~\lambda^*_i\geq 0,~\theta^*_j\geq 0$, and $\gamma^*_{ij}\geq 0$~,
%     \item (Complementary slackness)~~$\forall i\in \Rider_k,j\in \Driver,(i,j)\in E_k:$ 
%     \begin{itemize}
%         \item  $\gamma^*_{ij}=0$ or $\left(\gamma^*_{ij}>0~\textrm{and}~ x^*_{k,ij}=0\right)~,$
%         \item $\lambda^*_{i}=0$ or $\left(\lambda^*_{i}>0~\textrm{and}~ \sum_{j: (i,j)\in E_k}x^*_{k,ij}=1\right)~,$
%         \item  $\theta^*_{j}=0$ or $\left(\theta^*_{j}>0~\textrm{and}~ y_j+\sum_{i: (i,j)\in E_k}x^*_{k,ij} =1\right)~.$
%     \end{itemize}
% \end{itemize}
% \end{proposition}
% With the above ingredients, we prove the structural lemma.
% \begin{proof}[Proof of \Cref{lemma:structure}]
% We first show the uniformity property. 
% For $j\in \Driver_k^{(0)}$,
% note that $$w_j\left(1-
%     f_k\left(y_j + \sum_{i:(i,j)\in E_k}x^*_{k,ij}\right)
%     \right)
%     =w_j(1 - f_k(1))=0=c^{(0)}.$$ 
%     For vertices in $\Driver_k^{(l)}$ 
%     with $l\in [L_k]$,
%     since
%     they are in the same connected component of $G_k'[\Rider_k\setminus\Rider_k^{(0)},\Driver\setminus \Driver_k^{(0)}]$,
%     it is sufficient to restrict attention to $j, j'\in\Driver_k^{(l)}$
%     such that
%     there exists a vertex $i\in\Rider_k^{(l)}$ such that $x^*_{k,ij}>0$ and $x^*_{k,ij'}>0$ (and therefore, $\gamma^*_{ij}=\gamma^*_{ij'}=0$, because of the complementary slackness in \Cref{prop:kkt}). Also, $\theta^*_j=\theta^*_{j'}=0$, again because of complementary slackness and the fact that $y_j+\sum_{i:(i,j)\in E_k}x^*_{k,ij}<1$ and $y_{j'}+\sum_{i: (i,j')\in E_k}x^*_{k,ij'}<1$.
% Now, applying the stationarity condition in \Cref{prop:kkt}, we have:
% $$
% w_j\left(1-
%     f_k\left(y_j + \sum_{i:(i,j)\in E_k}x^*_{k,ij}\right)
%     \right)
% -\lambda^*_i-\theta^*_j+\gamma^*_{ij}
% =0=
% w_{j'}\left(1-
%     f_k\left(y_{j'} + \sum_{i: (i,j')\in E_k}x^*_{k,ij'}\right)
%     \right)
% -\lambda^*_i-\theta^*_{j'}+\gamma^*_{ij'}~,
% $$
% and therefore 
% $w_j\left(1-
%     f_k\left(y_j + \sum_{i:(i,j)\in E_k}x^*_{k,ij}\right)
%     \right)
%     =
%     w_{j'}\left(1-
%     f_k\left(y_{j'} + \sum_{i: (i,j')\in E_k}x^*_{k,ij'}\right)
%     \right)$, 
%     finishing the proof of the uniformity property. 
    
%     To show saturation property, 
%     note that $\lambda^*_i=
%     w_j\left(1-
%     f_k\left(y_j + \sum_{i:(i,j)\in E_k}x^*_{k,ij}\right)
%     \right)>0$ for any $i \in \Rider_k^{(l)}, j \in \Driver_k^{(l)}$ with $l \in[L_k]$ such that $x_{ij}^* > 0$, simply because $f_k(1)=1$ and $f_k(x)$ is (strictly) monotone increasing.
%     Again, by using complementary slackness, we have $\sum_{j:(i,j)\in E_k}x^*_{k,ij}=1$, which proves the saturation property.

% Now suppose there exists an edge $(i,j')\in E_k$, where $i\in \Rider_k^{(l)}$ and $j'\in \Driver_k^{(l')}$, for $l,l'\in[0:L_k], l\neq l'$. 
% First note that there should 
% exist a vertex $j\in\Driver_k^{(l)}$ so that $x^*_{k,ij}>0$; this holds because $i$ is either fully matched by $\xbf_k^*$ if $l\in[L_k]$ 
% -- thanks to the saturation property --  
% or $l=0$ and $i$ is connected to a vertex  $j\in\Driver_k^{(0)}$ with $x^*_{k,ij'}>0$ by definition. 
% Because of complementary slackness $\gamma^*_{ij}=0$. 
% Now, by writing the stationarity condition of \Cref{prop:kkt} for the edge $(i,j')$, and noting that 
% $w_{j'}\left(1-
%     f_k\left(y_{j'} + \sum_{i: (i,j')\in E_k}x^*_{k,ij'}\right)
%     \right)=c^{(l')}$ 
% because of the uniformity property, we have:
% $$
% c^{(l')}-\lambda^*_i-\theta^*_{j'}+\gamma^*_{ij'}=0~,
% $$
% By writing the same condition for the edge $(i,j)$ we have: 
% $$
% c^{(l)} - \lambda^*_i - \theta^*_{j}=0~,
% $$
% and therefore 
% $$
% c^{(l)}\geq c^{(l)}-\theta^*_{j}
% =c^{(l')}-\theta^*_{j'}+\gamma^*_{ij'}
% \geq 
% c^{(l')}-\theta^*_{j'}
% $$
% If $l'=0$, then clearly $c^{(l)}\geq 0= c^{(l')}$. 
% If $l'\in [L_k]$, then $\sum_{i': (i',j')\in E_k}x^*_{i'j'}+y_{j'}<1$ 
% and $\theta^*_{j'}=0$ because of complementary slackness. Therefore, $c^{(l)}\geq c^{(l')}$, which finishes the proof of the monotonicity property.
% \end{proof}

% \input{tex/apx-b-matching-proof}
% \input{tex/apx-adword-proof}

% \section{Algorithms in Extension Problems}
% \label{apx:algorithms}
% \input{tex/apx-algorithms}


\input{tex/apx-kkt}

\input{tex/apx-numerical}

\input{tex/apx-open}

==> FN_ multi-stage matching + configuration allocation (MS Journal)/tex/apx-adword-proof.tex <==
\subsection{\texorpdfstring{Proof of \Cref{thm:adwords fractional} and \Cref{thm:adwords integral}}{Lg}}
\label{apx:adwords}

To prove our theorems, we start with a structural decomposition lemma 
as before. This time, our structural decomposition is slightly different, and in fact much simpler. 
% We omits its proof as it basically repeats 
% the argument for its analog in 
% vertex weighted
% matching problem (\Cref{lemma:structure}).
% The main difference between \Cref{lemma:structure adwords} and \Cref{lemma:structure}
% is the closed-form expression 
% in uniformity property.

\begin{lemma}[\emph{Structural decomposition --
AdWords}]
\label{lemma:structure adwords}
Fix any $k \in [K - 1]$.
Let $\xbf^*_k$ be the optimal solution of convex program~\ref{eq:concave-adwords-k}. Consider the subgraph $G'_k=(\Rider_k,\Driver,E'_k)$ of $G_k$, where $E'_k=\{(i,j)\in E_k :x^*_{k,ij}>0\}$. Let $\Driver^{(0)}_k$ be the set of offline vertices in $\Driver$ who exhausts their 
budgets by $\xbf^*_k$ given the current $\ybf$, and 
$\Rider^{(0)}_k$ be the set of online vertices who are neighbors of $\Driver^{(0)}_k$ in $G_k'$, that is, 
$$\Driver^{(0)}_k\triangleq \{j\in \Driver: y_j+\sum_{i:(i,j)\in E_k}b_{ij}x^*_{k,ij}=\budget_j\}~~\textrm{and}~~\Rider^{(0)}_k\triangleq \{i\in \Rider_k:\exists j\in \Driver^{(0)}_k, x^*_{k,ij}>0\}~.$$
Moreover, let $\Rider_k^{(1)} 
\triangleq \Rider_k\setminus\Rider_k^{(0)}$
and 
$\Driver_k^{(1)}
\triangleq
\Driver\setminus\Driver_k^{(0)}$.
Then:
\begin{enumerate}%[label=\roman*.]
    \item \underline{Uniformity}: ~$
    \forall
    i\in \Rider_k, j,j'\in \Driver:$
    if $x_{k,ij}^* > 0$ and 
    $x_{k,ij'}^* > 0$, then
    $$
    b_{ij}\left(1-
    f_k\left(
    \frac{y_j}{\budget_j}
    + \sum_{i':(i',j)\in E_k}
    \frac{b_{i' j}x^*_{k, i' j}}{\budget_j}
    \right)
    \right)=
    b_{ij'}\left(1-
    f_k\left(
    \frac{y_{j'}}{\budget_{j'}} + \sum_{i':(i',j')\in E_k}
    \frac{b_{i' j'}x^*_{k,i' j'}}{\budget_{j'}}
    \right)
    \right)$$
    For each online vertex $i\in \Rider_k$,
    if there exists an offline vertex $j$ such that $x_{l,ij}^* > 0$, define 
    $c_{k,i} \triangleq b_{ij}\left(1-
    f_k\left(
    \frac{y_j}{\budget_j}
    + \sum_{i':(i',j)\in E_k}
    \frac{b_{i' j}x^*_{k, i' j}}{\budget_j}
    \right)
    \right)$; otherwise
   \Big($\sum_{j:(i,j)\in E_k}x_{k,ij}^* = 0$\Big),
    define $c_{k,i} \triangleq 0$.
    \item \underline{Monotonicity}:  $\forall~ 
   (i,j)\in E_k$: 
   $$
   c_{k,i} \geq 
   b_{ij}\left(1-
    f_k\left(
    \frac{y_j}{\budget_j}
    + \sum_{i':(i',j)\in E_k}
    \frac{b_{i' j}x^*_{k, i' j}}{\budget_j}
    \right)
    \right)
   $$
    \item \underline{Saturation}: all online vertices in $\Rider_k^{(1)}$ are fully matched by $\xbf_k^*$, i.e., $\displaystyle\sum_{j:(i,j)\in E_k}x^*_{k,ij}=1, i\in\Rider_k^{(1)}$~.
\end{enumerate}
\end{lemma}
\ifMS \proof{\textsl{Proof.}}
\else \begin{proof}\fi
We first show the uniformity property. 
    Consider any online vertex $i \in \Rider_k^{(1)}$,
    offline vertices $j,j'\in \Driver$ such that
    $x_{k,ij}^* > 0$ and
    $x_{k,ij'}^* > 0$.
    By construction, $j,j'\in \Driver_k^{(1)}$.
    Thus, 
    $\gamma^*_{ij}=\gamma^*_{ij'}=0$, because of the complementary slackness in \Cref{prop:kkt}). Also, $\theta^*_j=\theta^*_{j'}=0$, again because of complementary slackness and the fact that $y_j+\sum_{i:(i,j)\in E_k}x^*_{k,ij}<1$ and $y_{j'}+\sum_{i: (i,j')\in E_k}x^*_{k,ij'}<1$.
Applying the stationarity condition in \Cref{prop:kkt}, we have:
\begin{align*}
 &b_{ij}\left(1-
    f_k\left(
    \frac{y_j}{\budget_j}
    + \sum_{i':(i',j)\in E_k}
    \frac{b_{i' j}x^*_{k, i' j}}{\budget_j}
    \right)
    \right)
-\lambda^*_i-\theta^*_j+\gamma^*_{ij}\\
=&~0
=
 b_{ij'}\left(1-
    f_k\left(
    \frac{y_{j'}}{\budget_{j'}} + \sum_{i':(i',j')\in E_k}
    \frac{b_{i' j'}x^*_{k,i' j'}}{\budget_{j'}}
    \right)
    \right)
-\lambda^*_i-\theta^*_{j'}+\gamma^*_{ij'}~,
\end{align*}
which
    finishes the proof of the uniformity property for 
    $i\in \Rider_k^{(1)}$. 
    

Now fix any online vertex $i\in \Rider_k^{(0)}$ and
offline vertex $j\in \Driver$ such that 
$x_{k,ij}^*$.
By complementary slackness, $\gamma_{ij}^* = 0$.
If $j\in \Driver_k^{(0)}$, then
$$
    b_{ij}\left(1-
    f_k\left(
    \frac{y_j}{\budget_j}
    + \sum_{i':(i',j)\in E_k}
    \frac{b_{i' j}x^*_{k, i' j}}{\budget_j}
    \right)
    \right)
    =b_{ij}(1 - f_k(1))=0.$$ 
    Due to stationarity condition, we know that 
    $\lambda_i^* = 0$. 
    If $j\in \Driver_k^{(1)}$, due to complementary slackness, we know that $\theta_j^* = 0$.
    Thus, applying stationarity condition again,
    we conclude that 
    $$    b_{ij}\left(1-
    f_k\left(
    \frac{y_j}{\budget_j}
    + \sum_{i':(i',j)\in E_k}
    \frac{b_{i' j}x^*_{k, i' j}}{\budget_j}
    \right)
    \right) = \lambda_i^* + \theta_j^* - \gamma_{ij}^* = 0.$$
    

    To show saturation property, 
    for any online vertex $i\in \Rider_k^{(1)}$,
    there should exist an offline vertex $j\in \Driver_k^{(1)}$
    such that $x_{k,ij}^* > 0$.\footnote{Without
    loss of generality, in this paper we assume that every online vertex
    has at least one edge to offline vertex set $\Driver$.}
    Note that $\lambda^*_i=
     b_{ij}\left(1-
    f_k\left(
    \frac{y_j}{\budget_j}
    + \sum_{i':(i',j)\in E_k}
    \frac{b_{i' j}x^*_{k, i' j}}{\budget_j}
    \right)
    \right)$ by stationarity condition of \Cref{prop:kkt}.
    Since $f_k(1)=1$, $f_k(x)$ is (strictly) monotone increasing
    and 
    $    \frac{y_j}{\budget_j}
    + \sum_{i':(i',j)\in E_k}
    \frac{b_{i' j}x^*_{k, i' j}}{\budget_j} < 1$,
    we know $\lambda_i^* > 0$.
    Again, by using complementary slackness, we have $\sum_{j:(i,j)\in E_k}x^*_{k,ij}=1$, which proves the saturation property.


Fix any $(i, j)\in E_k$ such that $x_{k,ij}^* = 0$.
Again, there should 
exist an offline vertex $j'\in\Driver$ 
so that $x^*_{k,ij}>0$. 
Because of complementary slackness $\gamma^*_{ij'}=0$. 
Now, by writing the stationarity condition of \Cref{prop:kkt} for the edge $(i,j)$,
we have:
$$
   b_{ij}\left(1-
    f_k\left(
    \frac{y_j}{\budget_j}
    + \sum_{i':(i',j)\in E_k}
    \frac{b_{i' j}x^*_{k, i' j}}{\budget_j}
    \right)
    \right)
    -\lambda^*_i-\theta^*_{j}+\gamma^*_{ij}=0~,
$$
By writing the same condition for the edge $(i,j')$, due
to uniformity property, we have: 
$$
c_{k,i} - \lambda^*_i - \theta^*_{j'}=0~,
$$
and therefore 
\begin{align*}
c_{k,i}&\geq c^{(l)}-\theta^*_{j'}
=b_{ij}\left(1-
    f_k\left(
    \frac{y_j}{\budget_j}
    + \sum_{i':(i',j)\in E_k}
    \frac{b_{i' j}x^*_{k, i' j}}{\budget_j}
    \right)
    \right)-\theta^*_{j}+\gamma^*_{ij}\\
&\geq 
b_{ij}\left(1-
    f_k\left(
    \frac{y_j}{\budget_j}
    + \sum_{i':(i',j)\in E_k}
    \frac{b_{i' j}x^*_{k, i' j}}{\budget_j}
    \right)
    \right)-\theta^*_{j}
\end{align*}
If $j\in\Driver_k^{(0)}$, 
then clearly $c_{k,i}\geq 0= 
b_{ij}\left(1-
    f_k\left(
    \frac{y_j}{\budget_j}
    + \sum_{i':(i',j)\in E_k}
    \frac{b_{i' j}x^*_{k, i' j}}{\budget_j}
    \right)
    \right)$. 
If $j\in \Driver_k^{(1)}$, then $\sum_{i': (i',j)\in E_k}x^*_{i'j}+y_{j}<1$ 
and $\theta^*_{j}=0$ because of complementary slackness. 
% Therefore, $c_{k,i}\geq 
% b_{ij}\left(1-
%     f_k\left(
%     \frac{y_j}{\budget_j}
%     + \sum_{i':(i',j)\in E_k}
%     \frac{b_{i' j}x^*_{k, i' j}}{\budget_j}
%     \right)
%     \right)$, which 
    This finishes the proof of the monotonicity property.
\ifMS \Halmos \fi

\ifMS
\endproof
\else
\end{proof}
\fi

We now present the proofs of \Cref{thm:adwords fractional} and \Cref{thm:adwords integral},
which are for fractional and integral algorithms, respectively.


\ifMS \proof{\textsl{Proof of \Cref{thm:adwords fractional}.}}
\else \begin{proof}[Proof of \Cref{thm:adwords fractional}]\fi
For each stage $k\in[K-1]$, let 
$\{x_{k, ij}^*\}_{(i,j)\in E_k}$
be the optimal solution of the program~\ref{eq:concave-adwords-k}. 
First, we define the following notations which will be useful in this proof:
\begin{align*}
\forall j\in \Driver,~k\in[K]:\quad\quad\quad 
& y^*_{k,j}\triangleq\sum_{s=1}^{k-1}\sum_{i:(i,j)\in E_s}
b_{ij} x^*_{s,ij}.
\end{align*}

Now consider the offline primal-dual linear program \ref{eq:LP-max-weight adwords}.
\begin{equation}
\tag{\textsc{Primal-Dual-AdWords}}
\label{eq:LP-max-weight adwords}
\arraycolsep=1.4pt\def\arraystretch{1}
\begin{array}{llllllll}
\max\quad\quad\quad&\displaystyle\sum_{(i,j)\in E}
b_{ij}x_{ij} &~~\text{s.t.}&
&\quad\quad\text{min}\quad\quad\quad &\displaystyle\sum_{i\in \Rider }{\alpha_i}+\displaystyle\sum_{j\in \Driver}{\budget_j\beta_j}&~~\text{s.t.} \\[1.4em]
 &\displaystyle\sum_{j:(i,j)\in E}{x_{ij}}\leq1 &~~i\in\Rider~,& 
& &\alpha_i+b_{ij}\beta_j\geq b_{ij}& (i,j)\in E~,\\[1.4em]
 &\displaystyle\sum_{i:(i,j)\in E}
 {b_{ij}x_{ij}}\leq \budget_j &~~j\in \Driver~, &
& &\alpha_i\geq 0 &i\in \Rider~, \\
 &x_{ij} \geq 0 &(i,j)\in E~. &
& &\beta_j\geq 0  &j\in \Driver~. 
\end{array}
\end{equation}
Once again, 
given the feasible primal (fractional) assignment $\{\xbf^*_k\}_{k\in[K]}$ produced by \Cref{alg:adwords fractional}, we construct a dual assignment so that,
\begin{itemize}
    \item Primal and dual have the same objective values: $\displaystyle\sum_{k\in[K]}\displaystyle\sum_{(i,j)\in E_k}
    b_{ij} x^*_{k,ij}=\sum_{i\in\Rider}\alpha_i+\sum_{j\in\Driver}\budget_j\beta_j$~,
    \item Dual is approximately feasible: $\forall (i,j)\in E: \alpha_i+b_{ij}\beta_j\geq \cratio{K}\cdot b_{ij}$~.
\end{itemize}

\noindent[\textit{Step \rom{1}}]~\emph{Dual assignment construction.}
First, set $\alpha_i\gets 0$ and $\beta_j\gets 0$ for all $i\in\Rider,j\in \Driver$. At each stage $k\in[0:K-1]$, update the dual variables as follows:
\begin{align*}
   &\forall i \in \Rider_k: &&
   \alpha_i\gets c_{k,i}
   \\
    &\forall j \in \Driver: &&\beta_{j}\gets\beta_{j}+\Delta\beta_{k,j}\\
    &&&\Delta\beta_{k,j}\triangleq 
    \left(\frac{ y_{k+1,j}^* -  y_{k,j}^*}{\budget_j}\right)
    f_k\left(\frac{ y_{k+1,j}^*}{\budget_j}\right)
\end{align*}
For the last stage $K$, note that $F_K(x)=0$
for all $x\in[0,1]$. Therefore, \Cref{alg:adwords fractional} essentially solves the maximum AdWords problem in the last stage graph $(\Rider_K, \Driver, E_K)$ where each $j\in\Driver$ has initial budget $\budget_j- y^*_{K, j}$. Let $\{\hat{\alpha}_{K,i}, \hat{\beta}_{K,j}\}_{i\in\Rider_K,j\in\Driver}$ 
be the \emph{optimal} dual solution of this LP. Then update the  dual variables as follows:
\begin{align*}
&\forall i\in\Rider_K:~~\alpha_i \gets \hat{\alpha}_{K,i} \\
&\forall j\in \Driver~:~~\beta_j\gets \beta_j+\Delta \beta_{K,j},~~\Delta\beta_{K, j} \triangleq \left(1 - 
\frac{ y^*_{K, j}}{\budget_j}\right)\hat{\beta}_{K,j}
\end{align*}

\noindent[\textit{Step \rom{2}}]~\emph{Comparing objective values in primal and dual.}
we first show that 
the objective value of the above dual assignment
is equal to the objective value of the primal assignment of \Cref{alg:adwords fractional}.
To show this, we consider 
each stage $k$ separately.
For the last stage $K$, 
this holds by construction.
For each stage $k < K$, note that the primal objective value is decomposed across pairs $(\Rider_k^{(l)}, \Driver_k^{(l)})$, $l=0,1$, simply because $x^*_{k,ij}>0$ only if $i$ and $j$ belong to the same pair (\Cref{lemma:structure adwords}). As these pairs partition sets of vertices $\Rider$ and $\Driver$, it is enough to compare the changes in the primal and dual objectives in each pair $(\Rider_k^{(l)}, \Driver_k^{(l)})$ separately. 
Notice that if $i \in \Rider_k^{(0)}$ then 
$c_{k, i} = 0$, and thus,
\begin{align*}
    \Delta(\textrm{Dual})^{(0)}\triangleq\sum_{i \in \Rider^{(0)}_k} \alpha_i
    +
    \sum_{j \in \Driver^{(0)}_k} \budget_j\Delta\beta_{k,j}
    &= 
    \sum_{j \in \Driver^{(0)}_k}\sum_{i:(i,j)\in E_0} b_{ij}x_{k, ij}^*\triangleq\Delta(\textrm{Primal})^{(0)}. 
\end{align*}
Similarly, 
\begin{align*}
     \Delta(\textrm{Dual})^{(1)}&\triangleq
     \sum_{i \in \Rider^{(1)}_k} \alpha_i
    +
    \sum_{j \in \Driver^{(1)}_k}\budget_j \Delta\beta_{k,j}
    =
    \sum_{i \in \Rider^{(1)}_k} c_{k,i}
    +
    \sum_{j \in \Driver^{(1)}_k}\sum_ {i:(i,j)\in E_k} 
    b_{ij}x_{k, ij}^*f_k\left(\frac{y_{k+1,j}^*}{\budget_j}\right)
    \\
    &=
    \sum_{i \in \Rider^{(1)}_k} c_{k,i}
    +
    \sum_{j \in \Driver^{(1)}_k}\sum_ {i:(i,j)\in E_k} 
    x_{k, ij}^*\left(b_{ij} - c_{k,i}\right)\\
    &=\sum_{j\in\Driver_k^{(1)}}\sum_{i:(i,j)\in E_k} 
    b_{ij}x_{k, ij}^*\triangleq \Delta(\textrm{Primal})^{(1)},
\end{align*}
where the last equality uses the saturation property in \Cref{lemma:structure adwords}.

\noindent[\textit{Step \rom{3}}]~\emph{Checking approximate feasibility of dual.}
To show approximate dual feasibility, it is enough to show that for any stage $k\in[K]$ and any arbitrary edge $(i, j) \in E_k$,
\begin{align}
\label{eq:dual constraint feasibility adwords}
    \alpha_i + \sum_{s = 1}^k b_{ij}\Delta\beta_{s, j}
    \geq 
    b_{ij}\left(1-(1-1/K)^K\right)
\end{align}
We next show \eqref{eq:dual constraint feasibility adwords}
holds for $k=1,2,\ldots,K-1$.
Fix any edge $(i,j)\in E_k$, we have:
\begin{align*}
     &\quad~\alpha_i + \sum_{s = 1}^{k}b_{ij}\Delta\beta_{s, j}\\
     &=c_{k,i} + 
    b_{ij}\left(\frac{y_{k+1,j}^* - 
    y_{k,j}^*}{\budget_j}
    \right)
    f_k\left(\frac{y_{k+1,j}^*}{\budget_j}\right)
    +
    \sum_{s= 1}^{k - 1} 
    b_{ij}\left(\frac{y_{s+1,j}^* - 
    y_{s,j}^*}{\budget_j}
    \right)
    f_s\left(\frac{y_{s+1,j}^*}{\budget_j}\right)
    \\
    &\geq 
    b_{ij}\left(1 - 
    f_k\left(\frac{y_{k+1,j}^*}{\budget_j}\right)
    \right)+ 
    b_{ij}\left(\frac{y_{k+1,j}^* - 
    y_{k,j}^*}{\budget_j}
    \right)
    f_k\left(\frac{y_{k+1,j}^*}{\budget_j}\right)
    +
    \sum_{s= 1}^{k - 1} 
    b_{ij}\left(\frac{y_{s+1,j}^* - 
    y_{s,j}^*}{\budget_j}
    \right)
    f_s\left(\frac{y_{s+1,j}^*}{\budget_j}\right)
    \\
    &\geq b_{ij} \cratio{K}~,
\end{align*}
where the first inequality uses monotonicity property in
\Cref{lemma:structure adwords},
and the second equality 
invokes \Cref{lem:polynomial inequality 2} for the sequence: 
$$
0=y^*_{1,j}/\budget_j\leq y^*_{2,j}/\budget_j\leq \ldots \leq 
y^*_{k,j}/\budget_j\leq 1-\sum_{i':(i',j)\in E_k}
x_{k, i'j}^*/\budget_j~.
$$
% \begin{align*}
%      & c_k^{(l)} + 
%     \left(\sum_{i'\in N_k(j)}x_{k, i'j}^*\right)
%     \left(w_j - c_k^{(l)}\right)
%     +
%     \sum_{s' = 1}^{k - 1} \Delta\beta_{s', j} \\
%     &\leq 
%     c_k^{(l')} + 
%     \left(\sum_{i'\in N_k(j)}x_{k, i'j}^*\right)
%     \left(w_j - c_k^{(l)}\right)
%     +
%     \sum_{s' = 1}^{k - 1} \Delta\beta_{s', j} \\
%     &=
%     \alpha_i + \sum_{s' = 1}^{k}\Delta\beta_{s', j}
% \end{align*}

So far, we have shown \eqref{eq:dual constraint feasibility adwords} 
holds for all stages $k < K$.
For the last stage $K$, and any edge $(i, j) \in E_K$,
notice that 
$\alpha_i+b_{ij}\Delta\beta_{K, j}
=\hat{\alpha}_{K,i} + b_{ij}(1 - y^*_{K, j})
\hat\beta_{K, j} \geq 
b_{ij}(1 - y^*_{K, j})$ by construction.
If $y^*_{K, j} = 0$, 
inequality \eqref{eq:dual constraint feasibility adwords} holds.
Otherwise, let $k' < K$ be the largest 
stage smaller than $K$ 
such that 
$\Delta\beta_{k',j} > 0$. By definition, we know that 
$y^*_{k' + 1, j} = y^*_{K,j}$. So we have:
\begin{align*}
    \alpha_i + \sum_{s = 1}^{K}b_{ij}\Delta\beta_{s, j}
    &\geq    
    b_{ij}(1 - y^*_{K, j})
    + \sum_{s = 1}^{K - 1}b_{ij}\Delta\beta_{s, j} = 
    b_{ij}(1 - y^*_{k'+1, j}) + \sum_{s = 1}^{k'}
    b_{ij}\Delta\beta_{s, j} \\
    &\geq 
    b_{ij}(1 - f_s(y^*_{k' + 1, j}))
    + \sum_{s = 1}^{k'}b_{ij}\Delta\beta_{s, j} 
    \geq b_{ij}(1 - (1 - 1/K)^K)~,
\end{align*}
where the first equality uses the fact $\Delta\beta_{s, j} = 0$ for all $s$
between $k' + 1$ and $K - 1$; the second inequality uses the fact that 
that $f_{s}(a) \geq a$ for all $a\in [0, 1]$ and $s\in[K - 1]$, 
and finally the last inequality holds by exactly the same argument as in the case of $k\in[K-1]$.\ifMS \Halmos \fi

\ifMS
\endproof
\else
\end{proof}
\fi

\ifMS \proof{\textsl{Proof of \Cref{thm:adwords integral}.}}
\else \begin{proof}[Proof of \Cref{thm:adwords integral}]\fi
Let 
$\{x_{k, ij}^*\}_{k\in[K],(i,j)\in E_k}$
be the fractional solution generated in \Cref{alg:adwords integral},
i.e., the optimal solution of the program~\ref{eq:concave-adwords-k}
with adjusted budgets $\{(1-\rho)\budget_j\}_{j\in \Driver}$. 
Based on the proof of \Cref{thm:adwords fractional}
for fractional solutions, we know that 
fractional solution 
$\{x_{k, ij}^*\}_{k\in [K], (i,j)\in E_k}$
is a $\cratio{K}$-approximation to 
the optimal objective in the linear program~\ref{eq:LP-max-weight adwords}
(a.k.a., optimal offline)
with adjusted budgets $\{(1-\rho)\budget_j\}_{j\in \Driver}$. 
Thus, $\{x_{k, ij}^*\}_{k\in [K], (i,j)\in E_k}$ 
is a $(1-\rho)\cratio{K}$-approximation
to the optimal offline with original budgets
$\{\budget_j\}_{j\in \Driver}$. 

Let $\{\hat x_{k, ij}^*\}_{k\in[K],(i,j)\in E_k}$
be the integral solution generated in \Cref{alg:adwords integral}.
For any stage $k\in [K]$,
any edge $(i, j) \in E_k$,
note that 
\begin{align*}
    \prob{\hat x_{k,ij}^* = 1} 
    =
    \prob{\text{vertex $j$ is sampled 
    for vertex $i$}}\cdot 
    \prob{\text{there is enough budget 
    for bid $b_{ij}$}}.
\end{align*}
where $\prob{\text{vertex $j$ is sampled 
    for vertex $i$}} = x_{k,ij}^*$
    by construction.
    Applying the multiplicative form of Chernoff bound 
    (\Cref{lem:chernoff}),
    we can lower-bound 
    $\prob{\text{there is enough budget 
    for bid $b_{ij}$}}$
    by $1 - 
    \exp\left(
    -\frac{\rho^2\minbudget}{2-\rho}\right)$.
    Thus, the integral solution
    $\{\hat x_{k, ij}^*\}_{k\in[K],(i,j)\in E_k}$ 
    is $(1 - \rho)(1 - 
    \exp\left(
    -\frac{\rho^2\minbudget}{2-\rho}\right))$-approximation to the optimal offline. 
    Finally, setting 
    $\rho = O\left(\sqrt{\frac{\log(\minbudget)}{\minbudget}}\right)$ 
    for a large enough constant in the big O notation
    finishes the proof.\ifMS \Halmos \fi

\ifMS
\endproof
\else
\end{proof}
\fi

\begin{lemma}[Multiplicative Chernoff Bound, \citealp{C-1952}]
\label{lem:chernoff}
Suppose $X_1,X_2,\ldots,X_t$ are independent random variables taking values in $\{0,1\}$. Let $X$ denote their sum and let $\mu=\expect[]{X}$ denote the sum's expected value. Then for any $\delta>0$,
$$
\prob{X> (1+\delta)\mu}\leq \exp\left(-\frac{\delta^2\mu}{2+\delta}\right)
$$
\end{lemma}

==> FN_ multi-stage matching + configuration allocation (MS Journal)/tex/apx-algorithms.tex <==
Here we present the algorithms 
for the extensions,
i.e.,
the multi-stage vertex weighted b-matching problem
and 
the multi-stage AdWords problem.

\begin{algorithm}
 	\caption{Polynomial Regularized Max Weight b-Matching (\PRMWBM)}
 	\label{alg:b-matching integral}
 	\KwIn{Number of batches/stages $K$,
 	Integral solution flag $\texttt{\textsl{Flag}}$.}
%  	\vspace{1mm}
%  	\KwOut{SS.}
 	    \vspace{2mm}
 	    
    $\forall j\in\Driver:~y_j\gets 0$.

 	\vspace{1mm}
 	\For{stage $k=1$ to $K$}
 	{
 	\vspace{2mm}
 	\tcc{$k^{\textrm{th}}$ batch of vertices in $\Rider$, denoted by $\Rider_k$, arrives. Let $E_k$ denote the set of edges incident to vertices in $\Rider_k$.}
 	\vspace{2mm}
 	
   Given $\{y_j\}_{j\in \Driver}$ and subgraph $G_k=(\Rider_k,\Driver,E_k)$, solve $\xbf_k^*$ from
   the convex program~\ref{eq:concave-k-bmatching integral}.

\If{$\texttt{Flag} == \text{False}$}{
$\forall j\in \Driver: y_j\gets y_j+\displaystyle\sum_{i\in\Rider_k}x^*_{k,ij}$.

Return $\xbf^*_k$ as the fractional b-matching allocation of stage $k$.
}
\Else{
Given $\xbf^*_k$, and
structural decomposition 
$\{(\Rider_k^{(l)}, \Driver_k^{(l)}\}_{l\in [0:L_k]}$, 
solve optimal vertex $\hat\xbf_k^*$ from
the linear program~\ref{eq:rounding k-bmatching} for all $l\in [0:L_k]$.

$\forall j\in \Driver: y_j\gets y_j+\displaystyle\sum_{i\in\Rider_k}\hat x^*_{k,ij}$.

Return $\hat\xbf^*_k$ as the integral b-matching allocation of stage $k$.
}
}
\end{algorithm}


\begin{algorithm}
 	\caption{Polynomial Regularized Fractional AdWords (\PRFAD)}
 	\label{alg:adwords fractional}
 	\KwIn{Number of batches/stages $K$}
%  	\vspace{1mm}
%  	\KwOut{SS.}
 	    \vspace{2mm}
 	    
    $\forall j\in\Driver:~y_j\gets 0$.

 	\vspace{1mm}
 	\For{stage $k=1$ to $K$}
 	{
 	\vspace{2mm}
 	\tcc{$k^{\textrm{th}}$ batch of vertices in $\Rider$, denoted by $\Rider_k$, arrives. Let $E_k$ denote the set of edges incident to vertices in $\Rider_k$.}
 	\vspace{2mm}
 	



   Given $\{y_j\}_{j\in \Driver}$ and subgraph $G_k=(\Rider_k,\Driver,E_k)$, solve $\xbf_k^*$
   from
   the convex program~\ref{eq:concave-adwords-k}.

$\forall j\in \Driver: y_j\gets y_j+\displaystyle\sum_{i\in\Rider_k}b_{ij}x^*_{k,ij}$.

Return $\xbf^*_k$ as the fractional AdWords allocation of stage $k$.

}
\end{algorithm}

\begin{algorithm}
 	\caption{Polynomial Regularized Integral AdWords (\PRIAD)}
 	\label{alg:adwords integral}
 	\KwIn{Number of batches/stages $K$, parameter $\rho\in[0,1]$}
%  	\vspace{1mm}
%  	\KwOut{SS.}
 	    \vspace{2mm}
 	    
    $\forall j\in\Driver:~y_j\gets 0,
    \hat y_j \gets 0$.
    
%     $\rho = \underset{\rho\in[0,1]}{\argmin}
% ~1-\left(1-\rho\right)\left(1 - \exp\left(-\frac{\rho^2\minbudget}
%     {2-\rho}\right)\right)$.

 	\vspace{1mm}
 	\For{stage $k=1$ to $K$}
 	{
 	\vspace{2mm}
 	\tcc{$k^{\textrm{th}}$ batch of vertices in $\Rider$, denoted by $\Rider_k$, arrives. Let $E_k$ denote the set of edges incident to vertices in $\Rider_k$.}
 	\vspace{2mm}
 	

    Given $\{y_j\}_{j\in \Driver}$ and subgraph  $G_k=(\Rider_k,\Driver,E_k)$, solve $\xbf_k^*$
   from
   the convex  program~\ref{eq:concave-adwords-k} with
    adjusted budgets $\{(1-\rho)\budget_j\}_{j\in \Driver}$,
    and used budgets $\{y_j\}_{j\in \Driver}$.
    
    $\hat\xbf_k^* \gets \mathbf 0$.
    
 	\For{online vertex $i \in \Rider_k$}{
 	Sample offline vertex $j\sim \{x_{k,ij}^*\}_{j:(i,j)\in E_k}$.
 	
 	\If{$\hat y_j + b_{ij} \leq \budget_j$}{
 	    $\hat x_{k,ij}^* \gets 1$.
 	    
 	    $\hat y_j \gets \hat y_j + b_{ij}$.
 	}
 	}

$\forall j\in \Driver: y_j\gets y_j+\displaystyle\sum_{i\in\Rider_k} b_{ij}x^*_{k,ij}$.

Return $\hat\xbf^*_k$ as the integral AdWords allocation of stage $k$.

}
\end{algorithm}

==> FN_ multi-stage matching + configuration allocation (MS Journal)/tex/apx-b-matching-proof.tex <==
\subsection{Proof of \texorpdfstring{\Cref{thm:b-matching integral}}{Lg}}
\label{apx:b-matching}

The proofs of the competitive ratio of the fractional
solution in \Cref{thm:b-matching integral}
is similar to 
the analog
proof in \Cref{sec:vertex-weight}.
Thus, we omit it and only show  
the proof of the competitive ratio of 
the integral solution in \Cref{thm:b-matching integral}.






\ifMS \proof{\textsl{Proof of \Cref{thm:b-matching integral} for integral solutions.}}
\else \begin{proof}[Proof of \Cref{thm:b-matching integral} for integral solutions]\fi
For each stage $k\in[K-1]$, let $\{(\Rider^{(0)}_k, \Driver^{(0)}_k),\dots, (\Rider^{(L_k)}_k, \Driver^{(L_k)}_k)\}$ be the 
structural decomposition of $(\Rider_k, \Driver, E_k)$ as in \Cref{lemma:structure budgeted allocation},
and $\{x_{k, ij}^*\}_{(i,j)\in E_k}$
be the optimal (fractional) solution of the program~\ref{eq:concave-k-bmatching integral}
and $\{\hat x_{k, ij}^*\}_{(i,j)\in E_k}$
be the optimal (integral) solution of the 
program~\ref{eq:rounding k-bmatching}. 
First, we define the following notations which will be useful in this proof:
\begin{align*}
\forall j\in \Driver,~k\in[K]:\quad\quad\quad 
&\hat y^*_{k,j}\triangleq\sum_{s=1}^{k-1}\sum_{i:(i,j)\in E_s}
\hat x^*_{s,ij},
\quad\quad\quad 
y^*_{k,j}\triangleq\sum_{s=1}^{k-2}\sum_{i:(i,j)\in E_s}
\hat x^*_{s,ij} + 
\sum_{i:(i,j)\in E_{k-1}}x^*_{k-1,ij}
% ,\\
%  &y^*_{0,j}=0.
\end{align*}

Now consider the offline primal-dual linear program \ref{eq:LP-max-weight b-matching}.
\begin{equation}
\tag{\textsc{Primal-Dual-bmatching}}
\label{eq:LP-max-weight b-matching}
\arraycolsep=1.4pt\def\arraystretch{1}
\begin{array}{llllllll}
\max\quad\quad\quad&\displaystyle\sum_{(i,j)\in E}w_jx_{ij} &~~\text{s.t.}&
&\quad\quad\text{min}\quad\quad\quad &\displaystyle\sum_{i\in \Rider }{\alpha_i}+\displaystyle\sum_{j\in \Driver}{\budget_j\beta_j}&~~\text{s.t.} \\[1.4em]
 &\displaystyle\sum_{j:(i,j)\in E}{x_{ij}}\leq1 &~~i\in\Rider~,& 
& &\alpha_i+\beta_j\geq w_j& (i,j)\in E~,\\[1.4em]
 &\displaystyle\sum_{i:(i,j)\in E}{x_{ij}}\leq \budget_j &~~j\in \Driver~, &
& &\alpha_i\geq 0 &i\in \Rider~, \\
 &x_{ij} \geq 0 &(i,j)\in E~. &
& &\beta_j\geq 0  &j\in \Driver~. 
\end{array}
\end{equation}
Once again, 
given the feasible primal (integral) assignment $\{\hat\xbf^*_k\}_{k\in[K]}$ produced by \Cref{alg:b-matching integral}, we construct a dual assignment so that,
\begin{itemize}
    \item Primal and dual have the same objective values: $\displaystyle\sum_{k\in[K]}\displaystyle\sum_{(i,j)\in E_k}w_j\hat x^*_{k,ij}=\sum_{i\in\Rider}\alpha_i+\sum_{j\in\Driver}\budget_j\beta_j$~,
    \item Dual is approximately feasible: $\forall (i,j)\in E: \alpha_i+\beta_j\geq (\cratio{K} - O(1/\minbudget))\cdot w_j$~.
\end{itemize}

\noindent[\textit{Step \rom{1}}]~\emph{Dual assignment construction.}
First, set $\alpha_i\gets 0$ and $\beta_j\gets 0$ for all $i\in\Rider,j\in \Driver$. At each stage $k\in[0:K-1]$, update the dual variables as follows:
\begin{align*}
   &\forall i \in \Rider^{(l)}_k,~l\in[0:L_k]: &&
   \alpha_i\gets \frac{1}{|\Rider^{(l)}_k|}
   \sum_{j\in \Driver_k^{(l)}}
       \left({\hat y_{k+1,j}^* - \hat y_{k,j}^*}\right)
    \left(1 - 
    f_k\left(\frac{\hat y_{k+1,j}^* - 1}{\budget_j}\right)
   \right)w_j
   \\
    &\forall j \in \Driver^{(l)},~l\in[0:L_k]: &&\beta_{j}\gets\beta_{j}+\Delta\beta_{k,j}\\
    &&&\Delta\beta_{k,j}\triangleq 
    \left(\frac{\hat y_{k+1,j}^* - \hat y_{k,j}^*}{\budget_j}\right)
    f_k\left(\frac{\hat y_{k+1,j}^* - 1}{\budget_j}\right)
    w_j 
\end{align*}
For the last stage $K$, note that $F_K(x)=0$
for all $x\in[0,1]$. Therefore, \Cref{alg:b-matching integral} essentially solves the maximum vertex weighted b-matching in the last stage graph $(\Rider_K, \Driver, E_K)$ where each $j\in\Driver$ has initial capacity $\budget_j-\hat y^*_{K, j}$. Let $\{\hat{\alpha}_{K,i}, \hat{\beta}_{K,j}\}_{i\in\Rider_K,j\in\Driver}$ 
be the \emph{optimal} dual solution of this LP. Then update the  dual variables as follows:
\begin{align*}
&\forall i\in\Rider_K:~~\alpha_i \gets \hat{\alpha}_{K,i} \\
&\forall j\in \Driver~:~~\beta_j\gets \beta_j+\Delta \beta_{K,j},~~\Delta\beta_{K, j} \triangleq \left(1 - 
\frac{\hat y^*_{K, j}}{\budget_j}\right)\hat{\beta}_{K,j}
\end{align*}

\noindent[\textit{Step \rom{2}}]~\emph{Comparing objective values in primal and dual.}
Note that by construction, the objective values in
primal and dual are equal (for each stage).

\noindent[\textit{Step \rom{3}}]~\emph{Checking approximate feasibility of dual.}
To show approximate dual feasibility, it is enough to show that for any stage $k\in[K]$ and any arbitrary edge $(i, j) \in E_k$,
\begin{align}
\label{eq:dual constraint feasibility b-matching}
    \alpha_i + \sum_{s = 1}^k\Delta\beta_{s, j}
    \geq 
    w_j\left(1-(1-1/K)^K - 3/\minbudget\right)
\end{align}
We next show inequality \eqref{eq:dual constraint feasibility b-matching}
holds for $k \in [K-1]$ 
and $k = K$ with slightly different arguments.
For any $k \in [K - 1]$, $l\in [0:L_k]$,
fix any edge $(\iprime, \jprime) \in E_k$
with 
online vertex $\iprime \in \Rider_k^{(l)}$.
We next 
show the following three inequalities \eqref{eq:dual constraint feasibility budgeted allocation fractional solution},
\eqref{eq:budgeted allocation alpha lower bound} 
and 
\eqref{eq:budgeted allocation beta lower bound}
hold. 
% (i) show that 
\begin{align}
\label{eq:dual constraint feasibility budgeted allocation fractional solution}
\begin{split}
    \frac{1}{|\Rider^{(l)}_k|}
    &\sum_{j\in \Driver^{(l)}_k}
    % \left(
    \left(y_{k+1,j}^* - \hat y_{k,j}^*\right)
    \left(1
    - 
    f_k\left(
    \frac{y_{k+1,j}^*}{\budget_{j}}
    \right)
    \right)
    w_j
    % \right) 
    \\
    &+
    \sum_{s = 1}^{k-1}
        \left(
    \frac{\hat y_{s+1,\jprime}^* - \hat y_{s, \jprime}^*}
    {\budget_{\jprime}}
    \right)\cdot 
     f_s
    \left(
    \frac{\hat y_{s + 1,\jprime}^*}
    {\budget_\jprime}\right)w_\jprime
    +
    \left(
    \frac{ y_{k+1,\jprime}^* -  \hat y_{k, \jprime}^*}
    {\budget_{\jprime}}
    \right)\cdot 
     f_k
    \left(
    \frac{ y_{k + 1,\jprime}^*}
    {\budget_{\jprime}}\right)w_\jprime \\
    &\qquad\qquad\qquad 
    \geq \left(1 - (1-1/K)^K\right)w_\jprime
    \end{split}
\end{align}
% (ii) shoaw that
and
\begin{align}
\label{eq:budgeted allocation alpha lower bound}
    \alpha_\iprime \geq 
    \frac{1}{|\Rider^{(l)}_k|}
    &\sum_{j\in \Driver^{(l)}_k}
    % \left(
    \left(y_{k+1,j}^* - \hat y_{k,j}^*\right)
    \left(1
    - 
    f_k\left(
    \frac{y_{k+1,j}^*}{\budget_{j}}
    \right)
    \right)
    w_j
    % \right) 
\end{align}
% and (iii) show that
and
\begin{align}
\label{eq:budgeted allocation beta lower bound}
\begin{split}
    &\sum_{s = 1}^k\Delta\beta_{s, \jprime} +
    \frac{3w_\jprime}{\budget_\jprime} 
    \\
    &\geq  
\sum_{s = 1}^{k-1}
        \left(
    \frac{\hat y_{s+1,\jprime}^* - \hat y_{s, \jprime}^*}
    {\budget_{\jprime}}
    \right)\cdot 
     f_s
    \left(
    \frac{\hat y_{s + 1,\jprime}^*}
    {\budget_\jprime}\right)w_\jprime
    +
    \left(
    \frac{ y_{k+1,\jprime}^* -  \hat y_{k, \jprime}^*}
    {\budget_{\jprime}}
    \right)\cdot 
     f_k
    \left(
    \frac{ y_{k + 1,\jprime}^*}
    {\budget_{\jprime}}\right)w_\jprime 
    \end{split}
\end{align}
Note that combining inequalities \eqref{eq:dual constraint feasibility budgeted allocation fractional solution},
\eqref{eq:budgeted allocation alpha lower bound} 
and 
\eqref{eq:budgeted allocation beta lower bound}
finishes the argument for inequality \eqref{eq:dual constraint feasibility b-matching}
on edge $(\iprime, \jprime) \in E_k$ with $k\in [K-1]$. 

\textsl{Proof of inequality \eqref{eq:dual constraint feasibility budgeted allocation fractional solution}.}
Let $l'\in [0:L_k]$ be the index s.t. 
offline vertex $\jprime \in \Driver_k^{(l')}$.
Due to monotonicity property
in \Cref{lemma:structure budgeted allocation},
we have 
$l \geq l'$ and $c_k^{(l)} \geq c_k^{(l')}$.
First, note that 
\begin{align*}
    c_k^{(l)} = 
    \frac{1}{|\Rider^{(l)}_k|}
    &\sum_{j\in \Driver^{(l)}_k}
    % \left(
    \left(y_{k+1,j}^* - \hat y_{k,j}^*\right)
    \left(1
    - 
    f_k\left(
    \frac{y_{k+1,j}^*}{\budget_{j}}
    \right)
    \right)
    w_j
\end{align*}
due to uniformity and saturation in \Cref{lemma:structure budgeted allocation}.\footnote{For $l = 0$,
the construction of $(\Rider_k^{(0)},\Driver_k^{(0)})$
suggests that 
$y_{k+1,j}^* = \budget_j$ for all $j \in \Driver_k^{(0)}$,
and thus
$\bar f_k\left(
    \frac{y_{k+1,j}^*}{\budget_{j}}
    \right) = 1$, which implies that
    the right hand side equals $c_k^{(0)} = 0$.
    For $l \in [L_k]$,
    since
    $\sum_{j\in \Driver_k^{(l)}}
    \left(y_{k+1,j}^* - \hat y_{k,j}\right) = 
    |\Rider_k^{(l)}|$ (due to saturation) and 
    for all $j\in \Driver_k^{(l)}$
    $w_{j}
    \left(1
    - 
    f_k\left(
    \frac{y_{k+1,j}^* - \hat y_{k,j}^*}
    {\budget_{j}}
    \right)
    \right) = c_k^{(l)}$ (due to uniformity),
    the right hand side equals $c_k^{(l)}$.
}
Hence, 
we can rewrite 
inequality \eqref{eq:dual constraint feasibility budgeted allocation fractional solution}
as 
\begin{align*}
    &c_k^{(l)} +    
    \sum_{s = 1}^{k-1}
        \left(
    \frac{\hat y_{s+1,\jprime}^* - \hat y_{s, \jprime}^*}
    {\budget_{\jprime}}
    \right)\cdot 
     f_s
    \left(
    \frac{\hat y_{s + 1,\jprime}^*}
    {\budget_\jprime}\right)w_\jprime
    +
    \left(
    \frac{ y_{k+1,\jprime}^* -  \hat y_{k, \jprime}^*}
    {\budget_{\jprime}}
    \right)\cdot 
     f_k
    \left(
    \frac{ y_{k + 1,\jprime}^*}
    {\budget_{\jprime}}\right)w_\jprime \\
    &\qquad\qquad\qquad 
    \geq \left(1 - (1-1/K)^K\right)w_\jprime
\end{align*}
which holds since $c_k^{(l)} \geq c_k^{(l')}$
and \Cref{lem:polynomial inequality 2}
for the sequence
$$
0=\hat y^*_{1,\jprime} / \budget_\jprime\leq 
\hat y^*_{2,\jprime}/ \budget_\jprime\leq \ldots \leq 
\hat y^*_{k,\jprime}/ \budget_\jprime\leq 1-\sum_{i:(i,\jprime)\in E_k}
x_{k, i\jprime}^*/ \budget_\jprime~.
$$

\textsl{Proof of inequality \eqref{eq:budgeted allocation alpha lower bound}.}
Since $f_k(\cdot)$ is weakly increasing,
and $y_{k+1,j}^* \geq \hat y_{k+1,j}^* - 1$ by construction,
we have 
$
    f_k\left(
    \frac{y_{k+1,j}^*}{\budget_{j}}
    \right) \geq 
     f_k\left(
    \frac{\hat y_{k+1,j}^* - 1}{\budget_{j}}
    \right)$.
    Thus,
    \begin{align*}
        \alpha_\iprime
        &= \frac{1}{|\Rider^{(l)}_k|}
   \sum_{j\in \Driver_k^{(l)}}
       \left({\hat y_{k+1,j}^* - \hat y_{k,j}^*}\right)
    \left(1 - 
    f_j\left(\frac{\hat y_{k+1,j}^* - 1}{\budget_j}\right)
   \right)w_j \\
   & \geq 
   \frac{1}{|\Rider^{(l)}_k|}
   \sum_{j\in \Driver_k^{(l)}}
       \left({\hat y_{k+1,j}^* - \hat y_{k,j}^*}\right)
    \left(1 - 
    f_j\left(\frac{ y_{k+1,j}^*}{\budget_j}\right)
   \right)w_j \\
   &=
       \frac{1}{|\Rider^{(l)}_k|}
    \sum_{j\in \Driver^{(l)}_k}
    % \left(
    \left(y_{k+1,j}^* - \hat y_{k,j}^*\right)
    \left(1
    - 
    f_k\left(
    \frac{y_{k+1,j}^*}{\budget_{j}}
    \right)
    \right)
    w_j
    \end{align*}
    where
    the last equality uses 
    the fact that 
    $\sum_{j\in \Driver^{(l)}_k}
    % \left(
    \left(\hat y_{k+1,j}^* - \hat y_{k,j}^*\right) = 
    \sum_{j\in \Driver^{(l)}_k}
    % \left(
    \left(y_{k+1,j}^* - \hat y_{k,j}^*\right)$
    (by the construction of $\hat \xbf^*$)
    and 
    uniformity in \Cref{lemma:structure budgeted allocation}.

\textsl{Proof of inequality \eqref{eq:budgeted allocation beta lower bound}.}
We start with the right hand side of inequality
\eqref{eq:budgeted allocation beta lower bound},
\begin{align*}
            &
\sum_{s = 1}^{k-1}
        \left(
    \frac{\hat y_{s+1,\jprime}^* - \hat y_{s, \jprime}^*}
    {\budget_{\jprime}}
    \right)\cdot 
     f_s
    \left(
    \frac{\hat y_{s + 1,\jprime}^*}
    {\budget_\jprime}\right)w_\jprime
    +
    \left(
    \frac{ y_{k+1,\jprime}^* -  \hat y_{k, \jprime}^*}
    {\budget_{\jprime}}
    \right)\cdot 
     f_k
    \left(
    \frac{ y_{k + 1,\jprime}^*}
    {\budget_{\jprime}}\right)w_\jprime 
    \\
    \leq &
\sum_{s = 1}^{k-1}
        \left(
    \frac{\hat y_{s+1,\jprime}^* - \hat y_{s, \jprime}^*}
    {\budget_{\jprime}}
    \right)\cdot 
     f_s
    \left(
    \frac{\hat y_{s + 1,\jprime}^*}
    {\budget_\jprime}\right)w_\jprime
    +
    \left(
    \frac{\hat y_{k+1,\jprime}^* -  \hat y_{k, \jprime}^*}
    {\budget_{\jprime}}
    \right)\cdot 
     f_k
    \left(
    \frac{ y_{k + 1,\jprime}^*}
    {\budget_{\jprime}}\right)w_\jprime 
    +
    \frac{w_\jprime}{\budget_\jprime}
    \\
    \leq&
\sum_{s = 1}^{k-1}
        \left(
    \frac{\hat y_{s+1,\jprime}^* - \hat y_{s, \jprime}^*}
    {\budget_{\jprime}}
    \right)\cdot 
    \left(
     f_s
    \left(
    \frac{\hat y_{s + 1,\jprime}^* - 1}
    {\budget_\jprime}\right)
    +
    \frac{1}{\budget_\jprime}
    \right)w_\jprime \\
    &\qquad\qquad\qquad\qquad\qquad\qquad
    +
    \left(
    \frac{\hat y_{k+1,\jprime}^* -  \hat y_{k, \jprime}^*}
    {\budget_{\jprime}}
    \right)\cdot 
    \left(
     f_k
    \left(
    \frac{\hat y_{k + 1,\jprime}^* - 1}
    {\budget_{\jprime}}\right)
    + \frac{2}{\budget_\jprime}
    \right)
    w_\jprime 
    +
    \frac{w_\jprime}{\budget_\jprime}
      \\
      =&
      \sum_{s=1}^k \Delta\beta_{s, \jprime}
      +
      \frac{\hat y_{k, \jprime}^*}
      {\budget_\jprime
      }
      \frac{w_\jprime}{\budget_\jprime}
      +
      \frac{\hat y_{k+1, \jprime}^*
      -\hat y_{k, \jprime}^*}
      {\budget_\jprime}
      \frac{2w_\jprime}{\budget_\jprime}
      +
      \frac{w_\jprime}{\budget_\jprime}
      \leq 
      \sum_{s=1}^k \Delta\beta_{s, \jprime} + \frac{3w_\jprime}{\budget_\jprime}
\end{align*}
where the first inequality 
uses the fact that $f_k(a) \leq 1$ 
for all $a\in[0, 1]$ and 
$\hat y_{k+1,\jprime}^* \geq 
 y_{k+1,\jprime}^*- 1$ by construction;
the second inequality uses the fact that
$f_k'(a) \in [0, 1]$ for all $a \in [0, 1]$.

% Therefore, combining step (i), (ii) and (iii), 
% we finish the argument that inequality \eqref{eq:dual constraint feasibility budgeted allocation}
% holds for $k < K$ case.

In $k = K$ case, 
consider any edge $(\iprime, \jprime) \in E_K$.
Notice that 
$\alpha_\iprime + \Delta\beta_{K, \jprime} \geq 
w_j\left(1 - \frac{\hat y_{K, \jprime}^*}
{\budget_\jprime}\right)$ by construction.
If $\hat y_{K, \jprime}^* = 0$, inequality \eqref{eq:dual constraint feasibility b-matching} holds immediately.
Otherwise, let $k' < K$ be the largest 
stage  
such that 
$\hat y_{k', \jprime}^* < 
\hat y_{k' + 1, \jprime}^* =
\hat y_{K, \jprime}^*$.
By construction, we know that
$\Delta\beta_{s,\jprime} = 0$
for all $s\in [k' + 1, K - 1]$.
Note that
\begin{align*}
    \alpha_i + \sum_{s = 1}^{K}
    \Delta\beta_{s, \jprime}
    &\geq    
    w_j\left(1 - 
    \frac{\hat y_{K, \jprime}^*}
    {\budget_\jprime}\right)
    + \sum_{s = 1}^{K - 1}
    \Delta\beta_{s, \jprime} 
    \\
    &= 
    w_j\left(1 - 
    \frac{\hat y_{k' + 1, \jprime}^*}
    {\budget_\jprime}\right)
    + \sum_{s = 1}^{k'}
    \Delta\beta_{s, \jprime}
    \\
    &\geq
    w_j\left(1 - 
    f_{k'}\left(\frac{\hat y_{k'+1, \jprime}^*}
    {\budget_\jprime}\right)\right)
    + \sum_{s = 1}^{k'}
    \Delta\beta_{s, \jprime}
    \\
    &\geq
    \left(1 - (1 - 1/K)^K\right)w_\jprime - 
    \frac{3w_j}
    {\budget_\jprime}
\end{align*}
where the third inequality uses the fact 
that $f_{s}(a) \geq a$ for all $a\in [0, 1]$
and $s \in [K - 1]$; and 
the fourth inequality uses the similar argument as in 
$k \in [K-1]$ case.\ifMS \Halmos \fi

\ifMS
\endproof
\else
\end{proof}
\fi


==> FN_ multi-stage matching + configuration allocation (MS Journal)/tex/apx-kkt.tex <==
\revcolor{\subsection{Proof of \Cref{lemma:structure}}
 \label{apx:kkt}
 
 We first define the Lagrangian dual function $\Lag_k(\cdot)$ and then re-state the KKT optimality conditions of $\xbf^*_k$ in our specific convex program.
\begin{definition}
\label{def:lagrange}
The \emph{Lagrangian dual} $\Lag_k(.)$ for the concave program~\ref{eq:concave-k-bmatching} is defined as:
\begin{align*}
    \Lag_k(\xbf,\lambdabf,\thetabf,\gammabf)\triangleq& \displaystyle\sum_{j\in \Driver}w_j\left(
        \sum_{i:(i,j)\in E_k}x_{ij} - 
        F_k\left(y_j+
        \sum_{i: (i,j)\in E_k}x_{ij}\right)
        \right) \\
    &-\sum_{i\in \Rider_k}\lambda_i\left(\sum_{j:(i,j)\in E_k}x_{ij}-1\right)
    -\sum_{j\in \Driver}\theta_j\left(\sum_{i:(i,j)\in E_k}x_{ij}+y_j-1\right)
    \\
    &+\sum_{(i,j)\in E_k}\gamma_{ij}x_{ij}~~,
\end{align*}
where $\{\lambda_i\}$, $\{\theta_j\}$, and $\{\gamma_{ij}\}$ are the \emph{Lagrange multipliers}, also known as the \emph{dual variables}, 
corresponding to different constraints 
in program~\ref{eq:concave-k-bmatching}.
\end{definition}
\begin{proposition}[KKT Conditions for Multi-stage Polynomial Regularized Matching]
\label{prop:kkt}
Suppose $\xbf_k^*$ is the optimal solution of the concave program \ref{eq:concave-k-bmatching}. 
Consider the Lagrangian dual $\Lag_k$, as in \Cref{def:lagrange}. Then:
\begin{equation*}
    \underset{\xbf}{\max}~\underset{\lambdabf,\thetabf,\gammabf}{\min}~\Lag_k(\xbf,\lambdabf,\thetabf,\gammabf)= \underset{\lambdabf,\thetabf,\gammabf}{\min}~\underset{\xbf}{\max}~\Lag_k(\xbf,\lambdabf,\thetabf,\gammabf)=\underset{\lambdabf,\thetabf,\gammabf}{\min}~\Lag_k(\xbf_k^*,\lambdabf,\thetabf,\gammabf)~~.
\end{equation*}
Moreover, if $\lambdabf^*$, $\thetabf^*$, and $\gammabf^*$ (together with $\xbf_k^*)$ are the solutions of the above minmax/maxmin, then:
\begin{itemize}
    \item (Stationarity)~~$\forall (i,j)\in E_k:~~\frac{\partial \Lag_k}
    {\partial x_{ij}}(\xbf_k^*,\lambdabf^*,\thetabf^*,\gammabf^*)=0,$
    \item (Dual feasibility)~~$\forall i\in \Rider_k,j\in \Driver,(i,j)\in E_k:~\lambda^*_i\geq 0,~\theta^*_j\geq 0$, and $\gamma^*_{ij}\geq 0$~,
    \item (Complementary slackness)~~$\forall i\in \Rider_k,j\in \Driver,(i,j)\in E_k:$ 
    \begin{itemize}
        \item  $\gamma^*_{ij}=0$ or $\left(\gamma^*_{ij}>0~\textrm{and}~ x^*_{k,ij}=0\right)~,$
        \item $\lambda^*_{i}=0$ or $\left(\lambda^*_{i}>0~\textrm{and}~ \sum_{j: (i,j)\in E_k}x^*_{k,ij}=1\right)~,$
        \item  $\theta^*_{j}=0$ or $\left(\theta^*_{j}>0~\textrm{and}~ y_j+\sum_{i: (i,j)\in E_k}x^*_{k,ij} =1\right)~.$
    \end{itemize}
\end{itemize}
\end{proposition}
With the above ingredients, we prove the structural lemma.

\ifMS \proof{\textsl{Proof of \Cref{lemma:structure}.}}
\else \begin{proof}[Proof of \Cref{lemma:structure}]\fi
We first show the uniformity property. 
For $j\in \Driver_k^{(0)}$,
note that $$w_j\left(1-
    f_k\left(y_j + \sum_{i:(i,j)\in E_k}x^*_{k,ij}\right)
    \right)
    =w_j(1 - f_k(1))=0=c^{(0)}.$$ 
    For vertices in $\Driver_k^{(l)}$ 
    with $l\in [L_k]$,
    since
    they are in the same connected component of $G_k'[\Rider_k\setminus\Rider_k^{(0)},\Driver\setminus \Driver_k^{(0)}]$,
    it is sufficient to restrict attention to $j, j'\in\Driver_k^{(l)}$
    such that
    there exists a vertex $i\in\Rider_k^{(l)}$ such that $x^*_{k,ij}>0$ and $x^*_{k,ij'}>0$ (and therefore, $\gamma^*_{ij}=\gamma^*_{ij'}=0$, because of the complementary slackness in \Cref{prop:kkt}). Also, $\theta^*_j=\theta^*_{j'}=0$, again because of complementary slackness and the fact that $y_j+\sum_{i:(i,j)\in E_k}x^*_{k,ij}<1$ and $y_{j'}+\sum_{i: (i,j')\in E_k}x^*_{k,ij'}<1$.
Now, applying the stationarity condition in \Cref{prop:kkt}, we have:
$$
w_j\left(1-
    f_k\left(y_j + \sum_{i:(i,j)\in E_k}x^*_{k,ij}\right)
    \right)
-\lambda^*_i-\theta^*_j+\gamma^*_{ij}
=0=
w_{j'}\left(1-
    f_k\left(y_{j'} + \sum_{i: (i,j')\in E_k}x^*_{k,ij'}\right)
    \right)
-\lambda^*_i-\theta^*_{j'}+\gamma^*_{ij'}~,
$$
and therefore 
$w_j\left(1-
    f_k\left(y_j + \sum_{i:(i,j)\in E_k}x^*_{k,ij}\right)
    \right)
    =
    w_{j'}\left(1-
    f_k\left(y_{j'} + \sum_{i: (i,j')\in E_k}x^*_{k,ij'}\right)
    \right)$, 
    finishing the proof of the uniformity property. 
    
    To show saturation property, 
    note that $\lambda^*_i=
    w_j\left(1-
    f_k\left(y_j + \sum_{i:(i,j)\in E_k}x^*_{k,ij}\right)
    \right)>0$ for any $i \in \Rider_k^{(l)}, j \in \Driver_k^{(l)}$ with $l \in[L_k]$ such that $x_{ij}^* > 0$, simply because $f_k(1)=1$ and $f_k(x)$ is (strictly) monotone increasing.
    Again, by using complementary slackness, we have $\sum_{j:(i,j)\in E_k}x^*_{k,ij}=1$, which proves the saturation property.

Now suppose there exists an edge $(i,j')\in E_k$, where $i\in \Rider_k^{(l)}$ and $j'\in \Driver_k^{(l')}$, for $l,l'\in[0:L_k], l\neq l'$. 
First note that there should 
exist a vertex $j\in\Driver_k^{(l)}$ so that $x^*_{k,ij}>0$; this holds because $i$ is either fully matched by $\xbf_k^*$ if $l\in[L_k]$ 
-- thanks to the saturation property --  
or $l=0$ and $i$ is connected to a vertex  $j\in\Driver_k^{(0)}$ with $x^*_{k,ij'}>0$ by definition. 
Because of complementary slackness $\gamma^*_{ij}=0$. 
Now, by writing the stationarity condition of \Cref{prop:kkt} for the edge $(i,j')$, and noting that 
$w_{j'}\left(1-
    f_k\left(y_{j'} + \sum_{i: (i,j')\in E_k}x^*_{k,ij'}\right)
    \right)=c^{(l')}$ 
because of the uniformity property, we have:
$$
c^{(l')}-\lambda^*_i-\theta^*_{j'}+\gamma^*_{ij'}=0~,
$$
By writing the same condition for the edge $(i,j)$ we have: 
$$
c^{(l)} - \lambda^*_i - \theta^*_{j}=0~,
$$
and therefore 
$$
c^{(l)}\geq c^{(l)}-\theta^*_{j}
=c^{(l')}-\theta^*_{j'}+\gamma^*_{ij'}
\geq 
c^{(l')}-\theta^*_{j'}
$$
If $l'=0$, then clearly $c^{(l)}\geq 0= c^{(l')}$. 
If $l'\in [L_k]$, then $\sum_{i': (i',j')\in E_k}x^*_{i'j'}+y_{j'}<1$ 
and $\theta^*_{j'}=0$ because of complementary slackness. Therefore, $c^{(l)}\geq c^{(l')}$, which finishes the proof of the monotonicity property. \ifMS \hfill\Halmos \fi
\ifMS
\endproof
\else
\end{proof}
\fi

\subsection{Proof of \Cref{lem:KKT restate}}
\label{apx:kkt-CA}
Let ($\lambdabf\starred, \thetabf\starred,
\mubf\starred, \pibf\starred,
\psibf\starred,\phibf\starred,\iotabf\starred$)
be the optimal solution in 
the Lagrangian dual program \ref{eq:convex dual}. The property
\ref{eq:cs} 
is satisfied by considering 
the complementary slackness
KKT conditions.
\ref{eq:stationary z}
is due to 
the
stationarity/first-order KKT condition
with respect to $z_{\rider,\config}$.
To show \ref{eq:stationary x}, note that 
the
stationarity/first-order KKT condition
with respect to $x_{\threeindex}$ implies that 
\begin{align*}
    \weight_{\threeindex}
    -
    \sum_{\wi\in[\totalweight]:
    \weightHat(\wi) \leq \weight_{\threeindex}}
    \left(\weightHat_\wi - \weightHat_{\wi-1}\right)
    \cdot 
    f_{k}(\cumcomsumptioni(\xbf\starred, \ybf\starred))
    -
    \thetai\starred 
    - \mui\starred + \psii\starred = 0
\end{align*}
Thus, it is sufficient to show that $\thetai\starred = 0$
for every advertiser $\driver$.
By complementary slackness in KKT conditions,
we know that $\thetai\starred = 0$ if 
$
\cumcomsumption_{\driver,0}(\xbf\starred, \ybf\starred)
~(\equiv
\sum_{\rider\in\Rider_k}
\sum_{\config\in\Config}
         x_{\threeindex}\starred
         +
         \sum_{\wi\in[\totalweight]}
         y_{\twoindex}\starred)~
         < 1$.

Now we consider any advertiser $\driver$ where 
$
\cumcomsumption_{\driver,0}(\xbf\starred, \ybf\starred)
% \sum_{\rider,\config:(\threeindex)\in E_k}
%          x_{\threeindex}\starred
%          +
%          \sum_{\wi\in[\totalweight]}
        %  y_{\twoindex}\starred 
         = 1$.
Let $\taup$ be the smallest index $\tau$ such that
(i) $y_{\driver,\taup}\starred > 0$ or 
(ii) there exists $x_{\threeindex}\starred > 0$ 
with $\weight_{\threeindex} = \weightHat_{\taup}$.
Note that by definition, for any $\wi \leq \taup$,
\begin{align}
\label{eq:full capacity F}
    f_{k}(\cumcomsumptioni(\xbf\starred,\ybf\starred)) &= 
% F\left(
%         \displaystyle\sum\limits_{
%         \substack{\rider,\config:
%         (\threeindex)\in E_k,\\
%         ~~\weight_{\threeindex}\geq 
%         \weightHat_\wi}
%         }
%         x_{\threeindex}
%         +
%         \displaystyle\sum\limits_{\wi' \geq \wi}
%         y_{\driver,\tau'}
%         \right)  
        % =
        f_k(1) = 1
\end{align}
We use similar arguments for both case (i) and case (ii).
\begin{itemize}
    \item Suppose $y_{\driver,\taup}\starred > 0$.   
We have that 
\begin{align*}
    0 
    &\overset{(a)}{=} 
    \weightHat_{\taup} - 
    \sum_{\wi\leq \taup}
    (\weightHat_{\wi} - \weightHat_{\wi - 1})
    \cdot 
    % F_{\twoindex}(\xbf\starred,\ybf\starred)
    f_{k}(\cumcomsumptioni(\xbf\starred,\ybf\starred))
    - \thetai\starred - \pi_{\driver,\taup}\starred 
    + \iota_{\driver,\taup}\starred  
    \\
    & \overset{(b)}{=} 
    \weightHat_{\taup} - 
    \sum_{\wi\leq \taup}
    (\weightHat_{\wi} - \weightHat_{\wi - 1})
    - \thetai\starred - \pi_{\driver,\taup}\starred 
    \overset{(c)}{\leq} 
    -\thetai\starred \overset{(d)}{\leq} 0
\end{align*}
where equation (a) is due to 
the stationarity/first-order KKT condition with respect to 
$y_{\driver,\taup}$;
equation (b) is due to the complementary slackness 
KKT condition (i.e., $\iota_{\driver,\taup}\starred\cdot y_{\driver,\taup}\starred = 0$) 
and equation~\eqref{eq:full capacity F};
and inequality (c) and (d) is due to the non-negativity of 
$\thetai^*$ and $\pi_{\driver,\taup}\starred$.

\item Similarly, suppose 
there exists $x_{\threeindex}\starred > 0$ 
with $\weight_{\threeindex} = \weightHat_{\taup}$. 
Applying the stationarity/first-order KKT condition with respect to 
$x_{\threeindex}\starred$ and invoking 
equation \eqref{eq:full capacity F}, we have
\begin{align*}
    0 
    &\overset{}{=} 
     \weight_{\threeindex}
    -
    \sum_{\wi\in[\totalweight]:
    \weightHat_\wi \leq \weight_{\threeindex}}
    \left(\weightHat_\wi - \weightHat_{\wi-1}\right)
    \cdot 
    % F_{\twoindex}(\xbf\starred, \ybf\starred)
    f_{k}(\cumcomsumptioni(\xbf\starred,\ybf\starred))
    -
    \thetai\starred 
    - \mui\starred + \psii\starred
    \\
    & \overset{}{=} 
    \weightHat_{\taup} - 
    \sum_{\wi\leq \taup}
    (\weightHat_{\wi} - \weightHat_{\wi - 1})
    - \thetai\starred - \mui\starred 
    \overset{}{\leq} 
    -\thetai\starred \overset{}{\leq} 0
\end{align*}
Thus, we conclude that $\thetai\starred = 0$ for all advertiser $\driver$,
and finish the proof of property~\ref{eq:stationary x}.
\halmos
\end{itemize}


\subsection{Proof of \Cref{lem:preempt monotone}}
\label{apx:kkt-CA-smallest}
Let ($\lambdabf\starred, \thetabf\starred,
\mubf\starred, \pibf\starred,
\psibf\starred,\phibf\starred,\iotabf\starred$)
be the optimal solution in 
the Lagrangian dual program \ref{eq:convex dual}.
Suppose $\comsumptioni - y_{\twoindex}^* > 0$
for $\driver\in \Driver$ and $\wi\in[\totalweight]$.
The stationarity/first-order KKT condition with respect to
$y_{\twoindex}$ implies that
\begin{align*}
    \weightHat_{\wi} - 
    \sum_{\wi'\leq \wi}
    (\weightHat_{\wi'} - \weightHat_{\wi' - 1})
    \cdot 
    % F_{\twoindex}(\xbf\starred,\ybf\starred)
    f_{k}(\cumcomsumption_{\driver,\wi'}(\xbf\starred,\ybf\starred))
    - \thetai\starred - \pi_{\driver,\wi}\starred 
    + \iota_{\driver,\wi}\starred  
    = 0
\end{align*}
Note that $\iota_{\twoindex} \geq 0$.
The complementary slackness in
KKT condition implies that 
$\pi_{\twoindex}\starred = 0$
since $\comsumptioni - y_{\twoindex}^* > 0$.
Additionally, as we already 
shown in \Cref{lem:KKT restate},
$\thetai\starred = 0$. Hence,
we have
\begin{align*}
    \weightHat_{\wi} - 
    \sum_{\wi'\leq \wi}
    (\weightHat_{\wi'} - \weightHat_{\wi' - 1})
    \cdot 
    % F_{\twoindex}(\xbf\starred,\ybf\starred)
    f_{k}(\cumcomsumption_{\driver,\wi'}(\xbf\starred,\ybf\starred)) \leq 0
\end{align*}
Since $f_k(a)\leq 1$ for all $a\in[0, 1]$
with equality hold when $a = 1$, we conclude that 
$f_{k}(\cumcomsumption_{\driver,\wi}(\xbf\starred,\ybf\starred)) = 1$ 
and $\cumcomsumption_{\driver,\wi}(\xbf\starred,\ybf\starred) = 1$.
\hfill\halmos

\subsection{Proof of \Cref{coro:cumulative comsumption monoton}}
\label{apx:kkt-CA-cor1}
To see the proof of the first item (\textbf{Distribution Monotonicity)}, by definition, $\cumcomsumptioni(\xbf\starred,\ybf\starred) \geq 
\sum_{\wi'\geq \wi} y_{\driver,\wi'}^*$. Thus
it is sufficient to show the statement when 
$\sum_{\wi'\geq \wi}\left(\comsumption_{\driver,\wi'}\kminused - y_{\driver,\wi'}^*\right) > 0$.
In this case, 
let index $\taup$ be the index such that 
$\taup \geq \wi$ and $\comsumption_{\driver,\wi\primed}\kminused - y_{\driver,\wi\primed}^*>0$.
By \Cref{lem:preempt monotone},
we have $ 
\cumcomsumption_{\driver,\taup}(\xbf\starred,\ybf\starred) = 1$.
Combining with the fact that 
$
\cumcomsumption_{\driver,\wi}(\xbf\starred,\ybf\starred)\geq 
\cumcomsumption_{\driver,\taup}(\xbf\starred,\ybf\starred)
$
and $\sum_{\wi'\geq \wi}\comsumption_{\driver,\wi'}\kminused \leq 1$ finishes the proof of the first item.

For the proof of the second item (\textbf{Only Disposing Smallest}), the argument is similar to \Cref{coro:cumulative comsumption monoton}.
Note that it is sufficient to show the statement 
when 
$\sum_{\wi'\geq \wi}\left(\comsumption_{\driver,\wi'}\kminused - y_{\driver,\wi'}^*\right) > 0$.
In this case, let index $\taup$ be the index such that 
$\taup \geq \wi$ and $\comsumption_{\driver,\wi\primed}\kminused - y_{\driver,\wi\primed}^*>0$.
By \Cref{lem:preempt monotone},
we have $
f_k(\cumcomsumption_{\driver,\taup}(\xbf\starred,\ybf\starred)) = 1$.
Combining with the fact that 
$
f_k(\cumcomsumption_{\driver,\taup}(\xbf\starred,\ybf\starred))
\leq
f_k(\cumcomsumption_{\driver,\wi}(\xbf\starred,\ybf\starred))\leq 1$,
we conclude that 
$f_k(\cumcomsumption_{\driver,\wi}(\xbf\starred,\ybf\starred)) = 1$ which finishes the proof.

\hfill\halmos

\subsection{Proof of \Cref{lem:dual restate theta K}}
\label{apx:last-stage-lemma}
Let $(\xbf\starred,\ybf\starred,\zbf\starred)$
be the optimal solution of the linear program
\ref{eq:convex primal} in the last stage.

Suppose $\weightHat_\wi < \thetai\starred$.
The complementary slackness 
(i.e., $y_{\twoindex}\cdot (\thetai\starred+\pi_{\twoindex\starred} - \weightHat_{\wi}) = 0$)
implies that $y_{\twoindex} = 0$.
Applying the complementary slackness (i.e., 
$\pi_{\twoindex}\starred\cdot(\comsumption_{\twoindex}\KMINUSED - y_{\twoindex}\starred) = 0$)
again, we conclude that $\comsumption_{\twoindex}\KMINUSED\cdot \pi_{\twoindex}\starred = 0$.

Suppose $\weightHat_\wi > \thetai\starred$.
We know that $\pi_{\twoindex}\starred 
\geq \weightHat_\wi - \thetai\starred > 0$.
Then the complementary slackness (i.e., 
$\pi_{\twoindex}\starred\cdot(\comsumption_{\twoindex}\KMINUSED - y_{\twoindex}\starred) = 0$)
suggests that $\comsumption_{\twoindex}\KMINUSED =
y_{\twoindex}\starred$.
Applying the complementary slackness 
(i.e., $y_{\twoindex}\cdot (\thetai\starred+\pi_{\twoindex\starred} - \weightHat_{\wi}) = 0$),
we conclude that 
$ \comsumption_{\twoindex}\KMINUSED
     \cdot 
     (
     \weightHat_{\wi} - \pi_{\twoindex}\starred)
    = 
     \comsumption_{\twoindex}\KMINUSED\cdot \thetai\starred$.
     
     Finally, 
     suppose $\weightHat_\wi = \thetai\starred$.
     As a sanity check, note that 
     equality $\comsumption_{\twoindex}\KMINUSED\cdot \pi_{\twoindex}\starred = 0$
     is equivalent to
     equality 
     $ \comsumption_{\twoindex}\KMINUSED
     \cdot 
     (
     \weightHat_{\wi} - \pi_{\twoindex}\starred)
    = 
     \comsumption_{\twoindex}\KMINUSED\cdot \thetai\starred$.
     If $y_{\twoindex}\starred = 0$,
     following the same argument as 
     the case $\weightHat_\wi < \thetai\starred$
     finishes the proof.
     Otherwise (i.e., $y_{\twoindex}\starred > 0$),
     following the same argument as 
     the case $\weightHat_\wi > \thetai\starred$
     finishes the proof.
\hfill\halmos


\subsection{Proof of \Cref{thm:main result configuration allocation}}
\label{apx:proof-primal-dual-CA}
Consider the suggested dual assignment in \Cref{sec:main proof}. We finish the proof in two steps.

\smallskip
\noindent[\textit{Step \rom{1}}]~\emph{Comparing objective values in primal and dual.}
we first show that 
the objective value of the above dual assignment
is equal to the objective value of the primal assignment of \Cref{alg:opt}.
To show this, we consider 
each stage $k$ separately.
For the last stage $K$, 
this holds by construction.
For each stage $k \in [K-1]$, note that
by \Cref{lem:preempt monotone}
the primal objective value is 
\begin{align*}
    \Delta(\textrm{Primal})\ked = 
    \sum\limits_{\rider\in\Rider_k}
    \sum_{\config\in\Config}
    \sum_{\driver\in\Driver}
    \weight_{\threeindex} \cdot x_{\threeindex}\ked
    -
    \sum_{\driver\in \Driver}
    \sum_{\wi\in[\totalweight]}
    \weightHat_{\wi}\cdot
    \left(\comsumptioni - y_{\twoindex}\ked
    \right)
\end{align*}
To consider the dual objective value, 
we start with the observation that 
\begin{align*}
    \alpha_\rider &= 
   \lambda_\rider\ked\\
   &\overset{(a)}{=} 
    \sum_{\config \in \Config}
   z_{\rider,\config}\ked\cdot 
   \lambda_\rider\ked
   \\
   &\overset{(b)}{=}
    \sum_{\config \in \Config}
   z_{\rider,\config}\ked\cdot 
   \left(
    \sum_{\driver\in \Driver}\alloci \cdot \mui\ked
    + \phii\ked 
    \right)
    \\
    &= 
    \sum_{\config \in \Config}
    \sum_{\driver\in \Driver}
    \alloci\cdot 
    z_{\rider,\config}\ked\cdot 
    \mui\ked
    +
    \sum_{\config \in \Config}
    z_{\rider,\config}\ked\cdot  \phii\ked
    \\
    &\overset{(c)}{=}
    \sum_{\config \in \Config}
    \sum_{\driver\in \Driver}
    x_{\threeindex}\ked\cdot
    \mui\ked   
    \\
    &\overset{(d)}{=}
    \sum_{\config \in \Config}
    \sum_{\driver\in \Driver}
    x_{\threeindex}\ked \cdot 
    \left(
    \weight_{\threeindex}
    -
    \sum_{\wi\in[\totalweight]:
    \weightHat(\wi) \leq \weight_{\threeindex}}
    \left(\weightHat_\wi - \weightHat_{\wi-1}\right)
    \cdot f_k\left(\cumcomsumptioni\ked\right)
    % -
    % \thetai\ked  
    + \psii\ked 
    \right) 
    \\
    &\overset{(e)}{=}
    \sum_{\config \in \Config}
    \sum_{\driver\in \Driver}
    x_{\threeindex}\ked \cdot 
    \left(
    \weight_{\threeindex}
    -
    \sum_{\wi\in[\totalweight]:
    \weightHat(\wi) \leq \weight_{\threeindex}}
    \left(\weightHat_\wi - \weightHat_{\wi-1}\right)
    \cdot f_k\left(\cumcomsumptioni\ked\right)
    % -
    % \thetai\ked  
    \right) 
\end{align*}
Here we heavily use \Cref{lem:KKT restate}:
\ref{eq:cs} for equality~(a)~(c)~(e),
\ref{eq:stationary z} for equality~(b),
and 
\ref{eq:stationary x} for equality~(d).
Thus, we can compute the dual objective as follows,
\begin{align*}
    \Delta(\textrm{Dual})\ked = 
    \sum_{\rider\in \Rider_k}
    \alpha_{\rider} 
    +
    \sum_{\driver\in \Driver}
    \Delta\beta_{\driver}\ked
    =
    \sum\limits_{\rider\in\Rider_k}
    \sum_{\config\in\Config}
    \sum_{\driver\in\Driver}
    \weight_{\threeindex} \cdot x_{\threeindex}\ked
    -
    \sum_{\driver\in \Driver}
    \sum_{\wi\in[\totalweight]}
    \weightHat_{\wi}\cdot
    \left(\comsumptioni - y_{\twoindex}\ked
    \right)
    \equiv
     \Delta(\textrm{Primal})\ked 
\end{align*}

\vspace{1mm}

\noindent[\textit{Step \rom{2}}]~\emph{Checking approximate feasibility of dual.} 
First, we show that all dual assignment are non-negative. 
Note that the non-negativity of $\alphabf$ and $\gammabf$
is guaranteed by construction. 
For $\betabf$, we show that $\Delta\beta_{\driver}\ked\geq 0$
for all $\driver\in \Driver$ and $k\in [K]$.
To see this, note that for any stage $k\in [K - 1]$
\begin{align}
    % \label{eq:beta reformulate}
% \begin{split}
\nonumber
    \Delta\beta_{\driver}\ked
    &=
    \sum_{\rider\in\Rider_k}
    \sum_{\config\in\Config}
    x_{\rider,\config,\driver}\ked
    \left(
    % \theta_{\driver}\ked + 
    \sum_{\wi\in[\totalweight]:
    \weightHat(\wi) \leq \weight_{\rider,\config,\driver}}
    \left(\weightHat_\wi - \weightHat_{\wi-1}\right)
    \cdot 
    f_k\left(\cumcomsumptioni\ked\right)
    \right)
    -
    \sum_{\wi\in[\totalweight]}
    \weightHat_{\wi}\cdot
    \left(\comsumption_{\twoindex}\kminused - y_{\twoindex}\ked
    \right)\\
\nonumber
    &
    \overset{(a)}{=}
    \sum_{\wi\in [\totalweight]}
    \left(\weightHat_\wi - \weightHat_{\wi-1}\right)
    \cdot
    \left(
    \displaystyle\sum\limits_{
        \substack{\rider\in\Rider_k,\config\in\Config:
    \\
        ~~\weight_{\rider,\config,\driver}\geq 
        \weightHat_\wi}
        }
        x_{\rider,\config,\driver}\ked
    \right)
    \cdot 
    % \left(
   f_k\left(\cumcomsumptioni\ked\right)
    % \right)
    -
    \sum_{\wi\in[\totalweight]}
    \left(\weightHat_{\wi} - \weightHat_{\wi-1}\right)\cdot
    % \left(
    \sum_{\wi'\geq \wi}\left(
    \comsumption_{\driver,\wi'}\kminused - y_{\driver,\wi'}\ked
    % \right)
    \right) 
    \\
\nonumber
    &
    \overset{(b)}{=}
    \sum_{\wi\in [\totalweight]}
    \left(\weightHat_\wi - \weightHat_{\wi-1}\right)
    \cdot
    \left(
    \displaystyle\sum\limits_{
        \substack{\rider\in\Rider_k,\config\in\Config:
        % (\rider,\config,\driver)\in E_s,
        \\
        ~~\weight_{\rider,\config,\driver}\geq 
        \weightHat_\wi}
        }
        x_{\rider,\config,\driver}\ked
    \right)
    \cdot 
    % \left(
   f_k\left(\cumcomsumptioni\ked\right)
    % \right)
    -
    \sum_{\wi\in[\totalweight]}
    \left(\weightHat_{\wi} - \weightHat_{\wi-1}\right)\cdot
    % \left(
    \sum_{\wi'\geq \wi}\left(
    \comsumption_{\driver,\wi'}\kminused - y_{\driver,\wi'}\ked
    % \right)
    \right) 
    \cdot 
    f_k\left(\cumcomsumptioni\ked\right)
    \\
    \label{eq:beta reformulate}
    &=
    \sum_{\wi\in [\totalweight]}
    \left(\weightHat_\wi - \weightHat_{\wi-1}\right)
    \cdot
    \left(
    \cumcomsumptioni\ked - \cumcomsumptioni\kminused
    \right)
    \cdot 
    % \left(
   f_k\left(\cumcomsumptioni\ked\right)
    \overset{(c)}{\geq} 0
    % \right)
\end{align}
where (a) is by changing the summation order,
(b) and (c) are due to
\Cref{coro:cumulative comsumption monoton}.
For the last stage $K$,
\begin{align*}
  \begin{split}
    \Delta\beta_{\driver}\KED
    &=
     \thetai\KED 
    -
    \displaystyle\sum_{\driver\in\Driver,\wi\in[\totalweight]}
    \comsumption_{\twoindex}\KMINUSED
    \cdot (\weightHat_{\wi} - \pi_{\twoindex}\KED)
    \overset{(a)}{\geq} 
     \thetai\KED 
    -
    \displaystyle\sum_{\driver\in\Driver,\wi\in[\totalweight]}
    \comsumption_{\twoindex}\KMINUSED
    \cdot \thetai\KED \geq 0
    \end{split}  
\end{align*}
where (a) uses the fact that $\thetai\KED + \pi_{\twoindex}\KED \geq \weightHat_{\wi}$ by definition.

Second, we show that $\alpha_{\rider} \geq 
    \displaystyle\sum_{\driver\in \Driver}
    \alloci \cdot \gamma_{\threeindex}$
    for all $\rider \in \Rider$.
    This inequality is satisfied 
    by the construction of $\alphabf$, $\gammabf$
    and \ref{eq:stationary z} in \Cref{lem:KKT restate}.
    
Finally, to finish the proof, 
it is sufficient for us to show
that for any stage $k\in [K]$
and $(\threeindex)\in E_k$,
\begin{align}
\label{eq:dual feasibility critical}
    \gamma_{\threeindex}
    +
    \sum_{s=1}^k
    \Delta\beta_\driver\sed \geq \cratio{K}\cdot \weight_{\threeindex}
\end{align}
We show inequality \eqref{eq:dual feasibility critical}
holds for any stage $k\in [K - 1]$ and
the last stage $K$ separately.

\vspace{2mm}
Fix an arbitrary stage $k\in[K - 1]$
and $(\threeindex)\in E_k$.
Let $\taup\in [\totalweight]$
be the index that $\weightHat_{\taup}=\weight_{\threeindex}$.
Note that
\begin{align*}
    \gamma_{\threeindex} &= \mui\ked
    \\
    &=
    %  \left(
    \weight_{\threeindex}
    -
    \sum_{\wi\in[\totalweight]:
    \weightHat(\wi) \leq \weight_{\threeindex}}
    \left(\weightHat_\wi - \weightHat_{\wi-1}\right)
    \cdot 
    f_k\left(\cumcomsumptioni\ked\right)
    % -
    % \thetai\ked  
    + \psii\ked  
    \\
    &\geq 
    \weight_{\threeindex}
    -
    \sum_{\wi\in[\totalweight]:
    \weightHat(\wi) \leq \weight_{\threeindex}}
    \left(\weightHat_\wi - \weightHat_{\wi-1}\right)
    \cdot 
    f_k\left(\cumcomsumptioni\ked\right)
    % -
    % \thetai\ked 
    \\
    &=
    \sum_{\wi\leq\taup}
    % \left(
    (\weightHat_{\wi} - \weightHat_{\wi-1})
    \cdot \left(1 - 
    f_k\left(\cumcomsumptioni\ked\right)
    \right)
    % \right)
    % -\thetai\ked
    % \right) 
\end{align*}
Combining with equality \eqref{eq:beta reformulate},
we have 
\begin{align*}
    \gamma_{\threeindex}
    +
    \sum_{s=1}^k
    \Delta\beta_\driver\sed
    \geq 
    \sum_{\wi\leq \taup} 
    (\weightHat_{\wi} - \weightHat_{\wi-1})
    \cdot 
    \left(
    1 - 
    f_k\left(\cumcomsumptioni\ked\right)
    +
    \sum_{s=1}^k
    \left(
    \cumcomsumptioni\ked - \cumcomsumptioni\kminused
    \right)
    \cdot 
    % \left(
   f_k\left(\cumcomsumptioni\ked\right)
    \right)
\end{align*}
Thus, to show
the approximated dual feasibility in
\eqref{eq:dual feasibility critical},
it is sufficient to show
\begin{align*}
    1 - 
    f_k\left(\cumcomsumptioni\ked\right)
    +
    \sum_{s = 1}^k
    \left(
    \cumcomsumptioni\sed - \cumcomsumptioni\sminused
    \right)
    \cdot 
   f_s\left(\cumcomsumptioni\sed\right)
   \geq  \cratio{K}~
   \qquad
   \forall \wi\leq \taup
\end{align*}
which is satisfied as the property of 
$\{f_k\}_{k\in [K]}$ 
by \Cref{lem:polynomial inequality 2} as follows.
% \begin{lemma}[\citealp{FN-21}]
% \label{lem:polynomial inequality}
% Fix any $K\in\N$ and $k\in [K - 1]$.
% For any $0 = a^{(0)} \leq a^{(1)} \leq \dots \leq a^{(k)} \leq 1$,
% % \begin{align*}
% $    1 - f_k\left(a^{(k)}\right) + \sum_{s = 1}^k \left(
%     a\sed - a\sminused
%     \right)
%     \cdot 
%     f_s\left(a\sed\right) 
%     \geq 
%     \cratio{K}.$
% % \end{align*}
% \end{lemma}


\vspace{2mm}
For the last stage $K$, 
fix any $(\threeindex)\in E_K$.
Let $\taup\in [T]$ be the index  
such that $\weightHat_{\taup} = \thetai\KED$.\footnote{Note that 
the optimal solution of the convex program \ref{eq:convex primal} 
as well as the outcome of 
\Cref{alg:opt} 
does not change if we enlarge the revenue level set $\{\weightHat_\wi\}$. 
Thus, it is without loss of generality to assume there exists index
$\taup$ such that $\weightHat_{\taup} = \thetai\KED$.}
% Note that for any $\wi < \taup$,
% we have $y_{\twoindex}\KED = 0$ 
% and thus
% $\pi_{\twoindex}\KED = 0$ 
% if $\comsumption_{\twoindex}\KMINUSED > 0 = y_{\twoindex}\KED$
% because of
% the complementary slackness in 
% program \ref{eq:convex dual K}
% and the definition of index $\taup$.
% Similarly, for any $\wi > \taup$, we have 
% $y_{\twoindex}\KED = \comsumption_{\twoindex}\KMINUSED$
% and thus 
% $\thetai\KED + \pi_{\twoindex}\KED = \weightHat_{\wi}$
% if $y_{\twoindex}\KED = \comsumption_{\twoindex}\KMINUSED > 0$;
% and for $\wi = \taup$, we have $\pi_{\twoindex}\KED = 0$ regardless.
Applying \Cref{lem:dual restate theta K}, we have
\begin{align}
\label{eq:beta K reformulate}
\begin{split}
    \Delta\beta_{\driver}\KED &=
    \thetai\KED 
    - 
    \displaystyle\sum_{\driver\in\Driver,\wi\in[\totalweight]}
    \comsumption_{\twoindex}\KMINUSED
    \cdot (\weightHat_{\wi} - \pi_{\twoindex}\KED)
    \\
    &= 
    \thetai\KED 
    -
    \sum_{\wi \geq \taup}
    \comsumption_{\twoindex}\KMINUSED \cdot \thetai\KED
    - 
    \sum_{\wi< \taup} 
    \comsumption_{\twoindex}\KMINUSED \cdot \weightHat_{\wi}
    \end{split}
\end{align}

We consider two subcases: 
$\weight_{\threeindex} < \thetai\KED$
and
$\weight_{\threeindex} \geq \thetai\KED$.

% Suppose $\weight_{\threeindex} \geq \thetai\KED$, note that 
% \begin{align*}
%     &\gamma_{\threeindex} + \sum_{s = 1}^K \Delta\beta_{\driver}\sed
%     - 
%     \cratio{K}\cdot \weight_{\threeindex}  \\
%     \overset{(a)}{=}~&
%     \mu_{\threeindex}\KED + 
%     \left(
%   \thetai\KED 
%   -
%     \sum_{\wi \geq \taup}
%     \comsumption_{\twoindex}\KMINUSED \cdot \thetai\KED
%     - 
%     \sum_{\wi < \taup} 
%     \comsumption_{\twoindex}\KMINUSED \cdot \weightHat_{\wi}
%     \right)
%     +
%     \sum_{s = 1}^{K-1} \Delta\beta_{\driver}\sed
%     - 
%     \cratio{K}\cdot \weight_{\threeindex}  
%     \\
%     \overset{(b)}{\geq}~&
%     \weight_{\threeindex}
%      -
%     \sum_{\wi \geq \taup}
%     \comsumption_{\twoindex}\KMINUSED \cdot \thetai\KED
%     - 
%     \sum_{\wi < \taup} 
%     \comsumption_{\twoindex}\KMINUSED \cdot \weightHat_{\wi}
%     +
%     \sum_{s = 1}^{K-1} \Delta\beta_{\driver}\sed
%     - 
%     \cratio{K}\cdot \weight_{\threeindex} 
%     \\
%     \overset{(c)}{\geq}~&
%     \thetai\KED
%      -
%     \sum_{\wi \geq \taup}
%     \comsumption_{\twoindex}\KMINUSED \cdot \thetai\KED
%     - 
%     \sum_{\wi < \taup} 
%     \comsumption_{\twoindex}\KMINUSED \cdot \weightHat_{\wi}
%     +
%     \sum_{s = 1}^{K-1} \Delta\beta_{\driver}\sed
%     - 
%     \cratio{K}\cdot\thetai\KED
%     \\
%     =~&
%     \weightHat_{\taup}
%      -
%     \sum_{\wi \geq \taup}
%     \comsumption_{\twoindex}\KMINUSED \cdot \weightHat_{\taup}
%     - 
%     \sum_{\wi < \taup} 
%     \comsumption_{\twoindex}\KMINUSED \cdot \weightHat_{\wi}
%     +
%     \sum_{s = 1}^{K-1} \Delta\beta_{\driver}\sed
%     - 
%     \cratio{K}\cdot\weightHat_{\taup}
%     \\
%     =~&
%     \sum_{\wi\leq \taup} 
%     \left(\weightHat_{\wi} - \weightHat_{\wi-1}\right)
%     \cdot 
%     \left(
%     1 - \cumcomsumption_{\twoindex}\KMINUSED
%     \right)
%     +
%     \sum_{s = 1}^{K-1} \Delta\beta_{\driver}\sed
%     - 
%     \cratio{K}\cdot\weightHat_{\taup}
%     \\
%     \overset{(d)}{\geq}~&
%     \sum_{\wi\leq \taup} 
%     \left(\weightHat_{\wi} - \weightHat_{\wi-1}\right)
%     \cdot 
%     \left(
%     1 - f_{K-1}\left(\cumcomsumption_{\twoindex}\KMINUSED\right)
%     \right)
%     +
%     \sum_{s = 1}^{K-1} \Delta\beta_{\driver}\sed
%     - 
%     \cratio{K}\cdot\weightHat_{\taup}
%     \\
%     \overset{(e)}{\geq}~&
%     0
% \end{align*}
% where (a) uses the construction of $\gamma_{\threeindex}$
% and equality~\eqref{eq:beta K reformulate};
% (b) uses the fact that 
% $\mu_{\threeindex}\KED + \thetai\KED \geq \weight_{\threeindex}$;
% (c) uses the assumption that $\weight_{\threeindex} \geq \thetai\KED$
% and the fact that $\cratio{K} \leq 1$;
% (d) uses the fact that $f_{K-1}(a) \geq a$ for all $a \in[0,1]$;
% and 
% (e) uses the similar argument as the one for stage $k\in [K-1]$.

Suppose $\weight_{\threeindex} < \thetai\KED$. 
Let $\taupp$ be the index such that $\weightHat_\taupp = \weight_{\threeindex}$.
By definition, $\taupp < \taup$.
% Note that in the case, $x_{\threeindex}\KED = 0$
% due to the complementary slackness.
% and for any index $\wi$ such that $\comsumption_{\twoindex}\KMINUSED > 0$
% we have $\wi \geq \taupp$.
\begin{align*}
    &\gamma_{\threeindex} + \sum_{s = 1}^K \Delta\beta_{\driver}\sed
    % - 
    % \cratio{K}\cdot \weight_{\threeindex}  
    \\
    \overset{(a)}{=}~&
    \mu_{\threeindex}\KED + 
    \left(
   \thetai\KED 
    -
    \sum_{\wi \geq \taup}
    \comsumption_{\twoindex}\KMINUSED \cdot \thetai\KED
    - 
    \sum_{\wi < \taup} 
    \comsumption_{\twoindex}\KMINUSED \cdot \weightHat_{\wi}
    \right)
    +
    \sum_{s = 1}^{K-1} \Delta\beta_{\driver}\sed
    % - 
    % \cratio{K}\cdot \weight_{\threeindex}  
    \\
    =~&
    \mu_{\threeindex}\KED + 
    \left(
   \thetai\KED 
    -
    \sum_{\wi \geq \taup}
    \comsumption_{\twoindex}\KMINUSED \cdot \thetai\KED
    - 
    \sum_{\wi =\taupp}^{\taup - 1} 
    \comsumption_{\twoindex}\KMINUSED \cdot \weightHat_{\wi}
    - 
    \sum_{\wi < \taupp} 
    \comsumption_{\twoindex}\KMINUSED \cdot \weightHat_{\wi}
    \right)
    +
    \sum_{s = 1}^{K-1} \Delta\beta_{\driver}\sed
    % - 
    % \cratio{K}\cdot \weight_{\threeindex} 
    \\
    \overset{(b)}{\geq}~&
    \mu_{\threeindex}\KED + 
    \left(
   \thetai\KED 
    -
    \sum_{\wi \geq \taup}
    \comsumption_{\twoindex}\KMINUSED \cdot \thetai\KED
    - 
    \sum_{\wi =\taupp}^{\taup - 1} 
    \comsumption_{\twoindex}\KMINUSED \cdot \thetai\KED
    - 
    \sum_{\wi < \taupp} 
    \comsumption_{\twoindex}\KMINUSED \cdot \weightHat_{\wi}
    \right)
    +
    \sum_{s = 1}^{K-1} \Delta\beta_{\driver}\sed
    % - 
    % \cratio{K}\cdot \weight_{\threeindex} 
    \\
    \overset{}{\geq}~&
    \left(
    1 - \sum_{\wi\geq\taupp}\comsumption_{\twoindex}\KMINUSED
    \right)
    \cdot \left(
    \mu_{\threeindex}\KED + 
   \thetai\KED 
   \right)
    - 
    \sum_{\wi < \taupp} 
    \comsumption_{\twoindex}\KMINUSED \cdot \weightHat_{\wi}
    +
    \sum_{s = 1}^{K-1} \Delta\beta_{\driver}\sed
    % - 
    % \cratio{K}\cdot \weight_{\threeindex} 
    \\
    \overset{(c)}{\geq}~&
    \left(
    1 - \sum_{\wi\geq\taupp}\comsumption_{\twoindex}\KMINUSED
    \right)
    \cdot \weight_{\threeindex}
    - 
    \sum_{\wi < \taupp} 
    \comsumption_{\twoindex}\KMINUSED \cdot \weightHat_{\wi}
    +
    \sum_{s = 1}^{K-1} \Delta\beta_{\driver}\sed
    % - 
    % \cratio{K}\cdot \weight_{\threeindex} 
    \\
    =~&
    \left(
    1 - \cumcomsumption_{\driver,\taupp}\KMINUSED
    \right)
    \cdot \weightHat_{\taupp}
    - 
    \sum_{\wi < \taupp} 
    \comsumption_{\twoindex}\KMINUSED \cdot \weightHat_{\wi}
    +
    \sum_{s = 1}^{K-1} \Delta\beta_{\driver}\sed
    % - 
    % \cratio{K}\cdot \weight_{\threeindex} 
    \\
    =~&
    \sum_{\wi\leq \taupp} 
    \left(\weightHat_{\wi} - \weightHat_{\wi-1}\right)
    \cdot 
    \left(
    1 - \cumcomsumption_{\twoindex}\KMINUSED
    \right)
    +
    \sum_{s = 1}^{K-1} \Delta\beta_{\driver}\sed
    \\
    \overset{(d)}{=}~&
    \sum_{\wi\leq \taupp} 
    \left(\weightHat_{\wi} - \weightHat_{\wi-1}\right)
    \cdot 
    \left(
    1 - f_{K-1}\left(\cumcomsumption_{\twoindex}\KMINUSED\right)
    \right)
    +
    \sum_{s = 1}^{K-1} \Delta\beta_{\driver}\sed
    \\
    \overset{(e)}{\geq}~&
    \cratio{K}\cdot \weightHat_{\taupp}
    =
    \cratio{K}\cdot \weight_{\threeindex}
\end{align*}
where (a) uses the construction of $\gamma_{\threeindex}$
and equality~\eqref{eq:beta K reformulate};
(b) uses the fact that $\weightHat_{\wi} \leq \thetai\KED$
for every $\wi\in[\taupp:\taup - 1]$;
(c) uses the fact that 
$\mu_{\threeindex}\KED + \thetai\KED \geq \weight_{\threeindex}$;
(d) uses the fact that $f_{K-1}(a) = a$ for all $a \in[0,1]$;
and 
(e) uses the similar argument as the one for stage $k\in [K-1]$.

Suppose $\weight_{\threeindex} \geq \thetai\KED$. 
Let $\taupp$ be the index such that $\weightHat_\taupp = \weight_{\threeindex}$.
By definition, $\taupp \geq \taup$.
\begin{align*}
    &\gamma_{\threeindex} + \sum_{s = 1}^K \Delta\beta_{\driver}\sed
    % - 
    % \cratio{K}\cdot \weight_{\threeindex}  
    \\
    \overset{}{=}~&
    \mu_{\threeindex}\KED + 
    \left(
   \thetai\KED 
    -
    \sum_{\wi \geq \taup}
    \comsumption_{\twoindex}\KMINUSED \cdot \thetai\KED
    - 
    \sum_{\wi < \taup} 
    \comsumption_{\twoindex}\KMINUSED \cdot \weightHat_{\wi}
    \right)
    +
    \sum_{s = 1}^{K-1} \Delta\beta_{\driver}\sed
    % - 
    % \cratio{K}\cdot \weight_{\threeindex}  
    \\
    =~&
    \mu_{\threeindex}\KED + 
    \left(
   \thetai\KED 
    -
    \sum_{\wi \geq \taupp}
    \comsumption_{\twoindex}\KMINUSED \cdot \thetai\KED
    - 
    \sum_{\wi =\taup}^{\taupp - 1} 
    \comsumption_{\twoindex}\KMINUSED \cdot \thetai\KED
    - 
    \sum_{\wi < \taup} 
    \comsumption_{\twoindex}\KMINUSED \cdot \weightHat_{\wi}
    \right)
    +
    \sum_{s = 1}^{K-1} \Delta\beta_{\driver}\sed
    % - 
    % \cratio{K}\cdot \weight_{\threeindex} 
    \\
    \overset{(a)}{\geq}~&
    \mu_{\threeindex}\KED + 
    \left(
   \thetai\KED 
    -
    \sum_{\wi \geq \taupp}
    \comsumption_{\twoindex}\KMINUSED \cdot \thetai\KED
    - 
    \sum_{\wi =\taup}^{\taupp - 1} 
    \comsumption_{\twoindex}\KMINUSED \cdot \weightHat_{\wi}
    - 
    \sum_{\wi < \taup} 
    \comsumption_{\twoindex}\KMINUSED \cdot \weightHat_{\wi}
    \right)
    +
    \sum_{s = 1}^{K-1} \Delta\beta_{\driver}\sed
    % - 
    % \cratio{K}\cdot \weight_{\threeindex} 
    \\
    \overset{}{\geq}~&
    \left(
    1 - \sum_{\wi\geq\taupp}\comsumption_{\twoindex}\KMINUSED
    \right)
    \cdot \left(
    \mu_{\threeindex}\KED + 
   \thetai\KED 
   \right)
    - 
    \sum_{\wi < \taupp} 
    \comsumption_{\twoindex}\KMINUSED \cdot \weightHat_{\wi}
    +
    \sum_{s = 1}^{K-1} \Delta\beta_{\driver}\sed
    % - 
    % \cratio{K}\cdot \weight_{\threeindex} 
    % \\
    % \overset{(c)}{\geq}~&
    % \left(
    % 1 - \sum_{\wi\geq\taupp}\comsumption_{\twoindex}\KMINUSED
    % \right)
    % \cdot \weight_{\threeindex}
    % - 
    % \sum_{\wi < \taupp} 
    % \comsumption_{\twoindex}\KMINUSED \cdot \weightHat_{\wi}
    % +
    % \sum_{s = 1}^{K-1} \Delta\beta_{\driver}\sed
    % % - 
    % % \cratio{K}\cdot \weight_{\threeindex} 
    % \\
    % =~&
    % \left(
    % 1 - \cumcomsumption_{\driver,\taupp}\KMINUSED
    % \right)
    % \cdot \weightHat_{\taupp}
    % - 
    % \sum_{\wi < \taupp} 
    % \comsumption_{\twoindex}\KMINUSED \cdot \weightHat_{\wi}
    % +
    % \sum_{s = 1}^{K-1} \Delta\beta_{\driver}\sed
    % % - 
    % % \cratio{K}\cdot \weight_{\threeindex} 
    % \\
    % =~&
    % \sum_{\wi\leq \taupp} 
    % \left(\weightHat_{\wi} - \weightHat_{\wi-1}\right)
    % \cdot 
    % \left(
    % 1 - \cumcomsumption_{\twoindex}\KMINUSED
    % \right)
    % +
    % \sum_{s = 1}^{K-1} \Delta\beta_{\driver}\sed
    % \\
    % \overset{(d)}{\geq}~&
    % \sum_{\wi\leq \taupp} 
    % \left(\weightHat_{\wi} - \weightHat_{\wi-1}\right)
    % \cdot 
    % \left(
    % 1 - f_{K-1}\left(\cumcomsumption_{\twoindex}\KMINUSED\right)
    % \right)
    % +
    % \sum_{s = 1}^{K-1} \Delta\beta_{\driver}\sed
    % \\
    % \overset{(e)}{\geq}~&
    % \cratio{K}\cdot \weightHat_{\taupp}
    % =
    % \cratio{K}\cdot \weight_{\threeindex}
\end{align*}
where (a) uses the fact that $\weightHat_{\wi}\geq \thetai\KED$
for every $\wi\in[\taup:\taupp-1]$,
and the remaining argument is identical to the subcase for $\weight_{\threeindex} < \thetai\KED$ which we omit here.
\hfill\halmos}

% \input{tex/vertex-weighted}


==> FN_ multi-stage matching + configuration allocation (MS Journal)/tex/apx-numerical.tex <==
\ydrevcolor{
\section{Numerical Experiments}
\label{apx:numerical}
In this section we provide 
numerical justifications for the performance of 
our multi-stage configuration allocation algorithm 
on synthetic instances. 
Our instances are motivated by the display-ad
application.
We compare the performance of our algorithm with both the batched-greedy
algorithm (that at each stage 
greedily picks the best local allocation) 
and the online-greedy
algorithm (that picks an ordering over vertices 
in each batch and greedily allocates), 
as well the optimum offline. 
We observe that the competitive ratio of 
our algorithm beats the
other algorithms in our simulations.

\newcommand{\wtp}{v}
\newcommand{\wtpij}{\wtp_{ij}}
\newcommand{\OnlineGR}{\texttt{Online-GR}}
\newcommand{\BatchedGR}{\texttt{Batched-GR}}

\paragraph{Experimental setup.}
We generate the following configuration allocation
problem instances.
There are 20 offline advertisers (i.e., $\Driver \triangleq [20]$)
and 100 arriving users 
(i.e., $\Rider \triangleq [100]$).\footnote{We also
ran our experiments by varying all parameters in our 
synthetic instances. We obtained similar results and verified
the robustness of our numerical findings.}
Each advertiser $j$ demands $n_j \triangleq 5$ 
number of impressions in total.
For each user $i\in\Rider$ and advertiser $j\in\Driver$,
we denote $\wtpij$ by the willingness-to-pay of advertiser $j$
for an impression from user $i$ (see the paragraph below about how 
we generate $\{\wtpij\}$).
For each user $i\in\Rider$, the platform needs to choose 
an advertising configuration $\config$
which specifies a subset of 
advertisers $\Driver_\config\subseteq\Driver$ 
to participate 
in a second-price auction for the arriving impression from user $i$:
the winning advertiser $j^* = \argmax_{j\in\Driver_\config}\wtpij$
with the highest willingness-to-pay 
receives the impression from user $i$,
and pays the per-impression price
equal to the second highest willingness-to-pay among participating advertisers,
i.e., $\alloci \triangleq \indicator{j = j^*}$ and 
$\weight_{\threeindex} \triangleq \wtp_{ij\primed}$
where $j\primed = \argmax_{j\in\Driver_\config\backslash \{j^*\}} 
\wtpij$.

We generate the willingness-to-pay quantities $\{\wtpij\}$ as follows.
First, we draw $20$ $(\triangleq T)$ i.i.d.\ samples from 
the exponential distribution,
and denote them as $\weightHat_1 \leq \dots \leq \weightHat_{T}$.
Next, we draw $20$ i.i.d.\ samples between $[1, 2]$
uniformly at random, and denote them as $\mu_1 \leq \dots \leq \mu_{20}$. 
For each user $i\in\Rider$ and advertiser $j\in\Driver$,
we set the willingness-to-pay $\wtpij \triangleq \weightHat_{\tau}$
where $\tau = \lceil\tau_{i} + \tau_{ij}\cdot \mu_j\rceil$ 
and 
both
$\tau_i$, $\tau_{ij}$ are drawn i.i.d.\ from $[0,\frac{T}{3}]$
uniformly at random.
Note that from the ex ante perspective, 
the willingness-to-pay $\{\wtpij\}$'s are 
symmetric over all users for each fixed advertiser $j$,
and increasing (i.e., stochastic dominant) with respect to advertiser $j$ (since $\mu_j$ is increasing in $j$) for each fixed user $i$.

We consider both scenarios where arriving users are ex ante symmetric 
and ex ante asymmetric, respectively.
In the symmetric-user (resp.\ asymmetric-user) scenario, 
for each user $i\in\Rider$,
we randomly generate $5$ feasible configurations, 
each of which corresponds to a second-price auction 
with 3 advertisers drawn uniformly at random from $\Driver$
(resp.\ $\Driver \backslash [\lfloor \frac{17\cdot i}{100} \rfloor]$).
We assume that there are $K$ stages, where
each stage $k\in[K]$
contains a batch of users $\Rider_k \triangleq [(k - 1)\cdot \lceil\frac{100}{K}\rceil + 1: \min\{100, k\cdot \lceil\frac{100}{K}\rceil\}]$.
Note that in the asymmetric-user scenario, 
the advertisers who can participate in the auction for user $i$
become more restrictive as $i$ increases.
In this way, policies have incentives to carefully 
preserve enough demands for later users.


\paragraph{Policies.} In our numerical experiments, we compare the expected revenue of four different policies/benchmark:
\begin{enumerate}
    \item \emph{Online greedy policy} ($\OnlineGR$):
    greedily decide the fractional allocation for each user $i = 1, 
    2, \dots, 100$.
    for each user $i = 1, 2, \dots, 100$,
    given the current allocation, $\OnlineGR$
    greedily finds the fractional allocation which maximizes the immediate revenue improvement for user $i$.
    
    \item \emph{Batched greedy policy} ($\BatchedGR$):
    for each stage $k\in[K]$,
    given the current allocation, $\BatchedGR$
    greedily finds the fractional allocation which maximizes the 
    immediate revenue improvement for users in batch~$\Rider_k$.
    
    \item \emph{Polynomial regularized max configuration allocation}
    ($\PRMCA$): this policy is \Cref{alg:opt} designed in
    \Cref{sec:extensions}.
    It attains the optimal competitive ratio $\Gamma(K)$.
    We numerically solve convex program \ref{eq:convex primal}
    in $\PRMCA$
    with the Frank–Wolfe algorithm (100 iterations per convex program,
    \citealp{FW-56}).
    
    \item \emph{Optimum offline solution}: this benchmark is
    the solution of linear program~\ref{eq:LP primal}
    in \Cref{sec:extension-model}. It upperbounds the expected revenue of
    any multi-stage allocation algorithms.
\end{enumerate}

\paragraph{Results.}
First, we randomly generate
100 configuration allocation problem instances 
for both user-symmetric and user-asymmetric scenarios 
with $K = 2$ and $K=5$ stages. 
For each instance, we simulate all three policies defined above,
and compute the ratio between the revenue of each policy
against the revenue of the optimum offline solution.
We summarize 
% the (unweighted) average of 
the competitive ratios for each policy 
in \Cref{table:numerical ratio different policies} and \Cref{fig:numerical ratio different policies}.
It can be observed that both $\BatchedGR$
and $\PRMCA$ which utilize the batch arrival 
outperform $\OnlineGR$, and the ratio between 
better from $K = 5$ batches to $K = 2$ batches.
Furthermore, $\PRMCA$ which hedges the batch-wise allocation
outperforms $\BatchedGR$ which greedily decides the
batch-wise allocation.
Specifically, by switching from $\OnlineGR$ (resp.\ $\BatchedGR$) to $\PRMCA$,
there are strictly more than 5\% revenue improvement 
in all scenarios.
\begin{table}[t]
    \centering
    \caption{The average competitive ratios for 
    different policies.}
    \label{table:numerical ratio different policies}
    \begin{tabular}[t]{lcccc}
    \toprule
    & \multicolumn{2}{c}{user-symmetric} & \multicolumn{2}{c}{user-asymmetric} \\
    \cmidrule{2-5}
     & $K = 2$ & $K = 5$ 
     & $K = 2$ & $K = 5$ 
     \\
     \midrule
     \OnlineGR & 0.913 & 0.913 & 0.849 & 0.849 \\
     \BatchedGR & 0.947 & 0.919 & 0.877 & 0.860 \\
     \PRMCA & 0.982 & 0.961 & 0.937 & 0.903 \\
    \bottomrule
    \end{tabular}
\end{table}

\begin{figure}[ht]
  \centering
       \subfloat[user-symmetric, $K = 2$]
      {\includegraphics[width=0.4\textwidth]{figs/symmetric-2.png}}
      \subfloat[user-symmetric, $K = 5$]
      {\includegraphics[width=0.4\textwidth]{figs/symmetric-5.png}}
      \\
       \subfloat[user-asymmetric, $K = 2$]
      {\includegraphics[width=0.4\textwidth]{figs/asymmetric-2.png}}
      \subfloat[user-asymmetric, $K = 5$]
      {\includegraphics[width=0.4\textwidth]{figs/asymmetric-5.png}}
      \\
  \caption{Box and whisker comparison of different policies in terms of the
  competitive ratios. Results are based on 100 iterations of Monte-Carlo simulation.
  }
   \label{fig:numerical ratio different policies}
\end{figure}

To illustrate the the benefit of batching, 
we also plots the average 
(over 100 configuration allocation problem instances) 
of the ratios for $\PRMCA$
and $\BatchedGR$ for $K = 1, \dots, 10$ for both 
user-symmetric and user-asymmetric scenario
in \Cref{fig:numerical vary K}. 
It can be observed that the average ratio is decreasing as 
the total number of stages $K$ increases, and 
$\PRMCA$ outperforms $\BatchedGR$ in both scenarios over all $K$. 

\begin{figure}[ht]
  \centering
       \subfloat[user-symmetric]
      {\includegraphics[width=0.4\textwidth]{figs/fig-ratio-vary-K-symmetric.png}}
      \subfloat[user-asymmetric]
      {\includegraphics[width=0.4\textwidth]{figs/fig-ratio-vary-K-asymmetric.png}}
  \caption{The average competitive ratios for 
  $\PRMCA$ and
  $\BatchedGR$ as functions of the total number of stages $K$.
  }
   \label{fig:numerical vary K}
\end{figure}

}

==> FN_ multi-stage matching + configuration allocation (MS Journal)/tex/apx-open.tex <==
\section{Future Directions and Open Problems}
\label{apx:open}
Several open questions arise from this work. 
The first question is to identify the optimal multi-stage algorithm and its competitive ratio
for the multi-stage \emph{integral} bipartite matching problem (i.e., the multi-stage version of the classic problem studied in \citealp{KVV-90}).  Showing whether our competitive ratio can be obtained in the integral matching problem for $K>2$ is still an open problem. 
\revcolor{Second, inspired by the importance of batched allocations in applications such as ride-sharing and cloud computing, one might want to study the multi-stage resource allocation where the resources are \emph{reusable}, similar to some recent work on online allocation of reusable resources \citep{FNS-19, feng2021online, goyal2020onlineb,gong2019online}. In such a setting, a resource after being assigned to a demand request will be available again for reassignment after a certain time durations, which can be deterministic (and fixed over time) or i.i.d. over time. Note that in such a problem formulation, resource usage durations are described in the number of stages it takes for a resource to be available again. Third, our multi-stage matching algorithms assume knowing the number of stages $K$ in advance. One can now investigate the question of having access to a predictor for $K$ and asks the question of obtaining robustness and consistency bounds (in the same style as in the learning-augmented online algorithm literature).}
Fourth, one can consider applying our developed machinery and framework in this paper to \revcolor{multi-stage assortment optimization~\citep{GNR-14},} multi-stage stochastic matching~\citep{MGS-12,JL-14}, or  multi-stage matching with stochastic rewards~\citep{mehta2012online}. \revcolor{We conjecture that our approach can be extended to all of these settings and help with improved competitive ratios. We leave further investigation around these directions and the possibility of extending our approach as open problems.}

\revcolor{Finally, 
it is also worthwhile to study
the benefit of batching under 
environments with additional structure.
Note that the optimal competitive ratio $\Gamma(K)$
converges to $1 - \frac{1}{e}$ at a linear rate as $K$ converges to infinity, i.e., $\Gamma(K)=1-\frac{1}{e}+O(\frac{1}{K})$. In other words, the benefit of batching 
decays quite fast in the worst-case analysis. However, this fast decay might be an artifact of the model and the fact that designer aims to have a robust multi-stage allocation algorithms that performs well under any problem instance.
To resolve this mystery, one can consider more refined models with additional (non-)stochastic structures,
and identify algorithms that benefit from batching, but this time with the goal of highlighting the benefit of the batching in a regime where the number of batches is super constant, but not very large. In such a model, another possible variable that can play a role is the average size of a batch. We leave all these investigations to future work.}


==> FN_ multi-stage matching + configuration allocation (MS Journal)/tex/b-matching.tex <==
Recall that the multi-stage vertex weighted b-matching
problem is a variant of 
the multi-stage vertex weighted matching 
where the matching constraint 
of each offline vertex $j\in\Driver$ is 
replaced with a capacity constraint $\budget_j$.
Let $\minbudget=\min_{j\in \Driver}\budget_j$
be the smallest capacity.
We
discuss how to modify 
\Cref{alg:b-matching}
to
output fractional solutions
for the $K$-stage vertex weighted b-matching problem
with competitive ratio $\cratio{K}$.
Finally, using a deterministic rounding technique,
we present a deterministic algorithm
that outputs \emph{integral} solutions 
with competitive ratio $
\cratio{K} - O(1/\minbudget)$.


\smallskip
\noindent\textbf{Fractional Multi-stage b-matching~} Consider a modification of 
\Cref{alg:b-matching}, where we replace the convex program~\ref{eq:concave-k-bmatching}
with the modified convex program~\ref{eq:concave-k-bmatching integral}
defined below,
    \begin{align}
 	\label{eq:concave-k-bmatching integral}
 	\tag{$\mathcal{P}^{\text{MWBM}}_k$}
    \begin{array}{lll}
       \xbf^*_k= \underset{\xbf}{\argmax} & 
        \displaystyle\sum_{(i,j) \in E_k}w_j 
        \frac{x_{ij}}{\budget_j} - \sum_{j\in \Driver}w_j F_k\left(\frac{y_j}{\budget_j}+
        \sum_{i : (i,j)\in E_k}\frac{x_{ij}}{\budget_j}\right)
        & \text{s.t.}\\
         &\displaystyle
         \sum_{j: (i,j)\in E_k} x_{ij} \leq 1
         & i\in \Rider_k\\
         & 
         \displaystyle\sum_{i: (i,j)\in E_k} x_{ij} \leq 
         \budget_j-y_j
         & j\in \Driver\\
         &
        x_{ij} \geq 0 &
        (i, j) \in E_k
    \end{array}
\end{align}
Similar to \Cref{sec:vertex-weight},
the convex program \ref{eq:concave-k-bmatching integral}
introduces the following structural decomposition (\Cref{lemma:structure budgeted allocation}).
We omits the proof of this lemma, as it follows exactly the same argument as its analog in the vertex weighted matching problem 
(\Cref{lemma:structure}).
% and its proof in \Cref{apx:skeleton}).
The main difference between \Cref{lemma:structure budgeted allocation} and \Cref{lemma:structure}
is the closed-form expression 
in uniformity property.

\begin{lemma}[{Structural Decomposition/Vertex Weighted b-matching}]
\label{lemma:structure budgeted allocation}
Fix any $k \in [K - 1]$.
Let $\xbf^*_k$ be the optimal solution of the convex program~\ref{eq:concave-k-bmatching integral}. Consider the subgraph $G'_k=(\Rider_k,\Driver,E'_k)$ of $G_k$, where $E'_k=\{(i,j)\in E_k :x^*_{k,ij}>0\}$. Let $\Driver^{(0)}_k$ be the set of offline vertices in $\Driver$ who exhausts their capacities by $\xbf^*_k$ given the current $\ybf$, and 
$\Rider^{(0)}_k$ be the set of online vertices who are neighbors of $\Driver^{(0)}_k$ in $G_k'$, that is, 
$$\Driver^{(0)}_k\triangleq \{j\in \Driver: y_j+\sum_{i:(i,j)\in E_k}x^*_{k,ij}=\budget_j\}~~\textrm{and}~~\Rider^{(0)}_k\triangleq \{i\in \Rider_k:\exists j\in \Driver^{(0)}_k, x^*_{k,ij}>0\}~.$$
Moreover, let the pairs 
$
\left\{\left(\Rider_k^{(l)},\Driver_k^{(l)}\right)\right\}_{l=1}^{L_k}$ 
identify the $L_k$ connected components of the induced subgraph $G_k'[\Rider_k\setminus\Rider_k^{(0)},\Driver\setminus\Driver_k^{(0)}]$ of $G_k'$. Then:
\begin{enumerate}%[label=\roman*.]
    \item \underline{Uniformity}: ~$\forall~ l\in[0:L_k],j,j'\in \Driveri_k:$ $$w_j\left(1-
    f_k\left(
    \frac{y_j}{\budget_j}
    + \sum_{i:(i,j)\in E_k}
    \frac{x^*_{k,ij}}{\budget_j}
    \right)
    \right)=
    w_{j'}\left(1-
    f_k\left(
    \frac{y_{j'}}{\budget_{j'}} + \sum_{i:(i,j')\in E_k}
    \frac{x^*_{k,ij'}}{\budget_{j'}}
    \right)
    \right)\triangleq c_k^{(l)}$$
    \item \underline{Monotonicity}:  $\forall~ l,l'\in[0:L_k]$: there exists no edge in $E_k$ between $\Rider_k^{(l)}$ and $\Driver_k^{(l')}$ if $c_k^{(l)}<c_k^{(l')}$. 
    \item \underline{Saturation}: $\forall~ l\in[L_k]$: all online vertices in $\Rider_k^{(l)}$ are fully matched by $\xbf_k^*$, i.e., $\displaystyle\sum_{j:(i,j)\in E_k}x^*_{k,ij}=1, i\in\Rider_k^{(l)}$~.
\end{enumerate}
\end{lemma}

\smallskip
\noindent\textbf{Rounding to an Integral Allocation~} To output integral solutions 
in 
the $K$-stage vertex weighted b-matching problem, 
we further round the fractional solution $\xbf_k^*$
to an integral solution $\hat\xbf_k^*$
for each stage $k$ as follows.
Let $\{(\Rider^{(0)}_k, \Driver^{(0)}_k),\dots, (\Rider^{(L_k)}_k, \Driver^{(L_k)}_k)\}$ be the 
structural decomposition of $(\Rider_k, \Driver, E_k)$ in \Cref{lemma:structure budgeted allocation}.
For any edge $(i, j)\in E_k$ such that 
$i\in \Rider_k^{(l)}$, $j \in \Driver_k^{(l')}$
and $l\not=l'$, we set $\hat x_{k,ij}^*\gets x_{k,ij}^* = 0$.
Denote the edges between $\Rider_k^{(l)}$ and $\Driver_k^{(l)}$
by $E_k^{(l)}$.
For each subgraph $(\Rider_k^{(l)}, \Driver_k^{(l)}, E_k^{(l)})$,
we set $\{\hat x_{k, ij}^*\}_{(i,j)\in E_k^{(l)}}$ to be an \emph{optimal vertex} of 
the following linear program
\ref{eq:rounding k-bmatching} (which can be found in polynomial time, for example by the simplex algorithm or ellipsoid method):

\begin{align}
 	\label{eq:rounding k-bmatching}
 	\tag{$\mathcal{P}^{\text{rounding}}_{k,l}$}
    \begin{array}{lll}
       \{\hat x_{k, ij}^*\}_{(i,j)\in E_k^{(l)}}= \underset{\xbf}{\argmax} & 
        \displaystyle\sum_{(i,j) \in E_k^{(l)}}x_{ij}
        & \text{s.t.}\\
         &\displaystyle
         \sum_{j: (i,j)\in E_k^{(l)}} x_{ij} \leq 1
         & i\in \Rider_k^{(l)}\\
         & 
         \displaystyle\sum_{i: (i,j)\in E_k^{(l)}} x_{ij} 
         \geq 
         \floor*{
         \displaystyle\sum_{i: (i,j)\in E_k^{(l)}} x_{k,ij}^*
         }
         & j\in \Driver_k^{(l)}\\
         \\
         & 
         \displaystyle\sum_{i: (i,j)\in E_k^{(l)}} x_{ij} 
         \leq 
         \floor*{
         \displaystyle\sum_{i: (i,j)\in E_k^{(l)}} x_{k,ij}^*
         } + 1
         & j\in \Driver_k^{(l)}\\
         &
        x_{ij} \geq 0 &
        (i, j) \in E_k^{(l)}
    \end{array}
\end{align}
where $\floor*{a}$ is the floor function that
outputs the greatest integer less than or equal to $a$.
Note that \ref{eq:rounding k-bmatching}
is a feasible program since $\{ x_{k, ij}^*\}_{(i,j)\in E_k^{(l)}}$
is a feasible solution.
Moreover, it can be easily checked that
the matrix defining the feasibility polytope in \ref{eq:rounding k-bmatching}, with entries in $\{0,\pm 1\}$, 
is indeed a  Totally Unimodular Matrix (TUM)
\citep[cf.][]{sch-03}. As a result, because all the lower-bound and upper-bound constraints are integers, all the vertices of this feasibility polytope are going to be integral.
Thus, $\hat\xbf_k^*$ is an integral optimal solution.
% \YF{Do we need a citation for TUM implying 
% integral solution?}.\RN{We need. Here is a good citation:~\cite{sch-03}}.



We are now ready to show the competitive ratio result of the multi-stage 
vertex weighted b-matching problem. We propose both fractional and integral versions of the \emph{Polynomial Regularized Maximum Weight b-Matching Algorithm} (\PRMWBM) -- see \Cref{alg:b-matching integral} 
% in \Cref{apx:algorithms} 
for a formal description. The analysis of this multi-stage algorithm is technical -- yet with several similarities to the proof of \Cref{thm:b-matching} -- and hence is deferred to \Cref{apx:b-matching}.

\begin{algorithm}
 	\caption{Polynomial Regularized Max Weight b-Matching (\PRMWBM)}
 	\label{alg:b-matching integral}
 	\KwIn{Number of batches/stages $K$,
 	Integral solution flag $\texttt{\textsl{Flag}}$.}
%  	\vspace{1mm}
%  	\KwOut{SS.}
 	    \vspace{2mm}
 	    
    $\forall j\in\Driver:~y_j\gets 0$.

 	\vspace{1mm}
 	\For{stage $k=1$ to $K$}
 	{
 	\vspace{2mm}
 	\tcc{$k^{\textrm{th}}$ batch of vertices in $\Rider$, denoted by $\Rider_k$, arrives. Let $E_k$ denote the set of edges incident to vertices in $\Rider_k$.}
 	\vspace{2mm}
 	
   Given $\{y_j\}_{j\in \Driver}$ and subgraph $G_k=(\Rider_k,\Driver,E_k)$, solve $\xbf_k^*$ from
   the convex program~\ref{eq:concave-k-bmatching integral}.

\If{$\texttt{Flag} == \text{False}$}{
$\forall j\in \Driver: y_j\gets y_j+\displaystyle\sum_{i\in\Rider_k}x^*_{k,ij}$.

Return $\xbf^*_k$ as the fractional b-matching allocation of stage $k$.
}
\Else{
Given $\xbf^*_k$, and
structural decomposition 
$\{(\Rider_k^{(l)}, \Driver_k^{(l)}\}_{l\in [0:L_k]}$, 
solve optimal vertex $\hat\xbf_k^*$ from
the linear program~\ref{eq:rounding k-bmatching} for all $l\in [0:L_k]$.

$\forall j\in \Driver: y_j\gets y_j+\displaystyle\sum_{i\in\Rider_k}\hat x^*_{k,ij}$.

Return $\hat\xbf^*_k$ as the integral b-matching allocation of stage $k$.
}
}
\end{algorithm}

\begin{theorem}[\textbf{Optimal Multi-stage Algorithm for Weighted Bipartite b-matching}]
\label{thm:b-matching integral}
In the $K$-stage fractional (resp.\ integral)
vertex weighted b-matching problem, the fractional (resp.\ integral) version of \PRMWBM ~(\Cref{alg:b-matching integral})
is $\cratio{K}$-competitive 
(resp.\ $\left(\cratio{K} - O(1/\minbudget)\right)$-competitive), where $\cratio{K}=\cratioexp$.
\end{theorem}
\begin{remark}[\textbf{Optimality of the $\boldsymbol{\cratio{K}}$ Competitive Ratio for b-matching}]
Note that the multi-stage vertex weighted
b-matching problem generalizes
the multi-stage 
(fractional) vertex 
weighted matching problem. Therefore
% (i.e., the former approximates the latter
% as $\minbudget\rightarrow\infty$),
\Cref{thm:tightness} implies that
the competitive ratio in \Cref{thm:b-matching integral} 
has the optimal dependence on $K$
in the multi-stage vertex weighted b-matching problem, i.e., no integral or fractional multi-stage algorithm can obtain a competitive ratio better than $\cratio{K}$.
\end{remark}


==> FN_ multi-stage matching + configuration allocation (MS Journal)/tex/conclusion.tex <==
\section{Conclusion and Discussions}
\label{sec:conclusion}
Motivated by the trade-off between batching and inefficiency in two-sided matching platforms, we studied the 
$K$-stage vertex weighted matching and its 
extension to the general model of configuration allocation with free-disposal. We designed optimal $\left(1-(1-1/K)^K\right)$-competitive 
fractional algorithms for these problems.
A key ingredient of our algorithms 
and analysis is 
a sequence of polynomials of decreasing degrees, used as regularizers of maximum weight matching. We also presented the idea of price-level regularization to handle weight heterogeneity of the allocation on the offline side, and showed our our approach can incorporate this form of regularization. Our work also identifies deep connections between convex duality and primal-dual analysis of multi-stage resource allocation algorithms.
There are several  open questions and future research directions stemming from this work. See Appendix~\ref{apx:open} for more discussions. 

% We also presented a deterministic rounding scheme
% with the competitive ratio $1-(1-1/K)^K 
% - O\left(1/\minbudget\right)$
% for the $K$-stage vertex weighted integral b-matching problem and 
% a randomized rounding scheme 
% with the competitive ratio $1-(1-1/K)^K 
% - O(\sqrt{\log(\minbudget)/\minbudget})$
% for the $K$-stage AdWords problem.


% Third, when batches have size one 
% (i.e., the fully online setting),
% identify the $K$-stage optimal algorithm and its 
% competitive ratio. For this last open problem, we conjecture the algorithms in this paper are optimal competitive.




% \section*{Acknowledgement}
% The authors would like to thank Yeganeh Alimohammadi for participating in the early stages of this project, and to Amin Saberi for helpful discussions regarding the presentation of this work. We are also grateful to Rene Caldentey, Ozan Candogan, and Niusha Navidi for helpful comments and feedback on an earlier version of this manuscript. 



==> FN_ multi-stage matching + configuration allocation (MS Journal)/tex/configuration-allocation-extensions.tex <==
\revcolor{\section{Extension: Multi-stage Configuration Allocation}
\label{sec:extensions}
In this section, we discuss how 
our approach can be generalized 
to the multi-stage configuration allocation problem. There are several key challenges towards this extension. First, in contrast to vertex weighted matching, here each unit of an advertiser's capacity can be allocated at \emph{different prices}. Thus, it is not clear how to use the regularization approach of the previous section. 
This important distinction also implies that a similar graph-based structural decomposition to analyze a potential convex programming based algorithm might not exist in this model, roughly because the degree of match-ability of an offline node might vary across different price levels. Finally, a configuration allocation algorithm should make disposal (preemption) decisions jointly with its allocation whenever needed. A priori, it is not clear how to incorporate preemption into our previous convex programs.\footnote{Note that edge-weighted online matching is a special case; hence disposals are definitely needed for having a bounded competitive ratio even when there is one offline node.} 

We start by introducing a novel algorithmic construct to address the above challenges. We present our new convex-programming based algorithm (\Cref{alg:opt}) based on this new technique in \Cref{sec:alg-convex}. Due to the lack of a structural decomposition, we study the key properties of this convex program directly in \Cref{sec:convex program} through convex duality. We then try to mimic the recursive primal-dual analysis of \Cref{sec:vertex-weight} in \Cref{sec:main proof}, with the major difference that we directly use the optimal Lagrangian dual solution of our convex programs in each stage to find an approximate dual certificate for our primal algorithm in the LP formulation of the offline problem.}

% that show the approximate optimality of our algorithm from our stage-wise convex program.s 


% We then set up the stage for our competitive analysis in \Cref{sec:convex program} by identifying a few key properties of the convex programs defining our algorithm in each stage $k\in[K]$ (by using convex duality). We then introduce our convex-programming based recursive primal-dual analysis in \Cref{sec:main proof}, in which we directly use the optimal Lagrangian dual solution of our convex programs in each stage to find an approximate dual certificate for our primal algorithm in the LP formulation of the offline problem.


\revcolor{\subsection{Price-level Regularized Convex Programs and Configuration Allocation}
\label{sec:alg-convex}
Before describing our algorithm, we make an
assumptions for simplicity (without loss of generality) that there exists a finite universe $0 = \weightHat_0 < \weightHat_1
< \dots < \weightHat_{\totalweight}$ of $T\in\mathbb{N}$ possible per-impression prices.
Namely, for each per-impression price $\weight_{\threeindex}$,
there exists an index $\wi\in[\totalweight]$ such that 
$\weight_{\threeindex} = \weightHat_\wi$.
As we will see soon, our algorithm does not need to know 
$\{\weightHat_\wi\}_{\wi\in[\totalweight]}$
ahead of time, and its competitive ratio will have no dependency on this finite set.\footnote{\label{footnote:weightHat}Notably, the discreetness assumption is mainly for ease of exposition, and our results can immediately be extended to the setting with continuous per-impression prices.}

\smallskip
\noindent\textbf{Overview of the Algorithm}~~~At each stage $k\in[K]$, our algorithm solves a stage-dependent convex program that is essentially a regularized version of the LP for a greedy allocation at that stage. Intuitively speaking, the main new ideas behind this convex program are:
\begin{enumerate}
    \item Regularizing the revenue function \emph{separately at different price levels} using a convex function in a structured fashion, in order to create a controlled hedging through maintaining balancedness in allocation separately at each price level, 
    \item Setting it up in a way that we can extract a balanced configuration allocation, together with the necessary amount of preemption at each price level, from the solution of the program.
\end{enumerate}
Formally, we solve the following convex program~\ref{eq:convex primal} in stage $k$ of our algorithm:
\begin{align}
\tag{$\mathcal{P}^{\textsc{MCA}}_k$}
\label{eq:convex primal}
&\arraycolsep=1.4pt\def\arraystretch{2.2}
\begin{array}{lll}
        \max\limits_{\xbf,\ybf,\zbf \geq \mathbf{0}}~~~~
        &
        \displaystyle\sum_{\rider\in\Rider_k}
        \displaystyle\sum_{\config\in\Config}
        \displaystyle\sum_{\driver\in\Driver}
        \weight_{\threeindex} 
        \cdot
        x_{\threeindex}
        - 
        \sum_{\driver\in\Driver}
        \sum_{\wi \in [\totalweight]}
        \weightHat_\wi \cdot 
        \left(
        \comsumptioni-
        y_{\twoindex}
        \right)&
        \\
        &
        \hspace{10mm}
        -
        \displaystyle\sum\limits_{\driver\in \Driver}
        \displaystyle\sum\limits_{\wi \in [\totalweight]}
        \left(
        \weightHat_\wi - \weightHat_{\wi - 1}
        \right)
        \cdot 
        F_k\left(
        \mathop{
        \displaystyle\sum
        x_{\threeindex}
        }
        \limits_{
        \substack{
        \rider\in\Rider_k,\config\in\Config:
        % (\threeindex)\in E_k,\\
        \\
        ~~\weight_{\threeindex}\geq 
        \weightHat_\wi}
        }
        % x_{\threeindex}
        +
        \displaystyle\sum\limits_{\wi' \geq \wi}
        y_{\driver,\wi'}
        \right)
        & \text{s.t.}
        \\
         &
        %  \mathop{
         \displaystyle\sum_{\rider\in\Rider_k}
         \displaystyle\sum_{\config\in\Config}
        %  x_{\threeindex}
        %  }
        %  \limits_{\rider,\config:(\threeindex)\in E_k}
         x_{\threeindex}
         +
         \displaystyle\sum_{\wi\in[\totalweight]}
         y_{\twoindex}
         \leq 1
         &
         \driver\in\Driver~,
         \\
         &
         \displaystyle\sum_{\config\in\Config} z_{\rider,\config}\leq 1
         &
         \rider\in\Rider_k~,
         \\
         &
         x_{\threeindex}\leq 
         \alloci\cdot z_{\rider,\config}
         &
        %  (\threeindex)\in E_k
        \rider\in\Rider_k,\config\in\Config,\driver\in\Driver~,
         \\
         &
         y_{\twoindex}\leq \comsumptioni
         &
         \driver\in \Driver, \wi\in[\totalweight]~.
        %  \\
        %  &x_{\threeindex}\geq 0,~z_{\rider,\config}\geq 0
        %  &\rider\in\Rider_k,\config\in\Config,\driver\in\Driver~, 
        %  \\
        %  &y_{\twoindex} \geq 0
        %  &\driver\in\Driver,\wi\in[\totalweight]~.
        %  \\
        \end{array}
\end{align}
This convex program depends on the set $\Rider_k$ of arriving users in stage $k$, the vector of impression numbers $\allocs\ked = \{\alloci\}_{\rider\in\Rider_k}$, and the vector of per-impression prices $\weightbf\ked = \{\weight_{\threeindex}\}_{\rider\in\Rider_k}$, all of which are revealed to the algorithm at the beginning of stage $k$. Furthermore, our algorithm keeps track of $\boldsymbol{\comsumption}\ked = \{\comsumption_{\twoindex}\ked\}$, where $\comsumption_{\twoindex}\ked$ is the fractional number of impressions that each advertiser $j$ is willing to pay for each per-impression price $\tau$ at the end of each stage $k$. The vector $\boldsymbol{\comsumption}^{(k-1)}$, which is basically the price distribution of top impressions allocated to advertiser $j$ with total capacity of $n_j=1$, captures the state of the allocation at the beginning of stage $k$. Notably, the above convex program \ref{eq:convex primal} depends on this state information  $\boldsymbol{\comsumption}\kminused$. As for the decision variables, variable $z_{\rider,\config}$
in the above program specifies the fractional allocation of
user $\rider\in\Rider_k$ with configuration $\config\in\Config$. Moreover, variable $x_{\threeindex}$
specifies the fractional number of impressions created by user $\rider$ form configuration $\config$ that advertiser $\driver$ is willing to pay for after the allocation of stage $k$,
and thus 
$\alloci\cdot z_{\rider,\config} - 
x_{\threeindex}$ impressions of user $\rider$ for advertiser $\driver$ are immediately preempted at the end of stage $k$.
Finally, variable $y_{\twoindex}$
specifies the total number of impressions of previous $k - 1$ stages that advertiser $\driver$ is still willing to pay for at 
per-impression price of 
$\weightHat_{\wi}$ \emph{after} allocation/preemption decisions of stage $k$. In other words,
$\comsumptioni - y_{\twoindex}$
number of impressions of advertiser $\driver$ which
were finalized in the previous $k-1$ stages at
per-impression price of $\weightHat_{\wi}$ will be preempted after stage $k$.  See \Cref{alg:opt} for a formal description.



% \noindent\textbf{Overview of the Algorithm}~~We summarize our proposed  multi-stage algorithm 
% in \Cref{alg:opt}, which heavily relies on solving a stage-dependent convex program \ref{eq:convex primal}  at each stage $k=1,2,\ldots,K$ to obtain its fractional configuration allocation in that stage.

% \begin{algorithm}[htb]
%  	\caption{Convex-programming Based Configuration Allocation}
%  	\label{alg:opt}
%  	\KwIn{Number of stages $K$, convex functions $\{F_k:[0,1]\rightarrow[0,1]\}_{k\in[K]}$}
%  	    \vspace{2mm}
 	    
%     $\forall \driver\in\Driver,\wi\in[\totalweight]:
%     ~\comsumption_{\twoindex}^{(0)}\gets 0$.

%  	\vspace{1mm}
%  	\For{stage $k=1$ to $K$}
%  	{
%  	\vspace{2mm}
%  	\tcc{$k^{\textrm{th}}$ batch of users
%  	in $\Rider$, denoted by $\Rider_k$, arrives. 
% %  	Let $E_k$ denote the set of edges incident to vertices in $\Rider_k$.
%  	}
%  	\vspace{2mm}
 	
%   Given $\boldsymbol{\comsumption}\kminused$,
%   $\Rider_k$,
% $\allocs\ked$ and $\weightbf\ked$, solve 
%   the optimal solution $(\xbf\starred,\ybf\starred,\zbf\starred)$
%   of the convex program~\ref{eq:convex primal} (after plugging the regularizer function $F_k$ in the program).


% $\forall \driver\in \Driver,\wi\in[\totalweight]:
% \comsumption_{\twoindex}\ked\gets
%         \mathop{
%         \displaystyle\sum
%         x_{\threeindex}\starred
%         }
%         \limits_{
%         \substack{
%         \rider\in\Rider_k,\config\in\Config:
%         % (\threeindex)\in E_k,\\
%         \\
%         ~~\weight_{\threeindex}= 
%         \weightHat_\wi}
%         }
%         % x_{\threeindex}
%         +
%         y_{\driver,\wi}\starred$.

% Return $(\xbf\starred,\ybf\starred,\zbf\starred)$
% as the fractional solution of stage $k$.
%  	}
% \end{algorithm}

% \newpage
\begin{algorithm}[htb]
 	\caption{Polynomial Regularized Max Configuration Allocation (\PRMCA)}
 	\label{alg:opt}
 	\KwIn{Number of stages $K$, convex functions $\{F_k:[0,1]\rightarrow[0,1]\}_{k\in[K]}$}
 	    \vspace{2mm}
 	    
    $\forall \driver\in\Driver,\wi\in[\totalweight]:
    ~\comsumption_{\twoindex}^{(0)}\gets 0$.

 	\vspace{1mm}
 	\For{stage $k=1$ to $K$}
 	{
 	\vspace{2mm}
 	\tcc{$k^{\textrm{th}}$ batch of users
 	in $\Rider$, denoted by $\Rider_k$, arrives. 
%  	Let $E_k$ denote the set of edges incident to vertices in $\Rider_k$.
 	}
 	\vspace{2mm}
 	
  Given $\boldsymbol{\comsumption}\kminused$,
  $\Rider_k$,
$\allocs\ked$ and $\weightbf\ked$, solve the convex program~\ref{eq:convex primal} to obtain $(\xbf\starred_k,\ybf\starred_k,\zbf\starred_k)$.
% \begin{align}
% \tag{$\mathcal{P}^{\textsc{CA}}_k$}
% \label{eq:convex primal}
% &\arraycolsep=1.4pt\def\arraystretch{2.2}
% \begin{array}{lll}
%         (\xbf\starred_k,\ybf\starred_k,\zbf\starred_k)=\argmax\limits_{\xbf,\ybf,\zbf \geq \mathbf{0}}~~~~
%         &
%         \displaystyle\sum_{\rider\in\Rider_k}
%         \displaystyle\sum_{\config\in\Config}
%         \displaystyle\sum_{\driver\in\Driver}
%         \weight_{\threeindex} 
%         \cdot
%         x_{\threeindex}
%         - 
%         \sum_{\driver\in\Driver}
%         \sum_{\wi \in [\totalweight]}
%         \weightHat_\wi \cdot 
%         \left(
%         \comsumptioni-
%         y_{\twoindex}
%         \right)&
%         \\
%         &
%         \hspace{10mm}
%         -
%         \displaystyle\sum\limits_{\driver\in \Driver}
%         \displaystyle\sum\limits_{\wi \in [\totalweight]}
%         \left(
%         \weightHat_\wi - \weightHat_{\wi - 1}
%         \right)
%         \cdot 
%         F_k\left(
%         \mathop{
%         \displaystyle\sum
%         x_{\threeindex}
%         }
%         \limits_{
%         \substack{
%         \rider\in\Rider_k,\config\in\Config:
%         % (\threeindex)\in E_k,\\
%         \\
%         ~~\weight_{\threeindex}\geq 
%         \weightHat_\wi}
%         }
%         % x_{\threeindex}
%         +
%         \displaystyle\sum\limits_{\wi' \geq \wi}
%         y_{\driver,\wi'}
%         \right)
%         & \text{s.t.}
%         \\
%          &
%         %  \mathop{
%          \displaystyle\sum_{\rider\in\Rider_k}
%          \displaystyle\sum_{\config\in\Config}
%         %  x_{\threeindex}
%         %  }
%         %  \limits_{\rider,\config:(\threeindex)\in E_k}
%          x_{\threeindex}
%          +
%          \displaystyle\sum_{\wi\in[\totalweight]}
%          y_{\twoindex}
%          \leq 1
%          &
%          \driver\in\Driver~,
%          \\
%          &
%          \displaystyle\sum_{\config\in\Config} z_{\rider,\config}\leq 1
%          &
%          \rider\in\Rider_k~,
%          \\
%          &
%          x_{\threeindex}\leq 
%          \alloci\cdot z_{\rider,\config}
%          &
%         %  (\threeindex)\in E_k
%         \rider\in\Rider_k,\config\in\Config,\driver\in\Driver~,
%          \\
%          &
%          y_{\twoindex}\leq \comsumptioni
%          &
%          \driver\in \Driver, \wi\in[\totalweight]~.
%         %  \\
%         %  &x_{\threeindex}\geq 0,~z_{\rider,\config}\geq 0
%         %  &\rider\in\Rider_k,\config\in\Config,\driver\in\Driver~, 
%         %  \\
%         %  &y_{\twoindex} \geq 0
%         %  &\driver\in\Driver,\wi\in[\totalweight]~.
%         %  \\
%         \end{array}
% \end{align}
$\forall \driver\in \Driver,\wi\in[\totalweight]:
\comsumption_{\twoindex}\ked\gets
        \mathop{
        \displaystyle\sum
        x_{\threeindex}\starred
        }
        \limits_{
        \substack{
        \rider\in\Rider_k,\config\in\Config:
        % (\threeindex)\in E_k,\\
        \\
        ~~\weight_{\threeindex}= 
        \weightHat_\wi}
        }
        % x_{\threeindex}
        +
        y_{\driver,\wi}\starred$.

Return $(\xbf\starred_k,\ybf_k\starred,\zbf_k\starred)$
as the fractional solution of stage $k$.

\tcc{$\zbf_k\starred:$~configuration allocation of stage $k$, $\boldsymbol{\comsumption}\kminused-\ybf_k\starred:$~preemption decisions of stage $k$.}
 	}
\end{algorithm}


% Our algorithm keeps track of the fractional number of impressions that each advertiser is willing to pay (i.e., it is a currently top impression considering the budget of $n_j=1$ for each advertiser $j$) at different per-impression prices until the end of the current stage. This information is captured by 
% $\boldsymbol{\comsumption}\ked = \{\comsumption_{\twoindex}\ked\}$, where $\comsumption_{\twoindex}\ked$
% is the total (fractional) number of impressions that
% advertiser $\driver$ is currently willing to pay 
% at per-impression price of $\weightHat_\wi$
% by the the end of stage $k$. At each stage $k$, 
% our algorithm solves a different convex program \ref{eq:convex primal}. This convex program depends on 
% the users $\Rider_k$ , the vector of impression numbers $\allocs\ked = \{\alloci\}_{\rider\in\Rider_k}$, and the vector of per-impression prices $\weightbf\ked = \{\weight_{\threeindex}\}_{\rider\in\Rider_k}$, both of which are revealed to the algorithm at the beginning of stage $k$. The convex program \ref{eq:convex primal} also depends on the vector
% $\boldsymbol{\comsumption}\kminused$, which basically captures the state of the algorithm at the end of the previous stage $k - 1$ (or equivalently, at the beginning of stage $k$).
% The optimal solution
% % $(\xbf\starred,\ybf\starred,\zbf\starred)$ 
% of
% \ref{eq:convex primal}
% determines the configuration allocation of users in this stage ($\zbf\starred$), as well as the number of paid impressions at each price level ($\xbf\starred,\ybf\starred$) until the end of this stage. Note that the solution of the convex program also encodes the number of preempted impressions at each price level during this stage and from previous stages. After $(\xbf\starred,\ybf\starred,\zbf\starred)$ are computed by solving the convex program, the algorithm updates the state variables $\boldsymbol{\comsumption}\kminused$ for stage $k$.


% \vspace{3mm}
% \noindent\textbf{Price-level Regularization}~~~At each stage $k\in[K]$, we consider solving a stage-dependent convex program~\ref{eq:convex primal} that is essentially a regularized version of the LP for a greedy allocation at that stage. Intuitively speaking, the main ideas behind these convex programs are:
% \begin{enumerate}
%     \item Regularizing the revenue function \emph{separately at different price levels} using a convex function in a structured fashion, in order to create a controlled hedging through the induced balancedness in allocation, and
%     \item Setting it up in a way that we can extract a balanced configuration allocation, together with the necessary amount of preemption at each price level, from the solution of the program.
% \end{enumerate}
% Note that the convex program of stage $k$ is parametric with respect to a regularizer function $F_k:[0,1]\rightarrow[0,1]$.
% % These convex programs 
% For $k\in[K - 1]$, $F_k(x) = \int_{0}^x f_k(t)\,dt$ for all $x\in[0,1]$, where $f_k$ is a non-negative monotone increasing function over $[0,1]$. Hence, $F_k$ is a monotone increasing and strictly convex function for $k\in[K-1]$. For $k=K$, we only need $F_k(x)=0$ for all $x\in[0,1]$. Below is the formal definition of the convex program~\ref{eq:convex primal} used in \Cref{alg:opt}.
% \begin{align}
% \tag{Convex-$\mathcal{P}_k$}
% \label{eq:convex primal}
% &\arraycolsep=1.4pt\def\arraystretch{2.2}
% \begin{array}{lll}
%         \max\limits_{\xbf,\ybf,\zbf \geq \mathbf{0}}~~~~
%         &
%         \displaystyle\sum_{\rider\in\Rider_k}
%         \displaystyle\sum_{\config\in\Config}
%         \displaystyle\sum_{\driver\in\Driver}
%         \weight_{\threeindex} 
%         \cdot
%         x_{\threeindex}
%         - 
%         \sum_{\driver\in\Driver}
%         \sum_{\wi \in [\totalweight]}
%         \weightHat_\wi \cdot 
%         \left(
%         \comsumptioni-
%         y_{\twoindex}
%         \right)&
%         \\
%         &
%         \hspace{10mm}
%         -
%         \displaystyle\sum\limits_{\driver\in \Driver}
%         \displaystyle\sum\limits_{\wi \in [\totalweight]}
%         \left(
%         \weightHat_\wi - \weightHat_{\wi - 1}
%         \right)
%         \cdot 
%         F_k\left(
%         \mathop{
%         \displaystyle\sum
%         x_{\threeindex}
%         }
%         \limits_{
%         \substack{
%         \rider\in\Rider_k,\config\in\Config:
%         % (\threeindex)\in E_k,\\
%         \\
%         ~~\weight_{\threeindex}\geq 
%         \weightHat_\wi}
%         }
%         % x_{\threeindex}
%         +
%         \displaystyle\sum\limits_{\wi' \geq \wi}
%         y_{\driver,\wi'}
%         \right)
%         & \text{s.t.}
%         \\
%          &
%         %  \mathop{
%          \displaystyle\sum_{\rider\in\Rider_k}
%          \displaystyle\sum_{\config\in\Config}
%         %  x_{\threeindex}
%         %  }
%         %  \limits_{\rider,\config:(\threeindex)\in E_k}
%          x_{\threeindex}
%          +
%          \displaystyle\sum_{\wi\in[\totalweight]}
%          y_{\twoindex}
%          \leq 1
%          &
%          \driver\in\Driver~,
%          \\
%          &
%          \displaystyle\sum_{\config\in\Config} z_{\rider,\config}\leq 1
%          &
%          \rider\in\Rider_k~,
%          \\
%          &
%          x_{\threeindex}\leq 
%          \alloci\cdot z_{\rider,\config}
%          &
%         %  (\threeindex)\in E_k
%         \rider\in\Rider_k,\config\in\Config,\driver\in\Driver~,
%          \\
%          &
%          y_{\twoindex}\leq \comsumptioni
%          &
%          \driver\in \Driver, \wi\in[\totalweight]~.
%         %  \\
%         %  &x_{\threeindex}\geq 0,~z_{\rider,\config}\geq 0
%         %  &\rider\in\Rider_k,\config\in\Config,\driver\in\Driver~, 
%         %  \\
%         %  &y_{\twoindex} \geq 0
%         %  &\driver\in\Driver,\wi\in[\totalweight]~.
%         %  \\
%         \end{array}
% \end{align}
% Given users $\Rider_k$
% and the revealed pair
% $\left(\allocs\ked,\weightbf\ked\right)$ 
% in stage $k\in [K]$, variable $z_{\rider,\config}$
% in the above program specifies the fractional allocation of
% user $\rider\in\Rider_k$ with configuration $\config\in\Config$. Moreover, variable $x_{\threeindex}$
% specifies the fractional number of impressions created by user $\rider$ form configuration $\config$ that advertiser $\driver$ is willing to pay for after the allocation of stage $k$,
% and thus 
% $\alloci\cdot z_{\rider,\config} - 
% x_{\threeindex}$ impressions of user $\rider$ for advertiser $\driver$ are immediately preempted at the end of stage $k$.
% Finally, variable $y_{\twoindex}$
% specifies the total number of impressions of previous $k - 1$ stages that advertiser $\driver$ is still willing to pay for at 
% per-impression price of 
% $\weightHat_{\wi}$ \emph{after} the allocation/preemption decision of stage $k$, i.e.,
% $\comsumptioni - y_{\twoindex}$
% number of impressions of advertiser $\driver$ which
% were finalized in the previous $k-1$ stages at
% per-impression price of $\weightHat_{\wi}$ will be preempted after stage $k$.


We are now ready to present the main result of this section. We prove this theorem in \Cref{sec:main proof}.

\begin{theorem}[\textbf{Optimal Multi-Stage Algorithm for Configuration Allocation}]
\label{thm:main result configuration allocation}
In the $K$-stage (fractional) configuration allocation problem,
 \PRMCA~(\Cref{alg:opt}) is $\cratio{K}$-competitive, where $\cratio{K}=\cratioexp$.
\end{theorem}




\begin{remark}
% [\textbf{Optimality of the $\boldsymbol{\cratio{K}}$ Competitive Ratio for Configuration Allocation Problem}]
We note that the multi-stage configuration allocation
problem generalizes the multi-stage edge-weighted matching with free-disposal~\citep{FKMMP-09}, budgeted allocation or AdWords with no disposal~\citep{MSVV-07}, and vertex weighted matching with no disposal~\citep{AGKM-11}. As we show later in \Cref{sec:lowerbound}, no integral or fractional multi-stage algorithm can obtain a competitive ratio better than $\cratio{K}$ in the multi-stage (unweighted) matching, and hence $\cratio{K}$ is the optimal competitive ratio for the multi-stage configuration allocation.
\end{remark}}



% The convex program \ref{eq:convex primal}
% plays a crucial role in our optimal 
% competitive algorithm.
% In \Cref{sec:program analysis}, we 
% provide detailed characterizations
% of 
% this convex program by considering its dual
% program.
% Then, 
% combining such characterizations with 
% a primal dual analysis framework,
% we proof the competitive ratio of 
% \Cref{alg:opt}
% in \Cref{sec:main proof}.


\revcolor{\subsection{Properties of Price-Level Regularized Convex Programs via Convex Duality}
\label{sec:convex program}
\input{tex/configuration-allocation-program-analysis}

\subsection{Competitive Ratio Analysis of \Cref{alg:opt}}
\label{sec:main proof}
\input{tex/configuration-allocation-main-proof}
}

==> FN_ multi-stage matching + configuration allocation (MS Journal)/tex/configuration-allocation-main-proof.tex <==
In this section we show the competitive ratio of $\cratio{K}$  for \Cref{alg:opt} as stated in \Cref{thm:main result configuration allocation}. 
Remember the optimum offline 
LP \ref{eq:LP primal} in \Cref{sec:prelim}. We start by considering its dual:
\vspace{1mm}
\begin{equation}
\tag{\textsc{OPT-PRIMAL-DUAL}}
\label{eq:LP}
\arraycolsep=1.4pt\def\arraystretch{1}
\begin{array}{llllllll}
\max\limits_{\xbf,\zbf\geq \boldsymbol{0}}
\quad~~&
% \mathop{\displaystyle\sum
% \weight_{\threeindex}\cdot}
% \limits_{(\threeindex)\in E}
\displaystyle\sum_{\rider\in\Rider}
\displaystyle\sum_{\config\in\Config}
\displaystyle\sum_{\driver\in\Driver}
 \weight_{\threeindex}\cdot x_{\threeindex}
&~\text{s.t.}&
&
\min\limits_{\alphabf,\betabf,\gammabf\geq \boldsymbol{0}}
\quad~~
&
\displaystyle\sum_{\rider\in \Rider }{\alpha_\rider}+
\displaystyle\sum_{\driver\in \Driver}{\beta_\driver}
&~~\text{s.t.} \\[1.4em]
 &
%  \mathop{\displaystyle\sum
%  x_{\threeindex} }
%  \limits_{\rider,\config:(\threeindex)\in E}
\displaystyle\sum_{\rider\in\Rider}
\displaystyle\sum_{\config\in\Config}
x_{\threeindex}
 \leq1 &
 \driver\in\Driver~,& 
& 
&\gamma_{\threeindex} 
+
\beta_\driver \geq \weight_{\threeindex}
& 
\rider\in \Rider,
\config\in\Config,
\driver\in\Driver~,
\\[1.4em]
 &
 \displaystyle\sum\limits_{\config\in\Config}
 z_{\rider,\config}
 \leq 1 
 &
 \rider\in \Rider~, &
& &\alpha_\rider 
\geq 
\displaystyle\sum\limits_{\driver\in \Driver}
\alloci\cdot \gamma_{\threeindex} &i\in \Rider, \config\in \Config~, \\[1.4em]
 &
 x_{\threeindex} \leq 
 \alloci \cdot z_{\rider,\config}
 &
\rider\in \Rider,
\config\in\Config,
\driver\in\Driver~,
 &
& &
 &
\end{array}
\end{equation}

Similar to \Cref{sec:primal-dual}, given the 
feasible primal assignment $\{\xbf\ked,\ybf\ked,\zbf\ked\}_{k\in[K]}$ produced by \Cref{alg:opt} (which leads to a final assignment of $\hat{\xbf}$ when considering the impressions disposals at the end), we construct a non-negative dual assignment so that,
\begin{itemize}
    \item Primal and dual have the same objective values: $$\displaystyle\sum_{\rider\in\Rider}
    \displaystyle\sum_{\config\in\Config}
    \displaystyle\sum_{\driver\in\Driver}\weight_{\threeindex}\cdot \hat{x}_{\threeindex}=\displaystyle\sum_{k\in[K]}\left(
    % \displaystyle\sum_{(\threeindex)\in 
    % E_k}
    \displaystyle\sum_{\rider\in\Rider_k}
    \displaystyle\sum_{\config\in\Config}
    \displaystyle\sum_{\driver\in\Driver}
    \weight_{\threeindex}\cdot x_{\threeindex}\ked - \sum_{\driver\in \Driver}
    \sum_{\wi\in[\totalweight]}
    \weightHat_{\wi}\cdot
    \left(\comsumptioni - y_{\twoindex}\ked
    \right)\right)
    =
    \displaystyle\sum_{\rider\in\Rider}\alpha_\rider
    +
    \displaystyle\sum_{\driver\in\Driver}\beta_\driver$$
    
     \vspace{1mm}
    \item Dual is approximately feasible: 
    % in particular,
    \begin{align*}
    \forall \rider\in\Rider,\config\in\Config,\driver\in\Driver:
    ~~
    &\gamma_{\threeindex}
    +
    \beta_\driver \geq \cratio{K}\cdot \weight_{\threeindex}
    \intertext{and}
    \forall \rider\in \Rider,\config\in\Config: 
    ~~
    &\alpha_{\rider} \geq 
    \displaystyle\sum_{\driver\in \Driver}
    \alloci \cdot \gamma_{\threeindex}
    \end{align*}
\end{itemize}
Existence of such a dual assignment will guarantee that 
\Cref{alg:opt}
is $\cratio{K}$-competitive.

Our dual assignment is constructed stage-by-stage.
First, set $\alpha_i\gets 0$, $\beta_j\gets 0$,
and $\gamma_{\threeindex} \gets 0$
for all $\rider\in\Rider,\config\in\Config,\driver\in\Driver$. 
At each stage $k\in[K-1]$, 
let $(\lambdabf\ked,\thetabf\ked,\mubf\ked,\psibf\ked,\phibf\ked)$
to denote 
$(\lambdabf\starred,\thetabf\starred,\mubf\starred,\psibf\starred,\phibf\starred)$ in \Cref{lem:KKT restate},
and $\cumcomsumptioni\ked$
to denote $\cumcomsumptioni(\xbf\ked,\ybf\ked)$.
Consider the following assignment corresponding to stages $k\in[K-1]$ for the dual program in \ref{eq:LP}:
\begin{align*}
   &\forall \rider \in \Rider_k: 
   &
   &\alpha_\rider\gets 
%   \sum_{\config \in \Config}
%   z_{\rider,\config}\ked\cdot 
   \lambda_\rider\ked
   \\
   &\forall \rider\in\Rider_k,
   \config\in\Config,
   \driver\in\Driver:
%   \in E_k:
   &
   &
   \gamma_{\threeindex} \gets
   \mu_{\threeindex}\ked 
   \\
    &\forall \driver \in \Driver: &&\beta_{\driver}\gets\beta_{\driver}+\Delta\beta_{\driver}\ked\\
    &&&
    \Delta\beta_{\driver}\ked
    \triangleq 
    \sum_{\rider\in\Rider_k}
    \sum_{\config\in\Config}
    % \sum_{\rider,\config:(\threeindex)\in E_k}
    x_{\threeindex}\ked
    \left(
    % \theta_{\driver}\ked + 
    \sum_{\wi\in[\totalweight]:
    \weightHat(\wi) \leq \weight_{\threeindex}}
    \left(\weightHat_\wi - \weightHat_{\wi-1}\right)
    \cdot 
    % F_{\twoindex}(\xbf\ked, \ybf\ked)
    f_k\left(\cumcomsumptioni\ked\right)
    \right)
    \\
    &&&
    \hspace{25mm}
    -
    \sum_{\wi\in[\totalweight]}
    \weightHat_{\wi}\cdot
    \left(\comsumptioni - y_{\twoindex}\ked
    \right)
\end{align*}
For the last stage $K$,
let $(\lambdabf\KED,\thetabf\KED,\mubf\KED,\pibf\KED)$
be the optimal solution of \ref{eq:convex dual K}.
We consider the following assignment corresponding to stage $K$ for the dual program in \ref{eq:LP}:
\begin{align*}
   &\forall \rider \in \Rider_k: 
   &
   &\alpha_\rider\gets 
   \lambda_\rider\KED
   \\
   &\forall (\threeindex) \in E_k:
   &
   &
   \gamma_{\threeindex} \gets
   \mu_{\threeindex}\KED 
   \\
    &\forall \driver \in \Driver: &&\beta_{\driver}\gets\beta_{\driver}+\Delta\beta_{\driver}\KED\\
    &&&
    \Delta\beta_{\driver}\KED
    \triangleq 
    \thetai\KED 
    -
    \sum_{\driver\in\Driver,\wi\in[\totalweight]}
    \comsumption_{\twoindex}\KMINUSED
    \cdot (\weightHat_{\wi} - \pi_{\twoindex}\KED)
\end{align*}


The rest of the proof is quite technical and we postpone to Appendix~\ref{apx:proof-primal-dual-CA}. Interestingly, the proof heavily relies on all the properties that we identified in \Cref{sec:convex program}; in particular, we use the \emph{``Connection''} (\Cref{lem:KKT restate}) combined with the \emph{``Disposing Smallest Price''} (\Cref{lem:preempt monotone}) and its corollary (\Cref{coro:cumulative comsumption monoton}) to show for all stages $k\in[K-1]$ we have an equal change in the dual and primal objectives. For the last stage $K$, this property holds by construction. In order to show the approximate dual feasibility for constraints corresponding to stages $k\in[K-1]$, again we rely on the \emph{``Connection''} (\Cref{lem:KKT restate}). However, showing dual approximate feasibility for the constraints corresponding to last stage is a bit different. There, we heavily use \emph{``Low Prices of Last Stage''} (first part of \Cref{lem:dual restate theta K}) and \emph{``High Prices of Last Stage''} (second part of \Cref{lem:dual restate theta K}) to do the analysis. 




==> FN_ multi-stage matching + configuration allocation (MS Journal)/tex/configuration-allocation-program-analysis.tex <==

Fix any stage $k\in[K]$. We now aim to identify/characterize some useful properties of the convex program \ref{eq:convex primal}. To simplify our study, we define the following notation for any $(\xbf,\ybf)$:
$$\cumcomsumptioni(\xbf,\ybf)\triangleq\sum
% \limits
_{
        \substack{\rider\in\Rider_k,\config\in\Config:
        \\
        ~~\weight_{\threeindex}\geq 
        \weightHat_\wi}
        }
        x_{\threeindex}
        +
        \sum_{\wi' \geq \wi}
        y_{\driver,\tau'}$$
Note that if 
$(\xbf\ked, \ybf\ked,\zbf\ked)$ is the fractional allocation selected by \Cref{alg:opt} (i.e., optimal solution of \ref{eq:convex primal}), then 
by definition, $\cumcomsumptioni(\xbf\ked,\ybf\ked) = \sum_{\tau'\geq \tau} \comsumption_{\twoindex}\ked$. In other words, $1-\cumcomsumptioni(\xbf\ked,\ybf\ked)$ is essentially the cumulative per-impression price distribution of advertiser $j$ at the end of stage $k$. Note that in the first $K - 1$ stages, 
the objective function in program~\ref{eq:convex primal}
is strictly concave,
while the convex program
degenerates to a linear program in the last stage $K$. For this reason, we study the properties of stages $k \in [K - 1]$
and the last stage $K$ separately. 

\smallskip
\noindent\textbf{Properties of Stage $\boldsymbol{k\in [K - 1]}$.}
To characterize the properties of the optimal solution in 
\ref{eq:convex primal} for stage $k\in[K-1]$,
we consider its 
Lagrangian relaxation 
and KKT optimality conditions.
Specifically, 
the Lagrangian dual \ref{eq:convex dual}
of \ref{eq:convex primal}
can be written as follows,
\begin{align*}
\arraycolsep=1.4pt\def\arraystretch{2.2}
    \tag{$\mathcal{D}^{\textsc{MCA}}_k$}
\label{eq:convex dual}
\begin{array}{ll}
   \min\limits_{\substack{\lambdabf,\thetabf,\mubf,\pibf,\\
   \psibf,\phibf,\iotabf\geq 0}} 
   &
   \max\limits_{\xbf,\ybf,\zbf\geq \mathbf{0}} 
           \displaystyle\sum_{\rider\in\Rider}
           \displaystyle\sum_{\config\in\Config}
           \displaystyle\sum_{\driver\in\Driver}
        \weight_{\threeindex} 
        \cdot
        x_{\threeindex}
        - 
        \sum_{\driver\in\Driver}
        \sum_{\wi \in [\totalweight]}
        \weightHat_\wi \cdot 
        \left(
        \comsumptioni-
        y_{\twoindex}
        \right)
    \\
     & 
        \hspace{10mm}
        -
        \displaystyle\sum\limits_{\driver\in \Driver}
        \displaystyle\sum\limits_{\wi \in [\totalweight]}
        \left(
        \weightHat_\wi - \weightHat_{\wi - 1}
        \right)
        \cdot 
        F_k\left(
        % \displaystyle\sum\limits_{
        % \substack{\rider,\config:
        % (\threeindex)\in E_k,\\
        % ~~\weight_{\threeindex}\geq 
        % \weightHat_\wi}
        % }
        % x_{\threeindex}
        % +
        % \displaystyle\sum\limits_{\wi\primed \geq \wi}
        % y_{\driver,\tau\primed}
        \cumcomsumptioni(\xbf,\ybf)
        \right)\\
        &
        \hspace{10mm}
        - 
        \displaystyle\sum_{\driver\in \Driver}
        \thetai\cdot 
        \left(
        % \mathop{
        % \displaystyle\sum
        %  x_{\threeindex}
        %  }
        %  \limits_{\rider,\config:(\threeindex)\in E_k}
        \displaystyle\sum_{\rider\in\Rider_k}
        \displaystyle\sum_{\config\in\Config}
         x_{\threeindex}
         +
         \displaystyle\sum_{\wi\in[\totalweight]}
         y_{\twoindex}
         - 1
        \right)
        -
        \displaystyle\sum_{\rider\in\Rider_k}
        \lambdai\cdot 
                \left(
        \displaystyle\sum_{\config\in\Config} z_{\rider,\config}
         - 1
        \right)
        \\
        &
        \hspace{10mm}
        -
        % \mathop{\displaystyle\sum
        % \mui}
        % \limits_{(\threeindex)\in E_k}
           \displaystyle\sum_{\rider\in\Rider}
           \displaystyle\sum_{\config\in\Config}
           \displaystyle\sum_{\driver\in\Driver}
           \mui\cdot 
        \left(x_{\threeindex} - \alloci\cdot z_{\rider,\config}
        \right)
        -
        \displaystyle\sum_{\driver\in \Driver}
        \displaystyle\sum_{\wi\in[\totalweight]}
        \pi_{\twoindex}\left(
        y_{\twoindex} - \comsumptioni
        \right)
        \\
        &
        \hspace{10mm}
        +
        % \mathop{\displaystyle\sum
        % \psii\cdot
        % }\limits_{(\threeindex)\in E_k}
           \displaystyle\sum_{\rider\in\Rider}
           \displaystyle\sum_{\config\in\Config}
           \displaystyle\sum_{\driver\in\Driver}
        \psii\cdot 
        x_{\threeindex}
        +
        % \mathop{\displaystyle\sum
        %  \phii  \cdot z_{\rider,\config}}
        % \limits_{\rider,\config:\exists (\threeindex)\in E_k}
        \displaystyle\sum_{\rider\in\Rider}
           \displaystyle\sum_{\config\in\Config}
           \phii  \cdot z_{\rider,\config}
        +
        \displaystyle\sum
        \limits_{\driver\in \Driver}
        \displaystyle\sum_{\wi\in[\totalweight]}
        % \cdot
        \iota_{\twoindex}\cdot
        y_{\twoindex}
\end{array}
\end{align*}
We start with the following lemma (proved in Appendix~\ref{apx:kkt-CA}) which builds 
a connection between the optimal solutions of
 \ref{eq:convex primal} and \ref{eq:convex dual}.
Briefly speaking, this lemma can be thought as
a collection of equalities extracted from
KKT conditions, which will later be used in the
competitive ratio analysis of \Cref{alg:opt}.
\begin{lemma}[Duality-based Connection]
\label{lem:KKT restate}
Fix any $k\in[K - 1]$.
Suppose $(\xbf\starred,\ybf\starred,\zbf\starred)$
is the optimal solution of the 
convex program \ref{eq:convex primal}.
There exists non-negative ($\lambdabf\starred, \thetabf\starred,
\mubf\starred, \psibf\starred,\phibf\starred$)
such that for all $(\threeindex)\in E_k$
\begin{align}
    \tag{complementary slackness}
    \label{eq:cs}
    \begin{split}
        % \thetai\starred
        % \left(
        % \displaystyle\sum_{\rider,\config:(\threeindex)\in E_k}
        %  x_{\threeindex}\starred
        %  +
        %  \displaystyle\sum_{\wi\in[\totalweight]}
        %  y_{\twoindex}\starred
        %  - 1
        % \right)
        % = 0 \\
        \lambdai\starred
                \left(
        \displaystyle\sum_{\config\in\Config} z_{\rider,\config}\starred
         - 1
        \right)
        =0
        \hspace{10mm}
        \mui\starred
        \left(x_{\threeindex}\starred
        - \alloci\cdot z_{\rider,\config}\starred
        \right) = 0
        \\
        \thetai\starred=0 \hspace{10mm}\psii\starred\cdot x_{\threeindex}\starred
        =0
        \hspace{10mm}
        \phii\starred\cdot z_{\rider,\config}\starred
        =0
    \end{split}
\end{align}
\begin{align}
    \label{eq:stationary z}
\tag{stationarity-1}
    \sum_{\driver\in \Driver}\alloci \cdot \mui\starred - \lambdai\starred + \phii\starred = 0
    % &
    % \hspace{10mm}
    % \forall \rider \in \Rider_k
    \\
\tag{stationarity-2}
\label{eq:stationary x}
    \weight_{\threeindex}
    -
    \sum\limits_{\wi\in[\totalweight]:
    \weightHat(\wi) \leq \weight_{\threeindex}}
    \left(\weightHat_\wi - \weightHat_{\wi-1}\right)
    \cdot 
    f_{k}(\cumcomsumptioni(\xbf\starred, \ybf\starred))
    % -
    % \thetai\starred 
    - \mui\starred + \psii\starred = 0
    % &
    % \hspace{10mm}
    % \forall (\threeindex)\in E_k 
\end{align}
\end{lemma}


Besides the above lemma, we intuitively expects that the optimal solution 
$(\xbf\starred,\ybf\starred,\zbf\starred)$
of \ref{eq:convex primal}
satisfies the following property:
whenever the entire capacity of a given advertiser is exhausted
and preemption is needed, 
it is optimal to dispose impressions which are allocated with the smallest price. 
% for any advertiser $\driver$,
% if there exists $x_{\threeindex}\starred > 0$
% and $\comsumptioni - y_{\twoindex} >0$,
% then we have $\weight_{\threeindex} \geq 
% \weightHat_{\wi}$,
% i.e., \Cref{alg:opt} only preempt  
% units of a advertiser from lower revenue level 
% to higher revenue level.
This intuition can be formalized below
and proved by convex duality (see Appendix~\ref{apx:kkt-CA-smallest}).
\begin{lemma}[Disposing Smallest Price]
\label{lem:preempt monotone}
Fix $k\in[K - 1]$.
Suppose $(\xbf\starred,\ybf\starred,\zbf\starred)$
is the optimal solution of \ref{eq:convex primal}.
For any advertiser $\driver\in \Driver$, and $\wi\in [\totalweight]$,
if $\comsumptioni - y_{\twoindex}^* > 0$,
then $\cumcomsumptioni(\xbf\starred,\ybf\starred) = 1$.
\end{lemma}

\Cref{lem:preempt monotone} gives us the following
corollary (proved in Appendix~\ref{apx:kkt-CA-cor1}), which again will later help with our competitive ratio analysis of \Cref{alg:opt}.


\begin{corollary}
Fix $k\in[K - 1]$.
\label{coro:cumulative comsumption monoton} 
Suppose $(\xbf\starred,\ybf\starred,\zbf\starred)$
is the optimal solution of \ref{eq:convex primal}. For any advertiser $\driver\in \Driver$, and $\wi\in [\totalweight]$, we have:
\begin{itemize}
    \item (\textbf{Distribution Monotonicity}) $\displaystyle\cumcomsumptioni(\xbf\starred,\ybf\starred) \geq 
\sum_{\wi'\geq \wi}\comsumptioni$.
\item (\textbf{Only Disposing Smallest}) $\displaystyle\sum_{\wi'\geq \wi}\left(\comsumption_{\driver,\wi'}\kminused - y_{\driver,\wi'}^*\right)
=
\sum_{\wi'\geq \wi}\left(\comsumption_{\driver,\wi'}\kminused - y_{\driver,\wi'}^*\right)
\cdot
f_k\left(\cumcomsumptioni(\xbf\starred,\ybf\starred)\right)$.
\end{itemize}
\end{corollary}


% \begin{corollary}
% Fix $k\in[K - 1]$.
% \label{coro:preempt complementary slackness}
% Suppose $(\xbf\starred,\ybf\starred,\zbf\starred)$
% is the optimal solution of \ref{eq:convex primal}.
% For any advertiser $\driver\in \Driver$, and $\wi\in [\totalweight]$,
% $\sum_{\wi'\geq \wi}\left(\comsumption_{\driver,\wi'}\kminused - y_{\driver,\wi'}^*\right)
% =
% \sum_{\wi'\geq \wi}\left(\comsumption_{\driver,\wi'}\kminused - y_{\driver,\wi'}^*\right)
% \cdot
% f_k\left(\cumcomsumptioni(\xbf\starred,\ybf\starred)\right)$.
% \end{corollary}

\smallskip
\noindent\textbf{Properties of the Last Stage $K$.}
For
stage $K$, 
note that $F_K(a) = 0$ for all $a \in [0, 1]$
and thus convex program \ref{eq:convex primal} 
degenerates to a linear program,
which solves the optimal configuration allocation
for the last stage graph under $\boldsymbol{\comsumption}\KMINUSED$.
This linear program \ref{eq:convex primal}  
admits a dual as follows,
\begin{align}
\tag{LP-$\mathcal{D}_K$}
\label{eq:convex dual K}
\arraycolsep=1.4pt\def\arraystretch{2.2}
    \begin{array}{lll}
    \min\limits_{\lambdabf,\thetabf,\mubf,\pibf\geq 0} &
    \displaystyle\sum_{\rider\in \Rider_K} \lambdai 
    +
    \displaystyle\sum_{\driver\in \Driver} \thetai
    -
    \displaystyle\sum_{\driver\in\Driver}
    \displaystyle\sum_{\wi\in[\totalweight]}
    \comsumption_{\twoindex}\KMINUSED
    \cdot (\weightHat_{\wi}- \pi_{\twoindex})
    &\text{s.t.}
    \\
    &
    \mui + \thetai \geq \weight_{\threeindex}
    & \rider\in\Rider_K, \config\in\Config,
    \driver\in \Driver~,
    \\
    &
    \thetai + \pi_{\twoindex} \geq \weightHat_{\wi}
    &
    \driver\in\Driver,\wi\in[\totalweight]~,
    \\
    &
    \lambdai \geq \displaystyle\sum_{\driver\in\Driver}
    \alloci\cdot \mui
    &
    \rider\in \Rider_K,
    \config\in \Config~.
    \end{array}
\end{align}

Technically speaking, the optimal 
solution of the dual program \ref{eq:convex dual K} for the last stage
satisfies the same KKT-like equalities/inequalities
as the solution of the Lagrangian dual program
\ref{eq:convex dual} for the first $K-1$ stages.
The main difference is the value of 
the optimal
$\thetai\starred$.
As we showed in \Cref{lem:KKT restate},
$\thetai\starred = 0$ in the first $K - 1$ stages.
This follows from 
the construction of function $F_k(\cdot)$, and in particular, the property that $\frac{d}{dx}F_k(1) = f_k(1) = 1$.
In contrast, $F_K\equiv 0$ in the last stage $K$,
and the value of the optimal $\thetai\starred$
can be strictly positive. It turns out this makes the competitive ratio analysis of \Cref{alg:opt} in the last stage a bit different from the previous stages. We introduce the following auxiliary lemma
to characterize the required properties of dual program \ref{eq:convex dual K} to help with this different part of the analysis. The proof is deferred to Appendix~\ref{apx:last-stage-lemma}.
\begin{lemma}
\label{lem:dual restate theta K}
Suppose 
$(\lambdabf\starred,\thetabf\starred,\mubf\starred,\pibf\starred)$
is the optimal solution of the dual program \ref{eq:convex dual K}.
For any advertiser $\driver\in\Driver$,
$\wi\in[\totalweight]$,
\begin{itemize}
    \item(\textbf{Low Prices of Last Stage}) \mbox{if $\weightHat_\wi\leq \thetai\starred $}:~~~~$\comsumption_{\twoindex}\KMINUSED\cdot \pi_{\twoindex}\starred = 0$
    \item(\textbf{High Prices of Last Stage}) \mbox{if $\weightHat_\wi>\thetai\starred $}:~~~~$\comsumption_{\twoindex}\KMINUSED
     \cdot 
     (
     \weightHat_{\wi} - \pi_{\twoindex}\starred)
    = 
     \comsumption_{\twoindex}\KMINUSED\cdot \thetai\starred$
\end{itemize}
% \begin{align*}
%     \comsumption_{\twoindex}\KMINUSED\cdot \pi_{\twoindex}\starred = 0
%     \;\;\mbox{if $\weightHat_\wi \leq \thetai\starred$; and}
%     \;\;
%      \comsumption_{\twoindex}\KMINUSED
%      \cdot 
%      (
%      \weightHat_{\wi} - \pi_{\twoindex}\starred)
%     = 
%      \comsumption_{\twoindex}\KMINUSED\cdot \thetai\starred
%     \;\;\mbox{if $\weightHat_\wi \geq \thetai\starred$}
% \end{align*}

% if $\weightHat_\wi \leq \thetai\starred$,
% then
% % \begin{align*}
%     $\comsumption_{\twoindex}\KMINUSED\cdot \pi_{\twoindex}\starred = 0$;
% % \end{align*}
% % \intertext{
% and if $\weightHat_\wi \geq \thetai\starred$,
% then
% % }
% % \begin{align*}
%     $\weightHat_{\wi} - \pi_{\twoindex}\starred 
%     = 
%     \thetai\starred$
% % \end{align*}
\end{lemma}

% First, we present the following lemma 
% which characterizes the optimal solution
% in program \ref{eq:convex primal}
% for stage $K$
% and its dual program 
% \ref{eq:convex dual K}.

% \begin{lemma}
% \label{lem:LP dual restated}
% Suppose $(\xbf\starred,\ybf\starred,\zbf\starred)$
% is 
% the optimal solution of the linear
% program \ref{eq:convex primal}
% for the last stage $K$ and
% $(\lambdabf\starred,\thetabf\starred,\mubf\starred,\pibf\starred)$
% is the optimal solution of the dual program \ref{eq:convex dual K}.
% Then,
% \begin{align}
%     \theta_{j}\starred =  
%      \weightHat_{\wi} - \pi_{\twoindex}\starred
%      \text{ if $y_{\twoindex}\starred > 0$}
% \end{align}
% \end{lemma}


==> FN_ multi-stage matching + configuration allocation (MS Journal)/tex/extensions_old.tex <==
\section{Extensions}
\label{sec:extensions Adwords}

In this section,
we discuss how 
our approach can be generalized 
to the multi-stage vertex weighted
b-matching problem, and 
the multi-stage AdWords problem.


\subsection{Multi-stage Vertex Weighted b-Matching}
\label{sec:weighted b-matching}
\input{tex/b-matching}

  
    
    \subsection{Multi-stage AdWords}
    \label{sec:adwords}
    \input{tex/adwords}



==> FN_ multi-stage matching + configuration allocation (MS Journal)/tex/fig-poly.tex <==
\begin{figure}[hbt!]
	\centering
	\subfloat[
    $k = K$
	]{
	\input{figs/fig-1}
	}
	\subfloat[
    $k = K - 1$
	]{
	\input{figs/fig-2}
	}
	\subfloat[
    $k = K - 2$
	]
	{
	\input{figs/fig-3}
	}
	\\
	\centering
	\subfloat[
    $k = K - 3$
	]{
	\input{figs/fig-4}
	}
	\subfloat[
    $k = K - 4$
	]{
	\input{figs/fig-5}
	}
	\subfloat[
    $k = K - 5$
	]
	{
	\input{figs/fig-6}
	}
	\caption{
	Polynomial regularizer $f_k(x)$
	in \Cref{prop:poly}
	(solid line)
	versus 
	$e^{x-1}$ (dashed line).
    }
	\label{fig:poly}
\end{figure}

==> FN_ multi-stage matching + configuration allocation (MS Journal)/tex/intro-configuration-allocation.tex <==
\newcommand{\cratio}[1]{\Gamma(#1)}
\newcommand{\cratioexp}{1-\left(1-\frac{1}{K}\right)^K}
\section{Introduction}
\label{sec:intro}
Thanks to ever-expanding popularity of online platforms and growth of web-based services, internet advertising has grown to become a major component of today's economy. Worldwide spending of internet advertising stood at an estimated 378 billion U.S. dollars in 2020---a figure that is forecast to constantly increase in the coming years, reaching a total of 646 billion U.S. dollars by 2024. The combination of the economic impact and the inherent flexibility of internet advertising not only has helped with the prevalence of this form of advertising, but it has also given rise to numerous important computational and economics problems, some of which pertain to real-time algorithmic allocation of ad opportunities to advertisers in various search and display advertising scenarios, e.g., see \cite{MSVV-07,FKMMP-09,BFMM-14,DHKMQ-16}. 

As digital consumption behaviors evolve, and new technologies provide new ways for users to interact with social media platforms and publishers, traditional forms of internet advertising are also being completely transformed. This brings new paradigms and challenges to the real-time ad allocation problem, and enriches the field with new and exciting research questions. A prominent example of this sort, which is the main motivating application behind our paper, is \emph{in-stream video advertising}. Nowadays, in-stream video advertising is rapidly growing,\footnote{According to \citet{Deloitte}, 80\% of U.S. consumers are now paying for streaming video service, up from 73\% before the COVID-19 pandemic began. Using ad spending as an indicator, video advertising will likely continue to grow for the foreseeable future. Video ad spending in the U.S. is increased from 8.92 billion U.S. dollars in 2017 to 10.18 billion U.S. dollars in 2019; it is also projected to reach as high as 12.66 billion U.S. dollars by 2024.} and plays an essential role in the business model of online video sharing platforms such as YouTube and Vimeo, on-demand/live streaming platforms and TVs such as Netflix, Roku, and Twitch, and even social live streaming platforms such as Facebook Live. In this application, when a user starts watching a new video session (e.g., on YouTube), an advertising opportunity to display \emph{video-ads}, and hence allocating user impressions to advertisers, is created. Video-ads refer to all  ad formats that appear before, during, or after a streaming video. These formats include in-stream advertising videos of different lengths, as well as the banner-like overlay and text- or image-based ads that appear over a video. See \Cref{fig:ad-formats} for specific video-ad formats that are currently used in YouTube.\footnote{See \url{https://support.google.com/youtube/answer/2375464?hl=en}}


\captionsetup[subfloat]{captionskip=0pt}
\begin{figure}[hbt!]
	\centering
	\subfloat[
   Skippable in-stream ads
	]{
\includegraphics[scale=0.42]{figs/skippable-video-ads.png}
	}
	\subfloat[Non-skippable in-stream ads]{
\includegraphics[scale=0.42]{figs/non-skippable-video-ads.png}
	}
	\subfloat[
   Bumper short ads
	]
	{
\includegraphics[scale=0.42]{figs/bumper-ads.png}
	}
	\\
	\centering
	\subfloat[
   Overlay ads
	]{
\includegraphics[scale=0.44]{figs/overlay-ads.png}
	}
	\subfloat[
   Clickable sponsored cards
	]{
\includegraphics[scale=0.44]{figs/sponsored-cards.png}
	}
	\vspace{1mm}
	\caption{
Different formats of video advertising in YouTube streaming; These formats can be used at different time-stamps of a YouTube video, and differ in their lengths, designs, and how users interact with them.}
	\label{fig:ad-formats}
\end{figure}

Given these ad format varieties, the real-time ad allocation for a sequence of arriving users is done by assigning each user (or equivalently, each video session) to one of feasible ``configurations". Here, a configuration can refer to an arrangement of video-ads of various lengths and formats for a subset of advertisers, showing up at different time-stamps of the user's video session.\footnote{It can also be the case that a long video session is divided into chunks, and then each chunk is assigned a separate configuration, i.e., is treated as a new video session.}  Particularly important in this application, the set of feasible configurations can model various user-level constraints such as \emph{exclusion} (e.g., competing advertisers can not be shown in the same video), \emph{frequency capping} (e.g., similar ads should not be shown back to back in the same video), or \emph{bundling} (e.g., when advertisers require that all or none of a set of related
ads be shown in the same video). 

While in-stream video ad allocation is a real-time application, it still admits a natural form of allowance for latency in showing ads to users. In fact, as several of these video-ads show up in the middle (or at the end) of users' video sessions, an ad allocator can delay the selection of a configuration for a session (or the current chunk of a long video session) from the beginning of the video to the first time-stamp that a video-ad is required to be displayed. This flexibility provides an immense opportunity for the ad allocator to \emph{batch} the arriving video sessions into large groups without any loss. More formally, a batch consists of the most recent group of users that should be assigned configurations in the same time frame. Given these batches, the ad allocator can make stage-wise allocation decisions as each batch of users arrives---in contrast to fully online decisions as each single user arrives---in order to make more profitable allocation decisions. 

\vspace{3mm}
\noindent\textbf{{Our Theoretical Lens}}~~Motivated by the above application, we study the design of multi-stage allocation algorithms for the configuration allocation problem under adversarial batch arrival. In this problem, we have online users (each corresponds to a new video session) that arrive in $K>0$ batches over a finite horizon,\footnote{We assume the parameter $K$ is fixed and known by the algorithm.} and offline advertisers that have ads to be displayed to the users in order to obtain impressions. Once a batch arrives, the multi-stage allocation algorithm (fractionally or integrally) assigns a feasible configuration to each user in that batch. These decisions are made stage-wise and are irrevocable. Each assigned configuration yields a certain number of impressions to each advertiser and charges the advertiser at a certain price per impression.  The per-impression prices of each feasible configuration assigned to a user, as well as the number of impressions reserved for different advertisers, are revealed when the batch corresponding to this user arrives. Depending on advertisers' long-term contracts, each advertiser is willing to pay for a certain number of impressions during the decision making horizon. Given this model, the goal of the algorithm is maximize the revenue (i.e., total collected prices) in the finite decision making horizon.

We measure the performance of our algorithm by its \emph{competitive ratio}, which is the worst-case ratio between the  revenue of the algorithm and a particular benchmark, given a fixed number of batches. Our goal is to design multi-stage competitive algorithms with respect to the in-hindsight optimal---also known as the optimum offline benchmark. One extreme regime of this problem is the fully offline when there is only a single large batch containing all the users---in which one can achieve the performance of the optimum offline. The other extreme regime is the fully online when each online user arrives as a batch of size one (no batching). While designing optimal competitive (fractional) allocation algorithms for the fully online version has been studied in the literature~\citep{DHKMQ-16}, the middle-ground multi-stage variant with fixed $K$ stages---when allocations are made batch-by-batch---is not studied. We now ask the following informal research question in this paper:

\smallskip
\begin{displayquote}
\emph{In the middle-ground multi-stage regime of configuration allocation problem with batch arrivals (in contrast to fully online and offline regimes), when we have $K >0$ number of batches, what is the optimal competitive ratio achievable by a multi-stage algorithm?}
\end{displayquote}


\vspace{3mm}
\noindent\textbf{{Main Result}}~~
%  \RN{@Yiding: I think what we have is good for a first draft, but it would be better if you can add a bit more technical content. Again, think about ways that either our algorithm or our analysis is creative. Also, it would be helpful to provide more context regarding the algorithm, polynomials we use, and the connection to the recursive equation (it's fine if it has overlap with FN-21; imagine it is very likely that a reviewer hasn't seen our previous paper and should be able to understand what's going on in this paper without looking at that paper. Finally, try to polish the writing of these paragraphs as much as you can while I am polishing the rest of the paper. I will get back to it later.}
As the main result of this paper,
we introduce and analyze an \emph{optimal competitive}
algorithm (\Cref{alg:opt})
for the fractional
multi-stage configuration 
allocation problem, which can easily be extended to the integral version under the large budget assumption (see \Cref{footnote:integral} on Page~9 for more details).
When there are $K$ stages,
\Cref{alg:opt} attains
the competitive ratio of 
$\cratio{K}\triangleq 1 - \left(1 - \frac{1}{K}\right)^K$. This ratio is  optimal for any fixed number of stages $K\in\mathbb{N}$, that is, no multi-stage algorithm---whether fractional or integral---can obtain a better competitive ratio than $\cratio{K}$ even in the special case of the multi-stage matching (thanks to the upper-bound result of \citealp{FN-21} for this special case). The competitive ratio function $\cratio{K} \in (1 - 1/e, 1]$
is monotone decreasing in $K$. 
It is equal to 1 at $K = 1$ and converges 
to $1 - 1/e$ as $K$ goes to infinity. Moreover, for any constant $K$, this ratio has a constant improvement over $1-1/e$ (which is the best achievable bound for the fully online version of this problem, thanks to the main result of \citealp{DHKMQ-16}). For example, this ratio is equal to $\frac{3}{4}$ for the two-stage version of the problem, and is equal to $\frac{19}{27}$ for the three-stage version.

\vspace{3mm}
\noindent\textbf{{Overview of the Techniques}}~~The first key technical ingredient 
in this work is the stage-dependent 
\emph{price-level regularized convex program}
\ref{eq:convex primal}
% stage-dependent convex programs
used in \Cref{alg:opt} for each stage $k\in[K]$.
It identifies a particularly \emph{balanced}
configuration assignment for each stage. 
The intuition behind the necessity of 
balancedness is simple and goes back to the classic work on online bipartite matching and its extensions \citep{KVV-90,KP-00,MSVV-07}. 
Consider a greedy algorithm
which selects the configuration assignment for the 
current stage
to maximizes the total revenue collected so far. 
This greedy algorithm can potentially suffer
a revenue loss due to the lack of enough balancedness, as an adversary can exploit this situation. While balancedness of the allocation in each stage is a property that at high-level should help the multi-stage algorithm to remain competitive against
the future stages constructed by an adversary, it is not clear at all how to use the structure of the problem (in particular, the fact that each advertiser essentially pays for impressions at different price levels) to introduce the required balancedness in each stage. Furthermore, it is not clear how to change the amount of balancedness over the span of $K$ stages. 
We use our convex programs
\ref{eq:convex primal}
to provide remedies for both of these challenges.

The configuration assignment
of the greedy algorithm 
can be solved by a linear program (LP).
Our convex program \ref{eq:convex primal}
is a regularized version of this LP
for the greedy algorithm.
In particular, 
% In these stage-dependent convex programs,
instead of maximizing the total revenue collected so far,
its objective is to maximizing total collected revenue minus a regularization term. This regularization term is the sum of different terms, where we have one regularizer term for each advertiser
at different possible per-impression price levels. 
For any fixed advertiser,
consider a quantity which keeps track of
the number of his impressions at each per-impression price (i.e., the number of impressions at different prices levels that the advertiser is willing to pay so far).
The regularizer term for this advertiser 
is a function
mapping the aforementioned quantity 
to a penalty in the objective of the
convex program \ref{eq:convex primal}
at each stage $k\in[K]$.


Intuitively speaking, 
\Cref{alg:opt} should incorporate ``more intense'' regularization
at early stages and then gradually shift towards no regularization
in the last stage. 
Our convex programs indeed capture such an intuition---it uses a particular sequence of polynomial functions with decreasing degrees
as the regularizer functions of stages $k=1,2,\ldots,K$.
This sequence of polynomial regularizers with decreasing degrees 
has been used in \citet{FN-21}, in which authors 
consider the multi-stage vertex-weighted bipartite matching problem (which is
a special case of our configuration allocation problem).
In their proposed scheme, the regularizers map 
the remaining capacity of each offline node to 
a penalty term in  the objective. 
As we mentioned above, 
in the configuration allocation problem,
the regularizers in \ref{eq:convex primal}
are mappings from 
the number of impressions at different per-impression price levels to non-negative penalties, and hence are of higher dimensions. At high-level, a similar paradigm plays a crucial role in 
\citet{DHKMQ-16},
in
which authors study the configuration allocation problem
with vertex arrival (rather than batch arrival). 
Namely, their model can be thought as the 
special case where
the number of stages $K$
is the number of online nodes 
(a.k.a., users), 
and in each stage only one user arrives.
They provide an optimal $(1-1/e)$-competitive algorithm for this fully online version.
% , which attains optimal competitive ratio in that problem. 
Their algorithm determines the configuration assignment using a continuous iterative method based on an adhoc, yet intuitive, rule.
Kind of surprisingly, as a side result in our paper, we find an alternative interpretation for this algorithm in \citet{DHKMQ-16}: the outcomes of the continuous procedures for each arriving user in
\citet{DHKMQ-16} are precisely captured by the optimal 
solution of our convex programs when we are in the special case of batch arrival with batches of size $1$ and we use \emph{the same exponential function} $f_k(x)=e^{x-1}$ 
as the regularizer functions 
for every single arriving user, rather than our polynomials (see \Cref{thm:main result} and statement of \Cref{alg:opt}).

% For any multi-stage configuration allocation 
% algorithm,
% in each stage, it needs to 
% (i) assign feasible configuration to each user
% arriving in that stage,
% and 
% (ii) keep track of impressions 
% for which each advertiser will pay.\footnote{Different impressions may have 
% different per-impression prices.}
% When there is $K = 1$ stage, 
% the optimal fractional 
% configuration allocation algorithm
% is a two-layer greedy algorithm --
% (i) fixing the impressions allocation, 
% it greedily charges each advertiser
% impressions with highest per-impression
% prices; 
% (ii) given (i) it
% greedily assigns users configurations 
% to maximize the revenue.
% Since the payment are charged 
% at the end of all stages,
% there is no loss 
% to greedily maintain a list of  
% impressions for which advertisers 
% are charged,
% even if there are $K > 1$ stages.
% Specifically, 
% suppose the greedy algorithm decides not to charge 
% an advertiser with an impression with certain per-impression
% price. It must be the case that there exists 
% other impressions with higher per-impression price allocated to this advertiser and fulfilled all his demand.
% As a consequence, the greedy algorithm will not 
% revert its decision and charge for that impression with lower per-impression in the future.
% On the other hand, 
% such two-layer greedy algorithm
% suffers from the lack of balancedness
% on configuration assignment, i.e., (ii).
% Hence, comparing to this two-layer greedy algorithm,
% \Cref{alg:opt} outputs 
% a more balanced configuration assignment
% that not only considers the additional revenue gain
% from the current stage, but also 
% provides hedging against the future stages.

% The outcome of the two-layer greedy algorithm 
% can be solved by a simple linear program.
% To formalize the idea of more balanced 
% configuration allocation,
% \Cref{alg:opt} solves specific convex program 
% \ref{eq:convex primal}
% which determines both 
% the configuration assignment and 
% the chargeable impression
% at each stage. 
% This approach which uses the convex program
% for the current stage decision
% is similar to \citet{FN-21},
% which studies multi-stage 
% fractional vertex-weighted matching.
% In their problem,
% for each stage, 
% the convex program 
% depends on the vector of remaining capacities
% of each offline nodes, and
% finds a feasible matching that maximizes 
% a regularized version of the total weight objective function.
% In contrast, 
% for our multi-stage configuration allocation problem
% (which can be thought as a generalized model 
% of multi-stage vertex-weighted matching),
% our convex program will depends on the chargeable 
% impressions in the previous stage,
% solves for a configuration assignment for the current 
% stage and update the chargeable impressions
% to maximize a similar regularized version of total revenue function.

To prove that \Cref{alg:opt} obtains the optimal competitive ratio of $\cratio{K}$,
we follow the now-universal primal dual analysis framework
\citep[cf.][]{DJK-13}:
we formulate the optimum offline as a linear program \ref{eq:LP primal}
and then consider its dual program \ref{eq:LP}. 
Due to the strong duality of linear programs, to provide a lower bound on the competitive ratio,
it is sufficient to
construct a dual assignment 
such that (i) the dual objective value is equal to the total revenue 
collected by \Cref{alg:opt} and (ii)
the dual constraints are
$\cratio{K}$-approximately satisfied. The main technical challenge, and the second key technical contribution in our paper, is how to connect our convex programs
\ref{eq:convex primal}
in each stage to a LP primal-dual analysis, or in other words, how to construct an approximate LP dual certificate for 
our primal algorithm (i.e., \Cref{alg:opt})
based on its convex-programming based structure.
% It turns out that 
% the optimal solution for the dual program
% of our convex program \ref{eq:convex primal}
% provide 
The constructed dual assignment
in our proposed novel primal-dual analysis 
is closely related to the \emph{theory of Fenchel/Lagrangian convex duality}~\citep[e.g., see][]{BV-04} for our convex programs 
\ref{eq:convex primal}
in \Cref{alg:opt}.


To be more precise and to provide more details, we 
consider the Lagrangian dual program
\ref{eq:convex dual}
of the convex program
\ref{eq:convex primal}, 
and use \emph{exactly} its optimal dual solution
to construct the dual assignment in the 
primal-dual analysis framework.
As a comparison to prior work, 
for the special case of multi-stage vertex-weighted matching,
\citet{FN-21} construct the dual assignment 
using a specific graph decomposition \citep[cf.][]{GKK-12,FN-21}, whose existence
is shown by 
% using 
convex programming. 
However, 
as it turns out, in general models such as edge-weighted matching problem 
or configuration allocation problem, similar convex programs
do not admit any similar structures, and hence do not induce any relevant graph decomposition or base function factorization. Thus, as we mentioned above, 
we use the optimal dual solutions 
in \ref{eq:convex dual}
to directly construct 
the dual assignment for \ref{eq:LP}. Surprisingly, with our proposed dual assignment, we can connect the analysis of the competitive ratio to a recursive functional equation across $K$ stages, which has exactly appeared before in \cite{FN-21}. This is indeed the reason  why a particular choice of polynomial regularizes, which is the solution of this recursive functional equation, attains the optimal $\cratio{K}$ competitive ratio.\footnote{See \cite{FN-21} for more context and the connection between the recursive equation and the mentioned polynomials.} We should highlight that the connection between LP primal-dual analysis and the convex duality in our paper is quite magical, and might be of independent interest in other online algorithm design problems. 







\vspace{3mm}
\noindent\textbf{{Related Literature}}~~Here is a summary of the literature directly related to our work.

\vspace{2mm}
\noindent\emph{Multi-stage matching.}~~Our work is closely related to \cite{feng2020two}, which studies the optimal competitive two-stage vertex weighted matching and pricing under both adversarial and stochastic settings, and \cite{FN-21}, which studies multi-stage fractional vertex-weighted matching under adversarial arrival. The current paper extends the multi-stage algorithm design framework and the convex-programming based recursive primal-dual analysis introduced in these two papers to the more complicated and general setting of configuration allocation problem with preemption (which includes bipartite edge-weighted matching with free-disposal and vertex-weighted matching without free-disposal as special cases). At high-level, our result is also related to the beautiful work of \cite{LS-17}. They diverge from ours as they focus on a different setting, which is the multi-stage bipartite matching and the edge arrival model. Another work that is conceptually related to ours is the recent work of \cite{housni2020matching}, which is inspired by the idea of robust multi-stage optimization~\citep[e.g.,][]{bertsimas2010optimality,bertsimas2011theory}. They consider a two-stage robust optimization for cost-minimization of the matching, where future demand uncertainty is modeled using a set of demand scenarios (specified explicitly or implicitly). Our model and results diverge drastically from this work, which makes them incomparable. 


% \noindent{\emph{Two-stage stochastic programming.}}
% Two-stage stochastic combinatorial
% optimization problems have been studied extensively in the 
% literature
% \citep[e.g.,][]{BL-11, CCP-05,SS-04,SS-07,IKMM-04, hanasusanto2015k,hanasusanto2018conic}.
% Also, see the excellent book of \cite{kuhn2006generalized} for more context regarding convex multi-stage stochastic programs.  For two-stage stochastic matching, various models with different objectives
% have been studied in \citet{KS-06, EGMS-10, KKU-08} and more recently in \cite{feng2020two}. Another work that is conceptually related to our two-stage matching problem is the recent work of \cite{housni2020matching}, which is inspired by the idea of robust multi-stage optimization~\citep[e.g.,][]{bertsimas2010optimality,bertsimas2011theory}. They consider a two-stage robust optimization for cost-minimization of the matching, where future demand uncertainty is modeled using a set of demand scenarios (specified explicitly or implicitly). Our model and results diverge drastically from this work, which makes them incomparable. 


\vspace{2mm}
\noindent\emph{Online bipartite allocations.}~~Our results are comparable to the literature on online bipartite matching (with vertex arrival) and its extensions, which is rooted in the seminal work of Karp, Vazirani, and Vazriani~\citep{KVV-90}. A simple non primal-dual proof of RANKING algorithm of \cite{KVV-90} is presented in \cite{birnbaum2008line}. An elegant primal-dual analysis is discovered later in \cite{DJK-13}. A rich body of literature has extended this simple formulation to more practical or more theoretically challenging two-sided online allocation scenarios such as the online budgeted allocation/AdWords~\citep{MSVV-07,BJN-07,HZZ-20} and the vertex weighted budgeted-matching~\citep{AGKM-11}. Other variants tailored to applications such as display advertising, ride-sharing, assortment optimization, and display advertising are also studied~\citep{FKMMP-09, mehta2012online,MGS-12,GNR-14,DHKMQ-16,HKTWZZ-18,GKMSW-19,FHTZ-20}. We further refer interested readers to a nice survey by \cite{mehta2013online}.

\vspace{2mm}
\noindent\emph{Competitive primal-dual analysis.}~~On the algorithmic side, a sequence of past work have developed an elegant primal-dual competitive analysis framework, which resembles some aspects of our recursive convex-programming based primal-dual analysis~\citep{BJN-07,DJK-13,devanur2012online,devanur2009adwords,esfandiari2015online,HKTWZZ-18,GKMSW-19,FHTZ-20,FNS-19}. The work closely related to ours is \cite{DHKMQ-16}, which basically studies the fully online version of the fractional configuration allocation problem (with preemption), under the name of ``whole page optimization'' (with applications to display ads). They provide the optimal $(1-\frac{1}{e})$-competitive algorithm for this problem and introduce a novel primal-dual framework, which has inspired some of the ideas in the current paper (e.g., regularizing the convex objective at different price levels). See \cite{buchbinder2009design} for a survey on the primal-dual technique in online algorithms, and specifically for designing and analyzing online bipartite allocation algorithms. 





%  Also, at high-level, our primal-dual analysis resembles some aspects of ~\cite{BJN-07,FKMMP-09,devanur2009adwords,devanur2012online,esfandiari2015online,HKTWZZ-18,FNS-19}.
 
%  Other related models are online bipartite stochastic matching~ \citep[e.g.,][]{feldman2009online,bahmani2010improved,MGS-12,mehta2014online,JL-14} and online bipartite matching with stochastic rewards~\citep[e.g.,][]{mehta2012online,goyal2020online,huang2020online}. We refer interested readers to a nice survey by \cite{mehta2013online} for further related work. Finally, related to us is also the literature on stochastic online packing and convex programming with large budgets~\citep[e.g.,][]{FMMS-10,DJSW-11,AD-14}. In particular, the role of concave regularizers have been studied in these settings for different purposes, e.g., fairness~\citep{agrawal2018proportional,balseiro2021regularized}, robustness to adversarial corruptions~\citep{balseiro2020best}, and obtaining blackbox reductions from Bayesian mechanism design to algorithm design~\citep{dughmi2021bernoulli}. 

\vspace{2mm}
\noindent\emph{Video-ads allocation.}
The popularity of in-stream video platforms has ignited 
a new research area related to video-ads, see 
a recent survey by \citet{FOG-21} for a detailed discussion.
There is a limited literature on
the algorithmic study of video-ads allocation.
Comparing to more traditional applications such as display ads,
video-ads (especially in-stream ads) 
have a distinct feature, which is the
need to be shown to the user during the video session.
\citet{DGNR-09} 
introduce the ``online story scheduling'' problem in which
the task is to schedule in-stream ads with 
different time lengths and per-unit prices for a single user in an online 
fashion, and
provide a constant competitive algorithm. 
Further improvements and 
studying other variants of this problem 
have been the focus in the literature, e.g., \citet{AP-19,LMQTYZ-16}.
\citet{BKK-09} study an alternative media scheduling problem 
for multiple users in an offline fashion.
\citet{SKFFC-17}
consider a variant of AdWords problem \citep{MSVV-07},
where each offline node (which is an in-stream ad in their model) is associated with 
a time length and every online node (i.e., a user) can be matched with multiple offline nodes as long as the total time length is below some threshold. 


% \vspace{2mm}
% \noindent\emph{Applications in revenue management and service operations.} From both methodological and application points of view, our work is related to several streams of work that focus to design online allocations and matching algorithms for problems in revenue management and service operations. These work pertain to practical applications in online retail, ride-sharing and other online platforms. Some examples are online assortment optimization (e.g., 
% \citealp{GNR-14,MS-19}), online assortment of reusable resources  (e.g.,
% \citealp{gong2019online,feng2019linear,goyal2020onlineb}), Bayesian online assortment with heterogeneous customers (e.g.,
% \citealp{rusmevichientong2020dynamic,feng2020near}), 
% online assortment with replenishment~\citep{feng2021online}, dynamic pricing with static calendar \citep{MSZ-18}, volunteer crowd-sourcing and nudging~\citep{manshadi2020online}, two-sided assortment optimization~\citep{aouad2020online}, two-stage stochastic matchings and approximate submodular covering for flexible network design~\citep{devalve2021approximate}, primal-dual approaches in the context of analyzing assemble-to-order systems~\citep{devalve2020primal}, online allocation strategies in two-sided media platforms~\citep{alaei2020revenue}, and finally the line of work on dynamic windowed supply-demand matching/queuing---with applications in ride-sharing (e.g., \cite{HKTWZZ-18, ashlagi2019edge,aouad2020dynamic,ozkan2020dynamic,ata2020dynamic,aveklouris2021matching,arnosti2021managing}).











==> FN_ multi-stage matching + configuration allocation (MS Journal)/tex/intro-old.tex <==
\newcommand{\cratio}[1]{\Gamma(#1)}
\newcommand{\cratioexp}{1-\left(1-\frac{1}{K}\right)^K}
\section{Introduction}
\label{sec:intro}

The process of matching arriving demand requests to the available supply in real-time is a central operational task in two-sided online marketplaces. Example application domains include allocating service requests to providers in platforms such as Uber/Lyft (ride requests to drivers), Amazon (delivery requests to dispatching centers), Microsoft Azure (requested jobs to servers in the cloud) and Google AdWords (keywords queries to advertisers in sponsored search). In these domains, the platform's economical goal is to make matching decisions as new demand arrives, so as to maximize certain objective functions such as efficiency or revenue. While making these over-time decisions, not only the platform should be concerned with respecting the overall supply feasibility constraints such as capacities or budgets, it should also take into account the dynamic or real-time aspect of decision making, and that there exists uncertainty in future arriving demand; these considerations can substantially impact the current decision of the platform, specially if it is aiming to optimize its objective function for the entire decision making horizon.

A canonical formulation to capture gist of some existing tensions in the above dynamic decision making scenarios is the (adversarial) online bipartite matching problem, originated from the seminal work of Karp, Vazirani, and Vazriani~\citep{KVV-90}. In this model, the online and offline vertices simply play the role of the arriving demand requests and the available supply, respectively. A rich body of literature has extended this simple formulation to more practical two-sided online allocation scenarios such as the online budgeted allocation/AdWords~\citep{MSVV-07} and the vertex weighted budgeted-matching~\citep{AGKM-11}. Other extensions and variants tailored to applications such as display advertising, ride-sharing, and assortment optimization are also studied~\citep{FKMMP-09, mehta2012online,MGS-12,GNR-14,HKTWZZ-18}. See \cite{mehta2013online} for a survey. On the algorithmic side, a sequence of past work have developed an elegant primal-dual framework to design and analyze online competitive algorithms in these problems~\citep{BJN-07,DJK-13,devanur2012online}. See \cite{buchbinder2009design} for a survey on the primal-dual technique in online algorithms, and specifically for designing and analyzing online bipartite allocation algorithms. 

A common theme in the above literature, which is practically relevant in truly real-time applications of matching, is that the platform has to match the arriving demand request to the available supply immediately---with almost no delay. However, in applications that allow for some latency---e.g., matching delivery requests to dispatching centers in Amazon or matching user jobs to computing servers in Azure cloud computing platform---the platform can delay its matching decision by \emph{batching} the demand requests. A batch consists of the most recent group of demand requests that are supposed to be matched to the available supply in the same time frame. While dividing the entire real-time sequence of demand requests into less number of batches---and hence larger batches---induces more latency, it clearly helps the platform to make improved matching decisions in terms of efficiency: indeed, real-time decision making with no latency is a special case where each arriving demand request forms a batch of size one; moreover, the offline decision making is also a special case where the entire set of demand requests forms one large batch, allowing for making the most efficient decision by picking the hindsight optimal matching. Even though in the middle-ground regime with a fixed number of batches of arbitrary sizes the efficiency is still less than the hindsight optimal, still the platform can enjoy more efficiency compared to the truly real-time setting---simply because it makes more informed decisions. To see numbers in practice, for example, ridesharing platforms such as Uber~\citep{Uber}, Lyft~\citep{Lyft} and DiDi~\citep{ZHMWZFGY-17} have reported substantial efficiency improvements due to shifting from match-as-you-go to batching-and-matching. Same phenomena is observed and reported in other corners of gig-economy such as cloud computing markets~\citep{AWS} and online food delivery~\citep{joshi2021batching}.\footnote{Notably, batching not only helps with improving the efficiency, it can also help with decreasing various forms of non-operational cost such as waste and environmental costs ~\citep{AWSwaste}}

\vspace{2mm}
\noindent{\textbf{Our Theoretical Lens~}} Motivated by the batching-and-matching paradigm in practice, and also to theoretically study the the inherent trade-off between batching and inefficiency in dynamic allocations, we revisit the literature on (adversarial) online bipartite allocation problems. In particular, we study the \emph{multi-stage} model in the context of the vertex weighted matching, and its extensions to vertex weighted b-matching~\citep{AGKM-11}  and the budgeted allocation problem (also known as the AdWords problem)~\citep{MSVV-07}. In these models, the online vertices are partitioned into $K>0$ fixed number of batches and arrive over the span of $K$ stages, one batch per stage. We study multi-stage matching algorithms that make irrevocable stage-wise matching decisions by allocating the arriving batch of vertices to the offline nodes at each stage. Such an algorithm should also respect the feasibility constraints on the supply side (which can be capacity constraints or budget restrictions, depending on the underlying problem formulation) and the matching constraints on the demand side for each arriving request.



We measure the performance of our algorithms by their \emph{competitive ratio}, which is the worst-case ratio between the expected total weight of the algorithm and a particular benchmark, given a fixed number of batches. Our goal is to design multi-stage competitive algorithms with respect to the in-hindsight optimal matching---also known as the optimal offline benchmark. Considering different degrees of batching by changing the batch sizes and number of stages, one extreme is when there is only a single large batch containing all the demand nodes (maximum batching), in which the algorithm can perform as good as the optimal offline. The other extreme is when each online vertex arrives as a batch of size one (no batching); this is the fully online regime and therefore the competitive ratio of any multi-stage algorithm is at most the best competitive ratio achievable in the online regime (importantly, as a function of the number of online vertices). We now ask the following informal question in this paper:

\vspace{2mm}
\begin{displayquote}
\emph{In the middle-ground multi-stage regime of bipartite allocation problems with batch arrivals (in contrast to fully online and offline regimes), when we have $K>0$ number of batches, what are the optimal competitive ratios achievable by multi-stage algorithms in these problems?}
\end{displayquote}
\vspace{2mm}

For the multi-stage variants of the problems we study, we rely on the standard formulations in \cite{AGKM-11} for the vertex weighted (b-)matching problem and in \cite{MSVV-07, buchbinder2009design} for the budgeted allocation/AdWords problem. See \Cref{sec:prelim} (Model and Notations) for more details. We are mostly interested in fractional $K$-stage algorithms in this paper, as most of our techniques and ideas can be demonstrated easier in this setting. For completeness, we also consider integral $K$-stage algorithms (possibly randomized) under the ``large budgets assumption'' in the vertex weighted b-matching problem, or equivalently under the small bid over budget assumption in the budgeted allocation problem (for details, refer to \Cref{sec:prelim}).

% \noindent{\textbf{Problem Formulations~}}
% An instance of our problems is a bipartite graph $G=(\Rider,\Driver,E)$, where vertices in $\Driver$ are offline and vertices in $\Rider$ arrive in $K\in\mathbb{N}$ batches. At each stage $k\in[K]$, a new batch $\Rider_k\subseteq \Rider$ arrives and reveals all edges incident to vertices in $\Rider_k$. The platform then makes an irrevocable decision by matching each vertex $i\in\Rider_K$ to at most one offline vertex in $\Driver$. This matching can be fractional or integral. The goal is to maximize the weight of the final matching after all batches arrive, while ensuring the feasibility constraints on the offline side. The objective function and the feasibility constraints are specific to the choice of the problem as follows:
% \begin{enumerate}[label=\textit{(\roman*)}]
%     \item \textit{Multi-stage vertex weighted b-matching:} each offline vertex $j\in\Driver$ has a non-negative weight $w_j$ and a capacity (i.e., budget) constraint $B_j$, that is, its matching degree cannot exceed $B_j$. The objective is the sum of weights of (fractionally) matched offline vertices. We also consider the special case of \emph{multi-stage vertex weighted matching}, in which $B_j=1$ for all $j\in\Driver$.
%     \item \textit{Multi-stage AdWords:}  each edge $(i,j)\in E$ has a non-negative weight $b_{ij}$---also known as the bid of $i$ for $j$. Without loss of generality, we assume $b_{ij}\in[0,1]$.\footnote{This assumption is just for simplicity, as it helps with making the large budget assumption in vertex weighted b-matching similar to small bid over budget assumption in the AdWords problem.} Each offline vertex $j\in \Driver$ has a budget constraint $B_j$, that is, the sum of the weights of edges matched to $j$ cannot exceed $B_j$. The objective is simply the total weights of the edges in the (fractional) matching.
% \end{enumerate}



\smallskip
\noindent{\textbf{Our Contributions~}}
 The main contribution of this paper is the following result.
 
\vspace{2mm}
\mybox{
\begin{displayquote}
{\textbf{(Main Result)} For the multi-stage vertex weighted matching with $K$ batches, we propose a fractional $K$-stage algorithm (\Cref{alg:b-matching}) that achieves a competitive ratio of $\cratio{K}\triangleq\cratioexp$. Moreover, by proposing an upper-bound instance, we show that no $K$-stage algorithm, fractional or integral, can have a competitive ratio better than $\cratio{K}$.}
\end{displayquote}}
\vspace{1mm}
\noindent The competitive ratio function $\cratio{K}\in(1-1/e,1]$ is monotone decreasing in $K$. It is equal to $1$ at $K=1$
and converges to $1-1/e$ as $K$ goes to infinity. For the special case of two-stage vertex weighted matching ($K=2$), our algorithm is $3/4$-competitive, which matches the result of \cite{feng2020two}. Also, for three stages ($K=3$), it has a competitive ratio of $19/27\approx 0.704$. To the best of our knowledge, this is the first bound beating $1-1/e\approx 0.63$ in the $K$-stage bipartite matching problems (weighted or unweighted) for any $K>2$.

We further extend our result to the fractional multi-stage vertex weighted b-matching and multi-stage budgeted allocation problems. We obtain these results by proposing natural adaptations of the previous algorithm for vertex weighted matching (\Cref{alg:b-matching integral} and \Cref{alg:adwords fractional}).  Following the same approach as in the vertex weighted matching problem, we show these adaptations are also $\cratio{K}$-competitive for these generalizations/variations of our base problem. Switching to integral allocations, we also design a simple rounding scheme for multi-stage vertex weighted b-matching, and show the resulting multi-stage integral algorithm obtains a competitive ratio no smaller than $\cratio{K}-O\left(\sfrac{1}{B_{\textrm{min}}}\right)$, where $B_{\text{min}}$ is the minimum capacity of an offline node. Finally, we design a different yet another simple rounding scheme for multi-stage budgeted allocation, and show the resulting multi-stage integral algorithm has a competitive ratio no smaller than $\cratio{K}-O\left(\sqrt{\sfrac{\log(B_{\text{min}})}{B_{\text{min}}}}\right)$. Here, $B_{\text{min}}$ should be interpreted as the maximum budget over bid ratio. See \Cref{tab:summary} for a summary of our results and how they are compared with the previous work.
\input{tex/result-table}

\smallskip
\noindent{\textbf{Overview of the Techniques~}} 
A greedy allocation will allocate the arriving batch of demand requests to the available pool of offline supply at each stage $k\in[K]$, so as to maximize the total weight. Such an allocation can potentially suffer from the lack of enough \emph{balancedness} on the supply side---a property that can help the multi-stage algorithm to remain competitive against the adversary in future stages of this dynamic allocation model. Hence, we aim to replace greedy with a more balanced allocation that (i) considers the matching weight of the current stage, and (ii) simultaneously provides \emph{hedging} against the future stages in a controlled fashion.
For the special case of online arrivals, this simple idea is the essence of the celebrated BALANCE algorithm~\citep{MSVV-07,AGKM-11}, which is optimal competitive under online arrivals. 

To systematically extend the above balanced matching idea under the online setting to the multi-stage setting---where a multi-stage algorithm can match multiple vertices of the arriving batch to the offline side---we propose using fractional matchings that are solutions to specific \emph{convex programs} at each stage. Given the vector of remaining capacities (or budgets) upon the arrival of a new batch, each convex program essentially finds a feasible fractional allocation that maximizes a regularized version of the total weight objective function. In particular, in order to favor more balanced fractional allocations, we choose our regularizers to be (strictly) concave functions of the final matching degrees (or allocation levels) of the offline vertices.

Considering the above algorithmic skeleton, one major question is how to pick the strictly concave regularizers to achieve our desired $\cratio{K}$ competitive ratio in $K$ stages. Our intuition suggests that an appropriate multi-stage algorithm requires hedging more in earlier stages and less in later stages, e.g., in the extreme case of the last stage, picking a maximum weight matching is optimal and no balancedness is required. To obtain the desired variation in the balancedness of our allocation, i.e., having a more balanced allocation early on and gradually pushing it towards a greedy allocation in later stages, we use a different regularizer at each stage. Informally speaking, we aim to incorporate ``more intense'' regularization at first and then gradually shift towards no regularization in the course of $K$ stages. To this end, we need to formalize the notion of intensity of regularization. 

Our key technical ingredient that formalizes the above intuitive notion is a particular sequence $f_1,f_2,\ldots,f_K:[0,1]\rightarrow [0,1]$ of \emph{polynomials of decreasing degrees}, where $f_k$ is a polynomial of degree $(K-k)$ associated to stage $k\in[K]$.  See \Cref{prop:poly} and \Cref{fig:poly}. Here, the regularization intensity of each polynomial is essentially governed by its degree---hence our sequences starts with the highest degree and goes in the descending order of polynomial degrees. We identify this sequence using a backward recursive equation (will be detailed later). We then show this sequence \emph{exactly} characterizes the regularizers of the optimal competitive multi-stage fractional algorithm.

More precisely, we use the primitive function $F_k(x)\triangleq\int_{0}^{x}f_k(y)dy$ to map the normalized fractional degree (or normalized allocation level) of each offline vertex to a penalty term in $[0,1]$ at stage $k$. We then subtract the weighted sum of these penalties from the total weight objective function to construct our regularized objective function; see convex programs \ref{eq:concave-k-bmatching} and \ref{eq:concave-adwords-k} for more details. Interestingly, the first-stage polynomial $f_1$ converges to $f(x)= e^{x-1}$ as $K$ goes to infinity. Also, in the special case of batches of size one, replacing the polynomial $f_k$ at all stages with \emph{the same function} $f(x)=e^{x-1}$ recovers the $(1-1/e)$-competitive BALANCE algorithms in \cite{AGKM-11} and \cite{MSVV-07} for the online vertex weighted b-matching and online budgeted allocation, respectively. 

\input{tex/fig-poly}

To analyze our polynomial regularized matching algorithms---inspired by the technique introduced in \cite{feng2020two} for two-stage matching---we use the strong duality of the convex programs, tied to a specific primal-dual analysis that is quite different from the known primal-dual analysis in the literature for various forms of online bipartite allocation problems (e.g., \cite{MSVV-07,AGKM-11,BJN-07}). The sketch of our analysis is roughly the following: The Karush–Kuhn–Tucker (KKT) conditions at each stage $k$ offer a structural decomposition of the subgraph induced by the $k^{\text{th}}$ batch. The special unweighted case of this decomposition coincides with the well-studied \emph{matching skeleton} introduced by~\cite{GKK-12}, which itself is closely related to the Edmonds-Gallai decomposition~\citep{edm-65,gal-64} of bipartite graphs. Using this decomposition, and by carefully using our polynomials $f_1,\ldots,f_k$, we propose a novel \emph{recursive primal-dual framework} to bound the competitive ratio of our fractional matchings. The resulting dual constructions, together with our recursive formulation, shows how to improve the competitive ratios from $(1-1/e)$ to $\cratio{K}$ in the multi-stage setting with $K$ batches. In other words, this new algorithmic construct extends the dual constructions in previous work~\citep{MSVV-07,AGKM-11,BJN-07} in a novel fashion to the multi-stage setting with batch arrivals. As a side dish, our technique provides a convex-programming based interpretation for the existing primal-dual proofs in the special case of the online setting. 

We further show the competitive ratio $\cratio{K}$ is the best achievable by any fractional multi-stage algorithm, whether deterministic or randomized, by showing an upper-bound instance for the special case of the unweighted multi-stage matching. Notably, this instance relies on batches of size more than one, and hence cannot be used as an upper-bound instance for the special case of online arrival where batch sizes are all one. See \Cref{fig:bad-example} for more details.



We finally turn our attention to the integral versions of the vertex weighted b-matching and AdWords problems, when the capacities are large (or equivalently, bid over budget ratios are small). By using the totally unimodularity of flow-type polytopes~\citep{sch-03}, we propose our deterministic rounding algorithm for the vertex weighted b-matching problem. The idea is finding integer lower and upper bounds on the fractional degrees of each offline vertex using the fractional solution of the convex program at each stage, and then searching for an integral matching satisfying these bounds.  For the AdWords problem, we use a straightforward variant of independent randomized rounding at each stage, after slightly reducing all the budgets. By applying standard concentration bounds for each offline vertex, we prove that maintaining feasibility of the resulting integral allocation only adds a small loss in expectation when the bid over budget ratios are small. 

\smallskip
\noindent\textbf{Managerial Insights~} Our study sheds insights on the role of batching in service operation of matching platforms, and provides algorithmic evidences on how they should adaptively tune their batched matching algorithms to achieve the right trade-off between \emph{``greedy-ness''} in the current decision and {``hedging''} for the sake of future decisions:
\begin{itemize}
    \item In settings that allow for latency---and hence allow for batching the demand arrivals---batched matching algorithms (versus fully online algorithms) can be used by the algorithm designer to obtain performance improvements.
    \item There is an inherent trade-off between the gain from batching (which is captured by the competitive ratio in our competitive analysis framework) and the degree of batching (which is captured by the inverse number of batches in our framework): with less number of batches/stages---which accounts for a higher degree of batching---a well-designed multi-stage matching algorithm can obtain a higher performance; moreover, it gets closer to the offline optimal matching as the degree of batching increases.\footnote{Of course, there is no free lunch here and the actual cost of batching is the induced latency in decision making.}
    \item When designing batched matching algorithms, our result suggests that pushing the matching to be more robust to future uncertainty early on (i.e., to be more balanced) and then pushing it to be more greedy later on will help with the performance in a finite horizon problem. In particular, we could formally capture this design aspect using our decreasing degree polynomial regularizers; However, in general, decreasing the degree of hedging induced by the matching algorithm over time to obtain improved performance is the main operational takeaway message of our work, and there might be other ways of performing this task in practice.
\end{itemize}




\smallskip
\noindent\textbf{Organization~} 
In \Cref{sec:vertex-weight}, we introduce our optimal competitive multi-stage algorithm for the vertex weighted bipartite matching problem (\Cref{sec:upper-bound}), then prove a competitive ratio lower bound for this algorithm (\Cref{sec:primal-dual}), and finally show that it \emph{exactly} matches the upper-bound on the competitive ratio of \emph{any} multi-stage algorithm (\Cref{sec:lowerbound}). We then switch to other variants of our base model in \Cref{sec:extensions}, and show the same results for its generalization to b-matching (\Cref{sec:weighted b-matching}) and its variation to multi-stage budgeted allocation/Adwords problem (\Cref{sec:adwords}). 
\subsection{Related Literature} Here is a summary of the literature directly related to our work.

\vspace{2mm}
\noindent\emph{Multi-stage matching.} A work closely related to ours is that of \cite{feng2020two}, which studies the optimal competitive two-stage vertex weighted matching and pricing under both adversarial and stochastic settings. We extend their result in the adversarial case to multi stages and settings beyond vertex weighted matching. Our result for the unweighted multi-stage matching is closely related to the beautiful work of \cite{LS-17}, which also uses the matching skeleton of \cite{GKK-12}, but for a different model. In their model, a batch of \emph{new edges} arrive in each stage. Their proposed algorithm first finds a maximum fractional matching using the matching skeleton in each stage, and then removes some of the edges sampled from this matching through a randomized procedure. This approach obtains an optimal $2/3$ competitive ratio for two stages and a non-optimal $1/2+O(2^{-K})$ competitive ratio for $K$ stages. 
\vspace{2mm}

\noindent{\emph{Two-stage stochastic programming.}}
Two-stage stochastic combinatorial
optimization problems have been studied extensively in the 
literature
\citep[e.g.,][]{BL-11, CCP-05,SS-04,SS-07,IKMM-04, hanasusanto2015k,hanasusanto2018conic}.
Also, see the excellent book of \cite{kuhn2006generalized} for more context regarding convex multi-stage stochastic programs.  For two-stage stochastic matching, various models with different objectives
have been studied in \citet{KS-06, EGMS-10, KKU-08} and more recently in \cite{feng2020two}. Another work that is conceptually related to our two-stage matching problem is the recent work of \cite{housni2020matching}, which is inspired by the idea of robust multi-stage optimization~\citep[e.g.,][]{bertsimas2010optimality,bertsimas2011theory}. They consider a two-stage robust optimization for cost-minimization of the matching, where future demand uncertainty is modeled using a set of demand scenarios (specified explicitly or implicitly). Our model and results diverge drastically from this work, which makes them incomparable. 


\vspace{2mm}
\noindent\emph{Online bipartite allocations.}
Our results are comparable to the literature on online bipartite matching (with vertex arrival) and its extensions. Related to us, \citet{AGKM-11} generalize the classic RANKING algorithm of \cite{KVV-90} to the setting where offline vertices are weighted. A simple non primal-dual proof of RANKING is presented in \cite{birnbaum2008line}. An elegant primal-dual analysis is discovered later in \cite{DJK-13}. Also, at high-level, our primal-dual analysis resembles some aspects of ~\cite{BJN-07,FKMMP-09,devanur2009adwords,devanur2012online,esfandiari2015online,HKTWZZ-18,FNS-19}. Other related models are online bipartite stochastic matching~ \citep[e.g.,][]{feldman2009online,bahmani2010improved,MGS-12,mehta2014online,JL-14} and online bipartite matching with stochastic rewards~\citep[e.g.,][]{mehta2012online,goyal2020online,huang2020online}. We refer interested readers to a nice survey by \cite{mehta2013online} for further related work. Finally, related to us is also the literature on stochastic online packing and convex programming with large budgets~\citep[e.g.,][]{FMMS-10,DJSW-11,AD-14}. In particular, the role of concave regularizers have been studied in these settings for different purposes, e.g., fairness~\citep{agrawal2018proportional,balseiro2021regularized}, robustness to adversarial corruptions~\citep{balseiro2020best}, and obtaining blackbox reductions from Bayesian mechanism design to algorithm design~\citep{dughmi2021bernoulli}. 

\vspace{2mm}
\noindent\emph{Applications in revenue management and service operations.} From both methodological and application points of view, our work is related to several streams of work that focus to design online allocations and matching algorithms for problems in revenue management and service operations. These work pertain to practical applications in online retail, ride-sharing and other online platforms. Some examples are online assortment optimization (e.g., 
\citealp{GNR-14,MS-19}), online assortment of reusable resources  (e.g.,
\citealp{gong2019online,feng2019linear,goyal2020onlineb}), Bayesian online assortment with heterogeneous customers (e.g.,
\citealp{rusmevichientong2020dynamic,feng2020near}), 
online assortment with replenishment~\citep{feng2021online}, dynamic pricing with static calendar \citep{MSZ-18}, volunteer crowd-sourcing and nudging~\citep{manshadi2020online}, two-sided assortment optimization~\citep{aouad2020online}, two-stage stochastic matchings and approximate submodular covering for flexible network design~\citep{devalve2021approximate}, primal-dual approaches in the context of analyzing assemble-to-order systems~\citep{devalve2020primal}, online allocation strategies in two-sided media platforms~\citep{alaei2020revenue}, and finally the line of work on dynamic windowed supply-demand matching/queuing---with applications in ride-sharing (e.g., \cite{HKTWZZ-18, ashlagi2019edge,aouad2020dynamic,ozkan2020dynamic,ata2020dynamic,aveklouris2021matching,arnosti2021managing}).



==> FN_ multi-stage matching + configuration allocation (MS Journal)/tex/intro.tex <==
\newcommand{\cratio}[1]{\Gamma(#1)}
\newcommand{\cratioexp}{1-\left(1-\frac{1}{K}\right)^K}
\section{Introduction}
\label{sec:intro}
\revcolor{
With the pervasiveness of online platforms and web-based services, internet advertising has grown to become a major component of today's economy. Worldwide spending of internet advertising stood at an estimated 521 billion U.S. dollars in 2021 --- a figure that is forecast to constantly increase in the coming years, reaching a total of 876.1 billion U.S. dollars by 2026.\footnote{See \url{https://www.statista.com/statistics/237974/online-advertising-spending-worldwide/}.} The combination of the economic impact and the inherent flexibility of internet advertising has helped with its prevalence as a modern market. At the same time, it has also given rise to numerous revenue management challenges and paradigms, some of which pertain to real-time algorithmic allocation of inventories of ad opportunities to advertisers in various search and display internet advertising scenarios, e.g., see \citet{MSVV-07,FKMMP-09,BFMM-14,DHKMQ-16}. 

As digital consumption behaviors change, and new technologies provide new ways for users to interact with social media platforms and publishers, traditional forms of real-time internet ad allocations  also evolve. A prominent example of this sort, which is one of the main motivating application behind our paper, is \emph{in-stream video advertising}. Nowadays, in-stream video advertising is rapidly growing~\footnote{According to \citet{Deloitte}, 80\% of U.S. consumers are now paying for streaming video services, up from 73\% before the COVID-19 pandemic began. Using ad spending as an indicator, video advertising will likely continue to grow for the foreseeable future. Video ad spending in the U.S. is increased from 8.92 billion U.S. dollars in 2017 to 55.34 billion U.S. dollars in 2021; it is also projected to reach as high as 78.45 billion U.S. dollars by 2023. See \url{https://www.statista.com/statistics/256272/digital-video-advertising-spending-in-the-us/}.} and is playing an essential role in the business model of online video sharing platforms such as YouTube and Vimeo, on-demand/live streaming platforms such as Netflix, Roku, and Twitch, and even social video streaming platforms such as TikTok. In this context, when a user starts watching a new video session (e.g., on YouTube), an advertising opportunity to display video-ads, and hence allocating user impressions to advertisers and charging them based on per-impression rates, is created. Video-ads refer to all possible ad formats in this context such as in-stream advertising videos of different lengths, as well as the banner-like overlay and text- or image-based ads that appear over a video. See \Cref{fig:ad-formats} for specific video-ad formats that are currently used in YouTube.\footnote{See \url{https://support.google.com/youtube/answer/2375464?hl=en}.}
Given these ad format varieties, the real-time ad allocation for a sequence of arriving users is done by displaying ads of one or multiple advertisers to each arriving user (or equivalently, each video session). It is important to add that such a dynamic environment is highly non-stationary (in terms of users that start watching videos) and hence enabling the platform to run a robust and prior free ad allocation policy is a common practice.

\captionsetup[subfloat]{captionskip=0pt}
\begin{figure}[hbt!]
	\centering
	\subfloat[
   Skippable in-stream ads
	]{
\includegraphics[scale=0.32]{figs/skippable-video-ads.png}
	}
	\subfloat[Non-skippable in-stream ads]{
\includegraphics[scale=0.32]{figs/non-skippable-video-ads.png}
	}
	\subfloat[
   Bumper short ads
	]
	{
\includegraphics[scale=0.32]{figs/bumper-ads.png}
	}
	\\
	\centering
	\subfloat[
   Overlay ads
	]{
\includegraphics[scale=0.34]{figs/overlay-ads.png}
	}
	\subfloat[
   Clickable sponsored cards
	]{
\includegraphics[scale=0.34]{figs/sponsored-cards.png}
	}
	\vspace{1mm}
	\caption{
Different formats of video advertising in YouTube streaming; These formats can be used at different time-stamps of a YouTube video, and differ in their lengths, designs, and how users interact with them.}
	\label{fig:ad-formats}
\end{figure}


While in-stream video advertising is a real-time application, it still admits a natural form of allowance for latency in displaying ads to the users. In particular, as several of the video-ads show up in the middle (or at the end) of users' video sessions, an ad allocator can delay the time of its decision for a session (or the current chunk of a long video session) from the beginning of the video to the first time-stamp that a video-ad is required to be displayed. This flexibility provides an immense opportunity to \emph{batch} the arriving video sessions, where a batch consists of the most recent group of users that their ad allocation decisions can be made in the same time frame. Given these batches, the goal of the ad allocator is to make allocation decisions as each batch of users arrives --- in contrast to fully online decisions as each single user arrives --- in order to maximize the revenue from the advertisers. This batching technique is indeed practiced in the web-based video advertising industry~\citep{personal}.

Besides video advertising, there are also other resource allocation applications with allowance for latency, e.g., matching delivery requests to dispatching centers in Amazon or matching user jobs to computing servers in Azure cloud computing platform. Even in fast-paced applications such as sponsored search, the ad decisions for the arriving search queries can still be delayed in the order of milliseconds, and hence batching is possible. In all of these applications, while dividing the entire real-time sequence of demand requests into less number of batches (of larger sizes) requires more latency, it clearly helps the platform to make improved allocation decisions in terms of its objective as it has more information about the sequence of arriving demand requests.\footnote{To see numbers in practice, for example, ridesharing platforms such as Uber~\citep{Uber}, Lyft~\citep{Lyft} and DiDi~\citep{ZHMWZFGY-17} have reported substantial efficiency improvements due to shifting from match-as-you-go to batching-and-matching. Same results are reported in other corners of gig-economy such as cloud computing markets~\citep{AWS} and online food delivery~\citep{joshi2021batching}. Notably, batching not only helps with improving the efficiency, it can also help with reducing non-operational forms of cost such as waste and environmental cost~\citep{AWSwaste}.}}

\vspace{2mm}
\revcolor{\noindent{\textbf{Our Theoretical Lens~}} Motivated by the batching-and-allocation paradigm in practical applications such as video advertising, and also to theoretically characterize the the inherent trade-off between batching and inefficiency in robust and prior-free dynamic allocations, we revisit the literature on (adversarial) online bipartite allocations, originated from the seminal work of \cite{KVV-90}, where the goal is to allocate the arriving demand vertices (online side) to the available supply vertices (offline side). We study several canonical settings in this literature under the \emph{multi-stage} arrival model, where the online vertices are partitioned into $K>0$ fixed number of batches and arrive over $K$ stages (one batch per each stage). In this model, once a batch arrives, every information in the problem instance related to this batch (which depends on the problem's specifications) is revealed to the multi-stage allocation algorithm. The algorithm then makes irrevocable stage-wise decisions by allocating the arriving batch of vertices to the offline side at each stage.

As our base model, we consider the \emph{multi-stage vertex weighted b-matching}~\citep{AGKM-11,DJK-13}. In this simple problem, online vertices arrive in $K>0$ batches. Then the multi-stage algorithm matches the arriving batches to the offline side while respecting the capacity constraints on the offline side. The goal is to maximize the total weight of the matching. 

Motivated by the video advertising application, we also consider an extension model called \emph{multi-stage configuration allocation}~\citep{DHKMQ-16}, which generalizes a rich set of multi-stage resource allocation problems including vertex-weighted b-matching, budgeted allocation (also known as ``AdWords''~\citep{MSVV-07}), and edge-weighted online matching with free-disposal~\citep{feldman2009online}. In this problem, we have online users (each corresponding to a new video session) that arrive in $K>0$ batches and offline advertisers that have ads to be displayed to these users so that they receive impressions from the users. Once a batch arrives, the multi-stage allocation algorithm assigns a feasible ``configuration'' to each user in that batch. Here, a configuration can refer to an arrangement of video-ads of various lengths and formats for a subset of advertisers, showing up at different time-stamps of the user's video session.\footnote{It can also be the case that a long video session is divided into chunks, and then each chunk is assigned a separate configuration, i.e., is treated as a new video session.}  Each assigned configuration yields a certain number of impressions to each advertiser and charges the advertiser at a certain price per impression. Depending on advertisers' long-term contracts, each advertiser is willing to pay for a certain number of impressions during the decision making horizon. Given this model, the goal is to maximize the revenue (i.e., total collected prices) in the finite decision making horizon. Particularly important in this model, the set of feasible configurations can model various complex user-level constraints.\footnote{\revcolor{To name a few, our model can capture exclusion (e.g., competing advertisers can not be shown in the same video), frequency capping (e.g., similar ads should not be shown back to back in the same video), and bundling (e.g., when advertisers require that all or none of a set of related ads be shown in the same video).}} }





% and to study a universal model that generalizes a rich set of multi-stage resource allocation problems including vertex-weighted b-matching, budgeted allocation (also known as ``AdWords'')~\citep{MSVV-07}), and edge-weighted online matching with free-disposal~\citep{feldman2009online}, we also study the 

% in the context of   and the budgeted allocation problem (also known as the AdWords problem)~\citep{MSVV-07}. 


% Such an algorithm should also respect the feasibility constraints on the supply side (which can be capacity constraints or budget restrictions, depending on the underlying problem formulation) and the matching constraints on the demand side for each arriving request.



% Even though in the middle-ground regime with a fixed number of batches of arbitrary sizes the efficiency is still less than the hindsight optimal, still the platform can enjoy more efficiency compared to the truly real-time setting---simply because it makes more informed decisions. 

% To see numbers in practice, for example, ridesharing platforms such as Uber~\citep{Uber}, Lyft~\citep{Lyft} and DiDi~\citep{ZHMWZFGY-17} have reported substantial efficiency improvements due to shifting from match-as-you-go to batching-and-matching. Same phenomena is observed and reported in other corners of gig-economy such as cloud computing markets~\citep{AWS} and online food delivery~\citep{joshi2021batching}.\footnote{Notably, batching not only helps with improving the efficiency, it can also help with decreasing various forms of non-operational cost such as waste and environmental costs ~\citep{AWSwaste}}














% Given these ad format varieties, the real-time ad allocation for a sequence of arriving users is done by assigning 

 







% The process of matching arriving demand requests to the available supply in real-time is a central operational task in two-sided online marketplaces. Example application domains include allocating service requests to providers in platforms such as Uber/Lyft (ride requests to drivers), Amazon (delivery requests to dispatching centers), Microsoft Azure (requested jobs to servers in the cloud) and Google AdWords (keywords queries to advertisers in sponsored search). In these domains, the platform's economical goal is to make matching decisions as new demand arrives, so as to maximize certain objective functions such as efficiency or revenue. While making these over-time decisions, not only the platform should be concerned with respecting the overall supply feasibility constraints such as capacities or budgets, it should also take into account the dynamic or real-time aspect of decision making, and that there exists uncertainty in future arriving demand; these considerations can substantially impact the current decision of the platform, specially if it is aiming to optimize its objective function for the entire decision making horizon.








\revcolor{We measure the performance of our algorithms by their \emph{competitive ratio}, which is the worst-case ratio between the expected objective value of the algorithm and the in-hindsight optimal solution --- also known as the optimal offline benchmark. Considering different degrees of batching by changing the number of batches $K$ and their sizes, one extreme regime of our problem is the fully offline setting when there is only a single large batch containing all the demand vertices. In this extreme regime one can achieve the performance of the optimum offline benchmark. The other extreme regime is the fully online setting when each online demand vertex arrives essentially as a batch of size one (no batching). Note that any competitive ratio lower-bound for the fully online setting establishes a lower-bound for the multi-stage setting, as any algorithm in the fully online setting can be used in the multi-stage setting by simply considering any arbitrary (synthetic) arrival order over vertices in each batch. We now ask the following research question in this paper:

\vspace{2mm}
\begin{displayquote}
\emph{In the middle-ground multi-stage regime of bipartite allocation problems with batch arrivals (in contrast to fully online and offline regimes), when we have $K>0$ number of batches, what are the optimal competitive ratios achievable by multi-stage algorithms in these problems?}
\end{displayquote}
\vspace{2mm}}

% Considering different degrees of batching by changing the number of stages $K$, on one extreme we have fully online decision making with no latency where each arriving demand vertex forms a batch of size one and $K$ is the number of demand vertices. 

% one extreme is when there is only a single large batch containing all the demand nodes (maximum batching), in which the algorithm can perform as good as the optimal offline. The other extreme is when each online vertex arrives as a batch of size one (no batching); this is the fully online regime and therefore the competitive ratio of any multi-stage algorithm is at most the best competitive ratio achievable in the online regime (importantly, as a function of the number of online vertices). We now ask the following informal question in this paper:


% Important to notice, online decision making with no latency is a special case where each arriving demand request forms a batch of size one; moreover, the offline decision making is also a special case where the entire set of demand requests forms one large batch, allowing for making the first-best decision by picking the hindsight optimal matching.



% For the multi-stage variants of the problems we study, we rely on the standard formulations in \cite{AGKM-11} for the vertex weighted (b-)matching problem and in \cite{MSVV-07, buchbinder2009design} for the budgeted allocation/AdWords problem. See \Cref{sec:prelim} (Model and Notations) for more details. We are mostly interested in fractional $K$-stage algorithms in this paper, as most of our techniques and ideas can be demonstrated easier in this setting. For completeness, we also consider integral $K$-stage algorithms (possibly randomized) under the ``large budgets assumption'' in the vertex weighted b-matching problem, or equivalently under the small bid over budget assumption in the budgeted allocation problem (for details, refer to \Cref{sec:prelim}).

% \noindent{\textbf{Problem Formulations~}}
% An instance of our problems is a bipartite graph $G=(\Rider,\Driver,E)$, where vertices in $\Driver$ are offline and vertices in $\Rider$ arrive in $K\in\mathbb{N}$ batches. At each stage $k\in[K]$, a new batch $\Rider_k\subseteq \Rider$ arrives and reveals all edges incident to vertices in $\Rider_k$. The platform then makes an irrevocable decision by matching each vertex $i\in\Rider_K$ to at most one offline vertex in $\Driver$. This matching can be fractional or integral. The goal is to maximize the weight of the final matching after all batches arrive, while ensuring the feasibility constraints on the offline side. The objective function and the feasibility constraints are specific to the choice of the problem as follows:
% \begin{enumerate}[label=\textit{(\roman*)}]
%     \item \textit{Multi-stage vertex weighted b-matching:} each offline vertex $j\in\Driver$ has a non-negative weight $w_j$ and a capacity (i.e., budget) constraint $B_j$, that is, its matching degree cannot exceed $B_j$. The objective is the sum of weights of (fractionally) matched offline vertices. We also consider the special case of \emph{multi-stage vertex weighted matching}, in which $B_j=1$ for all $j\in\Driver$.
%     \item \textit{Multi-stage AdWords:}  each edge $(i,j)\in E$ has a non-negative weight $b_{ij}$---also known as the bid of $i$ for $j$. Without loss of generality, we assume $b_{ij}\in[0,1]$.\footnote{This assumption is just for simplicity, as it helps with making the large budget assumption in vertex weighted b-matching similar to small bid over budget assumption in the AdWords problem.} Each offline vertex $j\in \Driver$ has a budget constraint $B_j$, that is, the sum of the weights of edges matched to $j$ cannot exceed $B_j$. The objective is simply the total weights of the edges in the (fractional) matching.
% \end{enumerate}



\revcolor{\smallskip
\noindent{\textbf{Our Contributions~}}
 The main contribution of this paper is the following result.
 
\vspace{2mm}
\mybox{
\begin{displayquote}
{\textbf{[Main Result]}~\emph{For the multi-stage vertex weighted matching (resp. multi-stage configuration allocation) problem with $K$ batches, we propose \Cref{alg:b-matching} (resp. \Cref{alg:opt}) that achieves a competitive ratio of $\cratio{K}\triangleq\cratioexp$. Moreover, by proposing an upper-bound instance, we show that no $K$-stage algorithm, fractional or integral, can have a competitive ratio better than $\cratio{K}$ in these problems.}}
\end{displayquote}}
\vspace{1mm}
\noindent The competitive ratio function $\cratio{K}\in(1-1/e,1]$ is monotone decreasing in $K$. It is equal to $1$ at $K=1$
and converges to $1-1/e$ as $K$ goes to infinity.\footnote{\revcolor{In fact, a simple asymptotic expansion shows that $\cratio{K}=\left(1-\frac{1}{e}\right)+\frac{1}{2eK}+O\left(\frac{1}{K^2}\right)$.}}. For the special case of two-stage vertex weighted matching ($K=2$), our algorithm is $3/4$-competitive, which matches the result of \cite{feng2020two}. Also, for three stages ($K=3$), it has a competitive ratio of $19/27\approx 0.704$. To the best of our knowledge, this is the first bound beating $1-1/e\approx 0.63$ in the $K$-stage bipartite matching problems (weighted or unweighted) for any $K>2$. While our results pertains to fractional allocations, they can easily be extended to the integral version under the large budget assumption. In fact, in the multi-stage configuration allocation problem (and all of its special cases) one can use a simple independent rounding schemes after slightly decreasing the capacities, and show the resulting multi-stage integral algorithm has a competitive ratio no smaller than $\cratio{K}-O\left(\sqrt{\sfrac{\log(B_{\text{min}})}{B_{\text{min}}}}\right)$ using standard concentration bounds (e.g., see \cite{DJSW-11} for technical details). Here, $B_{\text{min}}$ should be interpreted as the minimum capacity/required number of impressions of each offline node/advertiser.}

% We further extend our result to the fractional multi-stage vertex weighted b-matching and multi-stage budgeted allocation problems. We obtain these results by proposing natural adaptations of the previous algorithm for vertex weighted matching (\Cref{alg:b-matching integral} and \Cref{alg:adwords fractional}).  Following the same approach as in the vertex weighted matching problem, we show these adaptations are also $\cratio{K}$-competitive for these generalizations/variations of our base problem. Switching to integral allocations, we also design a simple rounding scheme for multi-stage vertex weighted b-matching, and show the resulting multi-stage integral algorithm obtains a competitive ratio no smaller than $\cratio{K}-O\left(\sfrac{1}{B_{\textrm{min}}}\right)$, where $B_{\text{min}}$ is the minimum capacity of an offline node. Finally, we design a different yet another simple rounding scheme for multi-stage budgeted allocation, and show the resulting multi-stage integral algorithm has a competitive ratio no smaller than $\cratio{K}-O\left(\sqrt{\sfrac{\log(B_{\text{min}})}{B_{\text{min}}}}\right)$. Here, $B_{\text{min}}$ should be interpreted as the maximum budget over bid ratio. See \Cref{tab:summary} for a summary of our results and how they are compared with the previous work.
% \input{tex/result-table}

\smallskip
\noindent{\textbf{Overview of the Main Technique~}} 
\revcolor{Considering the multi-stage vertex weighted matching problem first,} any greedy algorithm allocates the arriving batch of demand requests to the available pool of offline supply at each stage $k\in[K]$, so as to maximize the matching weight of the current stage. Such an allocation possibly suffers from the lack of enough \emph{balancedness} on the supply side --- a property that can help the algorithm to remain competitive against the adversary in future stages. To fix this issue, we replace greedy with a more balanced allocation that (i) takes into account the matching weight of each stage, and (ii) simultaneously provides \emph{hedging} against future stages in a controlled fashion.
For the special case of online arrivals, this simple idea is the essence of the celebrated BALANCE algorithm~\citep{AGKM-11}, which is optimal competitive under online arrivals. 

To systematically extend the above balanced matching idea under the online setting to the multi-stage setting --- where the algorithm can basically match multiple vertices of the arriving batch to the offline side --- we propose using specific \emph{stage-dependent convex programs} and output their optimal solution in each stage as the fractional matching of that stage. Given the vector of remaining capacities at the beginning of each stage, the convex program for this stage essentially finds a feasible fractional allocation that maximizes a regularized version of the total weight objective function. In particular, in order to favor more balanced fractional allocations, we choose our regularizers to be \emph{specific} (strictly) concave functions of the final matching degrees (or allocation levels) of the offline vertices. More precisely, we use the primitive function $F_k(x)\triangleq\int_{0}^{x}f_k(y)dy$ to map the normalized fractional degree (or normalized allocation level) of each offline vertex to a penalty term in $[0,1]$ at stage $k$. We then subtract the weighted sum of these penalties from the total weight objective function to construct our regularized objective function in that stage; see the convex program \ref{eq:concave-k-bmatching} used in \Cref{alg:b-matching}.

Considering the above algorithmic construct, one major question is how to pick these strictly concave regularizers to achieve our desired $\cratio{K}$ competitive ratio in $K$ stages. Our intuition suggests that an appropriate multi-stage algorithm requires hedging more in earlier stages and less in later stages, e.g., in the extreme case of the last stage, picking a maximum weight matching is optimal and no balancedness is required. To obtain the desired variation in the balancedness of our allocation, i.e., having a more balanced allocation early on and gradually pushing it towards a greedy allocation in later stages, we aim to incorporate ``more intense'' regularization at first and then gradually shift towards no regularization in the course of $K$ stages. 

Our key technical ingredient that formalizes the above intuitive notion of regularization intensity is introducing a particular sequence $f_1,f_2,\ldots,f_K:[0,1]\rightarrow [0,1]$ of \emph{polynomials of decreasing degrees}, where $f_k$ is a polynomial of degree $(K-k)$ associated to stage $k\in[K]$.  See \Cref{fig:poly} and \Cref{prop:poly}. Here, the regularization intensity of each polynomial is essentially governed by its degree --- hence our sequences starts with the highest degree and goes in the descending order of polynomial degrees. We identify this sequence using a backward recursive equation (will be detailed later). We then show this sequence \emph{exactly} characterizes the regularizers of the optimal competitive multi-stage algorithm.
% More precisely, we use the primitive function $F_k(x)\triangleq\int_{0}^{x}f_k(y)dy$ to map the normalized fractional degree (or normalized allocation level) of each offline vertex to a penalty term in $[0,1]$ at stage $k$. We then subtract the weighted sum of these penalties from the total weight objective function to construct our regularized objective function; see convex programs \ref{eq:concave-k-bmatching} and \ref{eq:concave-adwords-k} for more details.
Interestingly, the first-stage polynomial $f_1$ converges to $f(x)= e^{x-1}$ as $K$ goes to infinity. Also, in the special case of batches of size one, replacing the polynomial $f_k$ at all stages with \emph{the same function} $f(x)=e^{x-1}$ recovers the $(1-1/e)$-competitive BALANCE algorithms in \cite{AGKM-11} for the online vertex weighted b-matching.

\input{tex/fig-poly}

To analyze our polynomial regularized matching algorithms --- inspired by the technique introduced in \cite{feng2020two} for two-stage matching --- we use the strong duality of the convex programs, tied to a specific primal-dual analysis that is quite different from the known primal-dual analysis in the literature for various forms of online bipartite allocation problems. The sketch of our analysis is roughly the following: The Karush–Kuhn–Tucker (KKT) conditions at each stage $k$ offer a structural decomposition of the subgraph induced by the $k^{\text{th}}$ batch. The special unweighted case of this decomposition coincides with the well-studied \emph{matching skeleton} introduced by~\cite{GKK-12}, which itself is closely related to the Edmonds-Gallai decomposition~\citep{edm-65,gal-64} of bipartite graphs. Using this decomposition, and by carefully using our polynomials $f_1,\ldots,f_k$, we propose a novel \emph{recursive primal-dual framework} to bound the competitive ratio of our fractional matchings. The resulting dual constructions, together with our recursive formulation, shows how to improve the competitive ratios from $(1-1/e)$ to $\cratio{K}$ in the multi-stage setting with $K$ batches. In other words, this new algorithmic construct extends the dual constructions in previous work~\citep{MSVV-07,AGKM-11,BJN-07} in a novel fashion to the multi-stage setting with batch arrivals. As a side dish, our technique provides a convex-programming based interpretation for the existing primal-dual proofs in the special case of the online setting. 

\revcolor{
\smallskip
\noindent{\textbf{New Challenges for the Configuration Allocation~}}Switching to the multi-stage configuration allocation problem with free disposals, we aim to extend our earlier algorithm to this quite general model; nevertheless, as it turns out, our earlier algorithmic technique cannot be applied directly to the multi-stage configuration allocation problem because of three new fundamental technical challenges: (i)~\emph{Price-level treatment:} each advertiser pays for impressions at different price levels depending on the selected configuration, which is in a stark contrast to vertex-weighted matching where all impressions are essentially sold at the same price. Thus, it is not clear how to define a regularizer term to mimic the earlier approach,  (ii)~\emph{Lack of skeleton structure:} moving from matching to configuration allocation breaks several of the structural properties of the problem, most importantly the existence of a matching skeleton graph decomposition as mentioned earlier, which is crucial in the analysis of the multi-stage vertex-weighted matching, and (iii)~\emph{Managing preemption:} as the algorithm decides on the choice of the configuration at each time, it implicitly decides also on the number of impressions that each advertiser is responsible to pay at each price level at this point (and basically the rest are preempted); these price-level  dependent preemption or free-disposal decisions regarding previous impression-allocations are crucial to be able to obtain any bounded competitive algorithm, and a priori it is not  clear how to extend our previous approach to help with these preemption decisions.}



\revcolor{The first new key technical ingredient 
to circumvent the above challenges is the stage-dependent 
\emph{price-level regularized convex program}
\ref{eq:convex primal}
% stage-dependent convex programs
used by \Cref{alg:opt} in each stage $k\in[K]$. Similar to our previous convex programs, this new program maximizes the total revenue minus a regularization term by fractionally assigning a configuration to each user in batch $k$ and deciding which impressions should be preempted by each advertiser during stage $k$. This time, the regularization term is a summation of several terms, where we have one term for each advertiser
at \emph{each possible per-impression price level}. More precisely, we keep track of the price
distribution of top impressions allocated to each advertiser given her capacity
(i.e., the number of impressions at different per-impression price levels that the advertiser is willing to pay so far), instead of just her remaining capacity.
Having this distribution at the beginning of each stage $k$ as its input, the regularizer term corresponding to this advertiser is a separable function across all the price levels, where each term applies the primitive polynomial $F_k(x)$ in \Cref{prop:poly} to map the (normalized) number of allocated impressions at some price level to a penalty term in the objective. Intuitively speaking, this new form of regularization helps with gradually decreasing the hedging for each price level separately across stages.


The second new key technical ingredient is how to connect convex programs
\ref{eq:convex primal}
in each stage to an LP primal-dual analysis for the configuration allocation. As mentioned earlier, in contrast to the vertex-weighted matching, in general configuration allocation the resulting convex programs
\emph{do not admit} any matching skeleton or similar graph decompositions. The absence of this combinatorial structure, which has been the backbone of our previous primal-dual analysis, combined with price-level regularization and the need to incorporate preemption decisions in the analysis, make this new analysis more challenging. We circumvent this last obstacle by considering the Lagrangian dual program
\ref{eq:convex dual}
of the convex program
\ref{eq:convex primal}, 
and \emph{directly} using its optimal dual solution
to construct the dual assignment in the 
primal-dual analysis framework. Surprisingly, even with this different proposed dual assignment, we can connect the analysis of the competitive ratio to the same recursive functional equation across $K$ stages as before, and thus obtaining the $\cratio{K}$ competitive ratio by \Cref{alg:opt}. We should highlight that the connection between LP primal-dual analysis and the convex duality in our paper might be of independent interest in other online algorithm design problems. }

% As a comparison to
% \citet{FN-21}, they construct the dual assignment 
% using the generalized matching skeleton graph decomposition \citep[cf.][]{GKK-12,FN-21}. However, 
% as it turns out, in general models such as edge-weighted matching problem 
% or configuration allocation problem, similar convex programs
% \emph{do not admit} any similar structures, and hence do not induce any relevant graph decomposition or base function factorization. The absence of this structure, which has been the backbone of the primal-dual analysis in \cite{FN-21} for the special case of vertex-weighted matching, combined with price-level regularization and the need to incorporate preemption decisions in the analysis, make our analysis challenging.
% It turns out that 
% the optimal solution for the dual program
% of our convex program \ref{eq:convex primal}
% provide 

% The constructed dual assignment
% in our final proposed novel primal-dual analysis 
% is closely related to the \emph{theory of Fenchel/Lagrangian convex duality}~\citep[e.g., see][]{BV-04} for our convex programs 
% \ref{eq:convex primal}
% in \Cref{alg:opt}.
% To be more precise, we 

% consider the Lagrangian dual program
% \ref{eq:convex dual}
% of the convex program
% \ref{eq:convex primal}, 
% and use \emph{exactly} its optimal dual solution
% to construct the dual assignment in the 
% primal-dual analysis framework. Surprisingly, with our proposed dual assignment, we can connect the analysis of the competitive ratio to a recursive functional equation across $K$ stages, which has \emph{exactly} appeared before in \cite{FN-21}. This is indeed the reason  why a particular choice of polynomial regularizes, which is the solution of this recursive functional equation, attains the optimal $\cratio{K}$ competitive ratio.\footnote{See \cite{FN-21} for more context and the connection between the recursive equation and the mentioned polynomials.} We should highlight that the connection between LP primal-dual analysis and the convex duality in our paper might be of independent interest in other online algorithm design problems. 






We finally show the competitive ratio $\cratio{K}$ is the best achievable by any fractional multi-stage algorithm, whether deterministic or randomized, by showing an upper-bound instance for the special case of the unweighted multi-stage matching. Notably, this instance relies on batches of size more than one, and hence cannot be used as an upper-bound instance for the special case of online arrival where batch sizes are all one. See \Cref{fig:bad-example} for more details.



% We finally turn our attention to the integral versions of the vertex weighted b-matching and AdWords problems, when the capacities are large (or equivalently, bid over budget ratios are small). By using the totally unimodularity of flow-type polytopes~\citep{sch-03}, we propose our deterministic rounding algorithm for the vertex weighted b-matching problem. The idea is finding integer lower and upper bounds on the fractional degrees of each offline vertex using the fractional solution of the convex program at each stage, and then searching for an integral matching satisfying these bounds.  For the AdWords problem, we use a straightforward variant of independent randomized rounding at each stage, after slightly reducing all the budgets. By applying standard concentration bounds for each offline vertex, we prove that maintaining feasibility of the resulting integral allocation only adds a small loss in expectation when the bid over budget ratios are small. 

\smallskip
\noindent\textbf{Managerial Insights~} Our study sheds insights on the role of batching in service operation of matching platforms, and provides algorithmic evidences on how they should adaptively tune their batched matching algorithms to achieve the right trade-off between \emph{``greedy-ness''} in the current decision and {``hedging''} for the sake of future decisions \revcolor{in a prior-free non-stationary environment}:\footnote{\revcolor{We would like to reiterate that in our paper we make no assumptions on the number of nodes in each batch.}}
\begin{itemize}
    \item In settings that allow for latency---and hence allow for batching the demand arrivals---batched matching algorithms (versus fully online algorithms) can be used by the algorithm designer to obtain performance improvements, \revcolor{even when the environment is highly non-stationary}.
    \item There is an inherent trade-off between the gain from batching (which is captured by the competitive ratio in our competitive analysis framework) and the degree of batching (which is captured by the inverse number of batches in our framework) \revcolor{in prior-free non-stationary dynamic allocations}: with less number of batches/stages---which accounts for a higher degree of batching---a well-designed multi-stage matching algorithm can obtain a higher performance; moreover, it gets closer to the offline optimal matching as the degree of batching increases.\footnote{Of course, there is no free lunch here and the actual cost of batching is the induced latency in decision making.}
    \item When designing batched matching algorithms, our result suggests that pushing the matching to be more robust to future uncertainty early on (i.e., to be more balanced) and then pushing it to be more greedy later on will help with the performance in a finite horizon problem. In particular, we could formally capture this design aspect using our decreasing degree polynomial regularizers; However, in general, decreasing the degree of hedging induced by the matching algorithm over time to obtain improved performance is the main operational takeaway message of our work, and there might be other ways of performing this task in practice.
\end{itemize}




\revcolor{\smallskip
\noindent\textbf{Organization~} In \Cref{sec:prelim}, we start by formalizing both our baseline model (\Cref{sec:base-model}) and extension model (\Cref{sec:extension-model}).
In \Cref{sec:vertex-weight}, we introduce our first algorithm  by starting with some illustrative examples (\Cref{sec:example}). We then present this optimal competitive multi-stage algorithm for the vertex weighted bipartite matching problem (\Cref{sec:upper-bound}), and analyze its competitive ratio lower bound (\Cref{sec:primal-dual}). In \Cref{sec:extensions}, we switch to our extension model. We present our second algorithm, which is an optimal competitive multi-stage algorithm for the configuration allocation problem (\Cref{sec:alg-convex}), and characterize some of its properties (\Cref{sec:convex program}). We then analyze its competitive ratio lower bound (\Cref{sec:main proof}).
We finally show that our competitive ratio lower-bounds \emph{exactly} match the upper-bound on the competitive ratio of \emph{any} multi-stage algorithm (\Cref{sec:lowerbound}) and numerically evaluate the performance of our multi-stage algorithms on synthetic instances (Appendix~\ref{apx:numerical}).}

\subsection{Further Related Literature}
\label{sec:related}
Here is a summary of the other work in the literature directly related to our work.

\vspace{2mm}
\noindent\emph{Multi-stage matching.} \revcolor{Our work is closely related to \cite{feng2020two}, which studies the optimal competitive two-stage vertex weighted matching and pricing under both adversarial and stochastic settings. We extend their result in the adversarial case to multi stages and settings beyond vertex weighted matching (in particular to the more general settings of multi-stage edge-weighted matching and configuration allocation with free disposal). In \cite{feng2020two} basically there is a large class of convex programs that can be used in the first stage to introduce hedging. In our paper, we diverge by considering a \emph{different} form of convex-programming based matching where we use regularizers, and we show by changing the regularizer at each stage the optimal competitive ratio can be achieved for any $K$. Notably, both papers use a primal-dual analysis to analyze the underlying algorithm, but our dual construction in the analysis follows a different logic and has a different algebraic form (even for the special case of the two-stage problem).} Our result for the unweighted multi-stage matching is closely related to the beautiful work of \cite{LS-17}, which also uses the matching skeleton of \cite{GKK-12}, but for a different model of arrivals and online problem.

% In their model, a batch of \emph{new edges} arrive in each stage. Their proposed algorithm first finds a maximum fractional matching using the matching skeleton in each stage, and then removes some of the edges sampled from this matching through a randomized procedure. This approach obtains an optimal $2/3$ competitive ratio for two stages and a non-optimal $1/2+O(2^{-K})$ competitive ratio for $K$ stages. 
\vspace{2mm}

\noindent{\emph{Two-stage stochastic programming.}}
Two-stage stochastic combinatorial
optimization problems have been studied extensively in the 
literature
\citep[e.g.,][]{BL-11, CCP-05,SS-04,SS-07,IKMM-04, hanasusanto2015k,hanasusanto2018conic}.
Also, see the excellent book of \cite{kuhn2006generalized} for more context regarding convex multi-stage stochastic programs.  For two-stage stochastic matching, various models with different objectives
have been studied in \citet{KS-06, EGMS-10, KKU-08} and more recently in \cite{feng2020two}. Another work that is conceptually related to us is the recent work of \cite{housni2020matching}, which is inspired by the idea of robust multi-stage optimization~\citep[e.g.,][]{bertsimas2010optimality,bertsimas2011theory}. They consider a two-stage robust optimization for cost-minimization of the matching, where future demand uncertainty is modeled using a set of demand scenarios (specified explicitly or implicitly). Our model and results diverge drastically from this work.


\vspace{2mm}
\noindent\emph{Online bipartite allocations.}
Our results are comparable to the literature on online bipartite matching (with vertex arrival) and its extensions. Besides the work mentioned earlier, related to us is \cite{birnbaum2008line}, that gives a simple non primal-dual proof of RANKING algorithm of \cite{KVV-90} for online bipartite matching. An elegant primal-dual analysis is discovered later in \cite{DJK-13}. Also, at high-level, our primal-dual analysis resembles some aspects of ~\cite{BJN-07,FKMMP-09,devanur2009adwords,devanur2012online,esfandiari2015online,HKTWZZ-18,FNS-19}. Other related models are online bipartite stochastic matching~ \citep[e.g.,][]{feldman2009online,bahmani2010improved,MGS-12,mehta2014online,JL-14} and online bipartite matching with stochastic rewards~\citep[e.g.,][]{mehta2012online,goyal2020online,huang2020online}. We refer interested readers to a \revcolor{comprehensive} survey by \cite{mehta2013online} for further related work. Finally, related to us is also the literature on stochastic online packing and convex programming with large budgets~\citep[e.g.,][]{FMMS-10,DJSW-11,AD-14}. In particular, the role of concave regularizers have been studied in these settings for different purposes, e.g., fairness~\citep{agrawal2018proportional,balseiro2021regularized}, robustness to adversarial corruptions~\citep{balseiro2020best}, and obtaining blackbox reductions from Bayesian mechanism design to algorithm design~\citep{dughmi2021bernoulli}. 

\vspace{2mm}
\noindent\emph{Applications in revenue management and service operations.} From both methodological and application points of view, our work is related to several streams of work that focus to design online allocations and matching algorithms for problems in revenue management and service operations. These work pertain to practical applications in online retail, ride-sharing and other online platforms. Some examples are online assortment optimization (e.g., 
\citealp{GNR-14,MS-19}), online assortment of reusable resources  (e.g.,
\citealp{gong2019online,FNS-19,goyal2020onlineb}), Bayesian online assortment with heterogeneous customers (e.g.,
\citealp{rusmevichientong2020dynamic,feng2020near}), 
online assortment with replenishment~\citep{feng2021online}, dynamic pricing with static calendar \citep{MSZ-18}, volunteer crowd-sourcing and nudging~\citep{manshadi2020online}, two-sided assortment optimization~\citep{aouad2020online}, online allocation strategies in two-sided media platforms~\citep{alaei2020revenue}, \revcolor{online allocation of patient demand requests~\citep{golrezaei2021online}}, and finally the line of work on dynamic windowed supply-demand matching/queuing---with applications in ride-sharing (e.g., \citealp{ashlagi2019edge,aouad2020dynamic,ozkan2020dynamic,ata2020dynamic,aveklouris2021matching,arnosti2021managing}). \revcolor{Another recent work related to us is \cite{xie2022benefits} which studies the effect of delay (or equivalently look-ahead) in large-traffic stochastic stationary settings such as the multi-secretary problem~\citep{vera2021bayesian}. Our paper diverges from this work by considering non-stationary and adversarial arrival under batching instead of delay.}

% \subsection{from old intro}

% A canonical formulation to capture gist of some existing tensions in the above dynamic decision making scenarios is the (adversarial) online bipartite matching problem, originated from the seminal work of Karp, Vazirani, and Vazriani~\citep{KVV-90}. In this model, the online and offline vertices simply play the role of the arriving demand requests and the available supply, respectively. A rich body of literature has extended this simple formulation to more practical two-sided online allocation scenarios such as the online budgeted allocation/AdWords~\citep{MSVV-07} and the vertex weighted budgeted-matching~\citep{AGKM-11}. Other extensions and variants tailored to applications such as display advertising, ride-sharing, and assortment optimization are also studied~\citep{FKMMP-09, mehta2012online,MGS-12,GNR-14,HKTWZZ-18}. See \cite{mehta2013online} for a survey. On the algorithmic side, a sequence of past work have developed an elegant primal-dual framework to design and analyze online competitive algorithms in these problems~\citep{BJN-07,DJK-13,devanur2012online}. See \cite{buchbinder2009design} for a survey on the primal-dual technique in online algorithms, and specifically for designing and analyzing online bipartite allocation algorithms. 

\vspace{2mm}
\noindent\emph{Video-ads allocation.}
The popularity of in-stream video platforms has ignited 
a new research area related to video-ads, see 
a recent survey by \citet{FOG-21} for a detailed discussion.
There is a limited literature on
the algorithmic study of video-ads allocation.
Comparing to more traditional applications such as display ads,
video-ads (especially in-stream ads) 
have a distinct feature, which is the
need to be shown to the user during the video session.
\citet{DGNR-09} 
introduce the ``online story scheduling'' problem in which
the task is to schedule in-stream ads with 
different time lengths and per-unit prices for a single user in an online 
fashion, and
provide a constant competitive algorithm. 
Further improvements and 
studying other variants of this problem 
have been the focus in the literature, e.g., \citet{AP-19,LMQTYZ-16}.
\citet{BKK-09} study an alternative media scheduling problem 
for multiple users in an offline fashion.
\citet{SKFFC-17}
consider a variant of AdWords problem \citep{MSVV-07},
where each offline node (which is an in-stream ad in their model) is associated with 
a time length and every online node (i.e., a user) can be matched with multiple offline nodes as long as the total time length is below some threshold. 

==> FN_ multi-stage matching + configuration allocation (MS Journal)/tex/lower-bound.tex <==
\section{Competitive Ratio Upper-bound}
\label{sec:lowerbound}
In this section, we show a tight upper-bound of $\cratio{K}=\cratioexp$ on the worst-case competitive ratio of any multi-stage fractional matching algorithm, even for the special case of unweighted matching. This upper-bound clearly applies to the case of integral algorithms and the case of vertex weighted matching problem, and shows our earlier lower-bounds are the best achievable competitive ratios.


\begin{theorem}[\textbf{Tight Upper-bound for Multi-stage Matching}]
\label{thm:tightness}
No multi-stage fractional matching algorithm
can achieve a competitive ratio 
better than $\cratio{K}=\cratioexp$
in the $K$-stage (unweighted)
matching problem.
\end{theorem}
\smallskip
\noindent{\textbf{High-level Proof Overview}~} In order to show the upper-bound of $\cratio{K}$, we propose a distribution over deterministic instances of the multi-stage weighted fractional matching problem (i.e., a randomized instance), and show no fractional multi-stage algorithm obtains a competitive ratio better than $\cratio{K}$ over this randomized instance. To do so, we incorporate a simple factor revealing linear program whose optimal objective value provides an upper-bound on the competitive ratio of any feasible multi-stage matching algorithm. We then use LP primal-dual and by finding a feasible solution for its dual program we obtain the $\cratio{K}$ upper-bound. Interestingly, our upper-bound instance is a distribution over unweighted instances. Hence, the same upper-bound holds for the special case of multi-stage fractional matching in which all weights are equal.  

\begin{remark}[\textbf{Upper-bound for the Online Fractional Matching}]
\label{rem:online-matching-with-finite-nodes}
Notably, we need batches of size more than one in this instance, and hence our upper-bound \emph{does not} apply to the online matching problem with $K$ arrivals and batches of size $1$. So, while the competitive ratio $\cratio{K}$ is optimal for the multi-stage batch arrival problem, the competitive ratio of $\cratio{n}$ might not be optimal for the special case of online matching with $n$ vertex arrivals. To the best of our knowledge, the best known (almost) non-asymptotic competitive ratio upper-bound for the online fractional matching with $n$ arrivals is due to \cite{feige2019tighter}, where a bound of $\Theta(n)=\left(1-\frac{1}{e}\right)\left(1+\frac{1}{2n}\right)+O\left(\frac{1}{n^2}\right)$ is established. \revcolor{Note that a simple asymptotic expansion shows that $\Gamma(n)=\left(1-\frac{1}{e}\right)+\frac{1}{2en}+O\left(\frac{1}{n^2}\right) < \Theta(n)$, and hence the two bounds have a gap. Establishing the tight upper-bound for this problem is still open.}
 
\end{remark}
 
\subsection{Proof of \Cref{thm:tightness}}

Let $\M = K^K$.
Consider a bipartite graph 
$G=(\Rider,\Driver,E)$ with online vertices $\Rider$
and offline vertices $\Driver$,
where $\Rider = \Driver =
\{1,\dots, K\cdot \M\}= [K\M]$.
Online vertices $\Rider$
are partitioned into $K$ batches
$\{\Rider_1,\dots, \Rider_K\}$
where
the size of $\Rider_k$ is  $\left(\frac{K-1}{K}\right)^{k-1}\M$
for $k \in [K -1]$,
and $K\left(\frac{K-1}{K}\right)^{K-1}\M$
for $k = K$.
As a sanity check, notice that $\sum_{k = 1}^{K-1}
\left(\frac{K-1}{K}\right)^{k-1}\M +
K\left(\frac{K-1}{K}\right)^{K-1}\M = K\M$.

Let $\permu:[K\M]\rightarrow[K\M]$ be a uniform random permutation over $[K\M]$. Define the edge set $E$ of the graph $G$ as follows:
for each $k \in [K - 1]$,
each online vertex $i\in \Rider_k$
and offline vertex $j \in \Driver$,
there is an edge $(i, j)$ if $\permu(j) \leq K\,|\Rider_k|$;
for each online vertex $i\in\Rider_K$
and offline vertex $j\in \Driver$,
there is an edge $(i, j)$ if $\permu(j) \leq |\Rider_K|$.
Namely, at each stage $k$, we can partition offline vertices $\Driver$ into $\Driver_k$ and $\bar\Driver_k$
where $\Rider_k$ and $\Driver_k$
form a complete bipartite subgraph while 
there is no edge between $\Rider_k$
and $\bar\Driver_k$. The construction also ensures
that $\Driver_K \subseteq \Driver_{K - 1} \subseteq 
\dots \subseteq \Driver_1$. See \Cref{fig:bad-example} for an illustration of this randomized problem instance when permutation $\pi(i)=NK-i+1, i\in[NK]$ is realized.

\begin{figure}[hbt!]
	\centering
	
\includegraphics[trim=6.7cm 0cm 8.2cm 0cm,clip,width=0.8\textwidth]{figs/bad-example.pdf}
\caption{\label{fig:bad-example}The upper-bound instance when $\boldsymbol{\pi(i)=NK-i+1, i\in[NK]}$}
\end{figure}

First, we claim that there exists a perfect matching:
by backward induction on $k$ starting from $k=K$,
note that matching
all online vertices in
$\Rider_k$ with 
all offline vertices in
$
% \left\{
% j\in 
\Driver_k \backslash \Driver_{k+1} 
% \sum_{k' = k+1}^K |\Rider_{k'}| <
% \permu(j)
% \leq 
% \sum_{k' = k}^K |\Rider_{k'}|
% \right\}
$
for $k=1,2,\ldots,K$ produces a perfect matching between $\Rider$ and $\Driver$.

Next, we show that the expected size of the matching
produced by any given (possibly randomized) multi-stage fractional matching algorithm 
is at most $\cratio{K}\cdot K\M$,
where the expectation is taken over the randomness of the multi-stage algorithm
and the permutation $\permu$.
Let $\lusage_{k, j}^{\permu}$ be the expected degree
of offline vertex $j$ matched by the algorithm at stage $k$
under permutation $\permu$.
% The symmetry of our graph construction
% ensures that 
Note that:
$$\expect[\permu]{\lusage_{k, j}^{\permu} \condition j \not\in \Driver_k} = 0~~~~~\textrm{and}~~~~~\expect[\permu]{\lusage_{k, j}^{\permu} \condition j \in \Driver_k} 
= 
\expect[\permu]{\lusage_{k, j'}^{\permu}\condition j' \in \Driver_k}~$$ 
for all stages $k\in[K]$ and offline vertices $j, j'\in \Driver$.
The latter fact holds due to
the symmetry of our graph construction, i.e., conditioned on the event 
$[j\in\Driver_k~\&~j'\in \Driver_k]$,
it is an automorphism that exchanges $j$ and $j'$.
Thus, we can denote 
$\expect[\permu]{\lusage_{k, j}^{\permu} \condition j \in \Driver_k}$
by $\lusage_k$,
and write the following linear program and its dual 
to 
upper bound the expected size of the fractional matching
produced by any given (randomized or deterministic, integral or fractional) multi-stage algorithm:
\begin{equation*}
% \tag{\textsc{Primal-Dual-Upperbound}}
% \label{eq:LP-lower-bound}
\arraycolsep=1.4pt\def\arraystretch{1}
\begin{array}{llllllll}
\max\quad\quad\quad&
\displaystyle\sum_{k\in[K]}
|\Driver_k|\lusage_k
\qquad\qquad&\text{s.t.}&
&\quad\quad\text{min}\quad\quad\quad &
\mu + 
\displaystyle\sum_{k\in[K] }
{|\Rider_k|\zeta_k}
\qquad\qquad&\text{s.t.} \\[1.4em]
 &\displaystyle\sum_{k\in [K]}{\lusage_k}\leq 1~, & 
 & 
& &
\mu +|\Driver_k|\zeta_k
\geq |\Driver_k| & k\in[K]~,\\[1.4em]
 &
 |\Driver_k|\lusage_k
 \leq 
 |\Rider_k|&k\in [K]~, &
& &\mu\geq 0~, & \\
 &\lusage_k \geq 0 &k\in[K]~. &
& &\zeta_k \geq 0  &k\in [K]~. 
\end{array}
\end{equation*}
\ydrevcolor{Here, the variables are $\{\lusage_k\}_{k\in[K]}$
in the primal program and $\{\mu, \zeta_k\}_{k\in[K]}$ in the dual program. 
The primal objective function is the expected size of 
fractional matching induced by $\{\lusage_k\}_{k\in[K]}$,
the first primal constraint ensures that the total
expected allocation (over all $K$ stages) 
is at most one for each offline node,
and the second primal constraint
ensures that the expected 
fractional allocation on the offline side
is no more than the size of online nodes for each stage $k\in[K]$.}

Consider the following feasible dual solution 
with objective value $\cratio{K}\cdot K\M$
in the dual program:
$$\mu = |\Driver_K|~~~~,~~~~\zeta_k = \frac{|\Driver_k| - |\Driver_K|}{|\Driver_k|},~\forall k\in[K].$$
Invoking the weak duality between the above primal-dual linear
programs finishes 
the proof.\ifMS \hfill\Halmos \fi


==> FN_ multi-stage matching + configuration allocation (MS Journal)/tex/macros.tex <==

\TheoremsNumberedThrough 
\EquationsNumberedThrough
\usepackage{xfrac}
\usepackage{xcolor}
\usepackage{bbm}
%\usepackage[breakable, theorems, skins]{tcolorbox}
\usepackage{booktabs}
\usepackage{subfig}
\usepackage[ruled,vlined,linesnumbered]{algorithm2e}
\SetNoFillComment
% \DeclareRobustCommand{\mybox}[2][gray!10]{%
% \begin{tcolorbox}[   %% Adjust the following parameters at will.
%         left=0pt,
%         right=0pt,
%         top=0pt,
%         bottom=0pt,
%         colback=#1,
%         colframe=#1,
%         enlarge left by=0mm,
%         boxsep=15pt,
%         arc=5pt,outer arc=5pt,
%         ]
%         #2
% \end{tcolorbox}
% }


\usepackage[breakable, skins]{tcolorbox}
\DeclareRobustCommand{\mybox}[2][gray!10]{%
\begin{tcolorbox}[
        left=0.5pt,
        right=0.5pt,
        top=0.5pt,
        bottom=0.5pt,
        colback=#1,
        colframe=#1,
        width=\dimexpr\textwidth\relax, 
        enlarge left by=1mm,
        boxsep=3pt,
        arc=2pt,outer arc=2pt,
        code={\OneAndAHalfSpacedXII}
        ]
        #2
        
\end{tcolorbox}
}
\usepackage{csquotes}
\makeatletter
%Take the original environment definition and change the leftmargin to 1cm
\renewenvironment*{displayquote}
  {\begingroup\setlength{\leftmargini}{0.2cm}\csq@getcargs{\csq@bdquote{}{}}}
  {\csq@edquote\endgroup}
\makeatother



% \usepackage{csquotes}
% \makeatletter
% %Take the original environment definition and change the leftmargin to 1cm
% \renewenvironment*{displayquote}
%   {\begingroup\setlength{\leftmargini}{0.4cm}\csq@getcargs{\csq@bdquote{}{}}}
%   {\csq@edquote\endgroup}
% \makeatother
% \makeatletter

% %Take the original environment definition and change the leftmargin to 1cm
% \renewenvironment*{displayquote}
%   {\begingroup\setlength{\leftmargini}{0.6cm}\csq@getcargs{\csq@bdquote{}{}}}
%   {\csq@edquote\endgroup}
% \makeatother

\usepackage{mathtools}
%\usepackage{mathrsfs}
%\usepackage{dsfont}
\definecolor{cornellred}{rgb}{0.7, 0.11, 0.11}
\definecolor{maroon}{rgb}{0.52, 0, 0}
\definecolor{dgreen}{rgb}{0.0, 0.5, 0.0}
\definecolor{ballblue}{rgb}{0.13, 0.67, 0.8}
\definecolor{royalblue(web)}{rgb}{0.25, 0.41, 0.88}
\definecolor{bleudefrance}{rgb}{0.19, 0.55, 0.91}
\definecolor{royalazure}{rgb}{0.0, 0.22, 0.66}
\usepackage{hyperref}
\hypersetup{
	colorlinks = true,
	linkcolor=royalazure,
	urlcolor=royalazure,
	citecolor=royalazure,
	linkbordercolor = {white}
}
\usepackage{cleveref}
\usepackage{enumitem}
\usepackage{multirow}
%\DeclareRobustCommand*\cal{\@fontswitch\relax\mathcal}

\usepackage{pgf,tikz,pgfplots}
\pgfplotsset{compat=1.15}
\usetikzlibrary{arrows}
\usepackage{pgfplots}
\usetikzlibrary{patterns}
\usepgfplotslibrary{fillbetween}
\usetikzlibrary{intersections}
 %\usepackage{natbib}
% \setlength{\bibsep}{0.0pt}


\usetikzlibrary{arrows, decorations.markings}

% for double arrows a la chef
% adapt line thickness and line width, if needed
\tikzstyle{vecArrow} = [thick, decoration={markings,mark=at position
	1 with {\arrow[semithick]{open triangle 60}}},
	double distance=1.4pt, shorten >= 5.5pt,
	preaction = {decorate},
postaction = {draw,line width=1.4pt, white,shorten >= 4.5pt}]
\tikzstyle{innerWhite} = [semithick, white,line width=1.4pt, shorten >= 4.5pt]


% \ifMS
% \else
% \newtheorem{theorem}{Theorem}[section]
% \newtheorem{lemma}[theorem]{Lemma}
% \newtheorem*{lemma*}{Lemma}
% \newtheorem{proposition}[theorem]{Proposition}
% \newtheorem{corollary}[theorem]{Corollary}
% \newtheorem{observation}{Observation}
% \newtheorem{claim}{Claim}
% \newtheorem{remark}{Remark}
% \theoremstyle{definition}
% \newtheorem{definition}{Definition}[section]
% \theoremstyle{definition}
% % \newenvironment{example}[1][Example]{\begin{trivlist}
% % \item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
% %  	\newenvironment{remark}[1][Remark]{\begin{trivlist}
% %  \item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
% 	\newtheorem{assumption}[definition]{Assumption} 
% 		\newtheorem{example}[definition]{Example} 
% \fi

% 	\newenvironment{numberedassumption}[1]{%
% 		\renewcommand{\thedefinition}{#1}%
% \begin{assumption}}{\end{assumption}\addtocounter{definition}{-1}}

% 	\newenvironment{numberedremark}[1]{%
% 		\renewcommand{\thedefinition}{#1}%
% \begin{remark}}{\end{remark}\addtocounter{definition}{-1}}


%	\usepackage{accents}

	\usepackage[authoryear,round]{natbib}

% \usepackage{subfigure}





	\newcommand{\ubar}[1]{\underaccent{\bar}{#1}}
	\newcommand{\reals}{\mathbb{R}}
	\newcommand*{\R}{\mathbb{R}}





\ifMS
\else
	\DeclareMathOperator{\argmax}{argmax}
	\DeclareMathOperator{\argmin}{argmin}
\fi

\newcommand{\prob}[2][]{\text{\bf Pr}\ifthenelse{\not\equal{}{#1}}{_{#1}}{}\!\left[{\def\givenn{\middle|}#2}\right]}
\newcommand{\expect}[2][]{\text{\bf E}\ifthenelse{\not\equal{}{#1}}{_{#1}}{}\!\left[{\def\givenn{\middle|}#2}\right]}




\newcommand{\indicator}[1]{{\mathbbm{1}\left\{ #1 \right\}}}



\newcommand{\condition}{\,\mid\,}

	\DeclareMathOperator{\OPT}{\texttt{OPT}}
	\DeclareMathOperator{\MC}{\textrm{MaxCut}}
	\newcommand{\SDP}{\texttt{OPT-SDP}}
	\newcommand{\Ws}{\sum_{(i,j)\in E}w_{ij}}
	\newcommand{\OBJ}{\texttt{OBJ}}
	\newcommand{\Ycal}{\mathcal{Y}}
	\newcommand{\Ecal}{\mathcal{E}}
	\newcommand{\Zcal}{\mathcal{Z}}

	
	\DeclarePairedDelimiter{\norm}{\lVert}{\rVert}
	\DeclarePairedDelimiter{\card}{\lvert}{\rvert}
	\DeclarePairedDelimiter{\abs}{\lvert}{\rvert}
	\providecommand{\given}{}
	\DeclarePairedDelimiterX{\set}[1]\{\}{\renewcommand\given{\nonscript\:\delimsize\vert\nonscript\:\mathopen{}}#1}
	\let\Pr\relax
	\DeclarePairedDelimiterXPP{\Pr}[1]{\mathbb{P}}[]{}{\renewcommand\given{\nonscript\:\delimsize\vert\nonscript\:\mathopen{}}#1}
	\DeclarePairedDelimiterXPP{\Ex}[1]{\mathbb{E}}[]{}{\renewcommand\given{\nonscript\:\delimsize\vert\nonscript\:\mathopen{}}#1}
	\DeclarePairedDelimiter{\dotp}{\langle}{\rangle}
	\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
	\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}
	
\newcolumntype{P}[1]{>{\centering\arraybackslash}c{#1}}
	

	

	%%%-----------------Macros for this paper ------------------
	\newcommand{\RN}[1]{\textcolor{red}{\bf (Rad: #1)}}       
	\newcommand{\YF}[1]{\textcolor{green}{ (\em Yiding: \bf#1)}}





\newcommand*{\rom}[1]{\expandafter\romannumeral #1}
\newcommand{\Rom}[1]{\uppercase\expandafter{\romannumeral #1\relax}}
\newcommand{\valueDPsimple}{\mathcal{V}}



\newcommand{\onlineUnweightedRatioText}
{(1-\sfrac{1}{e}+\sfrac{1}{e^2})}
\newcommand{\onlineUnweightedRatio}
{1-\frac{1}{e}+\frac{1}{e^2}}
\newcommand{\onlineWeightedRatio}{0.7613}

\newcommand{\primed}{^\dagger}
\newcommand{\doubleprimed}{^\ddagger}

\newcommand{\mixap}{\alpha}

\newcommand{\combprob}{\lambda}
\newcommand{\matchprob}{q}
\newcommand{\matchprobi}{\matchprob_{\driver}}
\newcommand{\matchprobs}{\{\matchprob_\driver\}_{\driver\in[\totaldriver]}}
\newcommand{\msprob}{p}
\newcommand{\msprobi}{\msprob_\driver}
\newcommand{\matchprobHat}{\hat\matchprob}
\newcommand{\msprobHat}{\hat{\msprob}}
\newcommand{\msc}{c}
\newcommand{\msci}{\msc_\driver}

\newcommand{\msciHat}{\hat\msc_{j}}

\newcommand{\weight}{w}
\newcommand{\weightHat}{\hat{\weight}}
\newcommand{\weighti}{\weight_\driver}
\newcommand{\weights}{\{\weight_\driver\}_{\driver\in[\totaldriver]}}

\newcommand{\contribution}{\texttt{OBJ}}
\newcommand{\contributioni}{\contribution^{(\mspair)}}

\newcommand{\rider}{i}
\newcommand{\Rider}{U}
\newcommand{\RiderHat}{\hat \Rider}
\newcommand{\Rideri}{\Rider^{(\mspair)}}
\newcommand{\RideriHat}{\hat \Rider^{(\mspair)}}
\newcommand{\Riderj}{\Rider^{(j)}}
\newcommand{\driver}{j}
\newcommand{\Driver}{V}
\newcommand{\DriverHat}{\hat \Driver}
\newcommand{\Driveri}{\Driver^{(\mspair)}}
\newcommand{\DriveriHat}{\hat \Driver^{(\mspair)}}
%\newcommand{\Driverj}{D^{(j)}}
\newcommand{\Driverfirst}{S}
\newcommand{\DriverfirstHat}{\hat \Driverfirst}
\newcommand{\Driverfirsti}{\Driverfirst^{(\mspair)}}
\newcommand{\Driversecond}{\bar\Driverfirst}
\newcommand{\Driversecondi}{\bar\Driverfirst^{(\mspair)}}
\newcommand{\Driversecondb}{\tilde\Driverfirst}

\newcommand{\OPTHat}{\hat{\OPT}}
\newcommand{\GD}{\texttt{GD}}
\newcommand{\GDi}{\GD^{(\mspair)}}
\newcommand{\GDBar}{\underline{\GD}}
\newcommand{\MS}{\texttt{MS}}
\newcommand{\MSBar}{\underline{\MS}}
\newcommand{\MSi}{\MS^{(\mspair)}}

\newcommand{\xbf}{\mathbf{x}}
\newcommand{\zbf}{\mathbf{z}}
\newcommand{\ybf}{\mathbf{y}}
\newcommand{\lambdabf}{\boldsymbol{\lambda}}
\newcommand{\thetabf}{\boldsymbol{\theta}}
\newcommand{\gammabf}{\boldsymbol{\gamma}}

\newcommand{\Lag}{\mathcal{L}}

\newcommand{\OPTi}{\OPT^{(\mspair)}}

\newcommand{\GDHat}{\hat{\GD}}
\newcommand{\GDBarHat}{\hat{\GDBar}}
\newcommand{\MSHat}{\hat{\MS}}
\newcommand{\MSBarHat}{\hat{\MSBar}}

\newcommand{\N}{\mathbb{N}}

\newcommand{\totaldriver}{n}
\newcommand{\totalmspair}{L}
\newcommand{\totalmspairHat}{\hat L}
\newcommand{\mspair}{l}
\newcommand{\msfirst}{s}
\newcommand{\msfirsti}{\msfirst^{(\mspair)}}

\newcommand{\mssecond}{k}
\newcommand{\mssecondi}{\mssecond^{(\mspair)}}
\newcommand{\msseconds}{\{\mssecondi\}_{\mspair\in[\totalmspair]}}

\newcommand{\msfirsts}{\{\msfirsti\}_{\mspair\in[\totalmspair]}}
    
\newcommand{\msdriver}{n}
\newcommand{\msdriveri}{\msdriver^{(\mspair)}}
\newcommand{\msdrivers}{\{\msdriveri\}_{\mspair\in[\totalmspair]}}

    
\newcommand{\msrider}{m}
\newcommand{\msrideri}{\msrider^{(\mspair)}}
\newcommand{\msriders}{\{\msrideri\}_{\mspair\in[\totalmspair]}}

\newcommand{\mspairc}{\msc}
\newcommand{\mspairci}{\mspairc^{(\mspair)}}

\newcommand{\matchprobwithweights}{\{(\matchprobi,\weighti)\}_{\driver\in[\totaldriver]}}

\newcommand{\mspairinstance}{\{(\msdriveri,\msfirsti,\msrideri)\}_{\mspair\in[\totalmspair]}}

\newcommand{\mspairinstancenew}{\{(\msdriveri,\msfirsti,\msrideri,\mssecondi)\}_{\mspair\in[\totalmspair]}}

\newcommand{\RaHat}{\hat R_{\mathcal{A}}}
\newcommand{\RpHat}{\hat R_{\mathcal{P}}}

\newcommand{\weightp}{\bar\weight}
\newcommand{\weightdp}{\tilde\weight}
% \newcommand{\weightp}{\weight^{\dagger}}
% \newcommand{\weightdp}{\weight^{\ddagger}}

\newcommand{\driverTilde}{\tilde{\driver}}
\newcommand{\driverBar}{\bar{\driver}}

\newcommand{\val}{v}
\newcommand{\thresh}{t}
\newcommand{\Thresh}{\mathcal{T}}
\newcommand{\price}{p}
\newcommand{\acceptprob}{q}

\newcommand{\assignprob}{x}
\newcommand{\assignprobi}{\assignprob_{\rider\driver}}
\newcommand{\assignprobs}{\{\assignprobi\}_{(\rider,\driver)\in E}}

\newcommand{\assignvertexprob}{y}
\newcommand{\assignvertexprobi}{\assignvertexprob_{\rider}}
\newcommand{\assignvertexprobj}{\assignvertexprob_{\driver}}
\newcommand{\Ra}{R_{\mathcal{A}}}
\newcommand{\Rp}{R_{\mathcal{P}}}
\newcommand{\Rpa}{\tilde{R}_{\mathcal{P}}}
\newcommand{\Fu}{F_{i}}
\newcommand{\pb}{\mathbf{p}}
\newcommand{\RP}{\R_{\geq 0}}
\newcommand{\opt}{\texttt{OPT}}
\newcommand{\optoff}{\texttt{OPT}_{\textrm{offline}}}
\newcommand{\optoffmp}{\texttt{OPT}_{\textrm{offline-MP}}}
\newcommand{\opton}{\texttt{OPT}_{\textrm{online}}}
\newcommand{\maxmatch}{\textsc{Max-WeightMatch}^{\mathbf{w}}}
\newcommand{\maxmatchboth}{\textsc{Max-WeightMatch}^{\mathbf{\hat w}}}
\newcommand{\compratioM}{\Gamma_{\textrm{weighted-matching}}}
\newcommand{\compratioMUW}{\Gamma_{\textrm{matching}}}
\newcommand{\compratioMP}{\Gamma_{\textrm{matching-pricing}}}
\newcommand{\objr}{\texttt{OBJ}^{\Ra\cup\Rp}}
\newcommand{\objd}{\texttt{OBJ}^{D}}

\newcommand{\order}{\sigma}
\newcommand{\ordera}{\order_{\mathcal{A}}}
\newcommand{\orderp}{\order_{\mathcal{P}}}

\newcommand{\feasibles}{\mathcal{X}}
\newcommand{\quant}{q}


\newenvironment{numberedtheorem}[1]{%
\renewcommand{\thetheorem}{#1}%
\begin{theorem}}{\end{theorem}\addtocounter{theorem}{-1}}

\newenvironment{numberedproposition}[1]{%
\renewcommand{\thetheorem}{#1}%
\begin{proposition}}{\end{proposition}\addtocounter{theorem}{-1}}

\newenvironment{numberedlemma}[1]{%
\renewcommand{\thetheorem}{#1}%
\begin{lemma}}{\end{lemma}\addtocounter{theorem}{-1}}

\newcommand{\M}{N}
\newcommand{\permu}{\pi}

\newcommand{\lusage}{\xi}

\newcommand{\budget}{B}
\newcommand{\minbudget}{\budget_{\text{min}}}
\newcommand{\iprime}{{i^\dagger}}
\newcommand{\jprime}{{j^\dagger}}
\newcommand{\PRMWBM}{\texttt{PR-MWBM}}
\newcommand{\PRFAD}{\texttt{PR-F-AdWords}}
\newcommand{\PRIAD}{\texttt{PR-I-AdWords}}
\newcommand{\PRMCA}{\texttt{PR-MCA}}


\newcommand{\config}{c}
\newcommand{\Config}{C}
\newcommand{\threeindex}{\rider,\config,\driver}
\newcommand{\wi}{\tau}
\newcommand{\totalweight}{T}
\newcommand{\twoindex}{\driver,\wi}
\newcommand{\comsumption}{\eta}
\newcommand{\alloc}{\xi}
\newcommand{\alloci}{\alloc_{\threeindex}}
\newcommand{\allocs}{\boldsymbol{\alloc}}
% \newcommand{\weights}{\mathbf{\weight}}
\newcommand{\pibf}{\boldsymbol{\pi}}
\newcommand{\mubf}{\boldsymbol{\mu}}
\newcommand{\phibf}{\boldsymbol{\phi}}
\newcommand{\psibf}{\boldsymbol{\psi}}
\newcommand{\iotabf}{\boldsymbol{\iota}}
\newcommand{\lambdai}{\lambda_{\rider}}
\newcommand{\thetai}{\theta_{\driver}}
\newcommand{\mui}{\mu_{\threeindex}}
\newcommand{\phii}{\phi_{\rider,\config}}
\newcommand{\psii}{\psi_{\threeindex}}
\newcommand{\starred}{^*}
\newcommand{\ked}{^{(k)}}
\newcommand{\KED}{^{(K)}}
\newcommand{\sed}{^{(s)}}
\newcommand{\xbfi}{\xbf\ked}
\newcommand{\zbfi}{\zbf\ked}
\newcommand{\ybfi}{\ybf\ked}
\newcommand{\kminused}{^{(k-1)}}
\newcommand{\KMINUSED}{^{(K-1)}}
\newcommand{\sminused}{^{(s-1)}}
\newcommand{\alphabf}{\boldsymbol{\alpha}}
\newcommand{\betabf}{\boldsymbol{\beta}}
\newcommand{\comsumptioni}{\comsumption_{\twoindex}\kminused}
\newcommand{\taup}{{\tau\primed}}
\newcommand{\taupp}{{\tau\doubleprimed}}
\newcommand{\Eta}{H}
\newcommand{\cumcomsumption}{\Eta}
\newcommand{\cumcomsumptioni}{\cumcomsumption_{\twoindex}}

\newcommand{\ALG}{\texttt{ALG}}

\newcommand{\weightbf}{\mathbf{\weight}}

==> FN_ multi-stage matching + configuration allocation (MS Journal)/tex/multi-stage.tex <==
\section{Multi-stage Vertex Weighted Matching}
\label{sec:vertex-weight}
In this section we show the result
of the baseline model, 
which is an optimal competitive algorithm for the $K$-stage (fractional) vertex weighted matching problem. We start by a few simple examples to provide intuitions behind some of the main technical ideas used in the design of our algorithm. Then, in \Cref{sec:upper-bound}, we formally describe this algorithm and all of its ingredients. We then provide details of our new convex-programming based primal-dual framework in \Cref{sec:primal-dual}, and show how the recursive sequence of polynomials introduced in \Cref{prop:poly} help with analyzing the competitive ratio. 

% Note that in this section, for ease of exposition, 
% we focus on the the problem of designing fractional multi-stage allocations. 
% We extend our study to the integral vertex weighted b-matching
% and integral budgeted allocation, both  
% under the large budgets assumption, in \Cref{sec:extensions}.

\input{tex/example}

\input{tex/vertex-weighted}



==> FN_ multi-stage matching + configuration allocation (MS Journal)/tex/prelim.tex <==
\section{Preliminaries}
\smallskip
\label{sec:prelim}
%\subsection{Baseline Model: Multi-stage Edge-weighted Matching}
\subsection{Baseline Model: Multi-stage Vertex Weighted Matching}
\label{sec:base-model}
We study \emph{vertex weighted matching} as our baseline bipartite allocation model for matching arriving demands requests to available supply.
An instance of our model consists of a bipartite graph $\mathcal{G}=(\Rider,\Driver,E)$, where vertices 
in $\Driver$ (supply) are present offline 
and vertices in $\Rider$ (demand) arrive over time. 
Specifically, we consider a \emph{multi-stage arrival} model, 
in which vertices in $\Rider$ arrive in $K\in\mathbb{N}$ stages. 
We assume the number of stages $K$ is fixed and known by the algorithm. At each stage $k\in[K]$, a new subset of online vertices $\Rider_k\subseteq \Rider$ arrive, which we often call an arriving \emph{batch}, and reveal their incident edges in $E$. \revcolor{We assume $\lvert\Rider_k\rvert \geq 1$ and we make no further assumptions on $\Rider_k$'s.} We highlight that $\Rider=\cup_{k\in[K]}\Rider_k $ and $\Rider_k\cap\Rider_{k'}=\emptyset$ for $k\neq k'$. Each offline vertex $j$ has a total capacity $n_j$ for allocations, as well as a non-negative weight $w_j$ for each unit of allocation. 
After arrival of batch $k$, the multi-stage allocation algorithm makes an irrevocable allocation decision by allocating each vertex $i\in\Rider_K$ (which corresponds to one unit of demand) to the set of neighboring offline vertices $j\in\Driver, (i,j)\in E$ that have non-zero remaining capacity. Let $E_k$ denote the set of edges in $E$ incident to $\Rider_k$. 
We denote the allocation of stage $k$ by the vector $\xbf_{k}\in\mathbb{R}^{E_k}$, where $x_{k,ij}\in[0,1]$ is the amount of allocation of vertex $i$ to $j$. 
This allocation can be fractional or integral. We mostly focus on fractional allocations and assume $n_j=1$ for all the offline vertices $j\in\Driver$ without the loss of generality.\footnote{\revcolor{We are essentially considering fractional algorithms and adversarial arrivals; in such a setting, without the loss of generality, we can focus on adversaries that choose the input instance adaptively.}}  The goal of the multi-stage vertex weighted matching algorithm is to maximize the total weight of offline vertices in the (fractional) allocation, while ensuring  feasibility, i.e., each online (resp. offline) vertex uses no more than one unit of demand (resp. capacity).

\revcolor{\subsection{Extension Model: Multi-stage Configuration Allocation}
\label{sec:extension-model}
Motivated by the application of displaying video-ads in video streaming platforms, we also study the extension of our baseline model to \emph{multi-stage configuration allocation}. An instance of this model consists of a set of offline advertisers $\Driver$ who are willing to pay the platform to display their ads to its users and a set of arriving users $\Rider$ who are planning to watch videos on this platform. Specifically, 
the platform needs to choose
an advertising \emph{configuration} $\config\in\Config$
for each user (or equivalently, for each video session watched by a user), where $\Config$ is the set of feasible configurations.\footnote{Our model and results allow a different feasible set for each user, but we omit that for simplicity.} Fixing a user $\rider\in \Rider$,
choosing each configuration $\config\in\Config$ 
allocates a certain number of reserved impressions 
$\alloc_{\threeindex}$
at a non-negative per-impression price $\weight_{\threeindex}$
to each advertiser $\driver\in\Driver$.
% advertiser $\driver$'s impression 
% have been displayed to user $\rider$
% with per-unit price $\weight_{\threeindex}$.
Each advertiser $\driver$
demands $n_\driver$ number of impressions in total. We assume free-disposal, which means that the total allocated impressions to advertiser $j$ can exceed $n_j$, but she is eventually only paying for the top $n_j$ most expensive impressions. Similar to our baseline model in \Cref{sec:base-model}, users 
arrive to the platform over time
in $K\in\N$ stages. At each stage $k\in [K]$
a new batch of online users $\Rider_k\subseteq\Rider$
arrives. Upon the arrival of this batch, the video platform observes 
$\allocs\ked = \{\alloci\}_{\rider\in\Rider_k,\config\in\Config,\driver\in \Driver}$
and 
$\weightbf\ked = \{\weight_{\threeindex}\}_{\rider\in\Rider_k,\config\in\Config,\driver\in \Driver}$. Then the multi-stage allocation algorithm makes an irrevocable decision by
assigning a configuration to each user $\rider\in\Rider_k$. These configuration allocations can be integral or fractional. 
In this paper we focus on the fractional allocations~\footnote{\label{footnote:integral}Using standard randomized rounding techniques, all of our results for the fractional allocation problem, including the algorithm and its competitive analysis, can easily be extended to the setting with integral randomized allocations under the \emph{large budget assumptions}, i.e, in the asymptotic regime when $\underset{i,c,j}{\min}\frac{n_j}{\alloci}$ is large.} and assume $n_j=1$ for all advertisers $j\in\Driver$ without the loss of generality.\footnote{Since we allow fractional solutions, it is without
loss of generality to normalize the parameters after a simple change of variables, so that we can assume $n_\driver = 1$ for all $\driver\in \Driver$ without loss of generality. We omit details for brevity.}
 The goal of the multi-stage configuration allocation algorithm is to choose configurations for the users to maximize the total collected payments from allocating impressions to the advertisers at the end, which we also refer to as the revenue of the platform.}

\revcolor{
\smallskip
\noindent\textbf{LP Formulation and Offline Benchmark}~~To help with understanding our extension model, we formulate the
optimum offline solution in
the configuration allocation
problem as a simple linear program, denoted by  
\ref{eq:LP primal}:
    \begin{equation}
\tag{\textsc{PRIMAL-MCA}}
\label{eq:LP primal}
\arraycolsep=1.4pt\def\arraystretch{1}
\begin{array}{lllll}
\max\limits_{\xbf,\zbf\geq \mathbf{0}}
\quad\quad\quad&
% \mathop{\displaystyle\sum
\displaystyle\sum_{\rider\in\Rider}
\displaystyle\sum_{\config\in\Config}
\displaystyle\sum_{\driver\in\Driver}
\weight_{\threeindex}\cdot
% }
% \limits_{(\threeindex)\in E}
 x_{\threeindex}
&~~\text{s.t.}
% \min\limits_{\alphabf,\betabf,\gammabf}
% \quad\quad\quad 
% &
% \displaystyle\sum_{\rider\in \Rider }{\alpha_\rider}+
% \displaystyle\sum_{\driver\in \Driver}{\beta_\driver}
% &~~\text{s.t.} 
\\[1.4em]
 &
%  \mathop{\displaystyle\sum
\displaystyle\sum_{\rider\in\Rider}
\displaystyle\sum_{\config\in\Config}
 x_{\threeindex} 
%  }
%  \limits_{\rider,\config:(\threeindex)\in E}
 \leq
 n_{\driver} 
 &~~\driver\in\Driver~,
% \gamma_{\threeindex} 
% +
% \beta_\driver \geq \weight_{\threeindex}
% & (\threeindex)\in E~,
\\[1.4em]
 &
 \displaystyle\sum\limits_{\config\in\Config}
 z_{\rider,\config}
 \leq 1 
 &~~
 \rider\in \Rider~, 
% \alpha_\rider 
% \geq 
% \displaystyle\sum\limits_{\driver\in \Driver}
% \alloci\cdot \gamma_{\threeindex} &i\in \Rider, \config\in \Config~, 
\\[1.4em]
 &
 x_{\threeindex} \leq 
 \alloci \cdot z_{\rider,\config}
 &~~
\rider\in\Rider,\config\in\Config,\driver\in\Driver~. 
% \alpha_\rider 
% \geq 0 &\rider \in \Rider~, 
% \\[1.4em]
%  &x_{\threeindex} \geq 0 &(\threeindex)\in E~, &
% & &
% \beta_\driver\geq 0  &\driver\in \Driver~,
% \\[1.4em]
%  &z_{\rider,\config} \geq 0 &\rider\in\Rider, \config\in \Config~. &
% & &
% \gamma_{\threeindex} \geq 0  &(\threeindex)\in E~.
\end{array}
\end{equation}
In the above formulation, $z_{\rider,\config}$
is the fraction of configuration $\config$ assigned
to user $\rider$,
and $x_{\threeindex}$
is the (fractional) number of impressions
created by user $\rider$ for advertiser $\driver$ based on configuration $\config$ that the advertiser is finally willing to pay. Note that the number $x_{\threeindex}$ of impressions that the advertiser is willing to pay is no more than number of allocated impressions $\alloci \cdot z_{\rider,\config}$ from user $\rider$ under configuration $\config$, and the first quantity can be strictly smaller than the second (as advertiser $\driver$ should only pay for at most $n_\driver$ impressions overall). If an impression is allocated but the advertiser is not responsible to pay for it, we refer to that impression as being \emph{preempted} or \emph{freely disposed}. 


We finally note that the multi-stage configuration allocation problem
generalizes the multi-stage vertex weighted matching problem. Also, although we allow for free-disposal in the extension model as allocations of an advertiser's capacity can value differently (i.e., be at a different price level) for different users and configurations, for the special case of vertex weighted matching there is no point in free-disposal by any multi-stage algorithm, as all allocations of an offline node's capacity value the same. See the formal details in Appendix~\ref{apx:connection}. This distinction is the key that requires novel extensions of our techniques for the baseline model to capture different price levels.}

















% We study the \emph{edge-weighted matching with free disposal} as our baseline bipartite allocation model for matching arriving demands requests to available supply. An instance of our model consists of a weighted complete bipartite graph $\mathcal{G}=\left(\Rider,\Driver,[w_{ij}]\right)$, where vertices 
% in $\Driver$ (supply) are available offline 
% and vertices in $\Rider$ (demand) arrive over time. 
% Specifically, we consider a \emph{multi-stage arrival} model, 
% in which vertices in $\Rider$ arrive in $K\in\mathbb{N}$ stages. 
% We assume the number of stages $K$ is fixed and known by the algorithm. At each stage $k\in[K]$, a new subset of online vertices $\Rider_k\subseteq \Rider$ arrive, which we often call an arriving \emph{batch}. We highlight that $\Rider=\cup_{k\in[K]}\Rider_k $ and $\Rider_k\cap\Rider_{k'}=\emptyset$ for $k\neq k'$. Each edge $(i,j)\in \Rider\times\Driver$ has a non-negative weight $w_{ij}$, which determines the reward of allocating each unit of offline vertex $j$ to arriving vertex $i$.\footnote{Despite the graph $\mathcal{G}$ being complete, edge-weight $w_{ij}=0$ essentially means there exists no edge between $i$ and $j$.} Upon the arrival of batch $k$, all of the vertices $i\in\Rider_k$ reveal their incident edge weights $w_{ij}$ to the offline nodes $j\in\Driver$.
% Then the multi-stage allocation algorithm makes an irrevocable allocation decision by allocating each vertex $i\in\Rider_K$ (which corresponds to one unit of demand) to the set of \emph{available} neighboring offline vertices $j\in\Driver, (i,j)\in E$ . Let $E_k$ denote the set of edges in $E$ incident to $\Rider_k$. 
% We denote the allocation of stage $k$ by the vector $\xbf_{k}\in\mathbb{R}^{E_k}$, where $x_{k,ij}\in[0,1]$ is the amount of allocation of vertex $i$ to $j$. 
% This allocation can be fractional or integral. 

% Each offline vertex $j\in\Driver$ has a non-negative weight $w_j$ for each unit of allocation. 
% The goal of the multi-stage vertex weighted matching
% is to maximize the sum of the weight of the offline vertices in the (fractional) allocation, while ensuring the feasibility constraints -- 
% every demand/supply vertex can be matched at most 
% one unit.

\subsection{Competitive Ratio Analysis}

We measure the performance of our multi-stage algorithms by their \emph{competitive ratio}, which is the worst-case ratio between the expected total weight \revcolor{(or total revenue)} of the algorithm and the optimum offline benchmark given the entire problem instance (formally defined below).
\begin{definition}[\textbf{Competitive Ratio}]
	\label{def:competitive ratio}
	Fix the number of stages $K\in\mathbb{N}$. For $\alpha\in [0,1]$, a multi-stage allocation algorithm $\ALG$ is \emph{$\alpha$-competitive} against the optimum offline solution in the multi-stage vertex weighted matching \revcolor{(resp. multi-stage configuration allocation)} problem, if we have:
	\begin{align*}
		\inf\limits_{I \in\mathcal{I}^{(K)}}~~
		\frac{\ALG(I)}{\texttt{OPT}(I)}~
		\geq \alpha~,
	\end{align*}
	where $\mathcal{I}^{(K)}$ is the set of instances of the multi-stage vertex weighted matching  \revcolor{(resp. multi-stage configuration allocation)} problem with $K$ stages, 
	and $\ALG(I)$ and $\texttt{OPT}(I)$ are the total weights \revcolor{(resp. total revenue)} of the multi-stage algorithm $\ALG$ and optimum offline solution on an instance $I$, respectively. 
	For randomized multi-stage algorithms, we abuse the notation and $\ALG(I)$ denotes the expected total weight \revcolor{(resp. expected total revenue)} of the algorithm on an instance $I$.
\end{definition}

%  As an important note, we are mainly interested in the competitive ratio of fractional $K$-stage algorithms.

%  We also consider the asymptotic competitive ratio of integral $K$-stage algorithms (possibly randomized) under the ``large budgets assumption'' in the vertex weighted b-matching problem (i.e., under the assumption that $\min_j B_j=\Omega(1)$), or equivalently under the small bid over budget assumption in the budgeted allocation problem (i.e., under the assumption that $\max_{i,j} \frac{b_{ij}}{B_j}=o(1)$ or equivalently $\min_j B_j=\Omega(1)$ when $b_{ij}\in[0,1]$). 

\subsection{A Recursive Sequence of Polynomials}
\label{sec:poly}
As a novel technical ingredient of our proposed multi-stage allocation algorithms, we identify a particular sequence of polynomials of decreasing degrees. Our construction of these polynomials is recursive, which gives us a polynomial of degree $K-k$ for each stage $k=1,2,\ldots,K-1$. Here, we introduce these polynomials, describe this underlying recursive equation, and elaborate a bit more on some of their properties (\Cref{prop:poly}; see the proof in Appendxi~\ref{apx:poly}). Later, we first show in \Cref{sec:vertex-weight} how these polynomials help us to design an optimal competitive multi-stage algorithm for the vertex weighted matching and how to develop a primal-dual analysis framework that incorporates this recursive equation. \revcolor{Then we show how to extend these ideas and use our polynomials for the general multi-stage configuration allocation problem in \Cref{sec:extensions}, where we require treating allocations at different price levels differently --- as will be clear later.}

\begin{proposition}[{\textbf{{Sequence of Polynomial Regularizers}}}]
\label{prop:poly}
Consider a sequence of functions $f_1,f_2,\ldots,f_{K}:[0,1]\rightarrow[0,1]$
satisfying the following backward recursive equation:
\begin{itemize}
    \item $\forall x\in[0,1]:~f_{K}(x)=\mathbb{I}\{{x=1\}}$,
    where $\mathbb{I}(\cdot)$ is 
    the indicator function,
    \item $\forall x\in[0,1], k\in[K-1]:~f_{k}(x)=\underset{y\in[0,1-x]}{\max}~(1-y)f_{k+1}(x+y)$.
\end{itemize}
Then, the following statements hold:
\begin{enumerate}[label=(\roman*)]
    \item The function sequence $\{f_k\}_{k=1}^{K-1}$ is a sequence of $K-1$ polynomials with decreasing degrees, where $f_k(x)=(1-\frac{1-x}{K-k})^{K-k}$ for $k\in[K-1]$.\footnote{As a convention, we refer to $f_K(x)=\mathbb{I}\{x=1\}$ as a polynomial of degree $0$ (although not mathematically rigorous).}
    \item $f_k(x)$ is monotone increasing and continuous over $[0,1]$ for $k\in[K-1]$. Hence, $F_k(x)\triangleq \int_{0}^x f_k(y)dy$ is differentiable and strictly convex over $[0,1]$ for $k\in[K-1]$.
    \item $\forall k\in[K]$, $f_k(x)\leq e^{x-1}$ for $x\in[0,1]$. Moreover, the first function $f_1(x)=(1-\frac{1-x}{K-1})^{K-1}$ converges point-wise from below to the function $e^{x-1}$ as $K\to+\infty$ (see \Cref{fig:poly}).
    \item $\underset{y\in[0,1]}{\min}1-(1-y)f_1(y)=\cratioexp\triangleq\cratio{K}$
\end{enumerate}
\end{proposition}

The aforementioned polynomials $\{f_k\}_{k\in[K-1]}$ are drawn in \Cref{fig:poly}. As it is clear from this figure, these polynomials provide careful point-wise estimations for the exponential function $f(x)=e^{x-1}$ at different levels of precision. When these polynomials are used to regularize the maximum weight matching (or total revenue) objective functions, they provide different levels of ``hedging'' intensity against the future uncertainty in the arriving input exactly because of these different levels of estimation precision. This point will be clear in the upcoming sections.




==> FN_ multi-stage matching + configuration allocation (MS Journal)/tex/prelim_old.tex <==
\section{Preliminaries}
\smallskip
\label{sec:prelim}
\subsection{Baseline Model: Multi-stage Vertex Weighted Matching}
Our baseline model studies
\emph{multi-stage vertex weighted matching}
--
a bipartite allocation model
for matching arriving demand requests to available suppliers. 
An instance of our model consists of a bipartite graph $\mathcal{G}=(\Rider,\Driver,E)$, where vertices 
in $\Driver$ (supply) are available offline 
and vertices in $\Rider$ (demand) arrive over time. 
Specifically, we consider a \emph{multi-stage arrival} model, 
in which vertices in $\Rider$ arrive in $K\in\mathbb{N}$ stage. 
We assume the number of stages $K$ is fixed and known by the algorithm. At each stage $k\in[K]$, a new subset of online vertices $\Rider_k\subseteq \Rider$ arrive, which we often call an arriving \emph{batch}, and reveal their incident edges in $E$. 
We highlight that $\Rider=\cup_{k\in[K]}\Rider_k $ and $\Rider_k\cap\Rider_{k'}=\emptyset$ for $k\neq k'$. 
After arrival of batch $k$, the multi-stage allocation algorithm makes an irrevocable allocation decision by allocating each vertex $i\in\Rider_K$ (which corresponds to one unit of demand) to the set of \emph{available} neighboring offline vertices $j\in\Driver, (i,j)\in E$ . Let $E_k$ denote the set of edges in $E$ incident to $\Rider_k$. 
We denote the allocation of stage $k$ by the vector $\xbf_{k}\in\mathbb{R}^{E_k}$, where $x_{k,ij}\in[0,1]$ is the amount of allocation of vertex $i$ to $j$. 
This allocation can be fractional or integral. 

Each offline vertex $j\in\Driver$ has a non-negative weight $w_j$ for each unit of allocation. 
The goal of the multi-stage vertex weighted matching
is to maximize the sum of the weight of the offline vertices in the (fractional) allocation, while ensuring the feasibility constraints -- 
every demand/supply vertex can be matched at most 
one unit.

\subsection{Competitive Ratio Analysis}

We measure the performance of our multi-stage algorithms by their \emph{competitive ratio}, which is the worst-case ratio between the expected total weight of the algorithm and the optimum offline benchmark given the entire problem instance (formally defined below).
\begin{definition}[\textbf{Competitive Ratio}]
	\label{def:competitive ratio}
	Fix the number of stages $K\in\mathbb{N}$. For $\alpha\in [0,1]$, a multi-stage allocation algorithm $\ALG$ is \emph{$\alpha$-competitive} against the optimum offline solution in the multi-stage vertex weighted matching problem, if the following holds:
	\begin{align*}
		\inf\limits_{I \in\mathcal{I}}~~
		\frac{\ALG(I)}{\texttt{OPT}(I)}~
		\geq \alpha~,
	\end{align*}
	where $\mathcal{I}$ is the set of instances of the multi-stage vertex weighted matching problem, 
	and $\ALG(I)$ and $\texttt{OPT}(I)$ are the total weights of the multi-stage algorithm $\ALG$ and optimum offline solution on an instance $I$, respectively. 
	For randomized multi-stage algorithms, we abuse the notation and $\ALG(I)$ denotes the expected total weight of the algorithm on an instance $I$.
\end{definition}

 As an important note, we are mainly interested in the competitive ratio of fractional $K$-stage algorithms.
%  We also consider the asymptotic competitive ratio of integral $K$-stage algorithms (possibly randomized) under the ``large budgets assumption'' in the vertex weighted b-matching problem (i.e., under the assumption that $\min_j B_j=\Omega(1)$), or equivalently under the small bid over budget assumption in the budgeted allocation problem (i.e., under the assumption that $\max_{i,j} \frac{b_{ij}}{B_j}=o(1)$ or equivalently $\min_j B_j=\Omega(1)$ when $b_{ij}\in[0,1]$). 

\subsection{A Recursive Sequence of Polynomials}
As a novel technical ingredient of our proposed multi-stage allocation algorithms, we identify a particular sequence of polynomials of decreasing degrees. Our construction of these polynomials is recursive, which gives us a polynomial of degree $K-k$ for each stage $k=1,2,\ldots,K-1$. Here, we introduce these polynomials, describe this underlying recursive equation, and elaborate a bit more on some of their properties (\Cref{prop:poly}, proof in Appendxi~\ref{apx:poly}). Later, we first show in \Cref{sec:vertex-weight} how these polynomials help us to design an optimal competitive multi-stage algorithm for the vertex weighted matching and how to develop a primal-dual analysis framework that incorporates this recursive equation. Then we show how to extend these ideas to use our polynomials for the vertex weighted b-matching (\Cref{sec:weighted b-matching}) and budgeted allocation (\Cref{sec:adwords}) problems.

\begin{proposition}[{\textbf{{Sequence of Polynomial Regularizers}}}]
\label{prop:poly}
Consider a sequence of functions $f_1,f_2,\ldots,f_{K}:[0,1]\rightarrow[0,1]$
satisfying the following backward recursive equation:
\begin{itemize}
    \item $\forall x\in[0,1]:~f_{K}(x)=\mathbb{I}\{{x=1\}}$,
    where $\mathbb{I}(\cdot)$ is 
    the indicator function,
    \item $\forall x\in[0,1], k\in[K-1]:~f_{k}(x)=\underset{y\in[0,1-x]}{\max}~(1-y)f_{k+1}(x+y)$.
\end{itemize}
Then, the following statements hold:
\begin{enumerate}[label=(\roman*)]
    \item The function sequence $\{f_k\}_{k=1}^{K-1}$ is a sequence of $K-1$ polynomials with decreasing degrees, where $f_k(x)=(1-\frac{1-x}{K-k})^{K-k}$ for $k\in[K-1]$.\footnote{As a convention, we refer to $f_K(x)=\mathbb{I}\{x=1\}$ as a polynomial of degree $0$ (although not mathematically rigorous).}
    \item $f_k(x)$ is monotone increasing and continuous over $[0,1]$ for $k\in[K-1]$. Hence, $F_k(x)\triangleq \int_{0}^x f_k(y)dy$ is differentiable and strictly convex over $[0,1]$ for $k\in[K-1]$.
    \item $\forall k\in[K]$, $f_k(x)\leq e^{x-1}$ for $x\in[0,1]$. Moreover, the first function $f_1(x)=(1-\frac{1-x}{K-1})^{K-1}$ converges point-wise from below to the function $e^{x-1}$ as $K\to+\infty$ (see \Cref{fig:poly}).
    \item $\underset{y\in[0,1]}{\min}1-(1-y)f_1(y)=\cratioexp\triangleq\cratio{K}$
\end{enumerate}
\end{proposition}

The aforementioned polynomials $\{f_k\}_{k\in[K-1]}$ are drawn in \Cref{fig:poly}. As it is clear from this figure, these polynomials provide careful point-wise estimations for the exponential function $f(x)=e^{x-1}$ at different levels of precision. When these polynomials are used to regularize the maximum weight matching objective function, they provide different levels of ``hedging'' intensity against the future uncertainty in the arriving input exactly because of these different levels of estimation precision. This point will be clear in the next section.

\subsection{Extension Model: Multi-stage Configuration Allocation}
Motivated by the application of allocating video-ads,
this paper also considers the following
multi-stage configuration allocation problem.
It generalizes our baseline model.

There is a set of (offline) 
advertisers\footnote{Since 
the multi-stage configuration allocation problem
is motivated by the application of allocating video-ads,
we rename online demand vertices
(resp.\ offline supply vertices) in multi-stage vertex weighted matching 
as 
online users
(resp.\ offline advertisers) in this extension model.} 
$\Driver$.
Advertisers  
are willing to pay a video platform
to display their ads to a set of users $\Rider$ who are streaming videos in this platform.
% When a user
% start watching a video, 
% the video platform can allocate 
% impressions (i.e., exposure of a user 
% to a display ad) to advertisers.
% Specifically, we consider
% a \emph{multi-stage} arrival model, 
% in which users in $\Rider$
% arrive in $K\in\N$ stages.
% At each stage $k\in [K]$,
% a new subset of online users $\Rider_k\subseteq\Rider$
% arrives to the video platform.
Specifically, 
the video platform needs to determine
an advertising \emph{configuration} $\config\in\Config$
for each user (or equivalently, for each video session watched by a user), where $\Config$ is the set of feasible configurations.\footnote{Our model and results allow a different feasible set for each user, but we omit that for simplicity.} Fixing a user $\rider\in \Rider$,
each configuration $\config\in\Config$ 
specifies a certain number of reserved impressions 
$\alloc_{\threeindex}\in\mathbb{Z}_{\geq 0}$
and a per-impression price $\weight_{\threeindex}\in\mathbb{R}_{\geq 0}$
for each advertiser $\driver\in\Driver$.
% advertiser $\driver$'s impression 
% have been displayed to user $\rider$
% with per-unit price $\weight_{\threeindex}$.
Each advertiser $\driver$
demands $n_\driver\in\mathbb{Z}_{\geq 0}$ number of impressions in total
and is only willing to pay for 
at most that many impressions to
the video platform.
Users 
arrive at the video platform over time
in $K\in\N$ stages. At each stage $k\in [K]$,
a new subset of online users $\Rider_k\subseteq\Rider$
arrives at the video platform. Upon this arrival, the video platform observes $\Rider_k$, as well as 
$\allocs\ked = \{\alloci\}_{\rider\in\Rider_k,\config\in\Config,\driver\in \Driver}$
and 
$\weightbf\ked = \{\weight_{\threeindex}\}_{\rider\in\Rider_k,\config\in\Config,\driver\in \Driver}$.
We highlight that 
$\{\Rider_k\}_{k\in[K]}$
are disjoint and $\cup_{k\in[K]}\Rider_k = \Rider$. 


Our goal as the video platform is to design 
a multi-stage algorithm $\ALG$
for assigning configurations to the users in a stage-by-stage fashion as they arrive. Upon arrival of users $\Rider_k$ 
in stage $k\in [K]$,
$\ALG$ makes an 
irrevocable decision by
assigning a configuration 
to each user $\rider\in\Rider_k$. As we mentioned above, the assigned configuration of each user specifies 
the number of impressions and per-impression prices 
for each of the advertisers. 
These configuration decisions can be integral or fractional. 
In this paper we focus on the fractional allocations.\footnote{\label{footnote:integral}Using standard randomized rounding techniques, all of our results for the fractional allocation problem, including the algorithm and its competitive analysis, can easily be extended to the setting with integral randomized allocations under the \emph{large budget assumptions}, i.e, in the asymptotic regime when $\underset{i,c,j}{\min}\frac{n_j}{\alloci}$ is large.}
At the end of $K$ stages, given the assigned configurations by $\ALG$,  each advertiser only pays for 
at most $n_\driver$ number of allocated impressions in total. Moreover, they pay for an impression based on its per-impression price specified by the assigned configuration of the corresponding user. The goal of the algorithm is to maximize the total revenue collected at the end of $K$ stages.

\vspace{3mm}
\noindent\textbf{LP Formulation and Offline Benchmark}~~To help with understanding our extension model, we formulate the
optimum offline solution in
the configuration allocation
problem as a simple linear program, denoted by  
\ref{eq:LP primal}:
    \begin{equation}
\tag{\textsc{OFFLINE-OPT}}
\label{eq:LP primal}
\arraycolsep=1.4pt\def\arraystretch{1}
\begin{array}{lllll}
\max\limits_{\xbf,\zbf\geq \mathbf{0}}
\quad\quad\quad&
% \mathop{\displaystyle\sum
\displaystyle\sum_{\rider\in\Rider}
\displaystyle\sum_{\config\in\Config}
\displaystyle\sum_{\driver\in\Driver}
\weight_{\threeindex}\cdot
% }
% \limits_{(\threeindex)\in E}
 x_{\threeindex}
&~~\text{s.t.}
% \min\limits_{\alphabf,\betabf,\gammabf}
% \quad\quad\quad 
% &
% \displaystyle\sum_{\rider\in \Rider }{\alpha_\rider}+
% \displaystyle\sum_{\driver\in \Driver}{\beta_\driver}
% &~~\text{s.t.} 
\\[1.4em]
 &
%  \mathop{\displaystyle\sum
\displaystyle\sum_{\rider\in\Rider}
\displaystyle\sum_{\config\in\Config}
 x_{\threeindex} 
%  }
%  \limits_{\rider,\config:(\threeindex)\in E}
 \leq
 n_{\driver} 
 &~~\driver\in\Driver~,
% \gamma_{\threeindex} 
% +
% \beta_\driver \geq \weight_{\threeindex}
% & (\threeindex)\in E~,
\\[1.4em]
 &
 \displaystyle\sum\limits_{\config\in\Config}
 z_{\rider,\config}
 \leq 1 
 &~~
 \rider\in \Rider~, 
% \alpha_\rider 
% \geq 
% \displaystyle\sum\limits_{\driver\in \Driver}
% \alloci\cdot \gamma_{\threeindex} &i\in \Rider, \config\in \Config~, 
\\[1.4em]
 &
 x_{\threeindex} \leq 
 \alloci \cdot z_{\rider,\config}
 &~~
\rider\in\Rider,\config\in\Config,\driver\in\Driver~. 
% \alpha_\rider 
% \geq 0 &\rider \in \Rider~, 
% \\[1.4em]
%  &x_{\threeindex} \geq 0 &(\threeindex)\in E~, &
% & &
% \beta_\driver\geq 0  &\driver\in \Driver~,
% \\[1.4em]
%  &z_{\rider,\config} \geq 0 &\rider\in\Rider, \config\in \Config~. &
% & &
% \gamma_{\threeindex} \geq 0  &(\threeindex)\in E~.
\end{array}
\end{equation}
In the above formulation, $z_{\rider,\config}$
is the fraction of configuration $\config$ allocated
to user $\rider$,
and $x_{\threeindex}$
is the (fractional) number of impressions
created by user $\rider$ for advertiser $\driver$ based on configuration $\config$ that the advertiser is finally willing to pay. Note that the number $x_{\threeindex}$ of impressions that the advertiser is willing to pay is no more than number of allocated impressions $\alloci \cdot z_{\rider,\config}$ from user $\rider$ under configuration $\config$, and the first quantity can be strictly smaller than the second (as advertiser $\driver$ should only pay for at most $n_\driver$ impressions overall). If an impression is allocated but the advertiser is not responsible to pay for it, we refer to that impression as being \emph{preempted} or \emph{freely disposed}. 


\vspace{3mm}
\noindent\textbf{Connection to Baseline Model}~~As we mentioned above,
the multi-stage configuration allocation 
generalizes the multi-stage vertex weighted matching.
In particular, 
every instance in the vertex weighted matching 
can be thought as an
instance in configuration allocation as follows:
Each advertiser $\driver$ has a unit demand 
($n_\driver = 1$).
The feasible configuration set encodes 
all edges $E$ in baseline model
($\Config = E$).
More specifically, for every 
edge $(\rider\primed,\driver\primed)\in E$,
the corresponding
configuration $\config$ 
encodes the 
number of reserved impression $\{\alloci\}_{\rider,\driver}$
as 
$\alloci =\indicator{\rider = \rider\primed,
\driver = \driver\primed}$.
The 
per-impression price are identical for each advertiser
($\weight_{\threeindex} = \weight_{\rider',\config',\driver}$
for all $\rider,\rider',\config,\config'$).
Finally, note that
since per-impression price are identical for each advertiser
and number of reserved impression $\{\alloci\}$
is encoded as the aforementioned indicator function,
without loss of generality, 
we can restrict attention to online algorithms 
whose allocations never exceed demand $\{n_\driver\}$
of advertisers, and thus
no
preemption or free disposal is needed.


==> FN_ multi-stage matching + configuration allocation (MS Journal)/tex/prelim_older.tex <==
\section{Preliminaries}
\label{sec:prelim}
\smallskip
\noindent{\textbf{Model and Notation~}}
We consider a general bipartite allocation model for matching arriving demand requests to available suppliers. An instance of our model consists of a bipartite graph $\mathcal{G}=(\Rider,\Driver,E)$, where vertices in $\Driver$ (supply) are available offline and vertices in $\Rider$ (demand) arrive over time. Specifically, we consider a \emph{multi-stage arrival} model, in which vertices in $\Rider$ arrive in $K\in\mathbb{N}$ stage. We assume the number of stages $K$ is fixed and known by the algorithm. At each stage $k\in[K]$, a new subset of online vertices $\Rider_k\subseteq \Rider$ arrive, which we often call an arriving \emph{batch}, and reveal their incident edges in $E$. We highlight that $\Rider=\cup_{k\in[K]}\Rider_k $ and $\Rider_k\cap\Rider_{k'}=\emptyset$ for $k\neq k'$. After arrival of batch $k$, the multi-stage allocation algorithm makes an irrevocable allocation decision by allocating each vertex $i\in\Rider_K$ (which corresponds to one unit of demand) to the set of \emph{available} neighboring offline vertices $j\in\Driver, (i,j)\in E$ . Let $E_k$ denote the set of edges in $E$ incident to $\Rider_k$. We denote the allocation of stage $k$ by the vector $\mathbf{x}_{k}\in\mathbb{R}^{E_k}$, where $x_{k,ij}\in[0,1]$ is the amount of allocation of vertex $i$ to $j$. This allocation can be fractional or integral. 

The goal of the multi-stage allocation algorithm is to maximize the ``weight" of the final allocation after all batches arrive, while ensuring the \emph{feasibility constraints} on the offline side. The objective function and the feasibility constraints are specific to the choice of the problem as follows:
\begin{enumerate}[label=\textit{(\roman*)}]
\smallskip
    \item \underline{Multi-stage vertex weighted b-matching}: each offline vertex $j\in\Driver$ has a capacity constraint $B_j$, that is, the total (fractional) allocation amount at this vertex cannot exceed $B_j$. It also has a non-negative weight $w_j$ for each unit of allocation. The objective function is the sum of the weight of the offline vertices in the (fractional) allocation. We also consider the special case of \emph{multi-stage vertex weighted matching}, in which $B_j=1$ for all $j\in\Driver$.
    \smallskip
    \item\underline{Multi-stage budgeted allocation (AdWords)}:  each edge $(i,j)\in E$ has a non-negative weight $b_{ij}$ for each unit of allocation on this edge. Without loss of generality, we assume $b_{ij}\in[0,1]$.\footnote{This assumption is just for simplicity, as it helps with making the large budget assumption in vertex weighted b-matching similar to small bid over budget assumption in the budgeted allocation problem.} Each offline vertex $j\in \Driver$ has a budget constraint $B_j$, that is, the sum of the weights of edges incident to $j$ in the (fractional) allocation cannot exceed $B_j$. The objective function is the sum of the weight of all the edges in the (fractional) allocation.\footnote{This model can be interpreted as the multi-stage version of the AdWords problem, in which $V$ is the set of advertisers and $U$ is the set of arriving batched queries. In this application, $b_{ij}$ essentially denotes the bid of advertiser $j$ for query $i$ and $B_j$ is the budget of advertiser $j$.} 
\end{enumerate}

We measure the performance of our multi-stage algorithms by their \emph{competitive ratio}, which is the worst-case ratio between the expected total weight of the algorithm and the optimum offline benchmark given the entire problem instance (formally defined below).
\begin{definition}[\textbf{Competitive Ratio}]
	\label{def:competitive ratio}
	Fix the number of stages $K\in\mathbb{N}$. For $\alpha\in [0,1]$, a multi-stage allocation algorithm $\texttt{ALG}$ is \emph{$\alpha$-competitive} against the optimum offline solution in the multi-stage vertex weighted b-matching problem (resp. multi-stage budgeted allocation/AdWords problem), if the following holds:
	\begin{align*}
		\inf\limits_{I \in\mathcal{I}}~~
		\frac{\texttt{ALG}(I)}{\texttt{OPT}(I)}~
		\geq \alpha~,
	\end{align*}
	where $\mathcal{I}$ is the set of instances of the multi-stage vertex weighted b-matching problem (resp. multi-stage budgeted allocation problem), and $\texttt{ALG}(I)$ and $\texttt{OPT}(I)$ are the total weights of the multi-stage algorithm $\texttt{ALG}$ and optimum offline solution on an instance $I$, respectively. For randomized multi-stage algorithms, we abuse the notation and $\texttt{ALG}(I)$ denotes the expected total weight of the algorithm on an instance $I$.
\end{definition}

 As an important note, we are mainly interested in the competitive ratio of fractional $K$-stage algorithms. We also consider the asymptotic competitive ratio of integral $K$-stage algorithms (possibly randomized) under the ``large budgets assumption'' in the vertex weighted b-matching problem (i.e., under the assumption that $\min_j B_j=\Omega(1)$), or equivalently under the small bid over budget assumption in the budgeted allocation problem (i.e., under the assumption that $\max_{i,j} \frac{b_{ij}}{B_j}=o(1)$ or equivalently $\min_j B_j=\Omega(1)$ when $b_{ij}\in[0,1]$). 


\smallskip
\noindent{\textbf{A Recursive Sequence of Polynomials~}} As a novel technical ingredient of our proposed multi-stage allocation algorithms, we identify a particular sequence of polynomials of decreasing degrees. Our construction of these polynomials is recursive, which gives us a polynomial of degree $K-k$ for each stage $k=1,2,\ldots,K-1$. Here, we introduce these polynomials, describe this underlying recursive equation, and elaborate a bit more on some of their properties (\Cref{prop:poly}, proof in Appendxi~\ref{apx:poly}). Later, we first show in \Cref{sec:vertex-weight} how these polynomials help us to design an optimal competitive multi-stage algorithm for the vertex weighted matching and how to develop a primal-dual analysis framework that incorporates this recursive equation. Then we show how to extend these ideas to use our polynomials for the vertex weighted b-matching (\Cref{sec:weighted b-matching}) and budgeted allocation (\Cref{sec:adwords}) problems.

\begin{proposition}[{\textbf{{Sequence of Polynomial Regularizers}}}]
\label{prop:poly}
Consider a sequence of functions $f_1,f_2,\ldots,f_{K}:[0,1]\rightarrow[0,1]$
satisfying the following backward recursive equation:
\begin{itemize}
    \item $\forall x\in[0,1]:~f_{K}(x)=\mathbb{I}\{{x=1\}}$,
    where $\mathbb{I}(\cdot)$ is 
    the indicator function,
    \item $\forall x\in[0,1], k\in[K-1]:~f_{k}(x)=\underset{y\in[0,1-x]}{\max}~(1-y)f_{k+1}(x+y)$.
\end{itemize}
Then, the following statements hold:
\begin{enumerate}[label=(\roman*)]
    \item The function sequence $\{f_k\}_{k=1}^{K-1}$ is a sequence of $K-1$ polynomials with decreasing degrees, where $f_k(x)=(1-\frac{1-x}{K-k})^{K-k}$ for $k\in[K-1]$.\footnote{As a convention, we refer to $f_K(x)=\mathbb{I}\{x=1\}$ as a polynomial of degree $0$ (although not mathematically rigorous).}
    \item $f_k(x)$ is monotone increasing and continuous over $[0,1]$ for $k\in[K-1]$. Hence, $F_k(x)\triangleq \int_{0}^x f_k(y)dy$ is differentiable and strictly convex over $[0,1]$ for $k\in[K-1]$.
    \item $\forall k\in[K]$, $f_k(x)\leq e^{x-1}$ for $x\in[0,1]$. Moreover, the first function $f_1(x)=(1-\frac{1-x}{K-1})^{K-1}$ converges point-wise from below to the function $e^{x-1}$ as $K\to+\infty$ (see \Cref{fig:poly}).
    \item $\underset{y\in[0,1]}{\min}1-(1-y)f_1(y)=\cratioexp\triangleq\cratio{K}$
\end{enumerate}
\end{proposition}

We conclude this section by reminding the reader that the above polynomials $\{f_k\}_{k\in[K-1]}$ are drawn in \Cref{fig:poly}. As it is clear from this figure, these polynomials provide careful point-wise estimations for the exponential function $f(x)=e^{x-1}$ at different levels of precision. When these polynomials are used to regularize the maximum weight matching objective function, they provide different levels of ``hedging'' intensity against the future uncertainty in the arriving input exactly because of these different levels of estimation precision. This point will be clear in the next section.

==> FN_ multi-stage matching + configuration allocation (MS Journal)/tex/result-table.tex <==
\begin{table}[htb]
\small\addtolength{\tabcolsep}{-2pt}
\caption{Comparing our results to previous work}
\vspace{1mm}
\label{tab:summary}
%  	\smallskip
%\renewcommand{\thefootnote}{\fnsymbol{footnote}}
%\renewcommand*{\thefootnote}{\arabic{footnote}}

\renewcommand{\thefootnote}{\ifcase\value{footnote}\or(\textasteriskcentered)\or(\textdagger)\or(\textdagger)\or(\textdaggerdbl)\or(\textsection)\or(\textbardbl)\or(\textdollar)\or(\textdollar\textdollar)\or(\pounds)\or(\texteuro)\or(\#\#\#)\or(\#\#\#\#)\or($\infty$)\fi}
 	\footnotesize
\center
 	
% \begin{tabular}{|c|c|c|c|c|c|}
%     \cline{2-6}
%     \multicolumn{1}{c|}{}
%     &    	
%     \begin{minipage}{0.2\textwidth}
%  		{\begin{center}
%     \vspace{3pt}
%  			$K$-stage \\
%  			vertex weighted \\
%  			matching (\Cref{sec:vertex-weight})
%     \vspace{3pt}
%     \end{center}
%  		}
%  		\end{minipage}
%     & 
%         \multicolumn{2}{c|}{
%         \begin{minipage}{0.25\textwidth}
%  		{\begin{center}
%     \vspace{3pt}
%  			$K$-stage \\
%  			vertex weighted \\
%  			b-matching (\Cref{sec:weighted b-matching})
%     \vspace{3pt}
%     \end{center}
%  		}
%  		\end{minipage}
%  		}
%     & 
%     \multicolumn{2}{c|}{
%         \begin{minipage}{0.25\textwidth}
%  		{\begin{center}
%     \vspace{3pt}
%  			$K$-stage 
%  			AdWords \\
%  			(\Cref{sec:adwords})
%     \vspace{3pt}
%     \end{center}
%  		}
%  		\end{minipage}
%  		}
%     \\
%     \cline{2-6}
%     \multicolumn{1}{c|}{}
%     &
%     fractional & 
%     fractional & 
%             \begin{minipage}{0.12\textwidth}
%  		{\begin{center}
%     \vspace{3pt}
%  			integral,\\
%  			deterministic,\\
%  			($B\rightarrow +\infty$)
%     \vspace{3pt}
%     \end{center}
%  		}
%  		\end{minipage}
%     &
%     fractional &
%             \begin{minipage}{0.12\textwidth}
%  		{\begin{center}
%     \vspace{3pt}
%  			integral,\\
%  			randomized,\\
%  			($B\rightarrow +\infty$)
%     \vspace{3pt}
%     \end{center}
%  		}
%  		\end{minipage}
%     \\
%     \hline
%   	\begin{minipage}{0.2\textwidth}
%  		{\begin{center}
%     \vspace{3pt}
%  			Lower-bound \\
%  			(previous work)
%     \vspace{3pt}
%     \end{center}
%  		}
%  		\end{minipage}
%     &$1-\frac{1}{e}$ &$1-\frac{1}{e}$
%     &$1-\frac{1}{e}$
%     &$1-\frac{1}{e}$&$1-\frac{1}{e}$\\
%     \hline
%   	\begin{minipage}{0.2\textwidth}
%  		{\begin{center}
%     \vspace{3pt}
%  			Lower-bound \\
%  			(this work)
%     \vspace{3pt}
%     \end{center}
%  		}
%  		\end{minipage}
%     &\multicolumn{5}{c|}{
%     $\cratioexp
%     \xrightarrow{K\rightarrow+\infty}
%     1 - \frac{1}{e}$
%     }\\
%     \hline
%   	\begin{minipage}{0.2\textwidth}
%  		{\begin{center}
%     \vspace{3pt}
%  			Upper-bound \\
%  			(this work)
%     \vspace{3pt}
%     \end{center}
%  		}
%  		\end{minipage}
%     &\multicolumn{5}{c|}{
%         $\cratioexp
%     \xrightarrow{K\rightarrow+\infty}
%     1 - \frac{1}{e}$
%     }\\
%     \hline
% \end{tabular}
\begin{tabular}{|c|c|c|c|c|}
    \cline{2-5}
    \multicolumn{1}{c|}{}
    &    	
    
        \multicolumn{2}{c|}{
        \begin{minipage}{0.37\textwidth}
 		{\begin{center}
    \vspace{3pt}
 			$K$-stage vertex weighted b-matching\\
 			(\Cref{sec:vertex-weight} and \Cref{sec:weighted b-matching})
    \vspace{3pt}
    \end{center}
 		}
 		\end{minipage}
 		}
    & 
    \multicolumn{2}{c|}{
        \begin{minipage}{0.25\textwidth}
 		{\begin{center}
    \vspace{3pt}
 			$K$-stage 
 			AdWords \\
 			(\Cref{sec:adwords})
    \vspace{3pt}
    \end{center}
 		}
 		\end{minipage}
 		}
    \\
    \cline{2-5}
    \multicolumn{1}{c|}{}
    &
     
    fractional & 
            \begin{minipage}{0.12\textwidth}
 		{\begin{center}
    \vspace{3pt}
 			integral
    \vspace{3pt}
    \end{center}
 		}
 		\end{minipage}
    &
    fractional &
            \begin{minipage}{0.12\textwidth}
 		{\begin{center}
    \vspace{3pt}
 			integral
 			
    \vspace{3pt}
    \end{center}
 		}
 		\end{minipage}
    \\
    \hline
   	\begin{minipage}{0.2\textwidth}
 		{\begin{center}
    \vspace{3pt}
 			Lower-bound \\
 			\emph{(previous work)}
    \vspace{3pt}
    \end{center}
 		}
 		\end{minipage}
    &$1-\frac{1}{e}$\footnotemark[1]
    &$1-\frac{1}{e}-O\left(\frac{1}{B_{\textrm{min}}}\right)$\footnotemark[1]
    % \RN{can you check the bounds in this row? I haven't double checked them}
    &$1-\frac{1}{e}$\footnotemark[2]&$1-\frac{1}{e}-O\left(\frac{1}{B_{\textrm{min}}}\right)$\footnotemark[2]\\
    \hline
   	\begin{minipage}{0.2\textwidth}
 		{\begin{center}
    \vspace{3pt}
 			Lower-bound \\
 			\textbf{\emph{(this work)}}
    \vspace{3pt}
    \end{center}
 		}
 		\end{minipage}
    &$\cratioexp$
    &$\cratioexp-O\left(\frac{1}{B_{\textrm{min}}}\right)$
    &$\cratioexp$&$\cratioexp-O\left(\sqrt{\frac{\log(B_{\text{min}})}{{{B_{\text{min}}}}}}\right)$\\
    \hline
   	\begin{minipage}{0.2\textwidth}
 		{\begin{center}
    \vspace{3pt}
 			Upper-bound \\
 			\textbf{\emph{(this work)}}
    \vspace{3pt}
    \end{center}
 		}
 		\end{minipage}
    &  \multicolumn{2}{c|}{$\cratioexp$}
    &\multicolumn{2}{c|}{$\cratioexp$}\\
    \hline
\end{tabular}

 	\smallskip
\noindent\par

 	\begin{minipage}{0.65\textwidth}
 		{
 			\footnotesize
 			\footnotemark[1]~{\cite{AGKM-11}};~ 
 			\footnotemark[2]~{\cite{MSVV-07,BJN-07}};
 		}
 	\end{minipage}
 \end{table}

==> FN_ multi-stage matching + configuration allocation (MS Journal)/tex/tem.tex <==
\begin{proof}[Proof of \Cref{thm:b-matching}]

For each stage $k\in[1:K-1]$, let $\{(\Rider^{(0)}_k, \Driver^{(0)}_k),\dots, (\Rider^{(L_k)}_k, \Driver^{(L_k)}_k)\}$ be the 
structural decomposition of $(\Rider_k, D, E_k)$ as in \Cref{lemma:structure},
and $\{x_{k, ij}^*\}_{(i,j)\in E_k}$
be the optimal solution of the program~\ref{eq:concave-k-bmatching}. First, we define the following notations which will be useful in this proof:
\begin{align*}
\forall j\in \Driver,~k\in[K]:\quad\quad\quad &y^*_{k,j}\triangleq\sum_{s=1}^{k-1}\sum_{i:(i,j)\in E_s}x^*_{s,ij}
% ,\\
%  &y^*_{0,j}=0.
\end{align*}
Now, consider the offline primal-dual linear programs in \ref{eq:LP-max-weight}. Given the feasible primal assignment $\{\xbf^*_{k}\}_{k\in[K]}$, construct a dual assignment as follows. 
First, set $\alpha_i\gets 0$ and $\beta_j\gets 0$ for all $i\in\Rider,j\in \Driver$. At each stage $k\in[0:K-1]$, update the dual variables as follows:
\begin{align*}
   &\forall i \in \Rider^{(l)}_k,~l\in[0:L_k]: &&\alpha_i\gets c^{(l)}_k
   \\
    &\forall j \in \Driver^{(l)},~l\in[0:L_k]: &&\beta_{j}\gets\beta_{j}+\Delta\beta_{k,j}\\
    &&&\Delta\beta_{k,j}\triangleq \left(
\sum_{i:(i,j)\in E_k}x_{k,ij}^* \right)\cdot \left(w_j - c_k^{(l)}\right)\overset{(1)}{=}w_j(y^*_{k+1,j}-y^*_{k,j})f_k(y^*_{k+1,j})
\end{align*}
where in eq.~(1) above 
% \YF{label eq.~(1) is not defined in our paper}
we use the uniformity property and the definition of $c^{(l)}_k$ in \Cref{lemma:structure}. For the last stage $K$, note that $F_K(x)=0$. Therefore, \Cref{alg:b-matching} essentially solves the maximum vertex weighted matching in the last stage graph $(\Rider_K, \Driver, E_K)$ where each $j\in\Driver$ has initial capacity $1-y^*_{K, j}$. Let $\{\hat{\alpha}_{K,i}, \hat{\beta}_{K,j}\}_{i\in\Rider_K,j\in\Driver}$ 
be the \emph{optimal} dual solution of this LP. Then update the  dual variables as follows:
\begin{align*}
&\forall i\in\Rider_K:~~\alpha_i \gets \hat{\alpha}_{K,i} \\
&\forall j\in \Driver~:~~\beta_j\gets \beta_j+\Delta \beta_{K,j},~~\Delta\beta_{K, j} \triangleq (1 - y^*_{K, j})\hat{\beta}_{K,j}
\end{align*}



% Consider the following construction of dual solution.
% At stage $k < K$, let 
% $\bar f_k(x) \triangleq f_{K - k}(x) = \left(
% \frac{K - k - 1 + x}{K-k}
% \right)^{K-k}$, and 
% $\{(\Rider^{(0)}_k, \Driver^{(0)}_k),\dots, (\Rider^{(L)}_k, \Driver^{(L)}_k)\}$ be the 
% partition of $(\Rider_k, D, E_k)$ in \Cref{lemma:structure},
% and 
% $\{x_{k, ij}^*\}_{(i,j)\in E_k}$
% be the optimal solution  
% from the concave program~\eqref{eq:concave program k}
% solved by BWF.
% Construct the dual solution as follows,
% for any $k < K$ 
% \begin{align*}
%     \alpha_i &= c^{(l)}_k
%     \qquad \forall i \in \Rider^{(l)}_k \\
%     \Delta \beta_{k,j} &= \left(
%     % 1 - 
%     \sum_{i\in N_k(j)}x_{k,ij}^*
%     % - y_{k,j}
%     \right)\cdot 
%     \left(w_j - c_k^{(l)}\right)
%     \qquad \forall j \in \Driver^{(l)}
% \end{align*}
% where $N_k(j)$ denotes all neighbor vertices of item $j$
% in graph $(\Rider_k, D, E_k)$ at stage $k$.
The rest of the proof is done in two steps:
\vspace{1mm}

\noindent[\textit{Step \rom{1}}]~\emph{Comparing objective values in primal and dual.}
we first show that 
the objective value of the above dual assignment
is equal to the objective value of the primal assignment of \Cref{alg:b-matching}.
To show this, we consider 
each stage $k$ separately.
For the last stage $K$, 
this holds by construction.
For each stage $k < K$, note that the primal objective value is decomposed across pairs $(\Rider_k^{(l)}, \Driver_k^{(l)})$, $l=0,1,\ldots,L_k$, simply because $x^*_{k,ij}>0$ only if $i$ and $j$ belong to the same pair (\Cref{lemma:structure}). As these pairs partition sets of vertices $\Rider$ and $\Driver$, it is enough to compare the changes in the primal and dual objectives in each pair $(\Rider_k^{(l)}, \Driver_k^{(l)})$ separately. Notice that if $l = 0$ then $c^{(l)}_k = 0$, and thus,
\begin{align*}
    \Delta(\textrm{Dual})^{(0)}\triangleq\sum_{i \in \Rider^{(0)}_k} \alpha_i
    +
    \sum_{j \in \Driver^{(0)}_k} \Delta\beta_{k,j}
    &= 
    \sum_{j \in \Driver^{(0)}_k}\sum_{i:(i,j)\in E_0} w_jx_{k, ij}^*\triangleq\Delta(\textrm{Primal})^{(0)}. 
\end{align*}
Similarly, for $l \geq 1$, 
\begin{align*}
     \Delta(\textrm{Dual})^{(l)}&\triangleq\sum_{i \in \Rider^{(l)}_k} \alpha_i
    +
    \sum_{j \in \Driver^{(l)}_k} \Delta\beta_{k,j}
    =
    |\Rider^{(l)}_k|\cdot c^{(l)}_k
    +
    \sum_{j \in \Driver^{(l)}_k}\sum_ {i:(i,j)\in E_k} 
    x_{k, ij}^*\left(w_j - c^{(l)}_k\right)\\
    &= 
     |\Rider^{(l)}_k|\cdot c^{(l)}_k+\sum_{j\in\Driver_k^{(l)}}\sum_{i:(i,j)\in E_k} 
    w_jx_{k, ij}^*-c^{(l)}_k\sum_{i\in\Rider_k}\left(\sum_{j:(i,j)\in E}x^*_{k,ij}\right)\\
    &=\sum_{j\in\Driver_k^{(l)}}\sum_{i:(i,j)\in E_k} 
    w_jx_{k, ij}^*\triangleq \Delta(\textrm{Primal})^{(l)},
\end{align*}
where the last equality uses the saturation property in \Cref{lemma:structure} for $l\geq 1$.
\vspace{1mm}

\noindent[\textit{Step \rom{2}}]~\emph{Checking approximate feasibility of dual.} To show approximate dual feasibility, it is enough to show that for any stage $k\in[K]$ and any arbitrary edge $(i, j) \in E_k$,
\begin{align}
\label{eq:dual constraint feasibility}
    \alpha_i + \sum_{s = 1}^k\Delta\beta_{s, j}
    \geq 
    w_j\left(1-(1-1/K)^K\right)
\end{align}
We next show \eqref{eq:dual constraint feasibility}
holds for $k=1,2,\ldots,K-1$ by using the following technical lemma, which carefully uses our sequence of polynomial regularizers to establish a lower bound on the LHS of \eqref{eq:dual constraint feasibility}.

  \begin{lemma}
    \label{lem:polynomial inequality 2}
    For any $K \in \N,~1\leq k \leq K - 1$, any $x \in [0, 1]$, and
    any $0 = y_1 \leq 
    y_2 \leq \dots \leq y_k \leq  1 - x$,
    \begin{align*}
     (1-x)f_{k}(y_k + x) -
    \sum_{s = 1}^{k - 1} 
    (y_{s + 1} - y_s)
    f_{s}(y_{s + 1})
     \leq 1-\cratio{K}=
    (1-1/K)^K.
    \end{align*}
    \end{lemma}
Now assume $i \in \Rider_k^{(l)}$ and $j \in \Driver_k^{(l')}$, which implies $c^{(l')}_k \leq c^{(l)}_k$ (thanks to \Cref{lemma:structure}). Then we have:
\begin{align*}
     \alpha_i + \sum_{s = 1}^{k}\Delta\beta_{s, j}&=c_k^{(l)} + 
    \left(\sum_{i':(i',j)\in E_k}x_{k, i'j}^*\right)
    \left(w_j - c_k^{(l')}\right)
    +
    \sum_{s= 1}^{k - 1} \Delta\beta_{s, j} \\
    &\geq c_k^{(l')} + 
    \left(\sum_{i':(i',j)\in E_k}x_{k, i'j}^*\right)
    \left(w_j - c_k^{(l')}\right)
    +
    \sum_{s= 1}^{k - 1} \Delta\beta_{s, j} \\
    &=w_j\left(1-f_k\left(y^*_{k,j}+\sum_{i':(i',j)\in E_k}x_{k, i'j}^*\right)+\left(\sum_{i':(i',j)\in E_k}x_{k, i'j}^*\right)f_k\left(y^*_{k,j}+\sum_{i':(i',j)\in E_k}x_{k, i'j}^*\right)\right)\\
    &+ \sum_{s= 1}^{k - 1} \Delta\beta_{s, j} \\
    &=w_j\left(1-\left(1-\sum_{i':(i',j)\in E_k}x_{k, i'j}^*\right)f_k\left(y^*_{k,j}+\sum_{i':(i',j)\in E_k}x_{k, i'j}^*\right)+\sum_{s=1}^{k-1}\left(y^*_{s+1,j}-y^*_{s,j}\right)f_k\left(y^*_{s+1,j}\right)\right)\\
    &\geq w_j \cratio{K}~,
\end{align*}
where the first inequality uses $c^{(l')}_k \leq c^{(l)}_k$, the second equality uses the expression for $c^{(l')}_k$ in \Cref{lemma:structure} due to uniformity, and the last inequality invokes \Cref{lem:polynomial inequality 2} for the sequence: 
$$
0=y^*_{1,j}\leq y^*_{2,j}\leq \ldots \leq y^*_{k,j}\leq 1-\sum_{i':(i',j)\in E_k}x_{k, i'j}^*~.
$$
% \begin{align*}
%      & c_k^{(l)} + 
%     \left(\sum_{i'\in N_k(j)}x_{k, i'j}^*\right)
%     \left(w_j - c_k^{(l)}\right)
%     +
%     \sum_{s' = 1}^{k - 1} \Delta\beta_{s', j} \\
%     &\leq 
%     c_k^{(l')} + 
%     \left(\sum_{i'\in N_k(j)}x_{k, i'j}^*\right)
%     \left(w_j - c_k^{(l)}\right)
%     +
%     \sum_{s' = 1}^{k - 1} \Delta\beta_{s', j} \\
%     &=
%     \alpha_i + \sum_{s' = 1}^{k}\Delta\beta_{s', j}
% \end{align*}

So far, we have shown \eqref{eq:dual constraint feasibility} holds for all stages $k < K$.
For the last stage $K$, and any edge $(i, j) \in E_K$,
notice that 
$\alpha_i+\Delta\beta_{K, j}=\hat{\alpha}_{K,i} + \Delta\beta_{K, j} \geq 
w_j(1 - y^*_{K, j})$ by construction.
If $y^*_{K, j} = 0$, inequality \eqref{eq:dual constraint feasibility} holds. Otherwise, let $s^\dagger < K$ be the largest 
stage smaller than $K$ 
where 
there exists $l^\dagger$ 
such that 
$j \in \Driver_{s^\dagger}^{(l^\dagger)}$ and 
$\Delta\beta_{s^\dagger,j} > 0$. By definition, we know that 
$y^*_{s^\dagger, j} + \displaystyle\sum_{i':(i',j)\in E_{s^\dagger}}x_{s^\dagger, i'j}^* = y^*_{K,j}$. So we have:
\begin{align*}
    \alpha_i + \sum_{s = 1}^{K}\Delta\beta_{s, j}
    &\geq    
    w_j(1 - y^*_{K, j})
    + \sum_{s = 1}^{K - 1}\Delta\beta_{s, j} = 
    w_j(1 - y^*_{K, j}) + \sum_{s = 1}^{s^\dagger}\Delta\beta_{s, j} \\
    &\geq w_j\left(1 - f_{s^\dagger}(y^*_{K, j})\right) + \sum_{s = 1}^{s^\dagger}\Delta\beta_{s, j} =c^{(l^\dagger)}_{s^\dagger} + \sum_{s = 1}^{s^\dagger}\Delta\beta_{s, j} \\
    &\geq w_j(1 - (1 - 1/K)^K)~,
\end{align*}
where the first equality uses the fact $\Delta\beta_{s, j} = 0$ for all $s$
between $s^\dagger + 1$ and $K - 1$; the first inequality uses the fact that 
that $f_{s}(x) \geq x$ for all $x\in [0, 1]$, the second equality uses the definition of $c^{(l^\dagger)}_{s^\dagger}$ and the fact that $y^*_{s^\dagger, j} + \displaystyle\sum_{i':(i',j)\in E_{s^\dagger}}x_{s^\dagger, i'j}^* = y^*_{K,j}$; and finally the last inequality holds by exactly the same argument as in the case of $k<K$.
\end{proof}

==> FN_ multi-stage matching + configuration allocation (MS Journal)/tex/vertex-weighted.tex <==
\newcommand{\PRMWM}{\texttt{PR-MWM}}
\subsection{Polynomial Regularized Maximum Weight Matching}
\label{sec:upper-bound}







Recall the sequence of polynomials $f_1,f_2,\ldots,f_K$ defined in \Cref{sec:prelim} (see \Cref{prop:poly} and \Cref{fig:poly} for details). We are now ready to describe our main algorithm, which is an optimal competitive multi-stage algorithm for vertex weighted bipartite matching.

\smallskip
\noindent{\textbf{Overview of the Algorithm~}} Given the sequence of polynomials in \Cref{prop:poly}, our algorithm solves a different convex program
at each stage $k\in[K]$, and returns its unique optimal solution as the fractional matching of that stage. 
The program of stage $k$ is essentially a regularized maximum vertex weighted matching considering the current remaining capacity of each offline vertex. In this convex program, the regularization is done by a weighted combination of polynomials $F_k(x)=\int_0^{x}f_k(y)dy$ over offline vertices, each evaluated at the fractional degree of the offline vertex at the end of the allocation. \revcolor{Notably, the convex program at stage $k$ depends on the current state of the allocations, which is captured by the vector of fractional degrees of each offline vertex $j$ at the beginning of stage $k$ denoted by $\mathbf{y}^{(k)}$.} 
See \Cref{alg:b-matching} for a formal description.


\begin{algorithm}[htb]
 	\caption{Polynomial Regularized Max Weight Matching (\PRMWM)}
 	\label{alg:b-matching}
 	\KwIn{Number of batches/stages $K$}
 	    \vspace{2mm}
 	    
    $\forall j\in\Driver:~y^{(0)}_j\gets 0$.

 	\vspace{1mm}
 	\For{stage $k=1$ to $K$}
 	{
 	\vspace{2mm}
 	\tcc{$k^{\textrm{th}}$ batch of vertices in $\Rider$, denoted by $\Rider_k$, arrives. Let $E_k$ denote the set of edges incident to vertices in $\Rider_k$.}
 	\vspace{2mm}
 	
   Given $\mathbf{y}^{(k-1)}$ and subgraph $G_k=(\Rider_k,\Driver,E_k)$, solve the convex program~\ref{eq:concave-k-bmatching}:
   \vspace{-1mm}
 		\begin{align}
 	\label{eq:concave-k-bmatching}\tag{$\mathcal{P}^{\text{VWM}}_k$}
    \begin{array}{lll}
       \xbf^*_k= \underset{\xbf\geq \mathbf{0}}{\argmax} & 
        \displaystyle\sum_{(i,j) \in E_k}w_j x_{ij} - \sum_{j\in \Driver}w_j F_k\big(y^{(k-1)}_j+
        \sum_{i : (i,j)\in E_k}x_{ij}\big)
        & \text{s.t.}\\
         &\displaystyle
         \sum_{j: (i,j)\in E_k} x_{ij} \leq 1
         & i\in \Rider_k\\
         & 
         \displaystyle\sum_{i: (i,j)\in E_k} x_{ij} \leq 1-y^{(k-1)}_j
         & j\in \Driver
    \end{array}
\end{align}
\tcc{Recall that the $k^{\text{th}}$ regularizer is defined as $F_k(x)\triangleq\displaystyle\int_0^{x}f_k(y)dy$.}

$\forall j\in \Driver: y^{(k)}_j\gets y^{(k-1)}_j+\displaystyle\sum_{i\in\Rider_k}x^*_{k,ij}$.

Return $\xbf^*_k$ as the fractional matching of stage $k$.
 	}
 

%  	\vspace{2mm}
%  	\emph{\underline{Pre-processing:}} Compute the optimal assignment $\{\curalloctypeopt\}$ of $\EAR{\typedistributionsequence}$ by invoking the offline assortment oracle  (\Cref{asp:oracle})
%  	\vspace{2mm}
 	
%  	\For{$t=1$ to $T$}{
%  	\tcc{consumer $t$ with type $\type_t\sim\typedistribution_t$ arrives} 
%  	\vspace{1mm}
 	
%  	\emph{\underline{Simulation:}} Upon realizing consumer type $\type_t$, sample $\hat{\assortment}_t\sim \{\curalloctypeopt\}_{\assortment\in\assortmentspace}$
 	
%  	\vspace{2mm}
%  	\emph{\underline{Discarding:}} Initialize $\bar\assortment_t\gets\hat\assortment_t$
 	
%  	\For{each product $i\in\hat\assortment_t$}{
%  	\vspace{1mm}
%  	Flip an independent coin and remove $i$ from $\bar\assortment_t$ with probability $\gamma$
 	
%  	\If {there is no available unit of product $i$}{
%  	Remove $i$ from $\bar\assortment_t$}}
 	
%  	\vspace{2mm}
%  	\emph{\underline{Post-processing:}} Let $\tilde{S}_t\gets \textsc{Sub-assortment Sampling} \left(\choice^{\type_t}, \bar\assortment_t,\{\choice(\hat\assortment_t, i)\}_{i\in \bar\assortment_t}\right)$
 	
%  	\tcc{Send a query call to Procedure~\ref{alg:sample assortment} with appropriate input arguments}
%  	\vspace{2mm}
 	
%  	Offer assortment $\tilde{\assortment}_t$ to consumer $t$
 	
%  	}
\end{algorithm}
We are now ready to describe the main result of this section.

\begin{theorem}[\textbf{Optimal Multi-Stage Algorithm for Weighted Bipartite Matching}]
\label{thm:b-matching}
In the $K$-stage (fractional) vertex weighted matching problem,
 \PRMWM~(\Cref{alg:b-matching}) is $\cratio{K}$-competitive, where $\cratio{K}=\cratioexp$.
\end{theorem}

\smallskip
\noindent{\textbf{High-level Proof Overview}~} In a nutshell, we analyze our convex programming based algorithm by following two steps. First, we apply the theory of convex duality to the convex programs corresponding to each stage, which guides us to build a convex program specific graph decomposition for each stage's subgraph. Intuitively speaking, the graph decomposition in each stage partitions the subgraph of that stage into groups of demand and supply nodes, so that in each group there exists a fully ``weighted balanced'' fractional matching (measured by some definition related to the convex program). Second, we try to find an assignment to the dual linear program of our optimum offline LP that is built stage by stage, and in each stage uses the graph decomposition of that stage. We suggest a particular graph-decomposition based dual assignment, where we use the same assignment for all supply nodes in the same group and the same assignment for all demand nodes in the same group. Further, we show the dual objective value is equal to the primal algorithm's objective value from our construction. We finally show this dual assignment is approximately feasible, where the approximation factor is $\cratio{K}$. It turns out that the approximate feasibility of our dual assignment boils down to the requirement that functions $f_1,f_2,\ldots,f_K$ satisfy the specific recursive equation in the second bullet of \Cref{prop:poly} for $k=1,2,\ldots,K-1$. Hence, our \PRMWM~algorithm (\Cref{alg:b-matching}) obtains the desired competitive ratio of $\cratio{K}$, as it uses the sequence of  polynomials of decreasing degrees in place of $f_1,\ldots,f_K$ that are the unique solution to mentioned recursive functional equation. See the details of this proof overview in \Cref{sec:primal-dual}.


\begin{remark}[\textbf{Batched Water-filling}]
\label{rem:batched-water}
For the special case of unweighted matching, it is not hard to see that the solution of the convex program \ref{eq:concave-k-bmatching} does \emph{not} depend on the choice of the regularizer function $F_k$ (it only needs to be a strictly convex function). The algorithm for this special case is indeed the batched water-filling algorithm that we investigated in our first example in \Cref{sec:example}. \revcolor{This algorithm is oblivious to the choice of the regularizer and does not even need to know $K$.} Note that while in that simple example the batched water-filling ended up with fully balancing the remaining capacities of all the offline vertices in the first stage graph, this is not going to be necessarily the case in an arbitrary graph at any stage. We should also highlight that this algorithm generalizes the classic water-filling/BALANCE algorithm for the online bipartite fractional matching~\citep{MSVV-07,DJK-13} to the setting where we have batches. Importantly, even though our polynomials are not \emph{explicitly} used by the algorithm, they still help with its competitive ratio analysis and showing that it is $\cratio{K}$-competitive. 
\end{remark}
\begin{remark}[\textbf{Vertex-weighted Online Bipartite Matching}]
Another important special case is when batches have size one, which is basically the online arrival problem. As mentioned earlier, by replacing $f_k(x)$ with $e^{x-1}$ in \emph{every stage}, the final allocation of our algorithm will be the same as the classic BALANCE algorithm for the fractional vertex weighted online matching \citep{AGKM-11, DJK-13}. In other words, the special case of our algorithm provides a convex programming based interpretations of the BALANCE algorithm.\footnote{To provide more details, BALANCE can be viewed as running a particular first-order iterative method for solving this convex program (basically running a slight variant of the Frank-Wolfe algorithm\citep{frank1956algorithm}).}
\end{remark}
\begin{remark}[\textbf{Unweighted Online Bipartite Matching}]
Our result implies the following simple corollary for the very special case of the classic online bipartite matching problem: the water-filling/BALANCE algorithm is $\cratio{n}$ competitive for the (unweighted) online bipartite matching problem with a fixed number of $n$ online vertices. Interestingly, this corollary was also observed in \cite{goel2008online}, but for the RANKING algorithm~\citep{KVV-90} instead of water-filling, and through a more refined combinatorial analysis of RANKING using a factor revealing LP. As we will see later in \Cref{sec:lowerbound} and \Cref{rem:online-matching-with-finite-nodes}, this bound is not necessarily tight for the online bipartite matching problem with $n$ online nodes---despite the fact that the competitive ratio $\cratio{K}$ is indeed optimal in multi-stage matching with $K$ stages (\Cref{thm:tightness}).
\end{remark}

\subsection{Recursive Primal-dual Analysis of \texorpdfstring{\Cref{alg:b-matching}}{Lg}}
\label{sec:primal-dual}
We prove \Cref{thm:b-matching} by 
a primal-dual argument that carefully uses our polynomials.  
Consider the offline primal LP of the maximum vertex weighted matching in graph $G=(\Rider,\Driver,E)$, and its dual:
\begin{equation}
\tag{\textsc{Primal-Dual-MWM}}
\label{eq:LP-max-weight}
\arraycolsep=1.4pt\def\arraystretch{1}
\begin{array}{llllllll}
\underset{\xbf\geq\mathbf{0}}{\max}\quad\quad\quad&\displaystyle\sum_{(i,j)\in E}w_jx_{ij} &~~\text{s.t.}&
&\quad\quad\underset{\boldsymbol{\alpha},\boldsymbol{\beta}\geq\mathbf{0}}{\text{min}}\quad\quad\quad &\displaystyle\sum_{i\in \Rider }{\alpha_i}+\displaystyle\sum_{j\in \Driver}{\beta_j}&~~\text{s.t.} \\[1.4em]
 &\displaystyle\sum_{j:(i,j)\in E}{x_{ij}}\leq1 &~~i\in\Rider~,& 
& &\alpha_i+\beta_j\geq w_j& (i,j)\in E~,\\[1.4em]
 &\displaystyle\sum_{i:(i,j)\in E}{x_{ij}}\leq 1 &~~j\in \Driver~, &
& & \\
\end{array}
\end{equation}
Given the feasible primal assignment $\{\xbf^*_k\}_{k\in[K]}$ produced by \Cref{alg:b-matching}, we construct a dual assignment so that,
\begin{itemize}
    \item Primal and dual have the same objective values: $\displaystyle\sum_{k\in[K]}\displaystyle\sum_{(i,j)\in 
    E_k}w_jx^*_{k,ij}=\sum_{i\in\Rider}\alpha_i+\sum_{j\in\Driver}\beta_j$~,
    \vspace{1mm}
    \item Dual is approximately feasible: $\forall (i,j)\in E: \alpha_i+\beta_j\geq \cratio{K}\cdot w_j$~.
\end{itemize}
Existence of such a dual assignment will guarantee that primal is $\cratio{K}$-competitive.

\revcolor{Our dual assignment is constructed stage-by-stage. Moreover, our construction relies on a structural decomposition of the subgraph in each stage $k$, which itself is tied to the solution of the convex program~\ref{eq:concave-k-bmatching} of stage $k$.  
We highlight that this decomposition is a slightly modified version of a simpler decomposition first introduced in \cite{feng2020two} (for only the first stage in a two-stage problem and for a slightly different convex program) which actually \emph{does not depend} on the choice of the convex function they used. It also extends the well-known matching skeleton for unweighted bipartite graphs~\citep{GKK-12}. Notably, in contrast to both of of these decompositions, this new decomposition actually \emph{depends} on the choice of the convex function used in its definition. This is a key technical property used in the analysis of our algorithm. We first define this decomposition in \Cref{lemma:structure} and show how it can be constructed through convex programming duality (KKT conditions). 
% See the proof of this lemma in \Cref{apx:skeleton}.
We then show how it helps us with our dual construction.}


\begin{proposition}[\revcolor{Stage-wise Structural Decomposition}]
\label{lemma:structure}
Fix any $k \in [K - 1]$.
Let $\xbf^*_k$ be the optimal solution of the convex program~\ref{eq:concave-k-bmatching}. Consider the subgraph $G'_k=(\Rider_k,\Driver,E'_k)$ of $G_k$, where $E'_k=\{(i,j)\in E_k :x^*_{k,ij}>0\}$. Let $\Driver^{(0)}_k$ be the set of offline vertices in $\Driver$ fully matched by $\xbf^*_k$ given the current $\ybf$, and 
$\Rider^{(0)}_k$ be the set of online vertices who are neighbors of $\Driver^{(0)}_k$ in $G_k'$, that is, 
$$\Driver^{(0)}_k\triangleq \{j\in \Driver: y_j+\sum_{i:(i,j)\in E_k}x^*_{k,ij}=1\}~~\textrm{and}~~\Rider^{(0)}_k\triangleq \{i\in \Rider_k:\exists j\in \Driver^{(0)}_k, x^*_{k,ij}>0\}~.$$
Moreover, let the pairs 
$\left\{\left(\Rider_k^{(l)},\Driver_k^{(l)}\right)\right\}_{l=1}^{L_k}$ 
identify the $L_k$ connected components of the induced subgraph $G_k'[\Rider_k\setminus\Rider_k^{(0)},\Driver\setminus\Driver_k^{(0)}]$ of $G_k'$. Then:
\begin{enumerate}%[label=\roman*.]
    \item \underline{Uniformity}: ~$\forall~ l\in[0:L_k],j,j'\in \Driveri_k:$ $$w_j\left(1-
    f_k\left(y_j + \sum_{i:(i,j)\in E_k}x^*_{k,ij}\right)
    \right)=
    w_{j'}\left(1-
    f_k\left(y_{j'} + \sum_{i:(i,j')\in E_k}x^*_{k,ij'}\right)
    \right)\triangleq c_k^{(l)}$$
    \item \underline{Monotonicity}:  $\forall~ l,l'\in[0:L_k]$: there exists no edge in $E_k$ between $\Rider_k^{(l)}$ and $\Driver_k^{(l')}$ if $c_k^{(l)}<c_k^{(l')}$. 
    \item \underline{Saturation}: $\forall~ l\in[L_k]$: all online vertices $i\in\Rider_k^{(l)}$ are fully matched by $\xbf_k^*$, i.e., $\displaystyle\sum_{j:(i,j)\in E_k}x^*_{k,ij}=1$.
\end{enumerate}
\end{proposition}

We prove the above graph-based structural decomposition by investigating the program~\ref{eq:concave-k-bmatching} through convex strong duality. See the details in Appendix~\ref{apx:kkt}. \revcolor{At a high-level, the above graph decomposition partitions the subgraph revealed at each stage $k$ based on a (weighted) notion of \emph{``match-ability''} of the offline nodes (i.e., $c_k^{(l)}$ values). Having such a partitioning helps us to identify a charging scheme, so that we can charge the primal contributions of our algorithm between the dual variables corresponding to offline and online nodes appropriately.} We now have all the ingredients to prove our main theorem of this section using a primal-dual analysis. 
% Note that 
% $0=c_k^{(0)}\leq c_k^{(1)}\leq \ldots\leq c_k^{(L_k)}$.

% \begin{definition}[batch-water-filling (BWF)]
% In any stage $k < K$, let 
% $\{y_{k, j}\}_{j\in D}$ be the capacity 
% of drivers which has been used so far,
% batch-water-filling (BWF) selects
% the fractional matching as the solution of 
% program \eqref{eq:concave program k} 
% on $(\Rider_k, D, E_k)$ 
% with initial capacity $\{y_{k, j}\}_{j\in D}$ and $K - k$.
% In the last stage $k = K$, 
% BWF selects the maximum weighted fractional matching.
% \end{definition}


% \begin{proof}
\ifMS \proof{\textsl{Proof of \Cref{thm:b-matching}.}}
\else \begin{proof}[Proof of \Cref{thm:b-matching}]\fi
For each stage $k\in[K-1]$, let $\{(\Rider^{(0)}_k, \Driver^{(0)}_k),\dots, (\Rider^{(L_k)}_k, \Driver^{(L_k)}_k)\}$ be the 
structural decomposition of $(\Rider_k, \Driver, E_k)$ as in \Cref{lemma:structure},
and $\{x_{k, ij}^*\}_{(i,j)\in E_k}$
be the optimal solution of the program~\ref{eq:concave-k-bmatching}. Note that if $c_k^{(l)}=c_k^{(l')}$ for $l\neq l'$ and some $k\in[K-1]$, we can simply merge the two pairs $\left(\Rider_k^{(l)},\Driver_k^{(l)}\right)$ and $\left(\Rider_k^{(l')},\Driver_k^{(l')}\right)$ to $\left(\Rider_k^{(l)}\cup \Rider_k^{(l')},\Driver_k^{(l)}\cup \Driver_k^{(l')}\right)$, and still our decomposition satisfies the three properties of \Cref{lemma:structure}; these properties are all we need for our technical arguments. Therefore, without loss of generality, we can assume $c_k^{(l)}$'s are non-identical. Moreover, $0=c_k^{(0)}<c_k^{(1)}<\ldots<c_k^{(L_k)}$.


First, we define the following notations which will be useful in this proof:
\begin{align*}
\forall j\in \Driver,~k\in[K]:\quad\quad\quad &y^*_{k,j}\triangleq\sum_{s=1}^{k-1}\sum_{i:(i,j)\in E_s}x^*_{s,ij}
% ,\\
%  &y^*_{0,j}=0.
\end{align*}
Now, consider the offline primal-dual linear programs in \ref{eq:LP-max-weight}. Given the feasible primal assignment $\{\xbf^*_{k}\}_{k\in[K]}$, construct a dual assignment as follows. First, set $\alpha_i\gets 0$ and $\beta_j\gets 0$ for all $i\in\Rider,j\in \Driver$. At each stage $k\in[K-1]$, update the dual variables as follows:
\begin{align*}
   &\forall i \in \Rider^{(l)}_k,~l\in[0:L_k]: &&\alpha_i\gets c^{(l)}_k
   \\
    &\forall j \in \Driver^{(l)}_k,~l\in[0:L_k]: &&\beta_{j}\gets\beta_{j}+\Delta\beta_{k,j}\\
    &&&\Delta\beta_{k,j}\triangleq \left(
\sum_{i:(i,j)\in E_k}x_{k,ij}^* \right)\cdot \left(w_j - c_k^{(l)}\right)\overset{(a)}{=}w_j(y^*_{k+1,j}-y^*_{k,j})f_k(y^*_{k+1,j})
\end{align*}
where in eq.\ (a) above 
% \YF{label eq.~(1) is not defined in our paper}
we use the uniformity property and the definition of $c^{(l)}_k$ in \Cref{lemma:structure}. For the last stage $K$, note that $F_K(x)=0$ for all $x\in[0,1]$. Therefore, \Cref{alg:b-matching} essentially solves the maximum vertex weighted matching in the last stage graph $(\Rider_K, \Driver, E_K)$ where each $j\in\Driver$ has initial capacity $1-y^*_{K, j}$. Let $\{\hat{\alpha}_{K,i}, \hat{\beta}_{K,j}\}_{i\in\Rider_K,j\in\Driver}$ 
be the \emph{optimal} dual solution of this LP. Then update the  dual variables as follows:
\begin{align*}
&\forall i\in\Rider_K:~~\alpha_i \gets \hat{\alpha}_{K,i} \\
&\forall j\in \Driver~:~~\beta_j\gets \beta_j+\Delta \beta_{K,j},~~\Delta\beta_{K, j} \triangleq (1 - y^*_{K, j})\hat{\beta}_{K,j}
\end{align*}



% Consider the following construction of dual solution.
% At stage $k < K$, let 
% $\bar f_k(x) \triangleq f_{K - k}(x) = \left(
% \frac{K - k - 1 + x}{K-k}
% \right)^{K-k}$, and 
% $\{(\Rider^{(0)}_k, \Driver^{(0)}_k),\dots, (\Rider^{(L)}_k, \Driver^{(L)}_k)\}$ be the 
% partition of $(\Rider_k, D, E_k)$ in \Cref{lemma:structure},
% and 
% $\{x_{k, ij}^*\}_{(i,j)\in E_k}$
% be the optimal solution  
% from the concave program~\eqref{eq:concave program k}
% solved by BWF.
% Construct the dual solution as follows,
% for any $k < K$ 
% \begin{align*}
%     \alpha_i &= c^{(l)}_k
%     \qquad \forall i \in \Rider^{(l)}_k \\
%     \Delta \beta_{k,j} &= \left(
%     % 1 - 
%     \sum_{i\in N_k(j)}x_{k,ij}^*
%     % - y_{k,j}
%     \right)\cdot 
%     \left(w_j - c_k^{(l)}\right)
%     \qquad \forall j \in \Driver^{(l)}
% \end{align*}
% where $N_k(j)$ denotes all neighbor vertices of item $j$
% in graph $(\Rider_k, D, E_k)$ at stage $k$.
The rest of the proof is done in two steps:
\vspace{1mm}

\noindent[\textit{Step \rom{1}}]~\emph{Comparing objective values in primal and dual.}
we first show that 
the objective value of the above dual assignment
is equal to the objective value of the primal assignment of \Cref{alg:b-matching}.
To show this, we consider 
each stage $k$ separately.
For the last stage $K$, 
this holds by construction.
For each stage $k \in [K-1]$, note that the primal objective value is decomposed across pairs $(\Rider_k^{(l)}, \Driver_k^{(l)})$, 
$l\in[0: L_k]$, 
simply because $x^*_{k,ij}>0$ only if $i$ and $j$ belong to the same pair (\Cref{lemma:structure}). As these pairs partition sets of vertices $\Rider$ and $\Driver$, it is enough to compare the changes in the primal and dual objectives in each pair $(\Rider_k^{(l)}, \Driver_k^{(l)})$ separately. Notice that if $l = 0$ then $c^{(l)}_k = 0$, and thus,
\begin{align*}
    \Delta(\textrm{Dual})^{(0)}\triangleq\sum_{i \in \Rider^{(0)}_k} \alpha_i
    +
    \sum_{j \in \Driver^{(0)}_k} \Delta\beta_{k,j}
    &= 
    \sum_{j \in \Driver^{(0)}_k}\sum_{i:(i,j)\in E_0} w_jx_{k, ij}^*\triangleq\Delta(\textrm{Primal})^{(0)}. 
\end{align*}
Similarly, for $l \in [L_k]$, 
\begin{align*}
     \Delta(\textrm{Dual})^{(l)}&\triangleq\sum_{i \in \Rider^{(l)}_k} \alpha_i
    +
    \sum_{j \in \Driver^{(l)}_k} \Delta\beta_{k,j}
    =
    |\Rider^{(l)}_k|\cdot c^{(l)}_k
    +
    \sum_{j \in \Driver^{(l)}_k}\sum_ {i:(i,j)\in E_k} 
    x_{k, ij}^*\left(w_j - c^{(l)}_k\right)\\
    &= 
     |\Rider^{(l)}_k|\cdot c^{(l)}_k+\sum_{j\in\Driver_k^{(l)}}\sum_{i:(i,j)\in E_k} 
    w_jx_{k, ij}^*-c^{(l)}_k\sum_{i\in\Rider_k}\left(\sum_{j:(i,j)\in E_k}x^*_{k,ij}\right)\\
    &=\sum_{j\in\Driver_k^{(l)}}\sum_{i:(i,j)\in E_k} 
    w_jx_{k, ij}^*\triangleq \Delta(\textrm{Primal})^{(l)},
\end{align*}
where the last equality uses the saturation property in \Cref{lemma:structure} 
for $l\in[L_k]$.
\vspace{1mm}

\noindent[\textit{Step \rom{2}}]~\emph{Checking approximate feasibility of dual.} 
To show approximate dual feasibility, it is enough to show that for any stage $k\in[K]$ and any arbitrary edge $(i, j) \in E_k$,
\begin{align}
\label{eq:dual constraint feasibility}
    \alpha_i + \sum_{s = 1}^k\Delta\beta_{s, j}
    \geq 
    w_j\left(1-(1-1/K)^K\right)
\end{align}
We next show \eqref{eq:dual constraint feasibility}
holds for $k\in[K-1]$ by using the following technical lemma, which carefully uses our sequence of polynomial regularizers to establish a lower bound on the LHS of \eqref{eq:dual constraint feasibility}.

  \begin{lemma}
    \label{lem:polynomial inequality 2}
    For any $K \in \N,~k \in [K - 1]$, 
    $x \in [0, 1]$, and
    any $0 = y_1 \leq 
    y_2 \leq \dots \leq y_k \leq  1 - x$,
    \begin{align*}
     (1-x)f_{k}(y_k + x) -
    \sum_{s = 1}^{k - 1} 
    (y_{s + 1} - y_s)
    f_{s}(y_{s + 1})
     \leq 1-\cratio{K}=
    (1-1/K)^K.
    \end{align*}
    \end{lemma}
Now assume $i \in \Rider_k^{(l)}$ and $j \in \Driver_k^{(l')}$, which implies $c^{(l')}_k \leq c^{(l)}_k$ (\Cref{lemma:structure}). Then we have:
\begin{align*}
     \alpha_i + \sum_{s = 1}^{k}\Delta\beta_{s, j}&=c_k^{(l)} + 
    \left(\sum_{i':(i',j)\in E_k}x_{k, i'j}^*\right)
    \left(w_j - c_k^{(l')}\right)
    +
    \sum_{s= 1}^{k - 1} \Delta\beta_{s, j} \\
    &\geq c_k^{(l')} + 
    \left(\sum_{i':(i',j)\in E_k}x_{k, i'j}^*\right)
    \left(w_j - c_k^{(l')}\right)
    +
    \sum_{s= 1}^{k - 1} \Delta\beta_{s, j} \\
    &=w_j\left(1-f_k\left(y^*_{k,j}+\sum_{i':(i',j)\in E_k}x_{k, i'j}^*\right)+\left(\sum_{i':(i',j)\in E_k}x_{k, i'j}^*\right)f_k\left(y^*_{k,j}+\sum_{i':(i',j)\in E_k}x_{k, i'j}^*\right)\right)\\
    &+ \sum_{s= 1}^{k - 1} \Delta\beta_{s, j} \\
    &=w_j\left(1-\left(1-\sum_{i':(i',j)\in E_k}x_{k, i'j}^*\right)f_k\left(y^*_{k,j}+\sum_{i':(i',j)\in E_k}x_{k, i'j}^*\right)+\sum_{s=1}^{k-1}\left(y^*_{s+1,j}-y^*_{s,j}\right)f_k\left(y^*_{s+1,j}\right)\right)\\
    &\geq w_j \cratio{K}~,
\end{align*}
where the first inequality uses $c^{(l')}_k \leq c^{(l)}_k$, the second equality uses the expression for $c^{(l')}_k$ in \Cref{lemma:structure} due to uniformity, and the last inequality invokes \Cref{lem:polynomial inequality 2} for the sequence: 
$$
0=y^*_{1,j}\leq y^*_{2,j}\leq \ldots \leq y^*_{k,j}\leq 1-\sum_{i':(i',j)\in E_k}x_{k, i'j}^*~.
$$
% \begin{align*}
%      & c_k^{(l)} + 
%     \left(\sum_{i'\in N_k(j)}x_{k, i'j}^*\right)
%     \left(w_j - c_k^{(l)}\right)
%     +
%     \sum_{s' = 1}^{k - 1} \Delta\beta_{s', j} \\
%     &\leq 
%     c_k^{(l')} + 
%     \left(\sum_{i'\in N_k(j)}x_{k, i'j}^*\right)
%     \left(w_j - c_k^{(l)}\right)
%     +
%     \sum_{s' = 1}^{k - 1} \Delta\beta_{s', j} \\
%     &=
%     \alpha_i + \sum_{s' = 1}^{k}\Delta\beta_{s', j}
% \end{align*}

So far, we have shown \eqref{eq:dual constraint feasibility} holds for all stages $k < K$.
For the last stage $K$, and any edge $(i, j) \in E_K$,
notice that 
$\alpha_i+\Delta\beta_{K, j}=\hat{\alpha}_{K,i} + (1 - y^*_{K, j})\hat\beta_{K, j} \geq 
w_j(1 - y^*_{K, j})$ by construction.
 If $y^*_{K, j} = 0$, inequality \eqref{eq:dual constraint feasibility} holds. Otherwise, let $k' < K$ be the latest stage before $K$ where 
there exists $l^\dagger$ 
such that 
$j \in \Driver_{k'}^{(l^\dagger)}$ and 
$\Delta\beta_{k',j} > 0$. By definition, we have
$y^*_{k', j} + \displaystyle\sum_{i':(i',j)\in E_{k'}}x_{k', i'j}^* = y^*_{k'+1,j}= y^*_{K,j}$. Therefore:
\begin{align*}
    \alpha_i + \sum_{s = 1}^{K}\Delta\beta_{s, j}
    &\geq    
    w_j(1 - y^*_{K, j})
    + \sum_{s = 1}^{K - 1}\Delta\beta_{s, j} = 
    w_j(1 - y^*_{K, j}) + \sum_{s = 1}^{k'}\Delta\beta_{s, j} \\
    &\geq w_j\left(1 - f_{k'}(y^*_{k'+1, j})\right) + \sum_{s = 1}^{k'}\Delta\beta_{s, j} =c^{(l^\dagger)}_{k'} + \sum_{s = 1}^{k'}\Delta\beta_{s, j} \\
    &\geq w_j(1 - (1 - 1/K)^K)~,
\end{align*}
where the first equality uses the fact $\Delta\beta_{s, j} = 0$ for all $s$
between $k' + 1$ and $K - 1$; the second inequality uses the fact that 
that $f_{s}(x) \geq x$ for all $x\in [0, 1]$ and $s\in [K - 1]$
and $y^*_{k'+1,j}= y^*_{K,j}$,
the second equality uses the definition of $c^{(l^\dagger)}_{k'}$; and finally the last inequality holds by exactly the same argument as in the case of $k\in[K-1]$.\ifMS \hfill\Halmos \fi
\ifMS
\endproof
\else
\end{proof}
\fi

We finish the analysis by proving the technical lemma used in the proof of \Cref{thm:b-matching}. It will be further used in the analysis of our multi-stage configuration allocation algorithm in \Cref{sec:extensions}.


\ifMS \proof{\textsl{Proof of \Cref{lem:polynomial inequality 2}.}}
\else \begin{proof}{proof}[Proof of \Cref{lem:polynomial inequality 2}]\fi
    We show the statement by induction on $k$.
    
    \vspace{2mm}
    \noindent\textsl{Base case $(k = 1)$.} 
    The left hand side of inequality becomes
    \begin{align*}
        (1-x)f_{1}(x) 
        \leq 
        1-\cratio{K},
    \end{align*}
    which holds because of \Cref{prop:poly}, part (vi). 
    
    \vspace{2mm}
    \noindent\textsl{Inductive step $(1< k\leq K-1)$}.
    For any instance $(K, k, x, y_1, \dots, y_k)$,
    consider another instance 
    $(K, k - 1, x'\triangleq y_k - y_{k - 1}, y_1, \dots, y_{k-1})$.
    Note that
    \begin{align*}
         &(1 - x)f_{k}(y_k + x) - 
     \sum_{s = 1}^{k - 1} 
    (y_{s + 1} - y_s)
    f_{s}(y_{s + 1}) \overset{(a)}{\leq} f_{k-1}(y_k)
    -
     \sum_{s = 1}^{k - 1} 
    (y_{s + 1} - y_s)
    f_{s}(y_{s + 1})\\
   &= \left(1-(y_k-y_{k-1})\right)f_{k - 1}(y_{k - 1} + (y_k - y_{k - 1}))-
    \sum_{s = 1}^{k - 2} 
    (y_{s + 1} - y_s)
    f_{s}(y_{s + 1})\\
    &=\left(1-x'\right)f_{k - 1}(y_{k - 1} + x')-
    \sum_{s = 1}^{k - 2} 
    (y_{s + 1} - y_s)
    f_{s}(y_{s + 1}) \overset{(b)}{\leq} 1-\cratio{K}~,
    \end{align*}
    % \begin{align*}
    %     &
    % 1 - (1 - x)f_{K - k}(y_k + x) + 
    %  \sum_{s = 1}^{k - 1} 
    % (y_{s + 1} - y_s)
    % f_{K - s}(y_{s + 1})\\
    %     &1 - (1 - 1/K)^K  \\
    %     \leq &
    %     1 - f_{K - k + 1}(y_{k - 1} + (y_k - y_{k - 1})) 
    %     + 
    % \sum_{s = 1}^{k - 2} 
    % (y_{s + 1} - y_s)
    % f_{K - s}(y_{s + 1})
    % +
    % (y_k-y_{k-1}) f_{K - {k - 1}}(y_{k - 1} + (y_k - y_{k - 1}))
    % \\
    % =&
    % 1 - f_{K - k + 1}(y_k)
    % +
    %  \sum_{s = 1}^{k - 1} 
    % (y_{s + 1} - y_s)
    % f_{K - s}(y_{s + 1})
    % \end{align*}
    where ineq.\ (a) uses
    \Cref{prop:poly} and the recursive definition of $\{f_k(x)\}_{k\in[K]}$, and ineq.\ (b) uses the induction hypothesis on instance 
    $(K, k - 1, x', y_1, \dots, y_{k-1})$, where $x'=y_k - y_{k - 1}$.\ifMS
\hfill\Halmos\fi
\ifMS\endproof
\else
\end{proof}
\fi



% by induction.

% \emph{Base case (stage 1).}
% Again, let $\{(R_1^{(0)}, D_1^{(0)}),\dots, (R_1^{(L)}, D_1^{(L)})\}$ be the 
% partition of $(R_1, D, E_1)$ in \Cref{lemma:structure}. 
% Consider an arbitrary edge $(i, j) \in E_1$.
% Due to the monotonicity property in 
% \Cref{lemma:structure}, without loss of generality,
% we assume
% $i \in R_1^{(l')}$ and $j \in D_1^{(l)}$ where $l \leq l'$
% and $c^{(l)}_1 \leq c^{(l')}_1$.
% \begin{align*}
%     \alpha_i + \Delta\beta_{1, j}
%     &=
%     c^{(l')}_1 +  
%     \left(
%         \sum_{i'\in N_1(j)}x_{1,i'j}^*
%     \right)\cdot 
%     \left(w_j - c_1^{(l)}\right)\\
%     &\geq 
%     c^{(l)}_1 +  
%     \left(
%         \sum_{i'\in N_1(j)}x_{1,i'j}^*
%     \right)\cdot 
%     \left(w_j - c_1^{(l)}\right) \\
%     &=
%     w_j\left(1-
%     \bar f_1\left(y_{1,j} + 
%     \sum_{i'\in N_1(j)}x^*_{1,i'j}\right)
%     \right)
%     +
%     w_j\left(
%         \sum_{i'\in N_1(j)}x_{1,i'j}^*
%     \right)
%     \bar f_1\left(y_{1,j} + 
%     \sum_{i'\in N_1(j)}x^*_{1,i'j}\right)
%     \\
%     &\geq 
%     w_j\left(\min_{x\in[0, 1]}1 - (1 - x)\cdot \bar f_1(x)\right) \\
%     % &=
%     % \min_{x\in[0, 1]}1 - (1 - x)\cdot
%     % \left(
%     % \frac{k-2 + x}{k-1}
%     % \right)^{k-1} \\
%     &=
%     w_j\left(1 - (1 - 1/K)^K)\right)
% \end{align*}
% where the third line uses the definition of $c^{(l)}_1$;
% and the fourth line uses 
% the fact that $y_{1,j} = 0$.

% \emph{Inductive step (stage $1 < k < K$).}
% Consider an arbitrary edge $(i, j) \in E_k$.
% If $y_{k, j} = 0$ at stage $k$,
% using the same argument as the base case, 
% the inductive statement holds.

% Now, we assume $y_{k, j} > 0$ at stage $k$.
% Due to monotonicity in \Cref{lemma:structure}, 
% without loss of generality,
% we assume
% $i \in \Rider_k^{(l')}$ and $j \in \Driver_k^{(l)}$ where $l \leq l'$
% and $c^{(l)}_k \leq c^{(l')}_k$.
% Let $s < k$ be the largest 
% stage smaller than $k$ 
% where 
% there exists $l^\dagger$ 
% such that 
% $j \in D_{s}^{(l^\dagger)}$ and 
% $\Delta\beta_{s,j} > 0$.
% By definition, we know that 
% $y_{s, j} + \sum_{i':(i', j)\in E_s}x_{s, i'j}^* = y_{k,j}$.
% By induction hypothesis at stage $s$,
% \begin{align*}
%     w_j\left(1 - (1 - 1/K)^K\right) &\leq 
%     c_{s}^{(l^\dagger)}
%     +
%     \sum_{s' = 1}^{s} \Delta\beta_{s', j} \\
%     &=
%     w_j\left(1 - \bar f_s(y_{k, j})\right)
%     +
%     \sum_{s' = 1}^{k - 1} \Delta\beta_{s', j} \\
%     &\leq 
%     w_j\left
%     (1 - 
%     \bar f_{k}\left(y_{k,j} + 
%     \sum_{i'\in N_k(j)}x_{k, i'j}^*
%     \right)
%     + \left(\sum_{i'\in N_k(j)}x_{k, i'j}^*\right)
%     \bar f_{k}\left(y_{k,j} + 
%     \sum_{i'\in N_k(j)}x_{k, i'j}^*
%     \right)
%     \right)\\
%     &\qquad +
%     \sum_{s' = 1}^{k - 1} \Delta\beta_{s', j} \\
%     &=
%     c_k^{(l)} + 
%     \left(\sum_{i'\in N_k(j)}x_{k, i'j}^*\right)
%     \left(w_j - c_k^{(l)}\right)
%     +
%     \sum_{s' = 1}^{k - 1} \Delta\beta_{s', j} \\
%     &\leq 
%     c_k^{(l')} + 
%     \left(\sum_{i'\in N_k(j)}x_{k, i'j}^*\right)
%     \left(w_j - c_k^{(l)}\right)
%     +
%     \sum_{s' = 1}^{k - 1} \Delta\beta_{s', j} \\
%     &=
%     \alpha_i + \sum_{s' = 1}^{k}\Delta\beta_{s', j}
% \end{align*}
% where the first inequality holds 
% due to induction hypothesis at stage $s$;
% the second inequality holds since 
% $y_{s, j} + \sum_{i'\in N_s(j)}x_{s, i'j}^* = y_{k,j}$
% and 
% $\Delta\beta_{s', j} = 0$ for all $s'$
% between $s + 1$ and $k - 1$;
% the third inequality holds due to 
% \Cref{lem:polynomial inequality}.

% So far, we have shown \eqref{eq:dual constraint feasibility} holds for all stage $k < K$.
% For the last stage $K$, and any edge $(i, j) \in E_K$,
% notice that 
% $\alpha_i + \Delta\beta_{K, j} \geq 
% w_j(1 - y_{K, j})$ by construction.
% If $y_{K, j} = 0$, inequality \eqref{eq:dual constraint feasibility} holds.
% Otherwise, with the similar argument in our inductive
% step, let $s, l^\dagger$ defined the same as before,
% \begin{align*}
%     \alpha_i + \sum_{s' = 1}^{K}\Delta\beta_{s', j}
%     &\geq    
%     w_j(1 - y_{K, j})
%     + \sum_{s' = 1}^{K - 1}\Delta\beta_{s', j} \\
%     &= 
%     w_j(1 - y_{K, j}) + \sum_{s' = 1}^{s}\Delta\beta_{s', j} \\
%     &\geq
%     c^{(l^\dagger)}_s
%     +\sum_{s' = 1}^{s}\Delta\beta_{s', j} \\
%     &\geq
%     (1 - (1 - 1/K)^K)w_j
% \end{align*}
% where the third inequality uses the fact 
% that $\bar f_{s}(a) \geq a$ for all $a\in [0, 1]$ and 
% the definition of $c^{(l^\dagger)}_s$.


    % \begin{lemma}
    % \label{lem:polynomial inequality}
    % For any $a, b \in [0, 1]$, 
    % and any $s, k \in \N$ s.t.
    % $s < k$,
    % \begin{align*}
    % (1-b)  f_s(a + b)
    % \leq 
    % f_k(a)
    % \end{align*}
    % \end{lemma}
    % \begin{proof}
    % First, observe that 
    % $f_k(a)$
    % is monotone increasing
    % in $k$ for any fixed $a \in [0, 1]$. 
    % Hence, it is sufficient to show
    % for any $a, b \in [0, 1]$,
    % and any $s \in \N$,
    % \begin{align}
    % \label{eq:polynomial inequality}
    % (1-b)  f_s(a + b)
    % \leq 
    % f_{s+1}(a)
    % \end{align}
    % Consider the first order condition
    % of the left hand side of inequality \eqref{eq:polynomial inequality} 
    % with respect to
    % $b$,
    % \begin{align*}
    %     -b\left(
    % \frac{s - 1 + a + b}{s}
    % \right)^{s-1}
    % -\left(
    % \frac{s - 1 +a + b}{s}
    % \right)^{s}
    % +
    % \left(
    % \frac{s - 1+a + b}{s}
    % \right)^{s - 1}
    % = 0
    % \end{align*}
    % Since $a, b$ are both 
    % weakly positive,
    % the first order condition
    % is equivalent to 
    % \begin{align*}
    %     1 - b = \left(
    % \frac{s - 1+a + b}{s}
    % \right)
    % \end{align*}
    % where the solution is $b^* = \frac{1 - a}{s+1}$.
    % Plug-in $b^*$ into the left hand side of inequality
    % \eqref{eq:polynomial inequality}, we get  
    % the right hand side of inequality
    % \eqref{eq:polynomial inequality}
    % exactly.
    % It is also easy to verify that 
    % inequality
    % \eqref{eq:polynomial inequality} 
    % holds for boundary $b$,
    % i.e.,
    % $b = 0$ and $b = 1$.
    % \end{proof}
    

==> tex/adwords.tex <==
Recall that multi-stage AdWords 
problem is a variant of the multi-stage vertex 
weighted matching where 
(i) the weights (a.k.a., bids)
$\{b_{ij}\}_{(i,j)\in E}$
are assigned to edges;
(ii)
the matching constraint of 
each offline vertex $j\in \Driver$ is replaced with the budget constraint $\budget_j$;
and the goal 
is to maximize the total bids 
(a.k.a., used budgets) in the allocation.
Let $\minbudget = 
\min_{j\in \Driver}\budget_j$
be the smallest budget.
We discuss how to modify 
\Cref{alg:b-matching}
to output {fractional} solutions
for the $K$-stage AdWords problem
with competitive ratio $\cratio{K}$.
Then, using a standard 
randomized rounding technique,
we present a \emph{randomized} algorithm
that produces \emph{integral} solutions 
with competitive ratio 
$\cratio{K} - 
O(\sqrt{\log(\minbudget)/\minbudget})$.



\smallskip
\noindent\textbf{Fractional Multi-stage AdWords~} Consider a modification of 
\Cref{alg:b-matching}, where
(i) the convex program~\ref{eq:concave-k-bmatching}
is replaced with 
the modified convex program~\ref{eq:concave-adwords-k}
defined below,
and 
(ii) the update rule of 
$\{y_j\}$ is modified as 
$\forall j\in \Driver: y_j\gets y_j+\displaystyle\sum_{i\in\Rider_k}
b_{ij}x^*_{k,ij}$.
See the \emph{Polynomial Regularized Fractional AdWords} (\PRFAD) algorithm for a formal description (\Cref{alg:adwords fractional}):
    \begin{align}
\label{eq:concave-adwords-k}\tag{$\mathcal{P}_k^{\text{AdWords}}$}
    \begin{array}{lll}
       \xbf^*_k= \underset{\xbf}{\argmax} & 
        \displaystyle\sum_{(i,j) \in E_k}
b_{ij} {x_{ij}}
- \sum_{j\in \Driver}
\budget_j F_k\left(
\frac{y_j}{\budget_j}+
\sum_{i : (i,j)\in E_k}
\frac{b_{ij}x_{ij}}{\budget_j}
        \right)
        & \text{s.t.}\\
         &\displaystyle
         \sum_{j: (i,j)\in E_k} x_{ij} \leq 1
         & i\in \Rider_k\\
         & 
         \displaystyle\sum_{i: (i,j)\in E_k} 
         b_{ij}x_{ij} \leq 
         \budget_j-y_j
         & j\in \Driver\\
         &
        x_{ij} \geq 0 &
        (i, j) \in E_k
    \end{array}
\end{align}

\begin{algorithm}
 	\caption{Polynomial Regularized Fractional AdWords (\PRFAD)}
 	\label{alg:adwords fractional}
 	\KwIn{Number of batches/stages $K$}
%  	\vspace{1mm}
%  	\KwOut{SS.}
 	    \vspace{2mm}
 	    
    $\forall j\in\Driver:~y_j\gets 0$.

 	\vspace{1mm}
 	\For{stage $k=1$ to $K$}
 	{
 	\vspace{2mm}
 	\tcc{$k^{\textrm{th}}$ batch of vertices in $\Rider$, denoted by $\Rider_k$, arrives. Let $E_k$ denote the set of edges incident to vertices in $\Rider_k$.}
 	\vspace{2mm}
 	



   Given $\{y_j\}_{j\in \Driver}$ and subgraph $G_k=(\Rider_k,\Driver,E_k)$, solve $\xbf_k^*$
   from
   the convex program~\ref{eq:concave-adwords-k}.

$\forall j\in \Driver: y_j\gets y_j+\displaystyle\sum_{i\in\Rider_k}b_{ij}x^*_{k,ij}$.

Return $\xbf^*_k$ as the fractional AdWords allocation of stage $k$.

}
\end{algorithm}


\smallskip
\noindent\textbf{Rounding to an Integral Allocation~} To output integral solutions
in the $K$-stage AdWords problem, 
we apply a standard randomized rounding technique
as follows.
% \YF{do we need a citation for this
% sampling technique?}
At each stage $k$, find the optimal fractional solution
$\xbf_k^*$ of the convex
program \ref{eq:concave-adwords-k}
with adjusted budgets
$\{(1-\rho)\hat\budget_j\}_{j\in \Driver}$,
where $\rho = O(\sqrt{\log(\minbudget)/\minbudget})$
for a large enough constant in the big O notation.
% \footnote{It is not hard to verify that 
% $\rho = O(\sqrt{\log(\minbudget)/\minbudget})$.
% }
For each online vertex $i\in \Rider_k$,
sample an offline vertex $j\in\Driver$ independently 
with probability $\{x_{k,ij}^*\}_{j:(i,j)\in E_k}$.
If the offline vertex $j$ has enough budget for bid $b_{ij}$, allocate the online vertex $i$ to the offline vertex $j$. Otherwise, leave the online vertex $i$ unmatched.
Finally, update $\{y_j\}_{j\in \Driver}$
with the fractional solution $\xbf_k^*$ as before.
We refer to this algorithm as \emph{Polynomial Regularized Integral AdWords} (\PRIAD). See \Cref{alg:adwords integral}
for a formal description.

\begin{algorithm}
 	\caption{Polynomial Regularized Integral AdWords (\PRIAD)}
 	\label{alg:adwords integral}
 	\KwIn{Number of batches/stages $K$, parameter $\rho\in[0,1]$}
%  	\vspace{1mm}
%  	\KwOut{SS.}
 	    \vspace{2mm}
 	    
    $\forall j\in\Driver:~y_j\gets 0,
    \hat y_j \gets 0$.
    
%     $\rho = \underset{\rho\in[0,1]}{\argmin}
% ~1-\left(1-\rho\right)\left(1 - \exp\left(-\frac{\rho^2\minbudget}
%     {2-\rho}\right)\right)$.

 	\vspace{1mm}
 	\For{stage $k=1$ to $K$}
 	{
 	\vspace{2mm}
 	\tcc{$k^{\textrm{th}}$ batch of vertices in $\Rider$, denoted by $\Rider_k$, arrives. Let $E_k$ denote the set of edges incident to vertices in $\Rider_k$.}
 	\vspace{2mm}
 	

    Given $\{y_j\}_{j\in \Driver}$ and subgraph  $G_k=(\Rider_k,\Driver,E_k)$, solve $\xbf_k^*$
   from
   the convex  program~\ref{eq:concave-adwords-k} with
    adjusted budgets $\{(1-\rho)\budget_j\}_{j\in \Driver}$,
    and used budgets $\{y_j\}_{j\in \Driver}$.
    
    $\hat\xbf_k^* \gets \mathbf 0$.
    
 	\For{online vertex $i \in \Rider_k$}{
 	Sample offline vertex $j\sim \{x_{k,ij}^*\}_{j:(i,j)\in E_k}$.
 	
 	\If{$\hat y_j + b_{ij} \leq \budget_j$}{
 	    $\hat x_{k,ij}^* \gets 1$.
 	    
 	    $\hat y_j \gets \hat y_j + b_{ij}$.
 	}
 	}

$\forall j\in \Driver: y_j\gets y_j+\displaystyle\sum_{i\in\Rider_k} b_{ij}x^*_{k,ij}$.

Return $\hat\xbf^*_k$ as the integral AdWords allocation of stage $k$.

}
\end{algorithm}

We are now ready to describe the competitive ratio results of the multi-stage AdWords problem.
The proofs are deferred to \Cref{apx:adwords}.

\begin{theorem}[\textbf{Optimal Multi-stage Algorithm for Fractional AdWords}]
\label{thm:adwords fractional}
% \RN{is the statement of this theorem correct?}
In the $K$-stage fractional 
AdWords problem, \PRFAD~(\Cref{alg:adwords fractional})
is $\cratio{K}$-competitive, where $\cratio{K}=\cratioexp$.
\end{theorem}
\begin{theorem}[\textbf{Optimal Multi-stage Algorithm for AdWords with Large Budgets}]
\label{thm:adwords integral}
% \RN{is the statement of this theorem correct?}
In the $K$-stage integral
AdWords problem, \PRIAD~(\Cref{alg:adwords integral})
is \ $\left(\cratio{K} - O(\sqrt{\log(\minbudget)/\minbudget})\right)$-competitive, where $\cratio{K}=\cratioexp$.
\end{theorem}


\begin{remark}[\textbf{Optimality of the $\boldsymbol{\cratio{K}}$ Competitive Ratio for AdWords}]
Again, since the multi-stage AdWords problem generalizes
the multi-stage (fractional) unweighted matching problem (i.e., when $b_{ij}\in\{0,1\}$ and all budgets are $B_j=1$), 
% (i.e., the former approximates the latter
% by setting $b_{ij} = w_j$ for all $(i,j)\in E$
% and letting $\minbudget\rightarrow\infty$),
\Cref{thm:tightness} implies that
the competitive ratios in Theorems~\ref{thm:adwords fractional} and \ref{thm:adwords integral}
% is tight for $K$ 
have the optimal dependence on $K$
in the multi-stage AdWords problem, i.e., no integral or fractional multi-stage algorithm can obtain a competitive ratio better than $\cratio{K}$.
\end{remark}


==> tex/apx-adword-proof.tex <==
\subsection{\texorpdfstring{Proof of \Cref{thm:adwords fractional} and \Cref{thm:adwords integral}}{Lg}}
\label{apx:adwords}

To prove our theorems, we start with a structural decomposition lemma 
as before. This time, our structural decomposition is slightly different, and in fact much simpler. 
% We omits its proof as it basically repeats 
% the argument for its analog in 
% vertex weighted
% matching problem (\Cref{lemma:structure}).
% The main difference between \Cref{lemma:structure adwords} and \Cref{lemma:structure}
% is the closed-form expression 
% in uniformity property.

\begin{lemma}[\emph{Structural decomposition --
AdWords}]
\label{lemma:structure adwords}
Fix any $k \in [K - 1]$.
Let $\xbf^*_k$ be the optimal solution of convex program~\ref{eq:concave-adwords-k}. Consider the subgraph $G'_k=(\Rider_k,\Driver,E'_k)$ of $G_k$, where $E'_k=\{(i,j)\in E_k :x^*_{k,ij}>0\}$. Let $\Driver^{(0)}_k$ be the set of offline vertices in $\Driver$ who exhausts their 
budgets by $\xbf^*_k$ given the current $\ybf$, and 
$\Rider^{(0)}_k$ be the set of online vertices who are neighbors of $\Driver^{(0)}_k$ in $G_k'$, that is, 
$$\Driver^{(0)}_k\triangleq \{j\in \Driver: y_j+\sum_{i:(i,j)\in E_k}b_{ij}x^*_{k,ij}=\budget_j\}~~\textrm{and}~~\Rider^{(0)}_k\triangleq \{i\in \Rider_k:\exists j\in \Driver^{(0)}_k, x^*_{k,ij}>0\}~.$$
Moreover, let $\Rider_k^{(1)} 
\triangleq \Rider_k\setminus\Rider_k^{(0)}$
and 
$\Driver_k^{(1)}
\triangleq
\Driver\setminus\Driver_k^{(0)}$.
Then:
\begin{enumerate}%[label=\roman*.]
    \item \underline{Uniformity}: ~$
    \forall
    i\in \Rider_k, j,j'\in \Driver:$
    if $x_{k,ij}^* > 0$ and 
    $x_{k,ij'}^* > 0$, then
    $$
    b_{ij}\left(1-
    f_k\left(
    \frac{y_j}{\budget_j}
    + \sum_{i':(i',j)\in E_k}
    \frac{b_{i' j}x^*_{k, i' j}}{\budget_j}
    \right)
    \right)=
    b_{ij'}\left(1-
    f_k\left(
    \frac{y_{j'}}{\budget_{j'}} + \sum_{i':(i',j')\in E_k}
    \frac{b_{i' j'}x^*_{k,i' j'}}{\budget_{j'}}
    \right)
    \right)$$
    For each online vertex $i\in \Rider_k$,
    if there exists an offline vertex $j$ such that $x_{l,ij}^* > 0$, define 
    $c_{k,i} \triangleq b_{ij}\left(1-
    f_k\left(
    \frac{y_j}{\budget_j}
    + \sum_{i':(i',j)\in E_k}
    \frac{b_{i' j}x^*_{k, i' j}}{\budget_j}
    \right)
    \right)$; otherwise
   \Big($\sum_{j:(i,j)\in E_k}x_{k,ij}^* = 0$\Big),
    define $c_{k,i} \triangleq 0$.
    \item \underline{Monotonicity}:  $\forall~ 
   (i,j)\in E_k$: 
   $$
   c_{k,i} \geq 
   b_{ij}\left(1-
    f_k\left(
    \frac{y_j}{\budget_j}
    + \sum_{i':(i',j)\in E_k}
    \frac{b_{i' j}x^*_{k, i' j}}{\budget_j}
    \right)
    \right)
   $$
    \item \underline{Saturation}: all online vertices in $\Rider_k^{(1)}$ are fully matched by $\xbf_k^*$, i.e., $\displaystyle\sum_{j:(i,j)\in E_k}x^*_{k,ij}=1, i\in\Rider_k^{(1)}$~.
\end{enumerate}
\end{lemma}
\ifMS \proof{\textsl{Proof.}}
\else \begin{proof}\fi
We first show the uniformity property. 
    Consider any online vertex $i \in \Rider_k^{(1)}$,
    offline vertices $j,j'\in \Driver$ such that
    $x_{k,ij}^* > 0$ and
    $x_{k,ij'}^* > 0$.
    By construction, $j,j'\in \Driver_k^{(1)}$.
    Thus, 
    $\gamma^*_{ij}=\gamma^*_{ij'}=0$, because of the complementary slackness in \Cref{prop:kkt}). Also, $\theta^*_j=\theta^*_{j'}=0$, again because of complementary slackness and the fact that $y_j+\sum_{i:(i,j)\in E_k}x^*_{k,ij}<1$ and $y_{j'}+\sum_{i: (i,j')\in E_k}x^*_{k,ij'}<1$.
Applying the stationarity condition in \Cref{prop:kkt}, we have:
\begin{align*}
 &b_{ij}\left(1-
    f_k\left(
    \frac{y_j}{\budget_j}
    + \sum_{i':(i',j)\in E_k}
    \frac{b_{i' j}x^*_{k, i' j}}{\budget_j}
    \right)
    \right)
-\lambda^*_i-\theta^*_j+\gamma^*_{ij}\\
=&~0
=
 b_{ij'}\left(1-
    f_k\left(
    \frac{y_{j'}}{\budget_{j'}} + \sum_{i':(i',j')\in E_k}
    \frac{b_{i' j'}x^*_{k,i' j'}}{\budget_{j'}}
    \right)
    \right)
-\lambda^*_i-\theta^*_{j'}+\gamma^*_{ij'}~,
\end{align*}
which
    finishes the proof of the uniformity property for 
    $i\in \Rider_k^{(1)}$. 
    

Now fix any online vertex $i\in \Rider_k^{(0)}$ and
offline vertex $j\in \Driver$ such that 
$x_{k,ij}^*$.
By complementary slackness, $\gamma_{ij}^* = 0$.
If $j\in \Driver_k^{(0)}$, then
$$
    b_{ij}\left(1-
    f_k\left(
    \frac{y_j}{\budget_j}
    + \sum_{i':(i',j)\in E_k}
    \frac{b_{i' j}x^*_{k, i' j}}{\budget_j}
    \right)
    \right)
    =b_{ij}(1 - f_k(1))=0.$$ 
    Due to stationarity condition, we know that 
    $\lambda_i^* = 0$. 
    If $j\in \Driver_k^{(1)}$, due to complementary slackness, we know that $\theta_j^* = 0$.
    Thus, applying stationarity condition again,
    we conclude that 
    $$    b_{ij}\left(1-
    f_k\left(
    \frac{y_j}{\budget_j}
    + \sum_{i':(i',j)\in E_k}
    \frac{b_{i' j}x^*_{k, i' j}}{\budget_j}
    \right)
    \right) = \lambda_i^* + \theta_j^* - \gamma_{ij}^* = 0.$$
    

    To show saturation property, 
    for any online vertex $i\in \Rider_k^{(1)}$,
    there should exist an offline vertex $j\in \Driver_k^{(1)}$
    such that $x_{k,ij}^* > 0$.\footnote{Without
    loss of generality, in this paper we assume that every online vertex
    has at least one edge to offline vertex set $\Driver$.}
    Note that $\lambda^*_i=
     b_{ij}\left(1-
    f_k\left(
    \frac{y_j}{\budget_j}
    + \sum_{i':(i',j)\in E_k}
    \frac{b_{i' j}x^*_{k, i' j}}{\budget_j}
    \right)
    \right)$ by stationarity condition of \Cref{prop:kkt}.
    Since $f_k(1)=1$, $f_k(x)$ is (strictly) monotone increasing
    and 
    $    \frac{y_j}{\budget_j}
    + \sum_{i':(i',j)\in E_k}
    \frac{b_{i' j}x^*_{k, i' j}}{\budget_j} < 1$,
    we know $\lambda_i^* > 0$.
    Again, by using complementary slackness, we have $\sum_{j:(i,j)\in E_k}x^*_{k,ij}=1$, which proves the saturation property.


Fix any $(i, j)\in E_k$ such that $x_{k,ij}^* = 0$.
Again, there should 
exist an offline vertex $j'\in\Driver$ 
so that $x^*_{k,ij}>0$. 
Because of complementary slackness $\gamma^*_{ij'}=0$. 
Now, by writing the stationarity condition of \Cref{prop:kkt} for the edge $(i,j)$,
we have:
$$
   b_{ij}\left(1-
    f_k\left(
    \frac{y_j}{\budget_j}
    + \sum_{i':(i',j)\in E_k}
    \frac{b_{i' j}x^*_{k, i' j}}{\budget_j}
    \right)
    \right)
    -\lambda^*_i-\theta^*_{j}+\gamma^*_{ij}=0~,
$$
By writing the same condition for the edge $(i,j')$, due
to uniformity property, we have: 
$$
c_{k,i} - \lambda^*_i - \theta^*_{j'}=0~,
$$
and therefore 
\begin{align*}
c_{k,i}&\geq c^{(l)}-\theta^*_{j'}
=b_{ij}\left(1-
    f_k\left(
    \frac{y_j}{\budget_j}
    + \sum_{i':(i',j)\in E_k}
    \frac{b_{i' j}x^*_{k, i' j}}{\budget_j}
    \right)
    \right)-\theta^*_{j}+\gamma^*_{ij}\\
&\geq 
b_{ij}\left(1-
    f_k\left(
    \frac{y_j}{\budget_j}
    + \sum_{i':(i',j)\in E_k}
    \frac{b_{i' j}x^*_{k, i' j}}{\budget_j}
    \right)
    \right)-\theta^*_{j}
\end{align*}
If $j\in\Driver_k^{(0)}$, 
then clearly $c_{k,i}\geq 0= 
b_{ij}\left(1-
    f_k\left(
    \frac{y_j}{\budget_j}
    + \sum_{i':(i',j)\in E_k}
    \frac{b_{i' j}x^*_{k, i' j}}{\budget_j}
    \right)
    \right)$. 
If $j\in \Driver_k^{(1)}$, then $\sum_{i': (i',j)\in E_k}x^*_{i'j}+y_{j}<1$ 
and $\theta^*_{j}=0$ because of complementary slackness. 
% Therefore, $c_{k,i}\geq 
% b_{ij}\left(1-
%     f_k\left(
%     \frac{y_j}{\budget_j}
%     + \sum_{i':(i',j)\in E_k}
%     \frac{b_{i' j}x^*_{k, i' j}}{\budget_j}
%     \right)
%     \right)$, which 
    This finishes the proof of the monotonicity property.
\ifMS \Halmos \fi

\ifMS
\endproof
\else
\end{proof}
\fi

We now present the proofs of \Cref{thm:adwords fractional} and \Cref{thm:adwords integral},
which are for fractional and integral algorithms, respectively.


\ifMS \proof{\textsl{Proof of \Cref{thm:adwords fractional}.}}
\else \begin{proof}[Proof of \Cref{thm:adwords fractional}]\fi
For each stage $k\in[K-1]$, let 
$\{x_{k, ij}^*\}_{(i,j)\in E_k}$
be the optimal solution of the program~\ref{eq:concave-adwords-k}. 
First, we define the following notations which will be useful in this proof:
\begin{align*}
\forall j\in \Driver,~k\in[K]:\quad\quad\quad 
& y^*_{k,j}\triangleq\sum_{s=1}^{k-1}\sum_{i:(i,j)\in E_s}
b_{ij} x^*_{s,ij}.
\end{align*}

Now consider the offline primal-dual linear program \ref{eq:LP-max-weight adwords}.
\begin{equation}
\tag{\textsc{Primal-Dual-AdWords}}
\label{eq:LP-max-weight adwords}
\arraycolsep=1.4pt\def\arraystretch{1}
\begin{array}{llllllll}
\max\quad\quad\quad&\displaystyle\sum_{(i,j)\in E}
b_{ij}x_{ij} &~~\text{s.t.}&
&\quad\quad\text{min}\quad\quad\quad &\displaystyle\sum_{i\in \Rider }{\alpha_i}+\displaystyle\sum_{j\in \Driver}{\budget_j\beta_j}&~~\text{s.t.} \\[1.4em]
 &\displaystyle\sum_{j:(i,j)\in E}{x_{ij}}\leq1 &~~i\in\Rider~,& 
& &\alpha_i+b_{ij}\beta_j\geq b_{ij}& (i,j)\in E~,\\[1.4em]
 &\displaystyle\sum_{i:(i,j)\in E}
 {b_{ij}x_{ij}}\leq \budget_j &~~j\in \Driver~, &
& &\alpha_i\geq 0 &i\in \Rider~, \\
 &x_{ij} \geq 0 &(i,j)\in E~. &
& &\beta_j\geq 0  &j\in \Driver~. 
\end{array}
\end{equation}
Once again, 
given the feasible primal (fractional) assignment $\{\xbf^*_k\}_{k\in[K]}$ produced by \Cref{alg:adwords fractional}, we construct a dual assignment so that,
\begin{itemize}
    \item Primal and dual have the same objective values: $\displaystyle\sum_{k\in[K]}\displaystyle\sum_{(i,j)\in E_k}
    b_{ij} x^*_{k,ij}=\sum_{i\in\Rider}\alpha_i+\sum_{j\in\Driver}\budget_j\beta_j$~,
    \item Dual is approximately feasible: $\forall (i,j)\in E: \alpha_i+b_{ij}\beta_j\geq \cratio{K}\cdot b_{ij}$~.
\end{itemize}

\noindent[\textit{Step \rom{1}}]~\emph{Dual assignment construction.}
First, set $\alpha_i\gets 0$ and $\beta_j\gets 0$ for all $i\in\Rider,j\in \Driver$. At each stage $k\in[0:K-1]$, update the dual variables as follows:
\begin{align*}
   &\forall i \in \Rider_k: &&
   \alpha_i\gets c_{k,i}
   \\
    &\forall j \in \Driver: &&\beta_{j}\gets\beta_{j}+\Delta\beta_{k,j}\\
    &&&\Delta\beta_{k,j}\triangleq 
    \left(\frac{ y_{k+1,j}^* -  y_{k,j}^*}{\budget_j}\right)
    f_k\left(\frac{ y_{k+1,j}^*}{\budget_j}\right)
\end{align*}
For the last stage $K$, note that $F_K(x)=0$
for all $x\in[0,1]$. Therefore, \Cref{alg:adwords fractional} essentially solves the maximum AdWords problem in the last stage graph $(\Rider_K, \Driver, E_K)$ where each $j\in\Driver$ has initial budget $\budget_j- y^*_{K, j}$. Let $\{\hat{\alpha}_{K,i}, \hat{\beta}_{K,j}\}_{i\in\Rider_K,j\in\Driver}$ 
be the \emph{optimal} dual solution of this LP. Then update the  dual variables as follows:
\begin{align*}
&\forall i\in\Rider_K:~~\alpha_i \gets \hat{\alpha}_{K,i} \\
&\forall j\in \Driver~:~~\beta_j\gets \beta_j+\Delta \beta_{K,j},~~\Delta\beta_{K, j} \triangleq \left(1 - 
\frac{ y^*_{K, j}}{\budget_j}\right)\hat{\beta}_{K,j}
\end{align*}

\noindent[\textit{Step \rom{2}}]~\emph{Comparing objective values in primal and dual.}
we first show that 
the objective value of the above dual assignment
is equal to the objective value of the primal assignment of \Cref{alg:adwords fractional}.
To show this, we consider 
each stage $k$ separately.
For the last stage $K$, 
this holds by construction.
For each stage $k < K$, note that the primal objective value is decomposed across pairs $(\Rider_k^{(l)}, \Driver_k^{(l)})$, $l=0,1$, simply because $x^*_{k,ij}>0$ only if $i$ and $j$ belong to the same pair (\Cref{lemma:structure adwords}). As these pairs partition sets of vertices $\Rider$ and $\Driver$, it is enough to compare the changes in the primal and dual objectives in each pair $(\Rider_k^{(l)}, \Driver_k^{(l)})$ separately. 
Notice that if $i \in \Rider_k^{(0)}$ then 
$c_{k, i} = 0$, and thus,
\begin{align*}
    \Delta(\textrm{Dual})^{(0)}\triangleq\sum_{i \in \Rider^{(0)}_k} \alpha_i
    +
    \sum_{j \in \Driver^{(0)}_k} \budget_j\Delta\beta_{k,j}
    &= 
    \sum_{j \in \Driver^{(0)}_k}\sum_{i:(i,j)\in E_0} b_{ij}x_{k, ij}^*\triangleq\Delta(\textrm{Primal})^{(0)}. 
\end{align*}
Similarly, 
\begin{align*}
     \Delta(\textrm{Dual})^{(1)}&\triangleq
     \sum_{i \in \Rider^{(1)}_k} \alpha_i
    +
    \sum_{j \in \Driver^{(1)}_k}\budget_j \Delta\beta_{k,j}
    =
    \sum_{i \in \Rider^{(1)}_k} c_{k,i}
    +
    \sum_{j \in \Driver^{(1)}_k}\sum_ {i:(i,j)\in E_k} 
    b_{ij}x_{k, ij}^*f_k\left(\frac{y_{k+1,j}^*}{\budget_j}\right)
    \\
    &=
    \sum_{i \in \Rider^{(1)}_k} c_{k,i}
    +
    \sum_{j \in \Driver^{(1)}_k}\sum_ {i:(i,j)\in E_k} 
    x_{k, ij}^*\left(b_{ij} - c_{k,i}\right)\\
    &=\sum_{j\in\Driver_k^{(1)}}\sum_{i:(i,j)\in E_k} 
    b_{ij}x_{k, ij}^*\triangleq \Delta(\textrm{Primal})^{(1)},
\end{align*}
where the last equality uses the saturation property in \Cref{lemma:structure adwords}.

\noindent[\textit{Step \rom{3}}]~\emph{Checking approximate feasibility of dual.}
To show approximate dual feasibility, it is enough to show that for any stage $k\in[K]$ and any arbitrary edge $(i, j) \in E_k$,
\begin{align}
\label{eq:dual constraint feasibility adwords}
    \alpha_i + \sum_{s = 1}^k b_{ij}\Delta\beta_{s, j}
    \geq 
    b_{ij}\left(1-(1-1/K)^K\right)
\end{align}
We next show \eqref{eq:dual constraint feasibility adwords}
holds for $k=1,2,\ldots,K-1$.
Fix any edge $(i,j)\in E_k$, we have:
\begin{align*}
     &\quad~\alpha_i + \sum_{s = 1}^{k}b_{ij}\Delta\beta_{s, j}\\
     &=c_{k,i} + 
    b_{ij}\left(\frac{y_{k+1,j}^* - 
    y_{k,j}^*}{\budget_j}
    \right)
    f_k\left(\frac{y_{k+1,j}^*}{\budget_j}\right)
    +
    \sum_{s= 1}^{k - 1} 
    b_{ij}\left(\frac{y_{s+1,j}^* - 
    y_{s,j}^*}{\budget_j}
    \right)
    f_s\left(\frac{y_{s+1,j}^*}{\budget_j}\right)
    \\
    &\geq 
    b_{ij}\left(1 - 
    f_k\left(\frac{y_{k+1,j}^*}{\budget_j}\right)
    \right)+ 
    b_{ij}\left(\frac{y_{k+1,j}^* - 
    y_{k,j}^*}{\budget_j}
    \right)
    f_k\left(\frac{y_{k+1,j}^*}{\budget_j}\right)
    +
    \sum_{s= 1}^{k - 1} 
    b_{ij}\left(\frac{y_{s+1,j}^* - 
    y_{s,j}^*}{\budget_j}
    \right)
    f_s\left(\frac{y_{s+1,j}^*}{\budget_j}\right)
    \\
    &\geq b_{ij} \cratio{K}~,
\end{align*}
where the first inequality uses monotonicity property in
\Cref{lemma:structure adwords},
and the second equality 
invokes \Cref{lem:polynomial inequality 2} for the sequence: 
$$
0=y^*_{1,j}/\budget_j\leq y^*_{2,j}/\budget_j\leq \ldots \leq 
y^*_{k,j}/\budget_j\leq 1-\sum_{i':(i',j)\in E_k}
x_{k, i'j}^*/\budget_j~.
$$
% \begin{align*}
%      & c_k^{(l)} + 
%     \left(\sum_{i'\in N_k(j)}x_{k, i'j}^*\right)
%     \left(w_j - c_k^{(l)}\right)
%     +
%     \sum_{s' = 1}^{k - 1} \Delta\beta_{s', j} \\
%     &\leq 
%     c_k^{(l')} + 
%     \left(\sum_{i'\in N_k(j)}x_{k, i'j}^*\right)
%     \left(w_j - c_k^{(l)}\right)
%     +
%     \sum_{s' = 1}^{k - 1} \Delta\beta_{s', j} \\
%     &=
%     \alpha_i + \sum_{s' = 1}^{k}\Delta\beta_{s', j}
% \end{align*}

So far, we have shown \eqref{eq:dual constraint feasibility adwords} 
holds for all stages $k < K$.
For the last stage $K$, and any edge $(i, j) \in E_K$,
notice that 
$\alpha_i+b_{ij}\Delta\beta_{K, j}
=\hat{\alpha}_{K,i} + b_{ij}(1 - y^*_{K, j})
\hat\beta_{K, j} \geq 
b_{ij}(1 - y^*_{K, j})$ by construction.
If $y^*_{K, j} = 0$, 
inequality \eqref{eq:dual constraint feasibility adwords} holds.
Otherwise, let $k' < K$ be the largest 
stage smaller than $K$ 
such that 
$\Delta\beta_{k',j} > 0$. By definition, we know that 
$y^*_{k' + 1, j} = y^*_{K,j}$. So we have:
\begin{align*}
    \alpha_i + \sum_{s = 1}^{K}b_{ij}\Delta\beta_{s, j}
    &\geq    
    b_{ij}(1 - y^*_{K, j})
    + \sum_{s = 1}^{K - 1}b_{ij}\Delta\beta_{s, j} = 
    b_{ij}(1 - y^*_{k'+1, j}) + \sum_{s = 1}^{k'}
    b_{ij}\Delta\beta_{s, j} \\
    &\geq 
    b_{ij}(1 - f_s(y^*_{k' + 1, j}))
    + \sum_{s = 1}^{k'}b_{ij}\Delta\beta_{s, j} 
    \geq b_{ij}(1 - (1 - 1/K)^K)~,
\end{align*}
where the first equality uses the fact $\Delta\beta_{s, j} = 0$ for all $s$
between $k' + 1$ and $K - 1$; the second inequality uses the fact that 
that $f_{s}(a) \geq a$ for all $a\in [0, 1]$ and $s\in[K - 1]$, 
and finally the last inequality holds by exactly the same argument as in the case of $k\in[K-1]$.\ifMS \Halmos \fi

\ifMS
\endproof
\else
\end{proof}
\fi

\ifMS \proof{\textsl{Proof of \Cref{thm:adwords integral}.}}
\else \begin{proof}[Proof of \Cref{thm:adwords integral}]\fi
Let 
$\{x_{k, ij}^*\}_{k\in[K],(i,j)\in E_k}$
be the fractional solution generated in \Cref{alg:adwords integral},
i.e., the optimal solution of the program~\ref{eq:concave-adwords-k}
with adjusted budgets $\{(1-\rho)\budget_j\}_{j\in \Driver}$. 
Based on the proof of \Cref{thm:adwords fractional}
for fractional solutions, we know that 
fractional solution 
$\{x_{k, ij}^*\}_{k\in [K], (i,j)\in E_k}$
is a $\cratio{K}$-approximation to 
the optimal objective in the linear program~\ref{eq:LP-max-weight adwords}
(a.k.a., optimal offline)
with adjusted budgets $\{(1-\rho)\budget_j\}_{j\in \Driver}$. 
Thus, $\{x_{k, ij}^*\}_{k\in [K], (i,j)\in E_k}$ 
is a $(1-\rho)\cratio{K}$-approximation
to the optimal offline with original budgets
$\{\budget_j\}_{j\in \Driver}$. 

Let $\{\hat x_{k, ij}^*\}_{k\in[K],(i,j)\in E_k}$
be the integral solution generated in \Cref{alg:adwords integral}.
For any stage $k\in [K]$,
any edge $(i, j) \in E_k$,
note that 
\begin{align*}
    \prob{\hat x_{k,ij}^* = 1} 
    =
    \prob{\text{vertex $j$ is sampled 
    for vertex $i$}}\cdot 
    \prob{\text{there is enough budget 
    for bid $b_{ij}$}}.
\end{align*}
where $\prob{\text{vertex $j$ is sampled 
    for vertex $i$}} = x_{k,ij}^*$
    by construction.
    Applying the multiplicative form of Chernoff bound 
    (\Cref{lem:chernoff}),
    we can lower-bound 
    $\prob{\text{there is enough budget 
    for bid $b_{ij}$}}$
    by $1 - 
    \exp\left(
    -\frac{\rho^2\minbudget}{2-\rho}\right)$.
    Thus, the integral solution
    $\{\hat x_{k, ij}^*\}_{k\in[K],(i,j)\in E_k}$ 
    is $(1 - \rho)(1 - 
    \exp\left(
    -\frac{\rho^2\minbudget}{2-\rho}\right))$-approximation to the optimal offline. 
    Finally, setting 
    $\rho = O\left(\sqrt{\frac{\log(\minbudget)}{\minbudget}}\right)$ 
    for a large enough constant in the big O notation
    finishes the proof.\ifMS \Halmos \fi

\ifMS
\endproof
\else
\end{proof}
\fi

\begin{lemma}[Multiplicative Chernoff Bound, \citealp{C-1952}]
\label{lem:chernoff}
Suppose $X_1,X_2,\ldots,X_t$ are independent random variables taking values in $\{0,1\}$. Let $X$ denote their sum and let $\mu=\expect[]{X}$ denote the sum's expected value. Then for any $\delta>0$,
$$
\prob{X> (1+\delta)\mu}\leq \exp\left(-\frac{\delta^2\mu}{2+\delta}\right)
$$
\end{lemma}

==> tex/apx-algorithms.tex <==
Here we present the algorithms 
for the extensions,
i.e.,
the multi-stage vertex weighted b-matching problem
and 
the multi-stage AdWords problem.

\begin{algorithm}
 	\caption{Polynomial Regularized Max Weight b-Matching (\PRMWBM)}
 	\label{alg:b-matching integral}
 	\KwIn{Number of batches/stages $K$,
 	Integral solution flag $\texttt{\textsl{Flag}}$.}
%  	\vspace{1mm}
%  	\KwOut{SS.}
 	    \vspace{2mm}
 	    
    $\forall j\in\Driver:~y_j\gets 0$.

 	\vspace{1mm}
 	\For{stage $k=1$ to $K$}
 	{
 	\vspace{2mm}
 	\tcc{$k^{\textrm{th}}$ batch of vertices in $\Rider$, denoted by $\Rider_k$, arrives. Let $E_k$ denote the set of edges incident to vertices in $\Rider_k$.}
 	\vspace{2mm}
 	
   Given $\{y_j\}_{j\in \Driver}$ and subgraph $G_k=(\Rider_k,\Driver,E_k)$, solve $\xbf_k^*$ from
   the convex program~\ref{eq:concave-k-bmatching integral}.

\If{$\texttt{Flag} == \text{False}$}{
$\forall j\in \Driver: y_j\gets y_j+\displaystyle\sum_{i\in\Rider_k}x^*_{k,ij}$.

Return $\xbf^*_k$ as the fractional b-matching allocation of stage $k$.
}
\Else{
Given $\xbf^*_k$, and
structural decomposition 
$\{(\Rider_k^{(l)}, \Driver_k^{(l)}\}_{l\in [0:L_k]}$, 
solve optimal vertex $\hat\xbf_k^*$ from
the linear program~\ref{eq:rounding k-bmatching} for all $l\in [0:L_k]$.

$\forall j\in \Driver: y_j\gets y_j+\displaystyle\sum_{i\in\Rider_k}\hat x^*_{k,ij}$.

Return $\hat\xbf^*_k$ as the integral b-matching allocation of stage $k$.
}
}
\end{algorithm}


\begin{algorithm}
 	\caption{Polynomial Regularized Fractional AdWords (\PRFAD)}
 	\label{alg:adwords fractional}
 	\KwIn{Number of batches/stages $K$}
%  	\vspace{1mm}
%  	\KwOut{SS.}
 	    \vspace{2mm}
 	    
    $\forall j\in\Driver:~y_j\gets 0$.

 	\vspace{1mm}
 	\For{stage $k=1$ to $K$}
 	{
 	\vspace{2mm}
 	\tcc{$k^{\textrm{th}}$ batch of vertices in $\Rider$, denoted by $\Rider_k$, arrives. Let $E_k$ denote the set of edges incident to vertices in $\Rider_k$.}
 	\vspace{2mm}
 	



   Given $\{y_j\}_{j\in \Driver}$ and subgraph $G_k=(\Rider_k,\Driver,E_k)$, solve $\xbf_k^*$
   from
   the convex program~\ref{eq:concave-adwords-k}.

$\forall j\in \Driver: y_j\gets y_j+\displaystyle\sum_{i\in\Rider_k}b_{ij}x^*_{k,ij}$.

Return $\xbf^*_k$ as the fractional AdWords allocation of stage $k$.

}
\end{algorithm}

\begin{algorithm}
 	\caption{Polynomial Regularized Integral AdWords (\PRIAD)}
 	\label{alg:adwords integral}
 	\KwIn{Number of batches/stages $K$, parameter $\rho\in[0,1]$}
%  	\vspace{1mm}
%  	\KwOut{SS.}
 	    \vspace{2mm}
 	    
    $\forall j\in\Driver:~y_j\gets 0,
    \hat y_j \gets 0$.
    
%     $\rho = \underset{\rho\in[0,1]}{\argmin}
% ~1-\left(1-\rho\right)\left(1 - \exp\left(-\frac{\rho^2\minbudget}
%     {2-\rho}\right)\right)$.

 	\vspace{1mm}
 	\For{stage $k=1$ to $K$}
 	{
 	\vspace{2mm}
 	\tcc{$k^{\textrm{th}}$ batch of vertices in $\Rider$, denoted by $\Rider_k$, arrives. Let $E_k$ denote the set of edges incident to vertices in $\Rider_k$.}
 	\vspace{2mm}
 	

    Given $\{y_j\}_{j\in \Driver}$ and subgraph  $G_k=(\Rider_k,\Driver,E_k)$, solve $\xbf_k^*$
   from
   the convex  program~\ref{eq:concave-adwords-k} with
    adjusted budgets $\{(1-\rho)\budget_j\}_{j\in \Driver}$,
    and used budgets $\{y_j\}_{j\in \Driver}$.
    
    $\hat\xbf_k^* \gets \mathbf 0$.
    
 	\For{online vertex $i \in \Rider_k$}{
 	Sample offline vertex $j\sim \{x_{k,ij}^*\}_{j:(i,j)\in E_k}$.
 	
 	\If{$\hat y_j + b_{ij} \leq \budget_j$}{
 	    $\hat x_{k,ij}^* \gets 1$.
 	    
 	    $\hat y_j \gets \hat y_j + b_{ij}$.
 	}
 	}

$\forall j\in \Driver: y_j\gets y_j+\displaystyle\sum_{i\in\Rider_k} b_{ij}x^*_{k,ij}$.

Return $\hat\xbf^*_k$ as the integral AdWords allocation of stage $k$.

}
\end{algorithm}

==> tex/apx-b-matching-proof.tex <==
\subsection{Proof of \texorpdfstring{\Cref{thm:b-matching integral}}{Lg}}
\label{apx:b-matching}

The proofs of the competitive ratio of the fractional
solution in \Cref{thm:b-matching integral}
is similar to 
the analog
proof in \Cref{sec:vertex-weight}.
Thus, we omit it and only show  
the proof of the competitive ratio of 
the integral solution in \Cref{thm:b-matching integral}.






\ifMS \proof{\textsl{Proof of \Cref{thm:b-matching integral} for integral solutions.}}
\else \begin{proof}[Proof of \Cref{thm:b-matching integral} for integral solutions]\fi
For each stage $k\in[K-1]$, let $\{(\Rider^{(0)}_k, \Driver^{(0)}_k),\dots, (\Rider^{(L_k)}_k, \Driver^{(L_k)}_k)\}$ be the 
structural decomposition of $(\Rider_k, \Driver, E_k)$ as in \Cref{lemma:structure budgeted allocation},
and $\{x_{k, ij}^*\}_{(i,j)\in E_k}$
be the optimal (fractional) solution of the program~\ref{eq:concave-k-bmatching integral}
and $\{\hat x_{k, ij}^*\}_{(i,j)\in E_k}$
be the optimal (integral) solution of the 
program~\ref{eq:rounding k-bmatching}. 
First, we define the following notations which will be useful in this proof:
\begin{align*}
\forall j\in \Driver,~k\in[K]:\quad\quad\quad 
&\hat y^*_{k,j}\triangleq\sum_{s=1}^{k-1}\sum_{i:(i,j)\in E_s}
\hat x^*_{s,ij},
\quad\quad\quad 
y^*_{k,j}\triangleq\sum_{s=1}^{k-2}\sum_{i:(i,j)\in E_s}
\hat x^*_{s,ij} + 
\sum_{i:(i,j)\in E_{k-1}}x^*_{k-1,ij}
% ,\\
%  &y^*_{0,j}=0.
\end{align*}

Now consider the offline primal-dual linear program \ref{eq:LP-max-weight b-matching}.
\begin{equation}
\tag{\textsc{Primal-Dual-bmatching}}
\label{eq:LP-max-weight b-matching}
\arraycolsep=1.4pt\def\arraystretch{1}
\begin{array}{llllllll}
\max\quad\quad\quad&\displaystyle\sum_{(i,j)\in E}w_jx_{ij} &~~\text{s.t.}&
&\quad\quad\text{min}\quad\quad\quad &\displaystyle\sum_{i\in \Rider }{\alpha_i}+\displaystyle\sum_{j\in \Driver}{\budget_j\beta_j}&~~\text{s.t.} \\[1.4em]
 &\displaystyle\sum_{j:(i,j)\in E}{x_{ij}}\leq1 &~~i\in\Rider~,& 
& &\alpha_i+\beta_j\geq w_j& (i,j)\in E~,\\[1.4em]
 &\displaystyle\sum_{i:(i,j)\in E}{x_{ij}}\leq \budget_j &~~j\in \Driver~, &
& &\alpha_i\geq 0 &i\in \Rider~, \\
 &x_{ij} \geq 0 &(i,j)\in E~. &
& &\beta_j\geq 0  &j\in \Driver~. 
\end{array}
\end{equation}
Once again, 
given the feasible primal (integral) assignment $\{\hat\xbf^*_k\}_{k\in[K]}$ produced by \Cref{alg:b-matching integral}, we construct a dual assignment so that,
\begin{itemize}
    \item Primal and dual have the same objective values: $\displaystyle\sum_{k\in[K]}\displaystyle\sum_{(i,j)\in E_k}w_j\hat x^*_{k,ij}=\sum_{i\in\Rider}\alpha_i+\sum_{j\in\Driver}\budget_j\beta_j$~,
    \item Dual is approximately feasible: $\forall (i,j)\in E: \alpha_i+\beta_j\geq (\cratio{K} - O(1/\minbudget))\cdot w_j$~.
\end{itemize}

\noindent[\textit{Step \rom{1}}]~\emph{Dual assignment construction.}
First, set $\alpha_i\gets 0$ and $\beta_j\gets 0$ for all $i\in\Rider,j\in \Driver$. At each stage $k\in[0:K-1]$, update the dual variables as follows:
\begin{align*}
   &\forall i \in \Rider^{(l)}_k,~l\in[0:L_k]: &&
   \alpha_i\gets \frac{1}{|\Rider^{(l)}_k|}
   \sum_{j\in \Driver_k^{(l)}}
       \left({\hat y_{k+1,j}^* - \hat y_{k,j}^*}\right)
    \left(1 - 
    f_k\left(\frac{\hat y_{k+1,j}^* - 1}{\budget_j}\right)
   \right)w_j
   \\
    &\forall j \in \Driver^{(l)},~l\in[0:L_k]: &&\beta_{j}\gets\beta_{j}+\Delta\beta_{k,j}\\
    &&&\Delta\beta_{k,j}\triangleq 
    \left(\frac{\hat y_{k+1,j}^* - \hat y_{k,j}^*}{\budget_j}\right)
    f_k\left(\frac{\hat y_{k+1,j}^* - 1}{\budget_j}\right)
    w_j 
\end{align*}
For the last stage $K$, note that $F_K(x)=0$
for all $x\in[0,1]$. Therefore, \Cref{alg:b-matching integral} essentially solves the maximum vertex weighted b-matching in the last stage graph $(\Rider_K, \Driver, E_K)$ where each $j\in\Driver$ has initial capacity $\budget_j-\hat y^*_{K, j}$. Let $\{\hat{\alpha}_{K,i}, \hat{\beta}_{K,j}\}_{i\in\Rider_K,j\in\Driver}$ 
be the \emph{optimal} dual solution of this LP. Then update the  dual variables as follows:
\begin{align*}
&\forall i\in\Rider_K:~~\alpha_i \gets \hat{\alpha}_{K,i} \\
&\forall j\in \Driver~:~~\beta_j\gets \beta_j+\Delta \beta_{K,j},~~\Delta\beta_{K, j} \triangleq \left(1 - 
\frac{\hat y^*_{K, j}}{\budget_j}\right)\hat{\beta}_{K,j}
\end{align*}

\noindent[\textit{Step \rom{2}}]~\emph{Comparing objective values in primal and dual.}
Note that by construction, the objective values in
primal and dual are equal (for each stage).

\noindent[\textit{Step \rom{3}}]~\emph{Checking approximate feasibility of dual.}
To show approximate dual feasibility, it is enough to show that for any stage $k\in[K]$ and any arbitrary edge $(i, j) \in E_k$,
\begin{align}
\label{eq:dual constraint feasibility b-matching}
    \alpha_i + \sum_{s = 1}^k\Delta\beta_{s, j}
    \geq 
    w_j\left(1-(1-1/K)^K - 3/\minbudget\right)
\end{align}
We next show inequality \eqref{eq:dual constraint feasibility b-matching}
holds for $k \in [K-1]$ 
and $k = K$ with slightly different arguments.
For any $k \in [K - 1]$, $l\in [0:L_k]$,
fix any edge $(\iprime, \jprime) \in E_k$
with 
online vertex $\iprime \in \Rider_k^{(l)}$.
We next 
show the following three inequalities \eqref{eq:dual constraint feasibility budgeted allocation fractional solution},
\eqref{eq:budgeted allocation alpha lower bound} 
and 
\eqref{eq:budgeted allocation beta lower bound}
hold. 
% (i) show that 
\begin{align}
\label{eq:dual constraint feasibility budgeted allocation fractional solution}
\begin{split}
    \frac{1}{|\Rider^{(l)}_k|}
    &\sum_{j\in \Driver^{(l)}_k}
    % \left(
    \left(y_{k+1,j}^* - \hat y_{k,j}^*\right)
    \left(1
    - 
    f_k\left(
    \frac{y_{k+1,j}^*}{\budget_{j}}
    \right)
    \right)
    w_j
    % \right) 
    \\
    &+
    \sum_{s = 1}^{k-1}
        \left(
    \frac{\hat y_{s+1,\jprime}^* - \hat y_{s, \jprime}^*}
    {\budget_{\jprime}}
    \right)\cdot 
     f_s
    \left(
    \frac{\hat y_{s + 1,\jprime}^*}
    {\budget_\jprime}\right)w_\jprime
    +
    \left(
    \frac{ y_{k+1,\jprime}^* -  \hat y_{k, \jprime}^*}
    {\budget_{\jprime}}
    \right)\cdot 
     f_k
    \left(
    \frac{ y_{k + 1,\jprime}^*}
    {\budget_{\jprime}}\right)w_\jprime \\
    &\qquad\qquad\qquad 
    \geq \left(1 - (1-1/K)^K\right)w_\jprime
    \end{split}
\end{align}
% (ii) shoaw that
and
\begin{align}
\label{eq:budgeted allocation alpha lower bound}
    \alpha_\iprime \geq 
    \frac{1}{|\Rider^{(l)}_k|}
    &\sum_{j\in \Driver^{(l)}_k}
    % \left(
    \left(y_{k+1,j}^* - \hat y_{k,j}^*\right)
    \left(1
    - 
    f_k\left(
    \frac{y_{k+1,j}^*}{\budget_{j}}
    \right)
    \right)
    w_j
    % \right) 
\end{align}
% and (iii) show that
and
\begin{align}
\label{eq:budgeted allocation beta lower bound}
\begin{split}
    &\sum_{s = 1}^k\Delta\beta_{s, \jprime} +
    \frac{3w_\jprime}{\budget_\jprime} 
    \\
    &\geq  
\sum_{s = 1}^{k-1}
        \left(
    \frac{\hat y_{s+1,\jprime}^* - \hat y_{s, \jprime}^*}
    {\budget_{\jprime}}
    \right)\cdot 
     f_s
    \left(
    \frac{\hat y_{s + 1,\jprime}^*}
    {\budget_\jprime}\right)w_\jprime
    +
    \left(
    \frac{ y_{k+1,\jprime}^* -  \hat y_{k, \jprime}^*}
    {\budget_{\jprime}}
    \right)\cdot 
     f_k
    \left(
    \frac{ y_{k + 1,\jprime}^*}
    {\budget_{\jprime}}\right)w_\jprime 
    \end{split}
\end{align}
Note that combining inequalities \eqref{eq:dual constraint feasibility budgeted allocation fractional solution},
\eqref{eq:budgeted allocation alpha lower bound} 
and 
\eqref{eq:budgeted allocation beta lower bound}
finishes the argument for inequality \eqref{eq:dual constraint feasibility b-matching}
on edge $(\iprime, \jprime) \in E_k$ with $k\in [K-1]$. 

\textsl{Proof of inequality \eqref{eq:dual constraint feasibility budgeted allocation fractional solution}.}
Let $l'\in [0:L_k]$ be the index s.t. 
offline vertex $\jprime \in \Driver_k^{(l')}$.
Due to monotonicity property
in \Cref{lemma:structure budgeted allocation},
we have 
$l \geq l'$ and $c_k^{(l)} \geq c_k^{(l')}$.
First, note that 
\begin{align*}
    c_k^{(l)} = 
    \frac{1}{|\Rider^{(l)}_k|}
    &\sum_{j\in \Driver^{(l)}_k}
    % \left(
    \left(y_{k+1,j}^* - \hat y_{k,j}^*\right)
    \left(1
    - 
    f_k\left(
    \frac{y_{k+1,j}^*}{\budget_{j}}
    \right)
    \right)
    w_j
\end{align*}
due to uniformity and saturation in \Cref{lemma:structure budgeted allocation}.\footnote{For $l = 0$,
the construction of $(\Rider_k^{(0)},\Driver_k^{(0)})$
suggests that 
$y_{k+1,j}^* = \budget_j$ for all $j \in \Driver_k^{(0)}$,
and thus
$\bar f_k\left(
    \frac{y_{k+1,j}^*}{\budget_{j}}
    \right) = 1$, which implies that
    the right hand side equals $c_k^{(0)} = 0$.
    For $l \in [L_k]$,
    since
    $\sum_{j\in \Driver_k^{(l)}}
    \left(y_{k+1,j}^* - \hat y_{k,j}\right) = 
    |\Rider_k^{(l)}|$ (due to saturation) and 
    for all $j\in \Driver_k^{(l)}$
    $w_{j}
    \left(1
    - 
    f_k\left(
    \frac{y_{k+1,j}^* - \hat y_{k,j}^*}
    {\budget_{j}}
    \right)
    \right) = c_k^{(l)}$ (due to uniformity),
    the right hand side equals $c_k^{(l)}$.
}
Hence, 
we can rewrite 
inequality \eqref{eq:dual constraint feasibility budgeted allocation fractional solution}
as 
\begin{align*}
    &c_k^{(l)} +    
    \sum_{s = 1}^{k-1}
        \left(
    \frac{\hat y_{s+1,\jprime}^* - \hat y_{s, \jprime}^*}
    {\budget_{\jprime}}
    \right)\cdot 
     f_s
    \left(
    \frac{\hat y_{s + 1,\jprime}^*}
    {\budget_\jprime}\right)w_\jprime
    +
    \left(
    \frac{ y_{k+1,\jprime}^* -  \hat y_{k, \jprime}^*}
    {\budget_{\jprime}}
    \right)\cdot 
     f_k
    \left(
    \frac{ y_{k + 1,\jprime}^*}
    {\budget_{\jprime}}\right)w_\jprime \\
    &\qquad\qquad\qquad 
    \geq \left(1 - (1-1/K)^K\right)w_\jprime
\end{align*}
which holds since $c_k^{(l)} \geq c_k^{(l')}$
and \Cref{lem:polynomial inequality 2}
for the sequence
$$
0=\hat y^*_{1,\jprime} / \budget_\jprime\leq 
\hat y^*_{2,\jprime}/ \budget_\jprime\leq \ldots \leq 
\hat y^*_{k,\jprime}/ \budget_\jprime\leq 1-\sum_{i:(i,\jprime)\in E_k}
x_{k, i\jprime}^*/ \budget_\jprime~.
$$

\textsl{Proof of inequality \eqref{eq:budgeted allocation alpha lower bound}.}
Since $f_k(\cdot)$ is weakly increasing,
and $y_{k+1,j}^* \geq \hat y_{k+1,j}^* - 1$ by construction,
we have 
$
    f_k\left(
    \frac{y_{k+1,j}^*}{\budget_{j}}
    \right) \geq 
     f_k\left(
    \frac{\hat y_{k+1,j}^* - 1}{\budget_{j}}
    \right)$.
    Thus,
    \begin{align*}
        \alpha_\iprime
        &= \frac{1}{|\Rider^{(l)}_k|}
   \sum_{j\in \Driver_k^{(l)}}
       \left({\hat y_{k+1,j}^* - \hat y_{k,j}^*}\right)
    \left(1 - 
    f_j\left(\frac{\hat y_{k+1,j}^* - 1}{\budget_j}\right)
   \right)w_j \\
   & \geq 
   \frac{1}{|\Rider^{(l)}_k|}
   \sum_{j\in \Driver_k^{(l)}}
       \left({\hat y_{k+1,j}^* - \hat y_{k,j}^*}\right)
    \left(1 - 
    f_j\left(\frac{ y_{k+1,j}^*}{\budget_j}\right)
   \right)w_j \\
   &=
       \frac{1}{|\Rider^{(l)}_k|}
    \sum_{j\in \Driver^{(l)}_k}
    % \left(
    \left(y_{k+1,j}^* - \hat y_{k,j}^*\right)
    \left(1
    - 
    f_k\left(
    \frac{y_{k+1,j}^*}{\budget_{j}}
    \right)
    \right)
    w_j
    \end{align*}
    where
    the last equality uses 
    the fact that 
    $\sum_{j\in \Driver^{(l)}_k}
    % \left(
    \left(\hat y_{k+1,j}^* - \hat y_{k,j}^*\right) = 
    \sum_{j\in \Driver^{(l)}_k}
    % \left(
    \left(y_{k+1,j}^* - \hat y_{k,j}^*\right)$
    (by the construction of $\hat \xbf^*$)
    and 
    uniformity in \Cref{lemma:structure budgeted allocation}.

\textsl{Proof of inequality \eqref{eq:budgeted allocation beta lower bound}.}
We start with the right hand side of inequality
\eqref{eq:budgeted allocation beta lower bound},
\begin{align*}
            &
\sum_{s = 1}^{k-1}
        \left(
    \frac{\hat y_{s+1,\jprime}^* - \hat y_{s, \jprime}^*}
    {\budget_{\jprime}}
    \right)\cdot 
     f_s
    \left(
    \frac{\hat y_{s + 1,\jprime}^*}
    {\budget_\jprime}\right)w_\jprime
    +
    \left(
    \frac{ y_{k+1,\jprime}^* -  \hat y_{k, \jprime}^*}
    {\budget_{\jprime}}
    \right)\cdot 
     f_k
    \left(
    \frac{ y_{k + 1,\jprime}^*}
    {\budget_{\jprime}}\right)w_\jprime 
    \\
    \leq &
\sum_{s = 1}^{k-1}
        \left(
    \frac{\hat y_{s+1,\jprime}^* - \hat y_{s, \jprime}^*}
    {\budget_{\jprime}}
    \right)\cdot 
     f_s
    \left(
    \frac{\hat y_{s + 1,\jprime}^*}
    {\budget_\jprime}\right)w_\jprime
    +
    \left(
    \frac{\hat y_{k+1,\jprime}^* -  \hat y_{k, \jprime}^*}
    {\budget_{\jprime}}
    \right)\cdot 
     f_k
    \left(
    \frac{ y_{k + 1,\jprime}^*}
    {\budget_{\jprime}}\right)w_\jprime 
    +
    \frac{w_\jprime}{\budget_\jprime}
    \\
    \leq&
\sum_{s = 1}^{k-1}
        \left(
    \frac{\hat y_{s+1,\jprime}^* - \hat y_{s, \jprime}^*}
    {\budget_{\jprime}}
    \right)\cdot 
    \left(
     f_s
    \left(
    \frac{\hat y_{s + 1,\jprime}^* - 1}
    {\budget_\jprime}\right)
    +
    \frac{1}{\budget_\jprime}
    \right)w_\jprime \\
    &\qquad\qquad\qquad\qquad\qquad\qquad
    +
    \left(
    \frac{\hat y_{k+1,\jprime}^* -  \hat y_{k, \jprime}^*}
    {\budget_{\jprime}}
    \right)\cdot 
    \left(
     f_k
    \left(
    \frac{\hat y_{k + 1,\jprime}^* - 1}
    {\budget_{\jprime}}\right)
    + \frac{2}{\budget_\jprime}
    \right)
    w_\jprime 
    +
    \frac{w_\jprime}{\budget_\jprime}
      \\
      =&
      \sum_{s=1}^k \Delta\beta_{s, \jprime}
      +
      \frac{\hat y_{k, \jprime}^*}
      {\budget_\jprime
      }
      \frac{w_\jprime}{\budget_\jprime}
      +
      \frac{\hat y_{k+1, \jprime}^*
      -\hat y_{k, \jprime}^*}
      {\budget_\jprime}
      \frac{2w_\jprime}{\budget_\jprime}
      +
      \frac{w_\jprime}{\budget_\jprime}
      \leq 
      \sum_{s=1}^k \Delta\beta_{s, \jprime} + \frac{3w_\jprime}{\budget_\jprime}
\end{align*}
where the first inequality 
uses the fact that $f_k(a) \leq 1$ 
for all $a\in[0, 1]$ and 
$\hat y_{k+1,\jprime}^* \geq 
 y_{k+1,\jprime}^*- 1$ by construction;
the second inequality uses the fact that
$f_k'(a) \in [0, 1]$ for all $a \in [0, 1]$.

% Therefore, combining step (i), (ii) and (iii), 
% we finish the argument that inequality \eqref{eq:dual constraint feasibility budgeted allocation}
% holds for $k < K$ case.

In $k = K$ case, 
consider any edge $(\iprime, \jprime) \in E_K$.
Notice that 
$\alpha_\iprime + \Delta\beta_{K, \jprime} \geq 
w_j\left(1 - \frac{\hat y_{K, \jprime}^*}
{\budget_\jprime}\right)$ by construction.
If $\hat y_{K, \jprime}^* = 0$, inequality \eqref{eq:dual constraint feasibility b-matching} holds immediately.
Otherwise, let $k' < K$ be the largest 
stage  
such that 
$\hat y_{k', \jprime}^* < 
\hat y_{k' + 1, \jprime}^* =
\hat y_{K, \jprime}^*$.
By construction, we know that
$\Delta\beta_{s,\jprime} = 0$
for all $s\in [k' + 1, K - 1]$.
Note that
\begin{align*}
    \alpha_i + \sum_{s = 1}^{K}
    \Delta\beta_{s, \jprime}
    &\geq    
    w_j\left(1 - 
    \frac{\hat y_{K, \jprime}^*}
    {\budget_\jprime}\right)
    + \sum_{s = 1}^{K - 1}
    \Delta\beta_{s, \jprime} 
    \\
    &= 
    w_j\left(1 - 
    \frac{\hat y_{k' + 1, \jprime}^*}
    {\budget_\jprime}\right)
    + \sum_{s = 1}^{k'}
    \Delta\beta_{s, \jprime}
    \\
    &\geq
    w_j\left(1 - 
    f_{k'}\left(\frac{\hat y_{k'+1, \jprime}^*}
    {\budget_\jprime}\right)\right)
    + \sum_{s = 1}^{k'}
    \Delta\beta_{s, \jprime}
    \\
    &\geq
    \left(1 - (1 - 1/K)^K\right)w_\jprime - 
    \frac{3w_j}
    {\budget_\jprime}
\end{align*}
where the third inequality uses the fact 
that $f_{s}(a) \geq a$ for all $a\in [0, 1]$
and $s \in [K - 1]$; and 
the fourth inequality uses the similar argument as in 
$k \in [K-1]$ case.\ifMS \Halmos \fi

\ifMS
\endproof
\else
\end{proof}
\fi


==> tex/b-matching.tex <==
Recall that the multi-stage vertex weighted b-matching
problem is a variant of 
the multi-stage vertex weighted matching 
where the matching constraint 
of each offline vertex $j\in\Driver$ is 
replaced with a capacity constraint $\budget_j$.
Let $\minbudget=\min_{j\in \Driver}\budget_j$
be the smallest capacity.
We
discuss how to modify 
\Cref{alg:b-matching}
to
output fractional solutions
for the $K$-stage vertex weighted b-matching problem
with competitive ratio $\cratio{K}$.
Finally, using a deterministic rounding technique,
we present a deterministic algorithm
that outputs \emph{integral} solutions 
with competitive ratio $
\cratio{K} - O(1/\minbudget)$.


\smallskip
\noindent\textbf{Fractional Multi-stage b-matching~} Consider a modification of 
\Cref{alg:b-matching}, where we replace the convex program~\ref{eq:concave-k-bmatching}
with the modified convex program~\ref{eq:concave-k-bmatching integral}
defined below,
    \begin{align}
 	\label{eq:concave-k-bmatching integral}
 	\tag{$\mathcal{P}^{\text{MWBM}}_k$}
    \begin{array}{lll}
       \xbf^*_k= \underset{\xbf}{\argmax} & 
        \displaystyle\sum_{(i,j) \in E_k}w_j 
        \frac{x_{ij}}{\budget_j} - \sum_{j\in \Driver}w_j F_k\left(\frac{y_j}{\budget_j}+
        \sum_{i : (i,j)\in E_k}\frac{x_{ij}}{\budget_j}\right)
        & \text{s.t.}\\
         &\displaystyle
         \sum_{j: (i,j)\in E_k} x_{ij} \leq 1
         & i\in \Rider_k\\
         & 
         \displaystyle\sum_{i: (i,j)\in E_k} x_{ij} \leq 
         \budget_j-y_j
         & j\in \Driver\\
         &
        x_{ij} \geq 0 &
        (i, j) \in E_k
    \end{array}
\end{align}
Similar to \Cref{sec:vertex-weight},
the convex program \ref{eq:concave-k-bmatching integral}
introduces the following structural decomposition (\Cref{lemma:structure budgeted allocation}).
We omits the proof of this lemma, as it follows exactly the same argument as its analog in the vertex weighted matching problem 
(\Cref{lemma:structure}).
% and its proof in \Cref{apx:skeleton}).
The main difference between \Cref{lemma:structure budgeted allocation} and \Cref{lemma:structure}
is the closed-form expression 
in uniformity property.

\begin{lemma}[{Structural Decomposition/Vertex Weighted b-matching}]
\label{lemma:structure budgeted allocation}
Fix any $k \in [K - 1]$.
Let $\xbf^*_k$ be the optimal solution of the convex program~\ref{eq:concave-k-bmatching integral}. Consider the subgraph $G'_k=(\Rider_k,\Driver,E'_k)$ of $G_k$, where $E'_k=\{(i,j)\in E_k :x^*_{k,ij}>0\}$. Let $\Driver^{(0)}_k$ be the set of offline vertices in $\Driver$ who exhausts their capacities by $\xbf^*_k$ given the current $\ybf$, and 
$\Rider^{(0)}_k$ be the set of online vertices who are neighbors of $\Driver^{(0)}_k$ in $G_k'$, that is, 
$$\Driver^{(0)}_k\triangleq \{j\in \Driver: y_j+\sum_{i:(i,j)\in E_k}x^*_{k,ij}=\budget_j\}~~\textrm{and}~~\Rider^{(0)}_k\triangleq \{i\in \Rider_k:\exists j\in \Driver^{(0)}_k, x^*_{k,ij}>0\}~.$$
Moreover, let the pairs 
$
\left\{\left(\Rider_k^{(l)},\Driver_k^{(l)}\right)\right\}_{l=1}^{L_k}$ 
identify the $L_k$ connected components of the induced subgraph $G_k'[\Rider_k\setminus\Rider_k^{(0)},\Driver\setminus\Driver_k^{(0)}]$ of $G_k'$. Then:
\begin{enumerate}%[label=\roman*.]
    \item \underline{Uniformity}: ~$\forall~ l\in[0:L_k],j,j'\in \Driveri_k:$ $$w_j\left(1-
    f_k\left(
    \frac{y_j}{\budget_j}
    + \sum_{i:(i,j)\in E_k}
    \frac{x^*_{k,ij}}{\budget_j}
    \right)
    \right)=
    w_{j'}\left(1-
    f_k\left(
    \frac{y_{j'}}{\budget_{j'}} + \sum_{i:(i,j')\in E_k}
    \frac{x^*_{k,ij'}}{\budget_{j'}}
    \right)
    \right)\triangleq c_k^{(l)}$$
    \item \underline{Monotonicity}:  $\forall~ l,l'\in[0:L_k]$: there exists no edge in $E_k$ between $\Rider_k^{(l)}$ and $\Driver_k^{(l')}$ if $c_k^{(l)}<c_k^{(l')}$. 
    \item \underline{Saturation}: $\forall~ l\in[L_k]$: all online vertices in $\Rider_k^{(l)}$ are fully matched by $\xbf_k^*$, i.e., $\displaystyle\sum_{j:(i,j)\in E_k}x^*_{k,ij}=1, i\in\Rider_k^{(l)}$~.
\end{enumerate}
\end{lemma}

\smallskip
\noindent\textbf{Rounding to an Integral Allocation~} To output integral solutions 
in 
the $K$-stage vertex weighted b-matching problem, 
we further round the fractional solution $\xbf_k^*$
to an integral solution $\hat\xbf_k^*$
for each stage $k$ as follows.
Let $\{(\Rider^{(0)}_k, \Driver^{(0)}_k),\dots, (\Rider^{(L_k)}_k, \Driver^{(L_k)}_k)\}$ be the 
structural decomposition of $(\Rider_k, \Driver, E_k)$ in \Cref{lemma:structure budgeted allocation}.
For any edge $(i, j)\in E_k$ such that 
$i\in \Rider_k^{(l)}$, $j \in \Driver_k^{(l')}$
and $l\not=l'$, we set $\hat x_{k,ij}^*\gets x_{k,ij}^* = 0$.
Denote the edges between $\Rider_k^{(l)}$ and $\Driver_k^{(l)}$
by $E_k^{(l)}$.
For each subgraph $(\Rider_k^{(l)}, \Driver_k^{(l)}, E_k^{(l)})$,
we set $\{\hat x_{k, ij}^*\}_{(i,j)\in E_k^{(l)}}$ to be an \emph{optimal vertex} of 
the following linear program
\ref{eq:rounding k-bmatching} (which can be found in polynomial time, for example by the simplex algorithm or ellipsoid method):

\begin{align}
 	\label{eq:rounding k-bmatching}
 	\tag{$\mathcal{P}^{\text{rounding}}_{k,l}$}
    \begin{array}{lll}
       \{\hat x_{k, ij}^*\}_{(i,j)\in E_k^{(l)}}= \underset{\xbf}{\argmax} & 
        \displaystyle\sum_{(i,j) \in E_k^{(l)}}x_{ij}
        & \text{s.t.}\\
         &\displaystyle
         \sum_{j: (i,j)\in E_k^{(l)}} x_{ij} \leq 1
         & i\in \Rider_k^{(l)}\\
         & 
         \displaystyle\sum_{i: (i,j)\in E_k^{(l)}} x_{ij} 
         \geq 
         \floor*{
         \displaystyle\sum_{i: (i,j)\in E_k^{(l)}} x_{k,ij}^*
         }
         & j\in \Driver_k^{(l)}\\
         \\
         & 
         \displaystyle\sum_{i: (i,j)\in E_k^{(l)}} x_{ij} 
         \leq 
         \floor*{
         \displaystyle\sum_{i: (i,j)\in E_k^{(l)}} x_{k,ij}^*
         } + 1
         & j\in \Driver_k^{(l)}\\
         &
        x_{ij} \geq 0 &
        (i, j) \in E_k^{(l)}
    \end{array}
\end{align}
where $\floor*{a}$ is the floor function that
outputs the greatest integer less than or equal to $a$.
Note that \ref{eq:rounding k-bmatching}
is a feasible program since $\{ x_{k, ij}^*\}_{(i,j)\in E_k^{(l)}}$
is a feasible solution.
Moreover, it can be easily checked that
the matrix defining the feasibility polytope in \ref{eq:rounding k-bmatching}, with entries in $\{0,\pm 1\}$, 
is indeed a  Totally Unimodular Matrix (TUM)
\citep[cf.][]{sch-03}. As a result, because all the lower-bound and upper-bound constraints are integers, all the vertices of this feasibility polytope are going to be integral.
Thus, $\hat\xbf_k^*$ is an integral optimal solution.
% \YF{Do we need a citation for TUM implying 
% integral solution?}.\RN{We need. Here is a good citation:~\cite{sch-03}}.



We are now ready to show the competitive ratio result of the multi-stage 
vertex weighted b-matching problem. We propose both fractional and integral versions of the \emph{Polynomial Regularized Maximum Weight b-Matching Algorithm} (\PRMWBM) -- see \Cref{alg:b-matching integral} 
% in \Cref{apx:algorithms} 
for a formal description. The analysis of this multi-stage algorithm is technical -- yet with several similarities to the proof of \Cref{thm:b-matching} -- and hence is deferred to \Cref{apx:b-matching}.

\begin{algorithm}
 	\caption{Polynomial Regularized Max Weight b-Matching (\PRMWBM)}
 	\label{alg:b-matching integral}
 	\KwIn{Number of batches/stages $K$,
 	Integral solution flag $\texttt{\textsl{Flag}}$.}
%  	\vspace{1mm}
%  	\KwOut{SS.}
 	    \vspace{2mm}
 	    
    $\forall j\in\Driver:~y_j\gets 0$.

 	\vspace{1mm}
 	\For{stage $k=1$ to $K$}
 	{
 	\vspace{2mm}
 	\tcc{$k^{\textrm{th}}$ batch of vertices in $\Rider$, denoted by $\Rider_k$, arrives. Let $E_k$ denote the set of edges incident to vertices in $\Rider_k$.}
 	\vspace{2mm}
 	
   Given $\{y_j\}_{j\in \Driver}$ and subgraph $G_k=(\Rider_k,\Driver,E_k)$, solve $\xbf_k^*$ from
   the convex program~\ref{eq:concave-k-bmatching integral}.

\If{$\texttt{Flag} == \text{False}$}{
$\forall j\in \Driver: y_j\gets y_j+\displaystyle\sum_{i\in\Rider_k}x^*_{k,ij}$.

Return $\xbf^*_k$ as the fractional b-matching allocation of stage $k$.
}
\Else{
Given $\xbf^*_k$, and
structural decomposition 
$\{(\Rider_k^{(l)}, \Driver_k^{(l)}\}_{l\in [0:L_k]}$, 
solve optimal vertex $\hat\xbf_k^*$ from
the linear program~\ref{eq:rounding k-bmatching} for all $l\in [0:L_k]$.

$\forall j\in \Driver: y_j\gets y_j+\displaystyle\sum_{i\in\Rider_k}\hat x^*_{k,ij}$.

Return $\hat\xbf^*_k$ as the integral b-matching allocation of stage $k$.
}
}
\end{algorithm}

\begin{theorem}[\textbf{Optimal Multi-stage Algorithm for Weighted Bipartite b-matching}]
\label{thm:b-matching integral}
In the $K$-stage fractional (resp.\ integral)
vertex weighted b-matching problem, the fractional (resp.\ integral) version of \PRMWBM ~(\Cref{alg:b-matching integral})
is $\cratio{K}$-competitive 
(resp.\ $\left(\cratio{K} - O(1/\minbudget)\right)$-competitive), where $\cratio{K}=\cratioexp$.
\end{theorem}
\begin{remark}[\textbf{Optimality of the $\boldsymbol{\cratio{K}}$ Competitive Ratio for b-matching}]
Note that the multi-stage vertex weighted
b-matching problem generalizes
the multi-stage 
(fractional) vertex 
weighted matching problem. Therefore
% (i.e., the former approximates the latter
% as $\minbudget\rightarrow\infty$),
\Cref{thm:tightness} implies that
the competitive ratio in \Cref{thm:b-matching integral} 
has the optimal dependence on $K$
in the multi-stage vertex weighted b-matching problem, i.e., no integral or fractional multi-stage algorithm can obtain a competitive ratio better than $\cratio{K}$.
\end{remark}


==> tex/extensions_old.tex <==
\section{Extensions}
\label{sec:extensions Adwords}

In this section,
we discuss how 
our approach can be generalized 
to the multi-stage vertex weighted
b-matching problem, and 
the multi-stage AdWords problem.


\subsection{Multi-stage Vertex Weighted b-Matching}
\label{sec:weighted b-matching}
\input{tex/b-matching}

  
    
    \subsection{Multi-stage AdWords}
    \label{sec:adwords}
    \input{tex/adwords}



==> tex/intro-configuration-allocation.tex <==
\newcommand{\cratio}[1]{\Gamma(#1)}
\newcommand{\cratioexp}{1-\left(1-\frac{1}{K}\right)^K}
\section{Introduction}
\label{sec:intro}
Thanks to ever-expanding popularity of online platforms and growth of web-based services, internet advertising has grown to become a major component of today's economy. Worldwide spending of internet advertising stood at an estimated 378 billion U.S. dollars in 2020---a figure that is forecast to constantly increase in the coming years, reaching a total of 646 billion U.S. dollars by 2024. The combination of the economic impact and the inherent flexibility of internet advertising not only has helped with the prevalence of this form of advertising, but it has also given rise to numerous important computational and economics problems, some of which pertain to real-time algorithmic allocation of ad opportunities to advertisers in various search and display advertising scenarios, e.g., see \cite{MSVV-07,FKMMP-09,BFMM-14,DHKMQ-16}. 

As digital consumption behaviors evolve, and new technologies provide new ways for users to interact with social media platforms and publishers, traditional forms of internet advertising are also being completely transformed. This brings new paradigms and challenges to the real-time ad allocation problem, and enriches the field with new and exciting research questions. A prominent example of this sort, which is the main motivating application behind our paper, is \emph{in-stream video advertising}. Nowadays, in-stream video advertising is rapidly growing,\footnote{According to \citet{Deloitte}, 80\% of U.S. consumers are now paying for streaming video service, up from 73\% before the COVID-19 pandemic began. Using ad spending as an indicator, video advertising will likely continue to grow for the foreseeable future. Video ad spending in the U.S. is increased from 8.92 billion U.S. dollars in 2017 to 10.18 billion U.S. dollars in 2019; it is also projected to reach as high as 12.66 billion U.S. dollars by 2024.} and plays an essential role in the business model of online video sharing platforms such as YouTube and Vimeo, on-demand/live streaming platforms and TVs such as Netflix, Roku, and Twitch, and even social live streaming platforms such as Facebook Live. In this application, when a user starts watching a new video session (e.g., on YouTube), an advertising opportunity to display \emph{video-ads}, and hence allocating user impressions to advertisers, is created. Video-ads refer to all  ad formats that appear before, during, or after a streaming video. These formats include in-stream advertising videos of different lengths, as well as the banner-like overlay and text- or image-based ads that appear over a video. See \Cref{fig:ad-formats} for specific video-ad formats that are currently used in YouTube.\footnote{See \url{https://support.google.com/youtube/answer/2375464?hl=en}}


\captionsetup[subfloat]{captionskip=0pt}
\begin{figure}[hbt!]
	\centering
	\subfloat[
   Skippable in-stream ads
	]{
\includegraphics[scale=0.42]{figs/skippable-video-ads.png}
	}
	\subfloat[Non-skippable in-stream ads]{
\includegraphics[scale=0.42]{figs/non-skippable-video-ads.png}
	}
	\subfloat[
   Bumper short ads
	]
	{
\includegraphics[scale=0.42]{figs/bumper-ads.png}
	}
	\\
	\centering
	\subfloat[
   Overlay ads
	]{
\includegraphics[scale=0.44]{figs/overlay-ads.png}
	}
	\subfloat[
   Clickable sponsored cards
	]{
\includegraphics[scale=0.44]{figs/sponsored-cards.png}
	}
	\vspace{1mm}
	\caption{
Different formats of video advertising in YouTube streaming; These formats can be used at different time-stamps of a YouTube video, and differ in their lengths, designs, and how users interact with them.}
	\label{fig:ad-formats}
\end{figure}

Given these ad format varieties, the real-time ad allocation for a sequence of arriving users is done by assigning each user (or equivalently, each video session) to one of feasible ``configurations". Here, a configuration can refer to an arrangement of video-ads of various lengths and formats for a subset of advertisers, showing up at different time-stamps of the user's video session.\footnote{It can also be the case that a long video session is divided into chunks, and then each chunk is assigned a separate configuration, i.e., is treated as a new video session.}  Particularly important in this application, the set of feasible configurations can model various user-level constraints such as \emph{exclusion} (e.g., competing advertisers can not be shown in the same video), \emph{frequency capping} (e.g., similar ads should not be shown back to back in the same video), or \emph{bundling} (e.g., when advertisers require that all or none of a set of related
ads be shown in the same video). 

While in-stream video ad allocation is a real-time application, it still admits a natural form of allowance for latency in showing ads to users. In fact, as several of these video-ads show up in the middle (or at the end) of users' video sessions, an ad allocator can delay the selection of a configuration for a session (or the current chunk of a long video session) from the beginning of the video to the first time-stamp that a video-ad is required to be displayed. This flexibility provides an immense opportunity for the ad allocator to \emph{batch} the arriving video sessions into large groups without any loss. More formally, a batch consists of the most recent group of users that should be assigned configurations in the same time frame. Given these batches, the ad allocator can make stage-wise allocation decisions as each batch of users arrives---in contrast to fully online decisions as each single user arrives---in order to make more profitable allocation decisions. 

\vspace{3mm}
\noindent\textbf{{Our Theoretical Lens}}~~Motivated by the above application, we study the design of multi-stage allocation algorithms for the configuration allocation problem under adversarial batch arrival. In this problem, we have online users (each corresponds to a new video session) that arrive in $K>0$ batches over a finite horizon,\footnote{We assume the parameter $K$ is fixed and known by the algorithm.} and offline advertisers that have ads to be displayed to the users in order to obtain impressions. Once a batch arrives, the multi-stage allocation algorithm (fractionally or integrally) assigns a feasible configuration to each user in that batch. These decisions are made stage-wise and are irrevocable. Each assigned configuration yields a certain number of impressions to each advertiser and charges the advertiser at a certain price per impression.  The per-impression prices of each feasible configuration assigned to a user, as well as the number of impressions reserved for different advertisers, are revealed when the batch corresponding to this user arrives. Depending on advertisers' long-term contracts, each advertiser is willing to pay for a certain number of impressions during the decision making horizon. Given this model, the goal of the algorithm is maximize the revenue (i.e., total collected prices) in the finite decision making horizon.

We measure the performance of our algorithm by its \emph{competitive ratio}, which is the worst-case ratio between the  revenue of the algorithm and a particular benchmark, given a fixed number of batches. Our goal is to design multi-stage competitive algorithms with respect to the in-hindsight optimal---also known as the optimum offline benchmark. One extreme regime of this problem is the fully offline when there is only a single large batch containing all the users---in which one can achieve the performance of the optimum offline. The other extreme regime is the fully online when each online user arrives as a batch of size one (no batching). While designing optimal competitive (fractional) allocation algorithms for the fully online version has been studied in the literature~\citep{DHKMQ-16}, the middle-ground multi-stage variant with fixed $K$ stages---when allocations are made batch-by-batch---is not studied. We now ask the following informal research question in this paper:

\smallskip
\begin{displayquote}
\emph{In the middle-ground multi-stage regime of configuration allocation problem with batch arrivals (in contrast to fully online and offline regimes), when we have $K >0$ number of batches, what is the optimal competitive ratio achievable by a multi-stage algorithm?}
\end{displayquote}


\vspace{3mm}
\noindent\textbf{{Main Result}}~~
%  \RN{@Yiding: I think what we have is good for a first draft, but it would be better if you can add a bit more technical content. Again, think about ways that either our algorithm or our analysis is creative. Also, it would be helpful to provide more context regarding the algorithm, polynomials we use, and the connection to the recursive equation (it's fine if it has overlap with FN-21; imagine it is very likely that a reviewer hasn't seen our previous paper and should be able to understand what's going on in this paper without looking at that paper. Finally, try to polish the writing of these paragraphs as much as you can while I am polishing the rest of the paper. I will get back to it later.}
As the main result of this paper,
we introduce and analyze an \emph{optimal competitive}
algorithm (\Cref{alg:opt})
for the fractional
multi-stage configuration 
allocation problem, which can easily be extended to the integral version under the large budget assumption (see \Cref{footnote:integral} on Page~9 for more details).
When there are $K$ stages,
\Cref{alg:opt} attains
the competitive ratio of 
$\cratio{K}\triangleq 1 - \left(1 - \frac{1}{K}\right)^K$. This ratio is  optimal for any fixed number of stages $K\in\mathbb{N}$, that is, no multi-stage algorithm---whether fractional or integral---can obtain a better competitive ratio than $\cratio{K}$ even in the special case of the multi-stage matching (thanks to the upper-bound result of \citealp{FN-21} for this special case). The competitive ratio function $\cratio{K} \in (1 - 1/e, 1]$
is monotone decreasing in $K$. 
It is equal to 1 at $K = 1$ and converges 
to $1 - 1/e$ as $K$ goes to infinity. Moreover, for any constant $K$, this ratio has a constant improvement over $1-1/e$ (which is the best achievable bound for the fully online version of this problem, thanks to the main result of \citealp{DHKMQ-16}). For example, this ratio is equal to $\frac{3}{4}$ for the two-stage version of the problem, and is equal to $\frac{19}{27}$ for the three-stage version.

\vspace{3mm}
\noindent\textbf{{Overview of the Techniques}}~~The first key technical ingredient 
in this work is the stage-dependent 
\emph{price-level regularized convex program}
\ref{eq:convex primal}
% stage-dependent convex programs
used in \Cref{alg:opt} for each stage $k\in[K]$.
It identifies a particularly \emph{balanced}
configuration assignment for each stage. 
The intuition behind the necessity of 
balancedness is simple and goes back to the classic work on online bipartite matching and its extensions \citep{KVV-90,KP-00,MSVV-07}. 
Consider a greedy algorithm
which selects the configuration assignment for the 
current stage
to maximizes the total revenue collected so far. 
This greedy algorithm can potentially suffer
a revenue loss due to the lack of enough balancedness, as an adversary can exploit this situation. While balancedness of the allocation in each stage is a property that at high-level should help the multi-stage algorithm to remain competitive against
the future stages constructed by an adversary, it is not clear at all how to use the structure of the problem (in particular, the fact that each advertiser essentially pays for impressions at different price levels) to introduce the required balancedness in each stage. Furthermore, it is not clear how to change the amount of balancedness over the span of $K$ stages. 
We use our convex programs
\ref{eq:convex primal}
to provide remedies for both of these challenges.

The configuration assignment
of the greedy algorithm 
can be solved by a linear program (LP).
Our convex program \ref{eq:convex primal}
is a regularized version of this LP
for the greedy algorithm.
In particular, 
% In these stage-dependent convex programs,
instead of maximizing the total revenue collected so far,
its objective is to maximizing total collected revenue minus a regularization term. This regularization term is the sum of different terms, where we have one regularizer term for each advertiser
at different possible per-impression price levels. 
For any fixed advertiser,
consider a quantity which keeps track of
the number of his impressions at each per-impression price (i.e., the number of impressions at different prices levels that the advertiser is willing to pay so far).
The regularizer term for this advertiser 
is a function
mapping the aforementioned quantity 
to a penalty in the objective of the
convex program \ref{eq:convex primal}
at each stage $k\in[K]$.


Intuitively speaking, 
\Cref{alg:opt} should incorporate ``more intense'' regularization
at early stages and then gradually shift towards no regularization
in the last stage. 
Our convex programs indeed capture such an intuition---it uses a particular sequence of polynomial functions with decreasing degrees
as the regularizer functions of stages $k=1,2,\ldots,K$.
This sequence of polynomial regularizers with decreasing degrees 
has been used in \citet{FN-21}, in which authors 
consider the multi-stage vertex-weighted bipartite matching problem (which is
a special case of our configuration allocation problem).
In their proposed scheme, the regularizers map 
the remaining capacity of each offline node to 
a penalty term in  the objective. 
As we mentioned above, 
in the configuration allocation problem,
the regularizers in \ref{eq:convex primal}
are mappings from 
the number of impressions at different per-impression price levels to non-negative penalties, and hence are of higher dimensions. At high-level, a similar paradigm plays a crucial role in 
\citet{DHKMQ-16},
in
which authors study the configuration allocation problem
with vertex arrival (rather than batch arrival). 
Namely, their model can be thought as the 
special case where
the number of stages $K$
is the number of online nodes 
(a.k.a., users), 
and in each stage only one user arrives.
They provide an optimal $(1-1/e)$-competitive algorithm for this fully online version.
% , which attains optimal competitive ratio in that problem. 
Their algorithm determines the configuration assignment using a continuous iterative method based on an adhoc, yet intuitive, rule.
Kind of surprisingly, as a side result in our paper, we find an alternative interpretation for this algorithm in \citet{DHKMQ-16}: the outcomes of the continuous procedures for each arriving user in
\citet{DHKMQ-16} are precisely captured by the optimal 
solution of our convex programs when we are in the special case of batch arrival with batches of size $1$ and we use \emph{the same exponential function} $f_k(x)=e^{x-1}$ 
as the regularizer functions 
for every single arriving user, rather than our polynomials (see \Cref{thm:main result} and statement of \Cref{alg:opt}).

% For any multi-stage configuration allocation 
% algorithm,
% in each stage, it needs to 
% (i) assign feasible configuration to each user
% arriving in that stage,
% and 
% (ii) keep track of impressions 
% for which each advertiser will pay.\footnote{Different impressions may have 
% different per-impression prices.}
% When there is $K = 1$ stage, 
% the optimal fractional 
% configuration allocation algorithm
% is a two-layer greedy algorithm --
% (i) fixing the impressions allocation, 
% it greedily charges each advertiser
% impressions with highest per-impression
% prices; 
% (ii) given (i) it
% greedily assigns users configurations 
% to maximize the revenue.
% Since the payment are charged 
% at the end of all stages,
% there is no loss 
% to greedily maintain a list of  
% impressions for which advertisers 
% are charged,
% even if there are $K > 1$ stages.
% Specifically, 
% suppose the greedy algorithm decides not to charge 
% an advertiser with an impression with certain per-impression
% price. It must be the case that there exists 
% other impressions with higher per-impression price allocated to this advertiser and fulfilled all his demand.
% As a consequence, the greedy algorithm will not 
% revert its decision and charge for that impression with lower per-impression in the future.
% On the other hand, 
% such two-layer greedy algorithm
% suffers from the lack of balancedness
% on configuration assignment, i.e., (ii).
% Hence, comparing to this two-layer greedy algorithm,
% \Cref{alg:opt} outputs 
% a more balanced configuration assignment
% that not only considers the additional revenue gain
% from the current stage, but also 
% provides hedging against the future stages.

% The outcome of the two-layer greedy algorithm 
% can be solved by a simple linear program.
% To formalize the idea of more balanced 
% configuration allocation,
% \Cref{alg:opt} solves specific convex program 
% \ref{eq:convex primal}
% which determines both 
% the configuration assignment and 
% the chargeable impression
% at each stage. 
% This approach which uses the convex program
% for the current stage decision
% is similar to \citet{FN-21},
% which studies multi-stage 
% fractional vertex-weighted matching.
% In their problem,
% for each stage, 
% the convex program 
% depends on the vector of remaining capacities
% of each offline nodes, and
% finds a feasible matching that maximizes 
% a regularized version of the total weight objective function.
% In contrast, 
% for our multi-stage configuration allocation problem
% (which can be thought as a generalized model 
% of multi-stage vertex-weighted matching),
% our convex program will depends on the chargeable 
% impressions in the previous stage,
% solves for a configuration assignment for the current 
% stage and update the chargeable impressions
% to maximize a similar regularized version of total revenue function.

To prove that \Cref{alg:opt} obtains the optimal competitive ratio of $\cratio{K}$,
we follow the now-universal primal dual analysis framework
\citep[cf.][]{DJK-13}:
we formulate the optimum offline as a linear program \ref{eq:LP primal}
and then consider its dual program \ref{eq:LP}. 
Due to the strong duality of linear programs, to provide a lower bound on the competitive ratio,
it is sufficient to
construct a dual assignment 
such that (i) the dual objective value is equal to the total revenue 
collected by \Cref{alg:opt} and (ii)
the dual constraints are
$\cratio{K}$-approximately satisfied. The main technical challenge, and the second key technical contribution in our paper, is how to connect our convex programs
\ref{eq:convex primal}
in each stage to a LP primal-dual analysis, or in other words, how to construct an approximate LP dual certificate for 
our primal algorithm (i.e., \Cref{alg:opt})
based on its convex-programming based structure.
% It turns out that 
% the optimal solution for the dual program
% of our convex program \ref{eq:convex primal}
% provide 
The constructed dual assignment
in our proposed novel primal-dual analysis 
is closely related to the \emph{theory of Fenchel/Lagrangian convex duality}~\citep[e.g., see][]{BV-04} for our convex programs 
\ref{eq:convex primal}
in \Cref{alg:opt}.


To be more precise and to provide more details, we 
consider the Lagrangian dual program
\ref{eq:convex dual}
of the convex program
\ref{eq:convex primal}, 
and use \emph{exactly} its optimal dual solution
to construct the dual assignment in the 
primal-dual analysis framework.
As a comparison to prior work, 
for the special case of multi-stage vertex-weighted matching,
\citet{FN-21} construct the dual assignment 
using a specific graph decomposition \citep[cf.][]{GKK-12,FN-21}, whose existence
is shown by 
% using 
convex programming. 
However, 
as it turns out, in general models such as edge-weighted matching problem 
or configuration allocation problem, similar convex programs
do not admit any similar structures, and hence do not induce any relevant graph decomposition or base function factorization. Thus, as we mentioned above, 
we use the optimal dual solutions 
in \ref{eq:convex dual}
to directly construct 
the dual assignment for \ref{eq:LP}. Surprisingly, with our proposed dual assignment, we can connect the analysis of the competitive ratio to a recursive functional equation across $K$ stages, which has exactly appeared before in \cite{FN-21}. This is indeed the reason  why a particular choice of polynomial regularizes, which is the solution of this recursive functional equation, attains the optimal $\cratio{K}$ competitive ratio.\footnote{See \cite{FN-21} for more context and the connection between the recursive equation and the mentioned polynomials.} We should highlight that the connection between LP primal-dual analysis and the convex duality in our paper is quite magical, and might be of independent interest in other online algorithm design problems. 







\vspace{3mm}
\noindent\textbf{{Related Literature}}~~Here is a summary of the literature directly related to our work.

\vspace{2mm}
\noindent\emph{Multi-stage matching.}~~Our work is closely related to \cite{feng2020two}, which studies the optimal competitive two-stage vertex weighted matching and pricing under both adversarial and stochastic settings, and \cite{FN-21}, which studies multi-stage fractional vertex-weighted matching under adversarial arrival. The current paper extends the multi-stage algorithm design framework and the convex-programming based recursive primal-dual analysis introduced in these two papers to the more complicated and general setting of configuration allocation problem with preemption (which includes bipartite edge-weighted matching with free-disposal and vertex-weighted matching without free-disposal as special cases). At high-level, our result is also related to the beautiful work of \cite{LS-17}. They diverge from ours as they focus on a different setting, which is the multi-stage bipartite matching and the edge arrival model. Another work that is conceptually related to ours is the recent work of \cite{housni2020matching}, which is inspired by the idea of robust multi-stage optimization~\citep[e.g.,][]{bertsimas2010optimality,bertsimas2011theory}. They consider a two-stage robust optimization for cost-minimization of the matching, where future demand uncertainty is modeled using a set of demand scenarios (specified explicitly or implicitly). Our model and results diverge drastically from this work, which makes them incomparable. 


% \noindent{\emph{Two-stage stochastic programming.}}
% Two-stage stochastic combinatorial
% optimization problems have been studied extensively in the 
% literature
% \citep[e.g.,][]{BL-11, CCP-05,SS-04,SS-07,IKMM-04, hanasusanto2015k,hanasusanto2018conic}.
% Also, see the excellent book of \cite{kuhn2006generalized} for more context regarding convex multi-stage stochastic programs.  For two-stage stochastic matching, various models with different objectives
% have been studied in \citet{KS-06, EGMS-10, KKU-08} and more recently in \cite{feng2020two}. Another work that is conceptually related to our two-stage matching problem is the recent work of \cite{housni2020matching}, which is inspired by the idea of robust multi-stage optimization~\citep[e.g.,][]{bertsimas2010optimality,bertsimas2011theory}. They consider a two-stage robust optimization for cost-minimization of the matching, where future demand uncertainty is modeled using a set of demand scenarios (specified explicitly or implicitly). Our model and results diverge drastically from this work, which makes them incomparable. 


\vspace{2mm}
\noindent\emph{Online bipartite allocations.}~~Our results are comparable to the literature on online bipartite matching (with vertex arrival) and its extensions, which is rooted in the seminal work of Karp, Vazirani, and Vazriani~\citep{KVV-90}. A simple non primal-dual proof of RANKING algorithm of \cite{KVV-90} is presented in \cite{birnbaum2008line}. An elegant primal-dual analysis is discovered later in \cite{DJK-13}. A rich body of literature has extended this simple formulation to more practical or more theoretically challenging two-sided online allocation scenarios such as the online budgeted allocation/AdWords~\citep{MSVV-07,BJN-07,HZZ-20} and the vertex weighted budgeted-matching~\citep{AGKM-11}. Other variants tailored to applications such as display advertising, ride-sharing, assortment optimization, and display advertising are also studied~\citep{FKMMP-09, mehta2012online,MGS-12,GNR-14,DHKMQ-16,HKTWZZ-18,GKMSW-19,FHTZ-20}. We further refer interested readers to a nice survey by \cite{mehta2013online}.

\vspace{2mm}
\noindent\emph{Competitive primal-dual analysis.}~~On the algorithmic side, a sequence of past work have developed an elegant primal-dual competitive analysis framework, which resembles some aspects of our recursive convex-programming based primal-dual analysis~\citep{BJN-07,DJK-13,devanur2012online,devanur2009adwords,esfandiari2015online,HKTWZZ-18,GKMSW-19,FHTZ-20,FNS-19}. The work closely related to ours is \cite{DHKMQ-16}, which basically studies the fully online version of the fractional configuration allocation problem (with preemption), under the name of ``whole page optimization'' (with applications to display ads). They provide the optimal $(1-\frac{1}{e})$-competitive algorithm for this problem and introduce a novel primal-dual framework, which has inspired some of the ideas in the current paper (e.g., regularizing the convex objective at different price levels). See \cite{buchbinder2009design} for a survey on the primal-dual technique in online algorithms, and specifically for designing and analyzing online bipartite allocation algorithms. 





%  Also, at high-level, our primal-dual analysis resembles some aspects of ~\cite{BJN-07,FKMMP-09,devanur2009adwords,devanur2012online,esfandiari2015online,HKTWZZ-18,FNS-19}.
 
%  Other related models are online bipartite stochastic matching~ \citep[e.g.,][]{feldman2009online,bahmani2010improved,MGS-12,mehta2014online,JL-14} and online bipartite matching with stochastic rewards~\citep[e.g.,][]{mehta2012online,goyal2020online,huang2020online}. We refer interested readers to a nice survey by \cite{mehta2013online} for further related work. Finally, related to us is also the literature on stochastic online packing and convex programming with large budgets~\citep[e.g.,][]{FMMS-10,DJSW-11,AD-14}. In particular, the role of concave regularizers have been studied in these settings for different purposes, e.g., fairness~\citep{agrawal2018proportional,balseiro2021regularized}, robustness to adversarial corruptions~\citep{balseiro2020best}, and obtaining blackbox reductions from Bayesian mechanism design to algorithm design~\citep{dughmi2021bernoulli}. 

\vspace{2mm}
\noindent\emph{Video-ads allocation.}
The popularity of in-stream video platforms has ignited 
a new research area related to video-ads, see 
a recent survey by \citet{FOG-21} for a detailed discussion.
There is a limited literature on
the algorithmic study of video-ads allocation.
Comparing to more traditional applications such as display ads,
video-ads (especially in-stream ads) 
have a distinct feature, which is the
need to be shown to the user during the video session.
\citet{DGNR-09} 
introduce the ``online story scheduling'' problem in which
the task is to schedule in-stream ads with 
different time lengths and per-unit prices for a single user in an online 
fashion, and
provide a constant competitive algorithm. 
Further improvements and 
studying other variants of this problem 
have been the focus in the literature, e.g., \citet{AP-19,LMQTYZ-16}.
\citet{BKK-09} study an alternative media scheduling problem 
for multiple users in an offline fashion.
\citet{SKFFC-17}
consider a variant of AdWords problem \citep{MSVV-07},
where each offline node (which is an in-stream ad in their model) is associated with 
a time length and every online node (i.e., a user) can be matched with multiple offline nodes as long as the total time length is below some threshold. 


% \vspace{2mm}
% \noindent\emph{Applications in revenue management and service operations.} From both methodological and application points of view, our work is related to several streams of work that focus to design online allocations and matching algorithms for problems in revenue management and service operations. These work pertain to practical applications in online retail, ride-sharing and other online platforms. Some examples are online assortment optimization (e.g., 
% \citealp{GNR-14,MS-19}), online assortment of reusable resources  (e.g.,
% \citealp{gong2019online,feng2019linear,goyal2020onlineb}), Bayesian online assortment with heterogeneous customers (e.g.,
% \citealp{rusmevichientong2020dynamic,feng2020near}), 
% online assortment with replenishment~\citep{feng2021online}, dynamic pricing with static calendar \citep{MSZ-18}, volunteer crowd-sourcing and nudging~\citep{manshadi2020online}, two-sided assortment optimization~\citep{aouad2020online}, two-stage stochastic matchings and approximate submodular covering for flexible network design~\citep{devalve2021approximate}, primal-dual approaches in the context of analyzing assemble-to-order systems~\citep{devalve2020primal}, online allocation strategies in two-sided media platforms~\citep{alaei2020revenue}, and finally the line of work on dynamic windowed supply-demand matching/queuing---with applications in ride-sharing (e.g., \cite{HKTWZZ-18, ashlagi2019edge,aouad2020dynamic,ozkan2020dynamic,ata2020dynamic,aveklouris2021matching,arnosti2021managing}).











==> tex/intro-old.tex <==
\newcommand{\cratio}[1]{\Gamma(#1)}
\newcommand{\cratioexp}{1-\left(1-\frac{1}{K}\right)^K}
\section{Introduction}
\label{sec:intro}

The process of matching arriving demand requests to the available supply in real-time is a central operational task in two-sided online marketplaces. Example application domains include allocating service requests to providers in platforms such as Uber/Lyft (ride requests to drivers), Amazon (delivery requests to dispatching centers), Microsoft Azure (requested jobs to servers in the cloud) and Google AdWords (keywords queries to advertisers in sponsored search). In these domains, the platform's economical goal is to make matching decisions as new demand arrives, so as to maximize certain objective functions such as efficiency or revenue. While making these over-time decisions, not only the platform should be concerned with respecting the overall supply feasibility constraints such as capacities or budgets, it should also take into account the dynamic or real-time aspect of decision making, and that there exists uncertainty in future arriving demand; these considerations can substantially impact the current decision of the platform, specially if it is aiming to optimize its objective function for the entire decision making horizon.

A canonical formulation to capture gist of some existing tensions in the above dynamic decision making scenarios is the (adversarial) online bipartite matching problem, originated from the seminal work of Karp, Vazirani, and Vazriani~\citep{KVV-90}. In this model, the online and offline vertices simply play the role of the arriving demand requests and the available supply, respectively. A rich body of literature has extended this simple formulation to more practical two-sided online allocation scenarios such as the online budgeted allocation/AdWords~\citep{MSVV-07} and the vertex weighted budgeted-matching~\citep{AGKM-11}. Other extensions and variants tailored to applications such as display advertising, ride-sharing, and assortment optimization are also studied~\citep{FKMMP-09, mehta2012online,MGS-12,GNR-14,HKTWZZ-18}. See \cite{mehta2013online} for a survey. On the algorithmic side, a sequence of past work have developed an elegant primal-dual framework to design and analyze online competitive algorithms in these problems~\citep{BJN-07,DJK-13,devanur2012online}. See \cite{buchbinder2009design} for a survey on the primal-dual technique in online algorithms, and specifically for designing and analyzing online bipartite allocation algorithms. 

A common theme in the above literature, which is practically relevant in truly real-time applications of matching, is that the platform has to match the arriving demand request to the available supply immediately---with almost no delay. However, in applications that allow for some latency---e.g., matching delivery requests to dispatching centers in Amazon or matching user jobs to computing servers in Azure cloud computing platform---the platform can delay its matching decision by \emph{batching} the demand requests. A batch consists of the most recent group of demand requests that are supposed to be matched to the available supply in the same time frame. While dividing the entire real-time sequence of demand requests into less number of batches---and hence larger batches---induces more latency, it clearly helps the platform to make improved matching decisions in terms of efficiency: indeed, real-time decision making with no latency is a special case where each arriving demand request forms a batch of size one; moreover, the offline decision making is also a special case where the entire set of demand requests forms one large batch, allowing for making the most efficient decision by picking the hindsight optimal matching. Even though in the middle-ground regime with a fixed number of batches of arbitrary sizes the efficiency is still less than the hindsight optimal, still the platform can enjoy more efficiency compared to the truly real-time setting---simply because it makes more informed decisions. To see numbers in practice, for example, ridesharing platforms such as Uber~\citep{Uber}, Lyft~\citep{Lyft} and DiDi~\citep{ZHMWZFGY-17} have reported substantial efficiency improvements due to shifting from match-as-you-go to batching-and-matching. Same phenomena is observed and reported in other corners of gig-economy such as cloud computing markets~\citep{AWS} and online food delivery~\citep{joshi2021batching}.\footnote{Notably, batching not only helps with improving the efficiency, it can also help with decreasing various forms of non-operational cost such as waste and environmental costs ~\citep{AWSwaste}}

\vspace{2mm}
\noindent{\textbf{Our Theoretical Lens~}} Motivated by the batching-and-matching paradigm in practice, and also to theoretically study the the inherent trade-off between batching and inefficiency in dynamic allocations, we revisit the literature on (adversarial) online bipartite allocation problems. In particular, we study the \emph{multi-stage} model in the context of the vertex weighted matching, and its extensions to vertex weighted b-matching~\citep{AGKM-11}  and the budgeted allocation problem (also known as the AdWords problem)~\citep{MSVV-07}. In these models, the online vertices are partitioned into $K>0$ fixed number of batches and arrive over the span of $K$ stages, one batch per stage. We study multi-stage matching algorithms that make irrevocable stage-wise matching decisions by allocating the arriving batch of vertices to the offline nodes at each stage. Such an algorithm should also respect the feasibility constraints on the supply side (which can be capacity constraints or budget restrictions, depending on the underlying problem formulation) and the matching constraints on the demand side for each arriving request.



We measure the performance of our algorithms by their \emph{competitive ratio}, which is the worst-case ratio between the expected total weight of the algorithm and a particular benchmark, given a fixed number of batches. Our goal is to design multi-stage competitive algorithms with respect to the in-hindsight optimal matching---also known as the optimal offline benchmark. Considering different degrees of batching by changing the batch sizes and number of stages, one extreme is when there is only a single large batch containing all the demand nodes (maximum batching), in which the algorithm can perform as good as the optimal offline. The other extreme is when each online vertex arrives as a batch of size one (no batching); this is the fully online regime and therefore the competitive ratio of any multi-stage algorithm is at most the best competitive ratio achievable in the online regime (importantly, as a function of the number of online vertices). We now ask the following informal question in this paper:

\vspace{2mm}
\begin{displayquote}
\emph{In the middle-ground multi-stage regime of bipartite allocation problems with batch arrivals (in contrast to fully online and offline regimes), when we have $K>0$ number of batches, what are the optimal competitive ratios achievable by multi-stage algorithms in these problems?}
\end{displayquote}
\vspace{2mm}

For the multi-stage variants of the problems we study, we rely on the standard formulations in \cite{AGKM-11} for the vertex weighted (b-)matching problem and in \cite{MSVV-07, buchbinder2009design} for the budgeted allocation/AdWords problem. See \Cref{sec:prelim} (Model and Notations) for more details. We are mostly interested in fractional $K$-stage algorithms in this paper, as most of our techniques and ideas can be demonstrated easier in this setting. For completeness, we also consider integral $K$-stage algorithms (possibly randomized) under the ``large budgets assumption'' in the vertex weighted b-matching problem, or equivalently under the small bid over budget assumption in the budgeted allocation problem (for details, refer to \Cref{sec:prelim}).

% \noindent{\textbf{Problem Formulations~}}
% An instance of our problems is a bipartite graph $G=(\Rider,\Driver,E)$, where vertices in $\Driver$ are offline and vertices in $\Rider$ arrive in $K\in\mathbb{N}$ batches. At each stage $k\in[K]$, a new batch $\Rider_k\subseteq \Rider$ arrives and reveals all edges incident to vertices in $\Rider_k$. The platform then makes an irrevocable decision by matching each vertex $i\in\Rider_K$ to at most one offline vertex in $\Driver$. This matching can be fractional or integral. The goal is to maximize the weight of the final matching after all batches arrive, while ensuring the feasibility constraints on the offline side. The objective function and the feasibility constraints are specific to the choice of the problem as follows:
% \begin{enumerate}[label=\textit{(\roman*)}]
%     \item \textit{Multi-stage vertex weighted b-matching:} each offline vertex $j\in\Driver$ has a non-negative weight $w_j$ and a capacity (i.e., budget) constraint $B_j$, that is, its matching degree cannot exceed $B_j$. The objective is the sum of weights of (fractionally) matched offline vertices. We also consider the special case of \emph{multi-stage vertex weighted matching}, in which $B_j=1$ for all $j\in\Driver$.
%     \item \textit{Multi-stage AdWords:}  each edge $(i,j)\in E$ has a non-negative weight $b_{ij}$---also known as the bid of $i$ for $j$. Without loss of generality, we assume $b_{ij}\in[0,1]$.\footnote{This assumption is just for simplicity, as it helps with making the large budget assumption in vertex weighted b-matching similar to small bid over budget assumption in the AdWords problem.} Each offline vertex $j\in \Driver$ has a budget constraint $B_j$, that is, the sum of the weights of edges matched to $j$ cannot exceed $B_j$. The objective is simply the total weights of the edges in the (fractional) matching.
% \end{enumerate}



\smallskip
\noindent{\textbf{Our Contributions~}}
 The main contribution of this paper is the following result.
 
\vspace{2mm}
\mybox{
\begin{displayquote}
{\textbf{(Main Result)} For the multi-stage vertex weighted matching with $K$ batches, we propose a fractional $K$-stage algorithm (\Cref{alg:b-matching}) that achieves a competitive ratio of $\cratio{K}\triangleq\cratioexp$. Moreover, by proposing an upper-bound instance, we show that no $K$-stage algorithm, fractional or integral, can have a competitive ratio better than $\cratio{K}$.}
\end{displayquote}}
\vspace{1mm}
\noindent The competitive ratio function $\cratio{K}\in(1-1/e,1]$ is monotone decreasing in $K$. It is equal to $1$ at $K=1$
and converges to $1-1/e$ as $K$ goes to infinity. For the special case of two-stage vertex weighted matching ($K=2$), our algorithm is $3/4$-competitive, which matches the result of \cite{feng2020two}. Also, for three stages ($K=3$), it has a competitive ratio of $19/27\approx 0.704$. To the best of our knowledge, this is the first bound beating $1-1/e\approx 0.63$ in the $K$-stage bipartite matching problems (weighted or unweighted) for any $K>2$.

We further extend our result to the fractional multi-stage vertex weighted b-matching and multi-stage budgeted allocation problems. We obtain these results by proposing natural adaptations of the previous algorithm for vertex weighted matching (\Cref{alg:b-matching integral} and \Cref{alg:adwords fractional}).  Following the same approach as in the vertex weighted matching problem, we show these adaptations are also $\cratio{K}$-competitive for these generalizations/variations of our base problem. Switching to integral allocations, we also design a simple rounding scheme for multi-stage vertex weighted b-matching, and show the resulting multi-stage integral algorithm obtains a competitive ratio no smaller than $\cratio{K}-O\left(\sfrac{1}{B_{\textrm{min}}}\right)$, where $B_{\text{min}}$ is the minimum capacity of an offline node. Finally, we design a different yet another simple rounding scheme for multi-stage budgeted allocation, and show the resulting multi-stage integral algorithm has a competitive ratio no smaller than $\cratio{K}-O\left(\sqrt{\sfrac{\log(B_{\text{min}})}{B_{\text{min}}}}\right)$. Here, $B_{\text{min}}$ should be interpreted as the maximum budget over bid ratio. See \Cref{tab:summary} for a summary of our results and how they are compared with the previous work.
\input{tex/result-table}

\smallskip
\noindent{\textbf{Overview of the Techniques~}} 
A greedy allocation will allocate the arriving batch of demand requests to the available pool of offline supply at each stage $k\in[K]$, so as to maximize the total weight. Such an allocation can potentially suffer from the lack of enough \emph{balancedness} on the supply side---a property that can help the multi-stage algorithm to remain competitive against the adversary in future stages of this dynamic allocation model. Hence, we aim to replace greedy with a more balanced allocation that (i) considers the matching weight of the current stage, and (ii) simultaneously provides \emph{hedging} against the future stages in a controlled fashion.
For the special case of online arrivals, this simple idea is the essence of the celebrated BALANCE algorithm~\citep{MSVV-07,AGKM-11}, which is optimal competitive under online arrivals. 

To systematically extend the above balanced matching idea under the online setting to the multi-stage setting---where a multi-stage algorithm can match multiple vertices of the arriving batch to the offline side---we propose using fractional matchings that are solutions to specific \emph{convex programs} at each stage. Given the vector of remaining capacities (or budgets) upon the arrival of a new batch, each convex program essentially finds a feasible fractional allocation that maximizes a regularized version of the total weight objective function. In particular, in order to favor more balanced fractional allocations, we choose our regularizers to be (strictly) concave functions of the final matching degrees (or allocation levels) of the offline vertices.

Considering the above algorithmic skeleton, one major question is how to pick the strictly concave regularizers to achieve our desired $\cratio{K}$ competitive ratio in $K$ stages. Our intuition suggests that an appropriate multi-stage algorithm requires hedging more in earlier stages and less in later stages, e.g., in the extreme case of the last stage, picking a maximum weight matching is optimal and no balancedness is required. To obtain the desired variation in the balancedness of our allocation, i.e., having a more balanced allocation early on and gradually pushing it towards a greedy allocation in later stages, we use a different regularizer at each stage. Informally speaking, we aim to incorporate ``more intense'' regularization at first and then gradually shift towards no regularization in the course of $K$ stages. To this end, we need to formalize the notion of intensity of regularization. 

Our key technical ingredient that formalizes the above intuitive notion is a particular sequence $f_1,f_2,\ldots,f_K:[0,1]\rightarrow [0,1]$ of \emph{polynomials of decreasing degrees}, where $f_k$ is a polynomial of degree $(K-k)$ associated to stage $k\in[K]$.  See \Cref{prop:poly} and \Cref{fig:poly}. Here, the regularization intensity of each polynomial is essentially governed by its degree---hence our sequences starts with the highest degree and goes in the descending order of polynomial degrees. We identify this sequence using a backward recursive equation (will be detailed later). We then show this sequence \emph{exactly} characterizes the regularizers of the optimal competitive multi-stage fractional algorithm.

More precisely, we use the primitive function $F_k(x)\triangleq\int_{0}^{x}f_k(y)dy$ to map the normalized fractional degree (or normalized allocation level) of each offline vertex to a penalty term in $[0,1]$ at stage $k$. We then subtract the weighted sum of these penalties from the total weight objective function to construct our regularized objective function; see convex programs \ref{eq:concave-k-bmatching} and \ref{eq:concave-adwords-k} for more details. Interestingly, the first-stage polynomial $f_1$ converges to $f(x)= e^{x-1}$ as $K$ goes to infinity. Also, in the special case of batches of size one, replacing the polynomial $f_k$ at all stages with \emph{the same function} $f(x)=e^{x-1}$ recovers the $(1-1/e)$-competitive BALANCE algorithms in \cite{AGKM-11} and \cite{MSVV-07} for the online vertex weighted b-matching and online budgeted allocation, respectively. 

\input{tex/fig-poly}

To analyze our polynomial regularized matching algorithms---inspired by the technique introduced in \cite{feng2020two} for two-stage matching---we use the strong duality of the convex programs, tied to a specific primal-dual analysis that is quite different from the known primal-dual analysis in the literature for various forms of online bipartite allocation problems (e.g., \cite{MSVV-07,AGKM-11,BJN-07}). The sketch of our analysis is roughly the following: The Karush–Kuhn–Tucker (KKT) conditions at each stage $k$ offer a structural decomposition of the subgraph induced by the $k^{\text{th}}$ batch. The special unweighted case of this decomposition coincides with the well-studied \emph{matching skeleton} introduced by~\cite{GKK-12}, which itself is closely related to the Edmonds-Gallai decomposition~\citep{edm-65,gal-64} of bipartite graphs. Using this decomposition, and by carefully using our polynomials $f_1,\ldots,f_k$, we propose a novel \emph{recursive primal-dual framework} to bound the competitive ratio of our fractional matchings. The resulting dual constructions, together with our recursive formulation, shows how to improve the competitive ratios from $(1-1/e)$ to $\cratio{K}$ in the multi-stage setting with $K$ batches. In other words, this new algorithmic construct extends the dual constructions in previous work~\citep{MSVV-07,AGKM-11,BJN-07} in a novel fashion to the multi-stage setting with batch arrivals. As a side dish, our technique provides a convex-programming based interpretation for the existing primal-dual proofs in the special case of the online setting. 

We further show the competitive ratio $\cratio{K}$ is the best achievable by any fractional multi-stage algorithm, whether deterministic or randomized, by showing an upper-bound instance for the special case of the unweighted multi-stage matching. Notably, this instance relies on batches of size more than one, and hence cannot be used as an upper-bound instance for the special case of online arrival where batch sizes are all one. See \Cref{fig:bad-example} for more details.



We finally turn our attention to the integral versions of the vertex weighted b-matching and AdWords problems, when the capacities are large (or equivalently, bid over budget ratios are small). By using the totally unimodularity of flow-type polytopes~\citep{sch-03}, we propose our deterministic rounding algorithm for the vertex weighted b-matching problem. The idea is finding integer lower and upper bounds on the fractional degrees of each offline vertex using the fractional solution of the convex program at each stage, and then searching for an integral matching satisfying these bounds.  For the AdWords problem, we use a straightforward variant of independent randomized rounding at each stage, after slightly reducing all the budgets. By applying standard concentration bounds for each offline vertex, we prove that maintaining feasibility of the resulting integral allocation only adds a small loss in expectation when the bid over budget ratios are small. 

\smallskip
\noindent\textbf{Managerial Insights~} Our study sheds insights on the role of batching in service operation of matching platforms, and provides algorithmic evidences on how they should adaptively tune their batched matching algorithms to achieve the right trade-off between \emph{``greedy-ness''} in the current decision and {``hedging''} for the sake of future decisions:
\begin{itemize}
    \item In settings that allow for latency---and hence allow for batching the demand arrivals---batched matching algorithms (versus fully online algorithms) can be used by the algorithm designer to obtain performance improvements.
    \item There is an inherent trade-off between the gain from batching (which is captured by the competitive ratio in our competitive analysis framework) and the degree of batching (which is captured by the inverse number of batches in our framework): with less number of batches/stages---which accounts for a higher degree of batching---a well-designed multi-stage matching algorithm can obtain a higher performance; moreover, it gets closer to the offline optimal matching as the degree of batching increases.\footnote{Of course, there is no free lunch here and the actual cost of batching is the induced latency in decision making.}
    \item When designing batched matching algorithms, our result suggests that pushing the matching to be more robust to future uncertainty early on (i.e., to be more balanced) and then pushing it to be more greedy later on will help with the performance in a finite horizon problem. In particular, we could formally capture this design aspect using our decreasing degree polynomial regularizers; However, in general, decreasing the degree of hedging induced by the matching algorithm over time to obtain improved performance is the main operational takeaway message of our work, and there might be other ways of performing this task in practice.
\end{itemize}




\smallskip
\noindent\textbf{Organization~} 
In \Cref{sec:vertex-weight}, we introduce our optimal competitive multi-stage algorithm for the vertex weighted bipartite matching problem (\Cref{sec:upper-bound}), then prove a competitive ratio lower bound for this algorithm (\Cref{sec:primal-dual}), and finally show that it \emph{exactly} matches the upper-bound on the competitive ratio of \emph{any} multi-stage algorithm (\Cref{sec:lowerbound}). We then switch to other variants of our base model in \Cref{sec:extensions}, and show the same results for its generalization to b-matching (\Cref{sec:weighted b-matching}) and its variation to multi-stage budgeted allocation/Adwords problem (\Cref{sec:adwords}). 
\subsection{Related Literature} Here is a summary of the literature directly related to our work.

\vspace{2mm}
\noindent\emph{Multi-stage matching.} A work closely related to ours is that of \cite{feng2020two}, which studies the optimal competitive two-stage vertex weighted matching and pricing under both adversarial and stochastic settings. We extend their result in the adversarial case to multi stages and settings beyond vertex weighted matching. Our result for the unweighted multi-stage matching is closely related to the beautiful work of \cite{LS-17}, which also uses the matching skeleton of \cite{GKK-12}, but for a different model. In their model, a batch of \emph{new edges} arrive in each stage. Their proposed algorithm first finds a maximum fractional matching using the matching skeleton in each stage, and then removes some of the edges sampled from this matching through a randomized procedure. This approach obtains an optimal $2/3$ competitive ratio for two stages and a non-optimal $1/2+O(2^{-K})$ competitive ratio for $K$ stages. 
\vspace{2mm}

\noindent{\emph{Two-stage stochastic programming.}}
Two-stage stochastic combinatorial
optimization problems have been studied extensively in the 
literature
\citep[e.g.,][]{BL-11, CCP-05,SS-04,SS-07,IKMM-04, hanasusanto2015k,hanasusanto2018conic}.
Also, see the excellent book of \cite{kuhn2006generalized} for more context regarding convex multi-stage stochastic programs.  For two-stage stochastic matching, various models with different objectives
have been studied in \citet{KS-06, EGMS-10, KKU-08} and more recently in \cite{feng2020two}. Another work that is conceptually related to our two-stage matching problem is the recent work of \cite{housni2020matching}, which is inspired by the idea of robust multi-stage optimization~\citep[e.g.,][]{bertsimas2010optimality,bertsimas2011theory}. They consider a two-stage robust optimization for cost-minimization of the matching, where future demand uncertainty is modeled using a set of demand scenarios (specified explicitly or implicitly). Our model and results diverge drastically from this work, which makes them incomparable. 


\vspace{2mm}
\noindent\emph{Online bipartite allocations.}
Our results are comparable to the literature on online bipartite matching (with vertex arrival) and its extensions. Related to us, \citet{AGKM-11} generalize the classic RANKING algorithm of \cite{KVV-90} to the setting where offline vertices are weighted. A simple non primal-dual proof of RANKING is presented in \cite{birnbaum2008line}. An elegant primal-dual analysis is discovered later in \cite{DJK-13}. Also, at high-level, our primal-dual analysis resembles some aspects of ~\cite{BJN-07,FKMMP-09,devanur2009adwords,devanur2012online,esfandiari2015online,HKTWZZ-18,FNS-19}. Other related models are online bipartite stochastic matching~ \citep[e.g.,][]{feldman2009online,bahmani2010improved,MGS-12,mehta2014online,JL-14} and online bipartite matching with stochastic rewards~\citep[e.g.,][]{mehta2012online,goyal2020online,huang2020online}. We refer interested readers to a nice survey by \cite{mehta2013online} for further related work. Finally, related to us is also the literature on stochastic online packing and convex programming with large budgets~\citep[e.g.,][]{FMMS-10,DJSW-11,AD-14}. In particular, the role of concave regularizers have been studied in these settings for different purposes, e.g., fairness~\citep{agrawal2018proportional,balseiro2021regularized}, robustness to adversarial corruptions~\citep{balseiro2020best}, and obtaining blackbox reductions from Bayesian mechanism design to algorithm design~\citep{dughmi2021bernoulli}. 

\vspace{2mm}
\noindent\emph{Applications in revenue management and service operations.} From both methodological and application points of view, our work is related to several streams of work that focus to design online allocations and matching algorithms for problems in revenue management and service operations. These work pertain to practical applications in online retail, ride-sharing and other online platforms. Some examples are online assortment optimization (e.g., 
\citealp{GNR-14,MS-19}), online assortment of reusable resources  (e.g.,
\citealp{gong2019online,feng2019linear,goyal2020onlineb}), Bayesian online assortment with heterogeneous customers (e.g.,
\citealp{rusmevichientong2020dynamic,feng2020near}), 
online assortment with replenishment~\citep{feng2021online}, dynamic pricing with static calendar \citep{MSZ-18}, volunteer crowd-sourcing and nudging~\citep{manshadi2020online}, two-sided assortment optimization~\citep{aouad2020online}, two-stage stochastic matchings and approximate submodular covering for flexible network design~\citep{devalve2021approximate}, primal-dual approaches in the context of analyzing assemble-to-order systems~\citep{devalve2020primal}, online allocation strategies in two-sided media platforms~\citep{alaei2020revenue}, and finally the line of work on dynamic windowed supply-demand matching/queuing---with applications in ride-sharing (e.g., \cite{HKTWZZ-18, ashlagi2019edge,aouad2020dynamic,ozkan2020dynamic,ata2020dynamic,aveklouris2021matching,arnosti2021managing}).



==> tex/prelim_old.tex <==
\section{Preliminaries}
\smallskip
\label{sec:prelim}
\subsection{Baseline Model: Multi-stage Vertex Weighted Matching}
Our baseline model studies
\emph{multi-stage vertex weighted matching}
--
a bipartite allocation model
for matching arriving demand requests to available suppliers. 
An instance of our model consists of a bipartite graph $\mathcal{G}=(\Rider,\Driver,E)$, where vertices 
in $\Driver$ (supply) are available offline 
and vertices in $\Rider$ (demand) arrive over time. 
Specifically, we consider a \emph{multi-stage arrival} model, 
in which vertices in $\Rider$ arrive in $K\in\mathbb{N}$ stage. 
We assume the number of stages $K$ is fixed and known by the algorithm. At each stage $k\in[K]$, a new subset of online vertices $\Rider_k\subseteq \Rider$ arrive, which we often call an arriving \emph{batch}, and reveal their incident edges in $E$. 
We highlight that $\Rider=\cup_{k\in[K]}\Rider_k $ and $\Rider_k\cap\Rider_{k'}=\emptyset$ for $k\neq k'$. 
After arrival of batch $k$, the multi-stage allocation algorithm makes an irrevocable allocation decision by allocating each vertex $i\in\Rider_K$ (which corresponds to one unit of demand) to the set of \emph{available} neighboring offline vertices $j\in\Driver, (i,j)\in E$ . Let $E_k$ denote the set of edges in $E$ incident to $\Rider_k$. 
We denote the allocation of stage $k$ by the vector $\xbf_{k}\in\mathbb{R}^{E_k}$, where $x_{k,ij}\in[0,1]$ is the amount of allocation of vertex $i$ to $j$. 
This allocation can be fractional or integral. 

Each offline vertex $j\in\Driver$ has a non-negative weight $w_j$ for each unit of allocation. 
The goal of the multi-stage vertex weighted matching
is to maximize the sum of the weight of the offline vertices in the (fractional) allocation, while ensuring the feasibility constraints -- 
every demand/supply vertex can be matched at most 
one unit.

\subsection{Competitive Ratio Analysis}

We measure the performance of our multi-stage algorithms by their \emph{competitive ratio}, which is the worst-case ratio between the expected total weight of the algorithm and the optimum offline benchmark given the entire problem instance (formally defined below).
\begin{definition}[\textbf{Competitive Ratio}]
	\label{def:competitive ratio}
	Fix the number of stages $K\in\mathbb{N}$. For $\alpha\in [0,1]$, a multi-stage allocation algorithm $\ALG$ is \emph{$\alpha$-competitive} against the optimum offline solution in the multi-stage vertex weighted matching problem, if the following holds:
	\begin{align*}
		\inf\limits_{I \in\mathcal{I}}~~
		\frac{\ALG(I)}{\texttt{OPT}(I)}~
		\geq \alpha~,
	\end{align*}
	where $\mathcal{I}$ is the set of instances of the multi-stage vertex weighted matching problem, 
	and $\ALG(I)$ and $\texttt{OPT}(I)$ are the total weights of the multi-stage algorithm $\ALG$ and optimum offline solution on an instance $I$, respectively. 
	For randomized multi-stage algorithms, we abuse the notation and $\ALG(I)$ denotes the expected total weight of the algorithm on an instance $I$.
\end{definition}

 As an important note, we are mainly interested in the competitive ratio of fractional $K$-stage algorithms.
%  We also consider the asymptotic competitive ratio of integral $K$-stage algorithms (possibly randomized) under the ``large budgets assumption'' in the vertex weighted b-matching problem (i.e., under the assumption that $\min_j B_j=\Omega(1)$), or equivalently under the small bid over budget assumption in the budgeted allocation problem (i.e., under the assumption that $\max_{i,j} \frac{b_{ij}}{B_j}=o(1)$ or equivalently $\min_j B_j=\Omega(1)$ when $b_{ij}\in[0,1]$). 

\subsection{A Recursive Sequence of Polynomials}
As a novel technical ingredient of our proposed multi-stage allocation algorithms, we identify a particular sequence of polynomials of decreasing degrees. Our construction of these polynomials is recursive, which gives us a polynomial of degree $K-k$ for each stage $k=1,2,\ldots,K-1$. Here, we introduce these polynomials, describe this underlying recursive equation, and elaborate a bit more on some of their properties (\Cref{prop:poly}, proof in Appendxi~\ref{apx:poly}). Later, we first show in \Cref{sec:vertex-weight} how these polynomials help us to design an optimal competitive multi-stage algorithm for the vertex weighted matching and how to develop a primal-dual analysis framework that incorporates this recursive equation. Then we show how to extend these ideas to use our polynomials for the vertex weighted b-matching (\Cref{sec:weighted b-matching}) and budgeted allocation (\Cref{sec:adwords}) problems.

\begin{proposition}[{\textbf{{Sequence of Polynomial Regularizers}}}]
\label{prop:poly}
Consider a sequence of functions $f_1,f_2,\ldots,f_{K}:[0,1]\rightarrow[0,1]$
satisfying the following backward recursive equation:
\begin{itemize}
    \item $\forall x\in[0,1]:~f_{K}(x)=\mathbb{I}\{{x=1\}}$,
    where $\mathbb{I}(\cdot)$ is 
    the indicator function,
    \item $\forall x\in[0,1], k\in[K-1]:~f_{k}(x)=\underset{y\in[0,1-x]}{\max}~(1-y)f_{k+1}(x+y)$.
\end{itemize}
Then, the following statements hold:
\begin{enumerate}[label=(\roman*)]
    \item The function sequence $\{f_k\}_{k=1}^{K-1}$ is a sequence of $K-1$ polynomials with decreasing degrees, where $f_k(x)=(1-\frac{1-x}{K-k})^{K-k}$ for $k\in[K-1]$.\footnote{As a convention, we refer to $f_K(x)=\mathbb{I}\{x=1\}$ as a polynomial of degree $0$ (although not mathematically rigorous).}
    \item $f_k(x)$ is monotone increasing and continuous over $[0,1]$ for $k\in[K-1]$. Hence, $F_k(x)\triangleq \int_{0}^x f_k(y)dy$ is differentiable and strictly convex over $[0,1]$ for $k\in[K-1]$.
    \item $\forall k\in[K]$, $f_k(x)\leq e^{x-1}$ for $x\in[0,1]$. Moreover, the first function $f_1(x)=(1-\frac{1-x}{K-1})^{K-1}$ converges point-wise from below to the function $e^{x-1}$ as $K\to+\infty$ (see \Cref{fig:poly}).
    \item $\underset{y\in[0,1]}{\min}1-(1-y)f_1(y)=\cratioexp\triangleq\cratio{K}$
\end{enumerate}
\end{proposition}

The aforementioned polynomials $\{f_k\}_{k\in[K-1]}$ are drawn in \Cref{fig:poly}. As it is clear from this figure, these polynomials provide careful point-wise estimations for the exponential function $f(x)=e^{x-1}$ at different levels of precision. When these polynomials are used to regularize the maximum weight matching objective function, they provide different levels of ``hedging'' intensity against the future uncertainty in the arriving input exactly because of these different levels of estimation precision. This point will be clear in the next section.

\subsection{Extension Model: Multi-stage Configuration Allocation}
Motivated by the application of allocating video-ads,
this paper also considers the following
multi-stage configuration allocation problem.
It generalizes our baseline model.

There is a set of (offline) 
advertisers\footnote{Since 
the multi-stage configuration allocation problem
is motivated by the application of allocating video-ads,
we rename online demand vertices
(resp.\ offline supply vertices) in multi-stage vertex weighted matching 
as 
online users
(resp.\ offline advertisers) in this extension model.} 
$\Driver$.
Advertisers  
are willing to pay a video platform
to display their ads to a set of users $\Rider$ who are streaming videos in this platform.
% When a user
% start watching a video, 
% the video platform can allocate 
% impressions (i.e., exposure of a user 
% to a display ad) to advertisers.
% Specifically, we consider
% a \emph{multi-stage} arrival model, 
% in which users in $\Rider$
% arrive in $K\in\N$ stages.
% At each stage $k\in [K]$,
% a new subset of online users $\Rider_k\subseteq\Rider$
% arrives to the video platform.
Specifically, 
the video platform needs to determine
an advertising \emph{configuration} $\config\in\Config$
for each user (or equivalently, for each video session watched by a user), where $\Config$ is the set of feasible configurations.\footnote{Our model and results allow a different feasible set for each user, but we omit that for simplicity.} Fixing a user $\rider\in \Rider$,
each configuration $\config\in\Config$ 
specifies a certain number of reserved impressions 
$\alloc_{\threeindex}\in\mathbb{Z}_{\geq 0}$
and a per-impression price $\weight_{\threeindex}\in\mathbb{R}_{\geq 0}$
for each advertiser $\driver\in\Driver$.
% advertiser $\driver$'s impression 
% have been displayed to user $\rider$
% with per-unit price $\weight_{\threeindex}$.
Each advertiser $\driver$
demands $n_\driver\in\mathbb{Z}_{\geq 0}$ number of impressions in total
and is only willing to pay for 
at most that many impressions to
the video platform.
Users 
arrive at the video platform over time
in $K\in\N$ stages. At each stage $k\in [K]$,
a new subset of online users $\Rider_k\subseteq\Rider$
arrives at the video platform. Upon this arrival, the video platform observes $\Rider_k$, as well as 
$\allocs\ked = \{\alloci\}_{\rider\in\Rider_k,\config\in\Config,\driver\in \Driver}$
and 
$\weightbf\ked = \{\weight_{\threeindex}\}_{\rider\in\Rider_k,\config\in\Config,\driver\in \Driver}$.
We highlight that 
$\{\Rider_k\}_{k\in[K]}$
are disjoint and $\cup_{k\in[K]}\Rider_k = \Rider$. 


Our goal as the video platform is to design 
a multi-stage algorithm $\ALG$
for assigning configurations to the users in a stage-by-stage fashion as they arrive. Upon arrival of users $\Rider_k$ 
in stage $k\in [K]$,
$\ALG$ makes an 
irrevocable decision by
assigning a configuration 
to each user $\rider\in\Rider_k$. As we mentioned above, the assigned configuration of each user specifies 
the number of impressions and per-impression prices 
for each of the advertisers. 
These configuration decisions can be integral or fractional. 
In this paper we focus on the fractional allocations.\footnote{\label{footnote:integral}Using standard randomized rounding techniques, all of our results for the fractional allocation problem, including the algorithm and its competitive analysis, can easily be extended to the setting with integral randomized allocations under the \emph{large budget assumptions}, i.e, in the asymptotic regime when $\underset{i,c,j}{\min}\frac{n_j}{\alloci}$ is large.}
At the end of $K$ stages, given the assigned configurations by $\ALG$,  each advertiser only pays for 
at most $n_\driver$ number of allocated impressions in total. Moreover, they pay for an impression based on its per-impression price specified by the assigned configuration of the corresponding user. The goal of the algorithm is to maximize the total revenue collected at the end of $K$ stages.

\vspace{3mm}
\noindent\textbf{LP Formulation and Offline Benchmark}~~To help with understanding our extension model, we formulate the
optimum offline solution in
the configuration allocation
problem as a simple linear program, denoted by  
\ref{eq:LP primal}:
    \begin{equation}
\tag{\textsc{OFFLINE-OPT}}
\label{eq:LP primal}
\arraycolsep=1.4pt\def\arraystretch{1}
\begin{array}{lllll}
\max\limits_{\xbf,\zbf\geq \mathbf{0}}
\quad\quad\quad&
% \mathop{\displaystyle\sum
\displaystyle\sum_{\rider\in\Rider}
\displaystyle\sum_{\config\in\Config}
\displaystyle\sum_{\driver\in\Driver}
\weight_{\threeindex}\cdot
% }
% \limits_{(\threeindex)\in E}
 x_{\threeindex}
&~~\text{s.t.}
% \min\limits_{\alphabf,\betabf,\gammabf}
% \quad\quad\quad 
% &
% \displaystyle\sum_{\rider\in \Rider }{\alpha_\rider}+
% \displaystyle\sum_{\driver\in \Driver}{\beta_\driver}
% &~~\text{s.t.} 
\\[1.4em]
 &
%  \mathop{\displaystyle\sum
\displaystyle\sum_{\rider\in\Rider}
\displaystyle\sum_{\config\in\Config}
 x_{\threeindex} 
%  }
%  \limits_{\rider,\config:(\threeindex)\in E}
 \leq
 n_{\driver} 
 &~~\driver\in\Driver~,
% \gamma_{\threeindex} 
% +
% \beta_\driver \geq \weight_{\threeindex}
% & (\threeindex)\in E~,
\\[1.4em]
 &
 \displaystyle\sum\limits_{\config\in\Config}
 z_{\rider,\config}
 \leq 1 
 &~~
 \rider\in \Rider~, 
% \alpha_\rider 
% \geq 
% \displaystyle\sum\limits_{\driver\in \Driver}
% \alloci\cdot \gamma_{\threeindex} &i\in \Rider, \config\in \Config~, 
\\[1.4em]
 &
 x_{\threeindex} \leq 
 \alloci \cdot z_{\rider,\config}
 &~~
\rider\in\Rider,\config\in\Config,\driver\in\Driver~. 
% \alpha_\rider 
% \geq 0 &\rider \in \Rider~, 
% \\[1.4em]
%  &x_{\threeindex} \geq 0 &(\threeindex)\in E~, &
% & &
% \beta_\driver\geq 0  &\driver\in \Driver~,
% \\[1.4em]
%  &z_{\rider,\config} \geq 0 &\rider\in\Rider, \config\in \Config~. &
% & &
% \gamma_{\threeindex} \geq 0  &(\threeindex)\in E~.
\end{array}
\end{equation}
In the above formulation, $z_{\rider,\config}$
is the fraction of configuration $\config$ allocated
to user $\rider$,
and $x_{\threeindex}$
is the (fractional) number of impressions
created by user $\rider$ for advertiser $\driver$ based on configuration $\config$ that the advertiser is finally willing to pay. Note that the number $x_{\threeindex}$ of impressions that the advertiser is willing to pay is no more than number of allocated impressions $\alloci \cdot z_{\rider,\config}$ from user $\rider$ under configuration $\config$, and the first quantity can be strictly smaller than the second (as advertiser $\driver$ should only pay for at most $n_\driver$ impressions overall). If an impression is allocated but the advertiser is not responsible to pay for it, we refer to that impression as being \emph{preempted} or \emph{freely disposed}. 


\vspace{3mm}
\noindent\textbf{Connection to Baseline Model}~~As we mentioned above,
the multi-stage configuration allocation 
generalizes the multi-stage vertex weighted matching.
In particular, 
every instance in the vertex weighted matching 
can be thought as an
instance in configuration allocation as follows:
Each advertiser $\driver$ has a unit demand 
($n_\driver = 1$).
The feasible configuration set encodes 
all edges $E$ in baseline model
($\Config = E$).
More specifically, for every 
edge $(\rider\primed,\driver\primed)\in E$,
the corresponding
configuration $\config$ 
encodes the 
number of reserved impression $\{\alloci\}_{\rider,\driver}$
as 
$\alloci =\indicator{\rider = \rider\primed,
\driver = \driver\primed}$.
The 
per-impression price are identical for each advertiser
($\weight_{\threeindex} = \weight_{\rider',\config',\driver}$
for all $\rider,\rider',\config,\config'$).
Finally, note that
since per-impression price are identical for each advertiser
and number of reserved impression $\{\alloci\}$
is encoded as the aforementioned indicator function,
without loss of generality, 
we can restrict attention to online algorithms 
whose allocations never exceed demand $\{n_\driver\}$
of advertisers, and thus
no
preemption or free disposal is needed.


==> tex/prelim_older.tex <==
\section{Preliminaries}
\label{sec:prelim}
\smallskip
\noindent{\textbf{Model and Notation~}}
We consider a general bipartite allocation model for matching arriving demand requests to available suppliers. An instance of our model consists of a bipartite graph $\mathcal{G}=(\Rider,\Driver,E)$, where vertices in $\Driver$ (supply) are available offline and vertices in $\Rider$ (demand) arrive over time. Specifically, we consider a \emph{multi-stage arrival} model, in which vertices in $\Rider$ arrive in $K\in\mathbb{N}$ stage. We assume the number of stages $K$ is fixed and known by the algorithm. At each stage $k\in[K]$, a new subset of online vertices $\Rider_k\subseteq \Rider$ arrive, which we often call an arriving \emph{batch}, and reveal their incident edges in $E$. We highlight that $\Rider=\cup_{k\in[K]}\Rider_k $ and $\Rider_k\cap\Rider_{k'}=\emptyset$ for $k\neq k'$. After arrival of batch $k$, the multi-stage allocation algorithm makes an irrevocable allocation decision by allocating each vertex $i\in\Rider_K$ (which corresponds to one unit of demand) to the set of \emph{available} neighboring offline vertices $j\in\Driver, (i,j)\in E$ . Let $E_k$ denote the set of edges in $E$ incident to $\Rider_k$. We denote the allocation of stage $k$ by the vector $\mathbf{x}_{k}\in\mathbb{R}^{E_k}$, where $x_{k,ij}\in[0,1]$ is the amount of allocation of vertex $i$ to $j$. This allocation can be fractional or integral. 

The goal of the multi-stage allocation algorithm is to maximize the ``weight" of the final allocation after all batches arrive, while ensuring the \emph{feasibility constraints} on the offline side. The objective function and the feasibility constraints are specific to the choice of the problem as follows:
\begin{enumerate}[label=\textit{(\roman*)}]
\smallskip
    \item \underline{Multi-stage vertex weighted b-matching}: each offline vertex $j\in\Driver$ has a capacity constraint $B_j$, that is, the total (fractional) allocation amount at this vertex cannot exceed $B_j$. It also has a non-negative weight $w_j$ for each unit of allocation. The objective function is the sum of the weight of the offline vertices in the (fractional) allocation. We also consider the special case of \emph{multi-stage vertex weighted matching}, in which $B_j=1$ for all $j\in\Driver$.
    \smallskip
    \item\underline{Multi-stage budgeted allocation (AdWords)}:  each edge $(i,j)\in E$ has a non-negative weight $b_{ij}$ for each unit of allocation on this edge. Without loss of generality, we assume $b_{ij}\in[0,1]$.\footnote{This assumption is just for simplicity, as it helps with making the large budget assumption in vertex weighted b-matching similar to small bid over budget assumption in the budgeted allocation problem.} Each offline vertex $j\in \Driver$ has a budget constraint $B_j$, that is, the sum of the weights of edges incident to $j$ in the (fractional) allocation cannot exceed $B_j$. The objective function is the sum of the weight of all the edges in the (fractional) allocation.\footnote{This model can be interpreted as the multi-stage version of the AdWords problem, in which $V$ is the set of advertisers and $U$ is the set of arriving batched queries. In this application, $b_{ij}$ essentially denotes the bid of advertiser $j$ for query $i$ and $B_j$ is the budget of advertiser $j$.} 
\end{enumerate}

We measure the performance of our multi-stage algorithms by their \emph{competitive ratio}, which is the worst-case ratio between the expected total weight of the algorithm and the optimum offline benchmark given the entire problem instance (formally defined below).
\begin{definition}[\textbf{Competitive Ratio}]
	\label{def:competitive ratio}
	Fix the number of stages $K\in\mathbb{N}$. For $\alpha\in [0,1]$, a multi-stage allocation algorithm $\texttt{ALG}$ is \emph{$\alpha$-competitive} against the optimum offline solution in the multi-stage vertex weighted b-matching problem (resp. multi-stage budgeted allocation/AdWords problem), if the following holds:
	\begin{align*}
		\inf\limits_{I \in\mathcal{I}}~~
		\frac{\texttt{ALG}(I)}{\texttt{OPT}(I)}~
		\geq \alpha~,
	\end{align*}
	where $\mathcal{I}$ is the set of instances of the multi-stage vertex weighted b-matching problem (resp. multi-stage budgeted allocation problem), and $\texttt{ALG}(I)$ and $\texttt{OPT}(I)$ are the total weights of the multi-stage algorithm $\texttt{ALG}$ and optimum offline solution on an instance $I$, respectively. For randomized multi-stage algorithms, we abuse the notation and $\texttt{ALG}(I)$ denotes the expected total weight of the algorithm on an instance $I$.
\end{definition}

 As an important note, we are mainly interested in the competitive ratio of fractional $K$-stage algorithms. We also consider the asymptotic competitive ratio of integral $K$-stage algorithms (possibly randomized) under the ``large budgets assumption'' in the vertex weighted b-matching problem (i.e., under the assumption that $\min_j B_j=\Omega(1)$), or equivalently under the small bid over budget assumption in the budgeted allocation problem (i.e., under the assumption that $\max_{i,j} \frac{b_{ij}}{B_j}=o(1)$ or equivalently $\min_j B_j=\Omega(1)$ when $b_{ij}\in[0,1]$). 


\smallskip
\noindent{\textbf{A Recursive Sequence of Polynomials~}} As a novel technical ingredient of our proposed multi-stage allocation algorithms, we identify a particular sequence of polynomials of decreasing degrees. Our construction of these polynomials is recursive, which gives us a polynomial of degree $K-k$ for each stage $k=1,2,\ldots,K-1$. Here, we introduce these polynomials, describe this underlying recursive equation, and elaborate a bit more on some of their properties (\Cref{prop:poly}, proof in Appendxi~\ref{apx:poly}). Later, we first show in \Cref{sec:vertex-weight} how these polynomials help us to design an optimal competitive multi-stage algorithm for the vertex weighted matching and how to develop a primal-dual analysis framework that incorporates this recursive equation. Then we show how to extend these ideas to use our polynomials for the vertex weighted b-matching (\Cref{sec:weighted b-matching}) and budgeted allocation (\Cref{sec:adwords}) problems.

\begin{proposition}[{\textbf{{Sequence of Polynomial Regularizers}}}]
\label{prop:poly}
Consider a sequence of functions $f_1,f_2,\ldots,f_{K}:[0,1]\rightarrow[0,1]$
satisfying the following backward recursive equation:
\begin{itemize}
    \item $\forall x\in[0,1]:~f_{K}(x)=\mathbb{I}\{{x=1\}}$,
    where $\mathbb{I}(\cdot)$ is 
    the indicator function,
    \item $\forall x\in[0,1], k\in[K-1]:~f_{k}(x)=\underset{y\in[0,1-x]}{\max}~(1-y)f_{k+1}(x+y)$.
\end{itemize}
Then, the following statements hold:
\begin{enumerate}[label=(\roman*)]
    \item The function sequence $\{f_k\}_{k=1}^{K-1}$ is a sequence of $K-1$ polynomials with decreasing degrees, where $f_k(x)=(1-\frac{1-x}{K-k})^{K-k}$ for $k\in[K-1]$.\footnote{As a convention, we refer to $f_K(x)=\mathbb{I}\{x=1\}$ as a polynomial of degree $0$ (although not mathematically rigorous).}
    \item $f_k(x)$ is monotone increasing and continuous over $[0,1]$ for $k\in[K-1]$. Hence, $F_k(x)\triangleq \int_{0}^x f_k(y)dy$ is differentiable and strictly convex over $[0,1]$ for $k\in[K-1]$.
    \item $\forall k\in[K]$, $f_k(x)\leq e^{x-1}$ for $x\in[0,1]$. Moreover, the first function $f_1(x)=(1-\frac{1-x}{K-1})^{K-1}$ converges point-wise from below to the function $e^{x-1}$ as $K\to+\infty$ (see \Cref{fig:poly}).
    \item $\underset{y\in[0,1]}{\min}1-(1-y)f_1(y)=\cratioexp\triangleq\cratio{K}$
\end{enumerate}
\end{proposition}

We conclude this section by reminding the reader that the above polynomials $\{f_k\}_{k\in[K-1]}$ are drawn in \Cref{fig:poly}. As it is clear from this figure, these polynomials provide careful point-wise estimations for the exponential function $f(x)=e^{x-1}$ at different levels of precision. When these polynomials are used to regularize the maximum weight matching objective function, they provide different levels of ``hedging'' intensity against the future uncertainty in the arriving input exactly because of these different levels of estimation precision. This point will be clear in the next section.

==> tex/result-table.tex <==
\begin{table}[htb]
\small\addtolength{\tabcolsep}{-2pt}
\caption{Comparing our results to previous work}
\vspace{1mm}
\label{tab:summary}
%  	\smallskip
%\renewcommand{\thefootnote}{\fnsymbol{footnote}}
%\renewcommand*{\thefootnote}{\arabic{footnote}}

\renewcommand{\thefootnote}{\ifcase\value{footnote}\or(\textasteriskcentered)\or(\textdagger)\or(\textdagger)\or(\textdaggerdbl)\or(\textsection)\or(\textbardbl)\or(\textdollar)\or(\textdollar\textdollar)\or(\pounds)\or(\texteuro)\or(\#\#\#)\or(\#\#\#\#)\or($\infty$)\fi}
 	\footnotesize
\center
 	
% \begin{tabular}{|c|c|c|c|c|c|}
%     \cline{2-6}
%     \multicolumn{1}{c|}{}
%     &    	
%     \begin{minipage}{0.2\textwidth}
%  		{\begin{center}
%     \vspace{3pt}
%  			$K$-stage \\
%  			vertex weighted \\
%  			matching (\Cref{sec:vertex-weight})
%     \vspace{3pt}
%     \end{center}
%  		}
%  		\end{minipage}
%     & 
%         \multicolumn{2}{c|}{
%         \begin{minipage}{0.25\textwidth}
%  		{\begin{center}
%     \vspace{3pt}
%  			$K$-stage \\
%  			vertex weighted \\
%  			b-matching (\Cref{sec:weighted b-matching})
%     \vspace{3pt}
%     \end{center}
%  		}
%  		\end{minipage}
%  		}
%     & 
%     \multicolumn{2}{c|}{
%         \begin{minipage}{0.25\textwidth}
%  		{\begin{center}
%     \vspace{3pt}
%  			$K$-stage 
%  			AdWords \\
%  			(\Cref{sec:adwords})
%     \vspace{3pt}
%     \end{center}
%  		}
%  		\end{minipage}
%  		}
%     \\
%     \cline{2-6}
%     \multicolumn{1}{c|}{}
%     &
%     fractional & 
%     fractional & 
%             \begin{minipage}{0.12\textwidth}
%  		{\begin{center}
%     \vspace{3pt}
%  			integral,\\
%  			deterministic,\\
%  			($B\rightarrow +\infty$)
%     \vspace{3pt}
%     \end{center}
%  		}
%  		\end{minipage}
%     &
%     fractional &
%             \begin{minipage}{0.12\textwidth}
%  		{\begin{center}
%     \vspace{3pt}
%  			integral,\\
%  			randomized,\\
%  			($B\rightarrow +\infty$)
%     \vspace{3pt}
%     \end{center}
%  		}
%  		\end{minipage}
%     \\
%     \hline
%   	\begin{minipage}{0.2\textwidth}
%  		{\begin{center}
%     \vspace{3pt}
%  			Lower-bound \\
%  			(previous work)
%     \vspace{3pt}
%     \end{center}
%  		}
%  		\end{minipage}
%     &$1-\frac{1}{e}$ &$1-\frac{1}{e}$
%     &$1-\frac{1}{e}$
%     &$1-\frac{1}{e}$&$1-\frac{1}{e}$\\
%     \hline
%   	\begin{minipage}{0.2\textwidth}
%  		{\begin{center}
%     \vspace{3pt}
%  			Lower-bound \\
%  			(this work)
%     \vspace{3pt}
%     \end{center}
%  		}
%  		\end{minipage}
%     &\multicolumn{5}{c|}{
%     $\cratioexp
%     \xrightarrow{K\rightarrow+\infty}
%     1 - \frac{1}{e}$
%     }\\
%     \hline
%   	\begin{minipage}{0.2\textwidth}
%  		{\begin{center}
%     \vspace{3pt}
%  			Upper-bound \\
%  			(this work)
%     \vspace{3pt}
%     \end{center}
%  		}
%  		\end{minipage}
%     &\multicolumn{5}{c|}{
%         $\cratioexp
%     \xrightarrow{K\rightarrow+\infty}
%     1 - \frac{1}{e}$
%     }\\
%     \hline
% \end{tabular}
\begin{tabular}{|c|c|c|c|c|}
    \cline{2-5}
    \multicolumn{1}{c|}{}
    &    	
    
        \multicolumn{2}{c|}{
        \begin{minipage}{0.37\textwidth}
 		{\begin{center}
    \vspace{3pt}
 			$K$-stage vertex weighted b-matching\\
 			(\Cref{sec:vertex-weight} and \Cref{sec:weighted b-matching})
    \vspace{3pt}
    \end{center}
 		}
 		\end{minipage}
 		}
    & 
    \multicolumn{2}{c|}{
        \begin{minipage}{0.25\textwidth}
 		{\begin{center}
    \vspace{3pt}
 			$K$-stage 
 			AdWords \\
 			(\Cref{sec:adwords})
    \vspace{3pt}
    \end{center}
 		}
 		\end{minipage}
 		}
    \\
    \cline{2-5}
    \multicolumn{1}{c|}{}
    &
     
    fractional & 
            \begin{minipage}{0.12\textwidth}
 		{\begin{center}
    \vspace{3pt}
 			integral
    \vspace{3pt}
    \end{center}
 		}
 		\end{minipage}
    &
    fractional &
            \begin{minipage}{0.12\textwidth}
 		{\begin{center}
    \vspace{3pt}
 			integral
 			
    \vspace{3pt}
    \end{center}
 		}
 		\end{minipage}
    \\
    \hline
   	\begin{minipage}{0.2\textwidth}
 		{\begin{center}
    \vspace{3pt}
 			Lower-bound \\
 			\emph{(previous work)}
    \vspace{3pt}
    \end{center}
 		}
 		\end{minipage}
    &$1-\frac{1}{e}$\footnotemark[1]
    &$1-\frac{1}{e}-O\left(\frac{1}{B_{\textrm{min}}}\right)$\footnotemark[1]
    % \RN{can you check the bounds in this row? I haven't double checked them}
    &$1-\frac{1}{e}$\footnotemark[2]&$1-\frac{1}{e}-O\left(\frac{1}{B_{\textrm{min}}}\right)$\footnotemark[2]\\
    \hline
   	\begin{minipage}{0.2\textwidth}
 		{\begin{center}
    \vspace{3pt}
 			Lower-bound \\
 			\textbf{\emph{(this work)}}
    \vspace{3pt}
    \end{center}
 		}
 		\end{minipage}
    &$\cratioexp$
    &$\cratioexp-O\left(\frac{1}{B_{\textrm{min}}}\right)$
    &$\cratioexp$&$\cratioexp-O\left(\sqrt{\frac{\log(B_{\text{min}})}{{{B_{\text{min}}}}}}\right)$\\
    \hline
   	\begin{minipage}{0.2\textwidth}
 		{\begin{center}
    \vspace{3pt}
 			Upper-bound \\
 			\textbf{\emph{(this work)}}
    \vspace{3pt}
    \end{center}
 		}
 		\end{minipage}
    &  \multicolumn{2}{c|}{$\cratioexp$}
    &\multicolumn{2}{c|}{$\cratioexp$}\\
    \hline
\end{tabular}

 	\smallskip
\noindent\par

 	\begin{minipage}{0.65\textwidth}
 		{
 			\footnotesize
 			\footnotemark[1]~{\cite{AGKM-11}};~ 
 			\footnotemark[2]~{\cite{MSVV-07,BJN-07}};
 		}
 	\end{minipage}
 \end{table}

==> tex/tem.tex <==
\begin{proof}[Proof of \Cref{thm:b-matching}]

For each stage $k\in[1:K-1]$, let $\{(\Rider^{(0)}_k, \Driver^{(0)}_k),\dots, (\Rider^{(L_k)}_k, \Driver^{(L_k)}_k)\}$ be the 
structural decomposition of $(\Rider_k, D, E_k)$ as in \Cref{lemma:structure},
and $\{x_{k, ij}^*\}_{(i,j)\in E_k}$
be the optimal solution of the program~\ref{eq:concave-k-bmatching}. First, we define the following notations which will be useful in this proof:
\begin{align*}
\forall j\in \Driver,~k\in[K]:\quad\quad\quad &y^*_{k,j}\triangleq\sum_{s=1}^{k-1}\sum_{i:(i,j)\in E_s}x^*_{s,ij}
% ,\\
%  &y^*_{0,j}=0.
\end{align*}
Now, consider the offline primal-dual linear programs in \ref{eq:LP-max-weight}. Given the feasible primal assignment $\{\xbf^*_{k}\}_{k\in[K]}$, construct a dual assignment as follows. 
First, set $\alpha_i\gets 0$ and $\beta_j\gets 0$ for all $i\in\Rider,j\in \Driver$. At each stage $k\in[0:K-1]$, update the dual variables as follows:
\begin{align*}
   &\forall i \in \Rider^{(l)}_k,~l\in[0:L_k]: &&\alpha_i\gets c^{(l)}_k
   \\
    &\forall j \in \Driver^{(l)},~l\in[0:L_k]: &&\beta_{j}\gets\beta_{j}+\Delta\beta_{k,j}\\
    &&&\Delta\beta_{k,j}\triangleq \left(
\sum_{i:(i,j)\in E_k}x_{k,ij}^* \right)\cdot \left(w_j - c_k^{(l)}\right)\overset{(1)}{=}w_j(y^*_{k+1,j}-y^*_{k,j})f_k(y^*_{k+1,j})
\end{align*}
where in eq.~(1) above 
% \YF{label eq.~(1) is not defined in our paper}
we use the uniformity property and the definition of $c^{(l)}_k$ in \Cref{lemma:structure}. For the last stage $K$, note that $F_K(x)=0$. Therefore, \Cref{alg:b-matching} essentially solves the maximum vertex weighted matching in the last stage graph $(\Rider_K, \Driver, E_K)$ where each $j\in\Driver$ has initial capacity $1-y^*_{K, j}$. Let $\{\hat{\alpha}_{K,i}, \hat{\beta}_{K,j}\}_{i\in\Rider_K,j\in\Driver}$ 
be the \emph{optimal} dual solution of this LP. Then update the  dual variables as follows:
\begin{align*}
&\forall i\in\Rider_K:~~\alpha_i \gets \hat{\alpha}_{K,i} \\
&\forall j\in \Driver~:~~\beta_j\gets \beta_j+\Delta \beta_{K,j},~~\Delta\beta_{K, j} \triangleq (1 - y^*_{K, j})\hat{\beta}_{K,j}
\end{align*}



% Consider the following construction of dual solution.
% At stage $k < K$, let 
% $\bar f_k(x) \triangleq f_{K - k}(x) = \left(
% \frac{K - k - 1 + x}{K-k}
% \right)^{K-k}$, and 
% $\{(\Rider^{(0)}_k, \Driver^{(0)}_k),\dots, (\Rider^{(L)}_k, \Driver^{(L)}_k)\}$ be the 
% partition of $(\Rider_k, D, E_k)$ in \Cref{lemma:structure},
% and 
% $\{x_{k, ij}^*\}_{(i,j)\in E_k}$
% be the optimal solution  
% from the concave program~\eqref{eq:concave program k}
% solved by BWF.
% Construct the dual solution as follows,
% for any $k < K$ 
% \begin{align*}
%     \alpha_i &= c^{(l)}_k
%     \qquad \forall i \in \Rider^{(l)}_k \\
%     \Delta \beta_{k,j} &= \left(
%     % 1 - 
%     \sum_{i\in N_k(j)}x_{k,ij}^*
%     % - y_{k,j}
%     \right)\cdot 
%     \left(w_j - c_k^{(l)}\right)
%     \qquad \forall j \in \Driver^{(l)}
% \end{align*}
% where $N_k(j)$ denotes all neighbor vertices of item $j$
% in graph $(\Rider_k, D, E_k)$ at stage $k$.
The rest of the proof is done in two steps:
\vspace{1mm}

\noindent[\textit{Step \rom{1}}]~\emph{Comparing objective values in primal and dual.}
we first show that 
the objective value of the above dual assignment
is equal to the objective value of the primal assignment of \Cref{alg:b-matching}.
To show this, we consider 
each stage $k$ separately.
For the last stage $K$, 
this holds by construction.
For each stage $k < K$, note that the primal objective value is decomposed across pairs $(\Rider_k^{(l)}, \Driver_k^{(l)})$, $l=0,1,\ldots,L_k$, simply because $x^*_{k,ij}>0$ only if $i$ and $j$ belong to the same pair (\Cref{lemma:structure}). As these pairs partition sets of vertices $\Rider$ and $\Driver$, it is enough to compare the changes in the primal and dual objectives in each pair $(\Rider_k^{(l)}, \Driver_k^{(l)})$ separately. Notice that if $l = 0$ then $c^{(l)}_k = 0$, and thus,
\begin{align*}
    \Delta(\textrm{Dual})^{(0)}\triangleq\sum_{i \in \Rider^{(0)}_k} \alpha_i
    +
    \sum_{j \in \Driver^{(0)}_k} \Delta\beta_{k,j}
    &= 
    \sum_{j \in \Driver^{(0)}_k}\sum_{i:(i,j)\in E_0} w_jx_{k, ij}^*\triangleq\Delta(\textrm{Primal})^{(0)}. 
\end{align*}
Similarly, for $l \geq 1$, 
\begin{align*}
     \Delta(\textrm{Dual})^{(l)}&\triangleq\sum_{i \in \Rider^{(l)}_k} \alpha_i
    +
    \sum_{j \in \Driver^{(l)}_k} \Delta\beta_{k,j}
    =
    |\Rider^{(l)}_k|\cdot c^{(l)}_k
    +
    \sum_{j \in \Driver^{(l)}_k}\sum_ {i:(i,j)\in E_k} 
    x_{k, ij}^*\left(w_j - c^{(l)}_k\right)\\
    &= 
     |\Rider^{(l)}_k|\cdot c^{(l)}_k+\sum_{j\in\Driver_k^{(l)}}\sum_{i:(i,j)\in E_k} 
    w_jx_{k, ij}^*-c^{(l)}_k\sum_{i\in\Rider_k}\left(\sum_{j:(i,j)\in E}x^*_{k,ij}\right)\\
    &=\sum_{j\in\Driver_k^{(l)}}\sum_{i:(i,j)\in E_k} 
    w_jx_{k, ij}^*\triangleq \Delta(\textrm{Primal})^{(l)},
\end{align*}
where the last equality uses the saturation property in \Cref{lemma:structure} for $l\geq 1$.
\vspace{1mm}

\noindent[\textit{Step \rom{2}}]~\emph{Checking approximate feasibility of dual.} To show approximate dual feasibility, it is enough to show that for any stage $k\in[K]$ and any arbitrary edge $(i, j) \in E_k$,
\begin{align}
\label{eq:dual constraint feasibility}
    \alpha_i + \sum_{s = 1}^k\Delta\beta_{s, j}
    \geq 
    w_j\left(1-(1-1/K)^K\right)
\end{align}
We next show \eqref{eq:dual constraint feasibility}
holds for $k=1,2,\ldots,K-1$ by using the following technical lemma, which carefully uses our sequence of polynomial regularizers to establish a lower bound on the LHS of \eqref{eq:dual constraint feasibility}.

  \begin{lemma}
    \label{lem:polynomial inequality 2}
    For any $K \in \N,~1\leq k \leq K - 1$, any $x \in [0, 1]$, and
    any $0 = y_1 \leq 
    y_2 \leq \dots \leq y_k \leq  1 - x$,
    \begin{align*}
     (1-x)f_{k}(y_k + x) -
    \sum_{s = 1}^{k - 1} 
    (y_{s + 1} - y_s)
    f_{s}(y_{s + 1})
     \leq 1-\cratio{K}=
    (1-1/K)^K.
    \end{align*}
    \end{lemma}
Now assume $i \in \Rider_k^{(l)}$ and $j \in \Driver_k^{(l')}$, which implies $c^{(l')}_k \leq c^{(l)}_k$ (thanks to \Cref{lemma:structure}). Then we have:
\begin{align*}
     \alpha_i + \sum_{s = 1}^{k}\Delta\beta_{s, j}&=c_k^{(l)} + 
    \left(\sum_{i':(i',j)\in E_k}x_{k, i'j}^*\right)
    \left(w_j - c_k^{(l')}\right)
    +
    \sum_{s= 1}^{k - 1} \Delta\beta_{s, j} \\
    &\geq c_k^{(l')} + 
    \left(\sum_{i':(i',j)\in E_k}x_{k, i'j}^*\right)
    \left(w_j - c_k^{(l')}\right)
    +
    \sum_{s= 1}^{k - 1} \Delta\beta_{s, j} \\
    &=w_j\left(1-f_k\left(y^*_{k,j}+\sum_{i':(i',j)\in E_k}x_{k, i'j}^*\right)+\left(\sum_{i':(i',j)\in E_k}x_{k, i'j}^*\right)f_k\left(y^*_{k,j}+\sum_{i':(i',j)\in E_k}x_{k, i'j}^*\right)\right)\\
    &+ \sum_{s= 1}^{k - 1} \Delta\beta_{s, j} \\
    &=w_j\left(1-\left(1-\sum_{i':(i',j)\in E_k}x_{k, i'j}^*\right)f_k\left(y^*_{k,j}+\sum_{i':(i',j)\in E_k}x_{k, i'j}^*\right)+\sum_{s=1}^{k-1}\left(y^*_{s+1,j}-y^*_{s,j}\right)f_k\left(y^*_{s+1,j}\right)\right)\\
    &\geq w_j \cratio{K}~,
\end{align*}
where the first inequality uses $c^{(l')}_k \leq c^{(l)}_k$, the second equality uses the expression for $c^{(l')}_k$ in \Cref{lemma:structure} due to uniformity, and the last inequality invokes \Cref{lem:polynomial inequality 2} for the sequence: 
$$
0=y^*_{1,j}\leq y^*_{2,j}\leq \ldots \leq y^*_{k,j}\leq 1-\sum_{i':(i',j)\in E_k}x_{k, i'j}^*~.
$$
% \begin{align*}
%      & c_k^{(l)} + 
%     \left(\sum_{i'\in N_k(j)}x_{k, i'j}^*\right)
%     \left(w_j - c_k^{(l)}\right)
%     +
%     \sum_{s' = 1}^{k - 1} \Delta\beta_{s', j} \\
%     &\leq 
%     c_k^{(l')} + 
%     \left(\sum_{i'\in N_k(j)}x_{k, i'j}^*\right)
%     \left(w_j - c_k^{(l)}\right)
%     +
%     \sum_{s' = 1}^{k - 1} \Delta\beta_{s', j} \\
%     &=
%     \alpha_i + \sum_{s' = 1}^{k}\Delta\beta_{s', j}
% \end{align*}

So far, we have shown \eqref{eq:dual constraint feasibility} holds for all stages $k < K$.
For the last stage $K$, and any edge $(i, j) \in E_K$,
notice that 
$\alpha_i+\Delta\beta_{K, j}=\hat{\alpha}_{K,i} + \Delta\beta_{K, j} \geq 
w_j(1 - y^*_{K, j})$ by construction.
If $y^*_{K, j} = 0$, inequality \eqref{eq:dual constraint feasibility} holds. Otherwise, let $s^\dagger < K$ be the largest 
stage smaller than $K$ 
where 
there exists $l^\dagger$ 
such that 
$j \in \Driver_{s^\dagger}^{(l^\dagger)}$ and 
$\Delta\beta_{s^\dagger,j} > 0$. By definition, we know that 
$y^*_{s^\dagger, j} + \displaystyle\sum_{i':(i',j)\in E_{s^\dagger}}x_{s^\dagger, i'j}^* = y^*_{K,j}$. So we have:
\begin{align*}
    \alpha_i + \sum_{s = 1}^{K}\Delta\beta_{s, j}
    &\geq    
    w_j(1 - y^*_{K, j})
    + \sum_{s = 1}^{K - 1}\Delta\beta_{s, j} = 
    w_j(1 - y^*_{K, j}) + \sum_{s = 1}^{s^\dagger}\Delta\beta_{s, j} \\
    &\geq w_j\left(1 - f_{s^\dagger}(y^*_{K, j})\right) + \sum_{s = 1}^{s^\dagger}\Delta\beta_{s, j} =c^{(l^\dagger)}_{s^\dagger} + \sum_{s = 1}^{s^\dagger}\Delta\beta_{s, j} \\
    &\geq w_j(1 - (1 - 1/K)^K)~,
\end{align*}
where the first equality uses the fact $\Delta\beta_{s, j} = 0$ for all $s$
between $s^\dagger + 1$ and $K - 1$; the first inequality uses the fact that 
that $f_{s}(x) \geq x$ for all $x\in [0, 1]$, the second equality uses the definition of $c^{(l^\dagger)}_{s^\dagger}$ and the fact that $y^*_{s^\dagger, j} + \displaystyle\sum_{i':(i',j)\in E_{s^\dagger}}x_{s^\dagger, i'j}^* = y^*_{K,j}$; and finally the last inequality holds by exactly the same argument as in the case of $k<K$.
\end{proof}
